Uplifting Bandits

We introduce a multi-armed bandit model where the reward is a sum of multiple random variables, and each action only alters the distributions of some of them. After each action, the agent observes the realizations of all the variables. This model is motivated by marketing campaigns and recommender systems, where the variables represent outcomes on individual customers, such as clicks. We propose UCB-style algorithms that estimate the uplifts of the actions over a baseline. We study multiple variants of the problem, including when the baseline and affected variables are unknown, and prove sublinear regret bounds for all of these. We also provide lower bounds that justify the necessity of our modeling assumptions. Experiments on synthetic and real-world datasets show the benefit of methods that estimate the uplifts over policies that do not use this structure.

==> Appendices/Concentration-deprecated.tex <==
In this section, we formally describe the probability model of the $\nArms$-arm uplifting bandit problem that we build upon for proving the regret upper bounds, before deriving several concentration results that are used throughout our analyses.

Our upper-bound analyses are based on the stack-feedback model.
That is, we have a collection of independent random vectors $(\vta[\valuev][\round])_{\arm\in\arms,\round\in\oneto{\nRuns}}$ such that the law of $\vta[\valuev][\round]$ is $\va[\distribution]$.
Each $(\vta[\valuev][\round])_{\round\in\oneto{\nRuns}}$ forms a stack, and when the learner chooses action $\arm$, they receives the vector from the top of the stack. In other words, the value of $\vta[\valuev][\round]$ is observed when the learner pulls $\arm$ for the $\round$-th time.
By abuse of notation, we will also use $\vta[\valuev][\round]$ to denote the value of the random variable (evaluated at some $\sample\in\samples$ with $\samples$ being the underlying probability space).
In most of our algorithms, we are interested in either of the following estimates
%
\begin{equation}
    \notag
    \vtav[\estalt{\meanReward}][\round]=\frac{\sum_{\runalt=1}^{\round}\vtav[\valuev][\runalt]}{\round},
    ~~~~~~
    \vtav[\est{\meanReward}][\run][0] =
    \frac{\sum_{\runalt=1}^{\run}\vtav[\valuev][\runalt][\vt[\arm][\runalt]]\one\{\indv\notin\va[\variables][\vt[\arm]]\}}{\max(1, \vtav[\pullcount][\run][0])}.
\end{equation}
%
Despite the apparent similarity between these two quantities, the key distinction is that the denominator of $\vtav[\estalt{\meanReward}][\round]$ is a constant while the denominator of $\vtav[\est{\meanReward}][\run][0]$ is also a random variable.
Therefore, deriving a concentration bound for the later will require a more delicate treatment.
We first state a concentration inequality for $\vtav[\estalt{\meanReward}][\round]$.
%
\begin{lemma}
\label{lem:iid-concentration}
Let $\smallproba\in(0,1)$. It holds
%
\begin{equation}
    \notag
    \prob\left(\abs{\vtav[\estalt{\meanReward}][\round]-\vav[\meanReward]}\ge\sqrt{\frac{2\log(1/\smallproba)}{\round}}\right)
    \le 2\smallproba.
\end{equation}
\end{lemma}
\begin{proof}
This is immediate from \eqref{eq:subgaussian-concentration} and the fact that $\vtav[\estalt{\meanReward}][\round]$ is $(1/\sqrt{\round})$-subgaussian.
\end{proof}
%
\cref{lem:iid-concentration} is sufficient for the analysis whenever $\vtav[\est{\meanReward}]$ is defined as in \eqref{eq:mean-estimate-a}.
In fact, in this case $\vtav[\est{\meanReward}]=\vtav[\estalt{\meanReward}][\vta[\pullcount]]$ as long as $\vta[\pullcount]\ge1$.
Therefore, if $\abs{\vtav[\estalt{\meanReward}][\round]-\vav[\meanReward]}\le\sqrt{2\log(1/\alt{\smallproba})/\round}$ for all relevant $\arm$ and $\indv$ we have indeed the desired concentration result.

For the more challenging case where an indicator of the probability event is also involved in the estimator, we will leverage on tools from martingale theory.
Let us first introduce a concentration inequality for martingale difference sequence based on \cite[Lem. 2]{BDHK+08} and \cite[Th. 1.2A]{Victor99}.

\begin{lemma}%[{{\cite[Lem. 2]{BDHK+08}}}]
\label{lem:DLP-ineq}
Let $(\vt[\filter][\runalt])_{\runalt=0}^{\run}$ be a filtration and $(\vt[\rv][\runalt])_{\runalt=1}^{\run}$ be a $(\vt[\filter][\runalt])$-adapted martingale difference sequence.
Suppose that there exists $\rvb>0$ such that $\exof{\vt[\rv][\runalt]^2\given{\vt[\filter][\runalt-1]}}\le\rvb^2$ and that the following conditional Bernstein condition is verified for all $\runalt\in\oneto{\run}$ and $\probmoment\ge2$,
\begin{equation}
    \notag
    \exof{\abs{\vt[\rv][\runalt]}^{\probmoment}\given{\vt[\filter][\runalt-1]}} \le \frac{\probmoment!}{2}\rvb^{\probmoment-2}\exof{\vt[\rv][\runalt]^2\given{\vt[\filter][\runalt-1]}}.
\end{equation}
Then, for any $\smallproba\in(0,1/e)$, it holds
%
\begin{equation}
    \notag
    \prob\left(\sum_{\runalt=1}^{\run}\vt[\rv][\runalt]
    \ge 2\max(2\noisedev,2\rvb\sqrt{\log(1/\smallproba)})\sqrt{\log(1/\smallproba)}
    \right) \le \max(\log_2(\run),1)\frac{\smallproba}{2},
\end{equation}
where $\noisedev=\sqrt{\sum_{\runalt=1}^{\run}\exof{\vt[\rv][\runalt]^2\given{\vt[\filter][\runalt-1]}}}$ is the square root of the sum of the conditional variances of $\vt[\rv][\runalt]$'s.
\end{lemma}
\begin{proof}
The proof of \cite[Lem. 2]{BDHK+08} essentially applies.
We just need to replace the use of Freedman’s inequality by the use of de la Peña's inequality \cite[Th. 1.2A]{Victor99} and define $\alpha_0=2\rvb\sqrt{\log(1/\smallproba)}$.
Also notice with this choice of $\alpha_0$ the condition $\smallproba<1/e$ guarantees $\alpha_0\ge2$ so $\ell\ge\log_2{\sqrt{\run}}-1$ already ensures $2^{\ell}\alpha_0\ge\rvb\sqrt{\run}$.
\end{proof}

In the following, $(\vt[\filter])_{\run}$ will represent the natural filtration associated to $(\vt[\valuev], \vt[\arm][\run+1])_{\run}$ such that both $\vt[\valuev]$ and $\vt[\arm][\run+1]$ are $\vt[\filter]$-measurable.

\begin{lemma}
\label{lem:indicator-concentration}
Let $(\eventalt)_{\runalt=1}^{\run}$ be a sequence of events such that $\vt[\eventalt][\runalt]\in\vt[\filter][\runalt-1]$.
We consider
\begin{equation}
    \notag
    \vta[\pullcount][\run][\eventalt] = \sum_{\runalt=1}^{\run}\one\{\vt[\eventalt][\runalt]\},
    ~~~~~
    \vtav[\est{\meanReward}][\run][\eventalt] =
    \frac{\sum_{\runalt=1}^{\run}\vtav[\valuev][\runalt][\vt[\arm][\runalt]]
    \one\{\vt[\eventalt][\runalt]\}}
    {\max(1, \vta[\pullcount][\run][\eventalt])}.
\end{equation}
%
Suppose that all the noise variables $\vav[\snoise]$ satisfy the Bernstein condition \eqref{eq:Bernstein} with $\noisedev=1$ and have their variance bounded by $1$ (this is automatically verified if the noises are $1$-subgaussian).
Then, we have the following concentration bound for $\vtav[\est{\meanReward}][\run][\eventalt]$
%
\begin{equation}
    \label{eq:indicator-estimate-concentration}
    \prob
    \left(
    \left|\vtav[\est{\meanReward}][\run][\eventalt] - \frac{\sum_{\runalt=1}^{\run}\vav[\meanReward][\vt[\arm][\runalt]]\one\{\vt[\eventalt][\runalt]\}}{ \max(1,\vta[\pullcount][\run][\eventalt])}\right|
    \ge
    4\sqrt{\frac{\log((\log(\run)/\log(2))\smallproba)}
    {\max(1,\vta[\pullcount][\run][\eventalt])}}
    + \frac{4\log((\log(\run)/\log(2))\smallproba)}
    {\max(1,\vta[\pullcount][\run][\eventalt])}
    \right)
    \le \smallproba
\end{equation}
\end{lemma}
\begin{proof}
Let $\vtav[\snoise][\runalt][\vt[\arm][\runalt]]=\vtav[\valuev][\runalt][\vt[\arm][\runalt]]-\vav[\meanReward][\vt[\arm][\runalt]]$.
We apply \cref{lem:DLP-ineq} with $\vt[\rv][\runalt]\subs\vtav[\snoise][\runalt][\vt[\arm][\runalt]]\one\{\vt[\eventalt][\runalt]\}$ and $\rvb\subs 1$.
The two conditions that involve $\rvb$ in \cref{lem:DLP-ineq} are indeed verified because
$\ex_{\runalt-1}[\abs{\vtav[\snoise][\runalt][\vt[\arm][\runalt]]\one\{\vt[\eventalt][\runalt]\}}^{\probmoment}]=\ex[\abs{\vav[\snoise][\vt[\arm][\runalt]]}^{\probmoment}]\one\{\vt[\eventalt][\runalt]\}$ for all $\probmoment\in\R$.
The equality with $\probmoment=2$ also shows that $\ex_{\runalt-1}[\vt[\rv][\runalt]^2]\le\one\{\vt[\eventalt][\runalt]\}$ and thus $\sum_{\runalt=1}^{\run}\ex_{\runalt-1}[\vt[\rv][\runalt]^2]\le\vta[\pullcount][\run][\eventalt]$.
\cref{lem:DLP-ineq} then ensures that for all $\alt{\smallproba}\in(0,1/e)$, it holds
%
\begin{equation}
    \notag
    \prob\left(\sum_{\runalt=1}^{\run}
    (\vtav[\valuev][\runalt][\vt[\arm][\runalt]]-\vav[\meanReward][\vt[\arm][\runalt]])\one\{\vt[\eventalt][\runalt]\}
    \ge 4\sqrt{\vta[\pullcount][\run][\eventalt]\log(1/\alt{\smallproba})}
    + 4\log(1/\alt{\smallproba})
    \right) \le \frac{\log(\run)\alt{\smallproba}}{2\log(2)}.
    %\le \log(\run)\alt{\smallproba}.
\end{equation}
%
Applying the same procedure to $\vt[\rv][\runalt]\subs-\vtav[\snoise][\runalt][\vt[\arm][\runalt]]\one\{\vt[\eventalt][\runalt]\}$ and using a union bound we get
%
\begin{equation}
    \notag
    \prob\left(\sum_{\runalt=1}^{\run}
    \abs{(\vtav[\valuev][\runalt][\vt[\arm][\runalt]]-\vav[\meanReward][\vt[\arm][\runalt]])\one\{\vt[\eventalt][\runalt]\}}
    \ge 4\sqrt{\vta[\pullcount][\run][\eventalt]\log(1/\alt{\smallproba})}
    + 4\log(1/\alt{\smallproba})
    \right) \le  \frac{\log(\run)\alt{\smallproba}}{\log(2)}.
\end{equation}
%
We obtain \eqref{eq:indicator-estimate-concentration} by dividing the inequality in $\prob$ by $\max(1,\vta[\pullcount][\run][\eventalt])$ and choose $\alt{\smallproba}=(\log(2)/\log(\run))\smallproba<1/e$.
\end{proof}

\begin{lemma}
Suppose that $\vav[\snoise][0]$ satisfies the Bernstein condition \eqref{eq:Bernstein} with $\noisedev=1$ and its variance is bounded by $1$.
Let $\smallproba\in(0,1/e)$. It holds
\begin{equation}
    \notag
    \prob
    \left(
    \abs{\vtav[\est{\meanReward}][\run][0] - \vav[\meanReward][0]}
    \ge
    4\sqrt{\frac{\log(2\run/\alt{\smallproba})}{\vtav[\pullcount][\run][0]}}
    + \frac{4\log(2\run/\alt{\smallproba})}{\vtav[\pullcount][\run][0]}
    \right)
    \le \smallproba.
\end{equation}
\end{lemma}
\begin{proof}
The result is immediate from \cref{lem:indicator-concentration} with the choice $\vt[\eventalt][\runalt]=\{\indv\notin\va[\variables][\runalt]\}$.
We also use the inequality $\log(\run)/(\log(2)\max(1,\vtav[\pullcount][\run][0]))\le2\run/\vtav[\pullcount][\run][0]$ and the fact that $\vav[\meanReward][\vt[\arm][\runalt]]\one\{\indv\notin\va[\variables][\runalt]\}=\vav[\meanReward][0]\one\{\indv\notin\va[\variables][\runalt]\}$.
\end{proof}

==> Appendices/Missing.tex <==
\input{Tables/Notations}


==> Appendices/Related.tex <==
% In this appendix we complete our related work by providing comparison to some other models in the bandit literature.

\paragraph{Causal Bandits\afterhead}
The term causal bandits captures the general idea that in a bandit model the generation of reward may be governed by some causal mechanism while the actions correspond to interventions on the underlying causal graph.
This idea was first formalized in \citep{lattimore2016causal} and subsequently explored in a series of work \cite{lee2018structural,lu2020regret,nair2021budgeted} that cover multiples variants of the problem, including both the minimization of simple and cumulative regrets.
Our problem fits into the causal bandit framework by regarding \cref{fig:model} as a simple causal graph where the variables consist of all the directed causes of the reward and the actions correspond to atomic interventions on the action nodes.
The observability of these direct causes are also key assumptions in many of the aforementioned works.
Moreover, in the unknown affected case our causal graph is in fact partially unknown.
This is an intriguing problem in causal bandits as argued by \citep{LMT21}.
While we have shown improvement of the algorithms for this specific model, a interesting question is whether similar improvement can still be shown in more general causal bandit models under the assumption that each actions only affects a limited number of variables of the causal graph.

\paragraph{Combinatorial Bandits\afterhead}
In combinatorial bandits~\cite{cesa2012combinatorial}, the learner selects at each round a subset of ground items depending on which the reward is computed.
In its simplest form, the reward is just the sum of the payoffs of the selected items.
Of particular relevance to us is the semi-bandit setting~\cite{CWY13,KWAS15}, which assumes that the payoffs of the selected items are also observed.
This structure of the reward and observability of individual payoffs both suggest a strong similarity between our model and semi-bandits.
However, this comes with an important conceptual difference: the set of items, or variables, for which we observe the outcomes are selected in semi-bandits, while for us they are fixed and inherent to the reward generation mechanism.
As an example, in example \ref{ex:movie}, combinatorial bandit models optimize the number of movies that are watched among the recommended ones, while we also consider non-recommended movies.
In fact, as argued in \citep{WLCB20}, a recommendation is only effective if the user actually watches the movie and would not watch it without the recommendation

On the other hand, mathematically, it is possible to fit our model into the stochastic combinatorial semi-bandit framework when the sets of affected variables are known.
For this, consider a semi-bandit problem with $\nVariables+\sum_{\arm\in\arms}\va[\nAffected]$ items that correspond to the random variables $\setdef{\vav[\valuev][0]}{\indv\in\variables}\union\bigcup_{\arm\in\arms}\setdef{\vav[\valuev]}{\indv\in\va[\variables]}$.
At each round, the learner selects $\nVariables$ items that depends on the taken action and observes the payoffs of the selected items.
More precisely, when action $\arm$ is taken, the selected items are $\setdef{\vav[\valuev][0]}{\indv\in\setcomplement{\va[\variables]}}\union\setdef{\vav[\valuev]}{\indv\in\va[\variables]}$.

In terms of algorithm, let us consider the \UpUCBwb algorithm described in \cref{algo:UpUCB}, which is based on selecting the action with the largest uplift index $\vta[\UPindexSum]=\sum_{\indv\in\va[\variables]}(\vtav[\UCBindex]-\vtav[\UCBindex][\run][0])$.
We notice that the quantity $\vta[\UCBindex]=\sum_{\indv\in\variables}\vtav[\UCBindex]=\vta[\UPindexSum]+\sum_{\indv\in\variables}\vtav[\UCBindex][\run][0]$ is indeed an upper confidence bound on the reward of action $\arm$ and \UpUCBwb is equivalent to choosing the action with the largest $\vta[\UCBindex]$ in each round.
This observation indeed reduces \UpUCBwb to CombUCB~\cite{CWY13,KWAS15} on the transformed model.
Nonetheless, the \UpUCBwb formulation has several advantages:
\begin{enumerate}[topsep=2pt, itemsep=1.5pt, parsep=2pt, leftmargin=*]%[\itshape i\upshape)]
    \item It captures the fact that we really care about is the uplifting effect and the variables affected by each action.
    \item The uplifting interpretation facilitates algorithm design in more involved situations as we have shown in \cref{sec:unknown-affected}.
    \item While the general analysis of CombUCB yields a regret in %$\bigoh((\nVariables+\sqrt{\nVariables\nArms\nAffected})\sqrt{\nRuns\log\nRuns})$ and
    $\bigoh((\nVariables^2+\nVariables\nArms\nAffected)\log\nRuns/\gapbandit)$, we have shown in \cref{thm:UpUCB-regret} that the regret of \UpUCBwb is in $\bigoh(\nAffected^2\log\nRuns/\gapbandit)$.
    Our analysis presented in \cref{apx:proof-UpUCBwb} also greatly benefits from the \UpUCBwb formulation of the algorihhm.
    %clearly indicates that the number of variables $\nVariables$ should have no effect in our regret bound, as we demonstrate immediately in the following theorem.
    %this will be discussed in more detail in the next paragraph. %\cref{subsec:UpUCB-regret}.
\end{enumerate}

% \vspace{0.4em}
% \begin{remark}
% With the CombUCB formulation of the algorithm, one can deduce the regret is in $\bigoh((\alt{\nVariables}\nArms\nAffected)\log\nRuns/\gapbandit)$
% %Indeed, it is rather straightforward to improve from $\nVariables$ to $\min(\nArms\nAffected,\nVariables)$
% by arguing that at most $\alt{\nVariables}\defeq\min(\nArms\nAffected,\nVariables)$ items are involved in the learning process.
% Our result further improves this by a factor of $\min(\nArms,\nVariables/\nAffected)$.
% \end{remark}




%The term uplift is borrowed from the field of uplift modeling \citep{radcliffe2007using,gutierrez2017causal}.
% We borrow the term uplift from {\em uplift modeling} \citep{radcliffe2007using,gutierrez2017causal}; the latter refers to a collection of techniques for modelling the incremental effect of an action on an individual's behavior.
% %The goal there is to design algorithms to model the incremental effect of an action on an individual's behavior
% At a high level, both uplifting modeling and \ac{MAB} %have the common goal of finding the optimal strategy
% are important tools for decision making, as they both help select an optimal action.
% Despite this apparent relation between the two concepts, few papers explicitly link them together.
% We believe this is because a combination of the two often just results in a redefinition of the reward, on top of which classic bandit algorithms can be applied. This approach was taken in \citep{sawant2018contextual,berrevoets2019optimising}.
% %Both papers alter the goal of the bandit problems and apply existing bandit algorithms to solve the transformed problem
% Instead, our paper
% %takes a different approach and
% focuses on bandit problems in which estimating the uplifts improves the statistical efficiency of the algorithms and designs algorithms for that purpose.

% To achieve this, we assume the reward to be the sum of a set of observable variables and leverage the \emph{sparsity} of an action's effects on these variables.
% The decomposition of reward and the observability of partial rewards also appear in semi-bandit \citep{CWY13,KWAS15}.
% However, there the reward is the sum of the the selected items while for us the set of variables is fixed for every action.
% On the other hand, understanding the benefit of sparsity in \ac{MAB} has been a research topic of emerging interest.
% Most of these works focus on sparsity of the parameter vectors in linear bandit, which could be of great interest in the high-dimensional setting, see \eg \citep{abbasi2012online,bastani2020online,hao2021information} and references therein.
% A notable exception is \citep{kwon2017sparse}, where the authors study a variant of the classical \ac{MAB} problem in which the sparsity is reflected by that fact that the number of arms with positive reward is small.
% Our work is orthogonal to all of these in that we look at a different form of sparsity. As we will see in \cref{subsec:contextual-linear}, while sparsity in parameter can be a cause of sparsity in action effect, the improvement of regret is established with a different mechanism.

%\citep{abbasi2012online,carpentier2012bandit,bastani2020online,hao2021information}


==> Appendices/UpUCB-GapUp-UBL.tex <==
% % \subsection{Known Lower Bound on Individual Uplift} \label{sec:part2}


% % \label{sec:part2}
% % Another type of knowledge that can help the learner exploit the structure is a lower bound on individual uplift.
% % This is defined as $\gapUplift>0$ such that for all $\arm\in\arms$ and $\indv\in\va[\variables]$, $\abs{\vav[\meanReward]-\vav[\meanReward][0]}\ge\gapUplift$.
% % Similar assumption were made by \citet{LMT21} to identify which node in the causal graph affects the reward variable.
% % Indeed, this gives us an indicator on how many times we need to take each action in order to identify all its affected variables.

% % Again in this scenario, we derive regret bounds for both when the baseline payoffs are known or not to the learner. 
% % Our algorithms combine UCB, successive elimination \cite{even2006action}, and the idea that the affected variables can be identified after an action is taken sufficiently many times.
% % Our regret bounds feature the ratio $\va[\gapbandit]/\gapUplift$, suggesting that this knowledge is helpful when $\gapUplift$ is relatively large. 
% % We defer details to~\cref{apx:unknown-affected-2}.

% In this second part of~\cref{sec:unknown-affected}, we assume a lower bound on individual uplift is known.
% This means the learner has access to $\gapUplift>0$ satisfying that for all $\arm\in\arms$ and $\indv\in\va[\variables]$, $\abs{\vav[\meanReward]-\vav[\meanReward][0]}\ge\gapUplift$.
% This gives us an indicator on how many times we need to take each action in order to identify all the affected variables. Similar assumption were made by \citet{LMT21} to identify which node in the causal graph affects the reward variable.

% Again in this scenario, we derive regret bounds for both when the baseline payoffs are known or not to the learner. 
% Our algorithms combine UCB, successive elimination \cite{even2006action}, and the idea that the affected variables can be identified after an action is taken sufficiently many times.
% Our regret bounds feature the ratio $\va[\gapbandit]/\gapUplift$, suggesting that this knowledge is helpful when $\gapUplift$ is relatively large. 

% %Our regret bound will feature the ratio $\va[\gapbandit]/\gapUplift$, suggesting that this information is helpful when $\gapUplift$ is relatively large.
% Hereinafter, for any $x,\alpha,\beta\in\R$ with $\alpha\le\beta$, we use $\clip(x,\alpha,\beta)$ to denote the clipping function that restricts $x$ to the interval $[\alpha,\beta]$, \ie $\clip(x,\alpha,\beta)=\max(\alpha,\min(\beta,x))$.

% \subsection{Known Baseline Payoffs}

% As we have seen in \cref{sec:unknown-affected},
% if the baseline payoffs $\va[\meanReward][0]$ are known, we can directly check whether $\vav[\meanReward][0]$ is in the confidence interval.
% Moreover, with the knowledge $\abs{\vav[\meanReward]-\vav[\meanReward][0]}\ge\gapUplift$ for all $\indv\in\va[\variables]$, we deduce that $\va[\variables]$ can be identified correctly with probability $1-2\nVariables\alt{\smallproba}$ after action $\arm$ is taken $\pullcount_0=\ceil{(8/\gapUplift^2)\log(1/\alt{\smallproba})}$ times.
% In fact, let $\vta[\valuev][1],\ldots,\vta[\valuev][\pullcount_0]$ be $\pullcount_0$ i.i.d. realizations of $\va[\valuev]\sim\va[\distribution]$ and $\vtav[\tilde{\meanReward}][\pullcount_0]=(\sum_{\run=1}^{\pullcount_0}\vtav[\valuev])/\pullcount_0$ be the empirical mean of variable $\indv$.
% %Choosing $\varepsilon\in(0,\gapUplift)$ such that $\pullcount_0=(8/(\gapUplift-\varepsilon)^2)\log(1/\alt{\smallproba})$.\footnote{Such $\varepsilon$ exists (and of course, is unique) because $\pullcount_0>(8/\gapUplift^2)\log(2\nVariables/\alt{\smallproba})$.}
% Applying the sub-Gaussian concentration inequality \eqref{eq:sub-Gaussian-concentration} gives
% %
% \begin{equation}
%     \prob\left(\abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward]}\ge\frac{\gapUplift}{2}\right)
%     \le2
%     \exp\left(-\frac{\pullcount_0\gapUplift^2}{8}\right)
%     \le 2\alt{\smallproba}.
%     %\frac{\alt{\smallproba}}{\nVariables}.
% \end{equation}
% %
% With a union bound we conclude that with probability at least $1-2\nVariables\alt{\smallproba}$ it holds for all $\indv$ that $\abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward]}<\gapUplift/2$.
% We distinguish between the following two situations
% %
% \begin{enumerate}
%     \item $\indv\in\va[\variables]$, then $\displaystyle \abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward][0]}\ge\abs{\vav[\meanReward]-\vav[\meanReward][0]}-\abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward]}>\gapUplift-\frac{\gapUplift}{2}=\frac{\gapUplift}{2}$.
%     \item $\indv\notin\va[\variables]$, then $\displaystyle \abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward][0]}=\abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward]}<\frac{\gapUplift}{2}$.
% \end{enumerate}
% %
% This implies that with the choice
% $\va[\setId] = \setdef{\indv\in\variables}{\abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward][0]}>\gapUplift/2}$, we have effectively $\prob(\va[\setId]=\va[\variables])\ge1-2\nVariables\alt{\smallproba}$.
% One natural algorithm is to thus first pull each arm $\pullcount_0$ times and run \UpUCB (\cref{algo:UpUCB-BL}) %(from~\cref{subsec:UpUCB-BL})
% in the remaining rounds by regarding $\va[\setId]$ as the variables that action $\arm$ affects.
% A direct computation shows that the regret of this algorithm is in
% $\bigoh(\sum_{\arm\in\arms:\va[\gapbandit]>0}(\va[\gapbandit]/\gapUplift+\va[\nAffected])^2\log\nRuns/\va[\gapbandit])$.
% %$\bigoh(\pullcount_0\sum_{\arm\in\arms}\va[\gapbandit]+(\nArms\nAffected^2)\log\nRuns/\gapbandit)$.

% However, $\pullcount_0$ can be arbitrarily large when $\gapUplift$ gets closer to $0$, and taking an action much fewer times is probably sufficient to deduce that action is not optimal (with high probability).
% We thus propose to implement the above idea in a more flexible manner:
% We run \UpUCB with the uplifting indices $\vta[\UPindexSum]=\sum_{\indv\in\vta[\setId]}(\vtav[\UCBindex]-\vav[\meanReward][0])$, where
% %
% \begin{equation}
%     \notag
%     \vta[\setId] =
%     \begin{cases}
%     \variables & \text{if} ~ \vta[\pullcount]<\pullcount_0,\\
%     \setdef{\indv\in\variables}{\abs{\vtav[\est{\meanReward}][\run][\vt[\arm]]-\vav[\meanReward][0]}>\gapUplift/2} & \text{otherwise}.
%     \end{cases}
% \end{equation}
% %
% %known baseline payoffs by assuming that all the actions affect all the variables.
% %Then, for each arm $\arm$, as long as its pull count exceeds $\pullcount_0$, we switch the index by considering $\va[\setId]$ as the affected set.
% This algorithm is summarized in \cref{algo:UpUCB-GapUp-BL} and has the following regret guarantee.

% \input{Algorithms/UpUCB_GapUp_BL}

% \begin{theorem}
% \label{thm:UpUCB-GapUp-BL-regret}
% Let $\alt{\smallproba}=\smallproba/(2\nArms\nVariables\nRuns)$. Then the regret of \UpUCBDelta (\cref{algo:UpUCB-GapUp-BL}), 
% with probability at least $1-\smallproba$, satisfies:
% %
% \begin{equation}
%     \label{eq:UpUCB-GapUp-BL-regret}
%     \vt[\reg][\nRuns] \le
%     \sum_{\arm\in\arms:\va[\gapbandit]>0}
%     \left(\frac{8\thinspace\clip(\va[\gapbandit]/\gapUplift,\va[\nAffected],\nVariables)^2\log(2\nArms\nVariables\nRuns/\smallproba)}{\va[\gapbandit]}+\va[\gapbandit]\right).
% \end{equation}
% \end{theorem}
% \begin{proof}
% As before, we prove \eqref{eq:UpUCB-GapUp-BL-regret} under the condition that $\event$ defined in \eqref{eq:UCB-L-event} occurs. Recall that we have shown in the proof of \cref{prop:UpUCB-L-BL-regret} that $\prob(\event)\ge1-\smallproba$ with our choice of $\alt{\smallproba}$, so this effectively leads to a high-probability regret bound.

% In the following we assume that $\event$ occurs and show that for any suboptimal action $\arm\in\arms$, it holds
% %
% \begin{equation}
%     \label{eq:UpUCB-GapUp-pullcount-bound}
%     \vta[\pullcount][\nRuns]
%     \le
%     \max\left(
%     \min\left(
%     \frac{8\log(1/\alt{\smallproba})}{\gapUplift^2},
%     \frac{8\nVariables^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right), \frac{8(\va[\nAffected])^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right)
%     +1.
% \end{equation}
% %
% The inequality \eqref{eq:UpUCB-GapUp-BL-regret} then follows directly from \eqref{eq:regret-decomp-apx} and a rearrangement of the terms.

% We first claim that for any $\arm\in\arms$ if $\vta[\pullcount]\ge\pullcount_0$ then $\vta[\setId]=\va[\variables]$.
% In fact, by the definition of $\pullcount_0$, $\vta[\pullcount]\ge\pullcount_0$ implies that $\vta[\radiusConf]<\gapUplift/2$.
% Therefore, as argued in the text, $\indv\in\vta[\setId]$ if and only if $\indv\in\va[\variables]$.
% Since $\vtav[\UPindex]\ge\vav[\meanUplift]$ for any $\arm$ and $\indv$, this also proves that $\vta[\UPindex]\ge\va[\uplift]$ always holds (we have either $\vta[\setId]=\variables$ or $\vta[\setId]=\va[\variables]$).

% Let $\run\in\intinterval{\nArms+1}{\nRuns}$ be the last time that a suboptimal action $\arm$ is taken so that $\vta[\pullcount][\nRuns]=\vta[\pullcount][\run-1]+1$.
% This indicates $\vta[\UPindexSum]\ge\vta[\UPindexSum][\run][\sol[\arm]]$, and hence $\vta[\UPindexSum]\ge\va[\uplift][\sol[\arm]]$.
% We distinguish between the following two cases:
% %
% \begin{enumerate}[itemsep=2.5pt,topsep=2.5pt,parsep=2.5pt]
%     \item $\vta[\pullcount][\run-1]<\pullcount_0$:
%     Then $\vta[\setId]=\variables$ so $\vta[\UPindexSum]=\sum_{\indv\in\variables}(\vtav[\UCBindex]-\va[\meanReward][0])
%     \le\va[\uplift]+2\nVariables\vta[\radiusConf][\run-1]$, which in turn leads to $\vta[\radiusConf][\run-1]\ge\va[\gapbandit]/(2\nVariables)$, or equivalently $\vta[\pullcount][\run-1]\le8\nVariables^2\log(1/\alt{\smallproba})/(\va[\gapbandit])^2$.
%     \item $\vta[\pullcount][\run-1]\ge\pullcount_0$:
%     Then $\vta[\setId]=\va[\variables]$ so $\vta[\UPindexSum]=\sum_{\indv\in\va[\variables]}(\vtav[\UCBindex]-\va[\meanReward][0])
%     \le\va[\uplift]+2\va[\nAffected]\vta[\radiusConf][\run-1]$, which in turn leads to $\vta[\radiusConf][\run-1]\ge\va[\gapbandit]/(2\va[\nAffected])$, or equivalently $\vta[\pullcount][\run-1]\le8(\va[\nAffected])^2\log(1/\alt{\smallproba})/(\va[\gapbandit])^2$.
% \end{enumerate}
% %
% Since we also have $\vta[\pullcount][\run-1]<\pullcount_0$ in the first case, the above gives
% %
% \begin{equation}
%     \notag
%     \vta[\pullcount][\run-1]
%     \le
%     \max\left(
%     \min\left(
%     \pullcount_0-1,\frac{8\nVariables^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right), \frac{8(\va[\nAffected])^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right).
% \end{equation}
% %
% Plugging in the definition of $\pullcount_0$ we get immediately \eqref{eq:UpUCB-GapUp-pullcount-bound}.
% \end{proof}

% \cref{thm:UpUCB-GapUp-BL-regret} shows that \cref{algo:UpUCB-GapUp-BL} provides a smooth transition between standard UCB and the strategy that identifies the affected variables of all the actions.
% When $\va[\gapbandit]/\gapUplift\ge\nVariables$, the loss of taking action $\arm$ is so large that UCB prevents it from being taken further even if $\vta[\pullcount]\le\pullcount_0$.
% Otherwise, the affected variables get identified after an action is taken sufficient number of times and the algorithm benefits from this knowledge to improve the estimate of the uplift.
% It is also quite straightforward to combine \cref{algo:UpUCB-L-BL} with \cref{algo:UpUCB-GapUp-BL} when both $\nAffected$ and $\gapUplift$ are known; this results in a regret bound that replaces $\clip(\va[\gapbandit]/\gapUplift,\va[\nAffected],\nVariables)$ by $\clip(\va[\gapbandit]/\gapUplift,\va[\nAffected],\nAffected)$ in \eqref{eq:UpUCB-GapUp-BL-regret}.

% \subsection{Unknown Baseline Payoffs}
% Several additional challenges emerge when we want to adapt the aforementioned strategies to the case where the baseline payoffs are unknown.
% First, without additional assumption, it is impossible to tell whether two arbitrarily close estimates indicate the same effect of two actions on a variable.
% Then, without a proper baseline to compare with, we can never exclude the possibility that all the variables are affected by all the actions.
% We will thus need to make the following much more stringent assumption.

% \begin{assumption}
% \label{asm:gapUplift-ubl}
% The effect of any two actions on a variable differ by at least $\gapUplift$ as long as one of them affects this variable, \ie for all $\arm\in\arms$, $\indv\in\va[\variables]$, and $\alt{\arm}\in\setexclude{\arms}{\{\arm\}}$, it holds $\abs{\vav[\meanReward]-\vav[\meanReward][\alt{\arm}]}\ge\gapUplift$.
% \end{assumption}

% \input{Algorithms/UpUCB_GapUp}

% In other words, $\gapbandit$ is not only a lower bound on individual uplift, but also a lower bound on (individual) effect gap.
% Second, with a UCB-style algorithm, the optimal actions may not be taken sufficiently many times, in which case we can only conservatively assume that they affect all the variables.
% This would incur additional regret in the analysis when $\va[\meanReward][0]$ is unknown. 
% %While this does not pose a problem when $\va[\meanReward][0]$ is known, it can cause extra regret when we apply the \ac{DiffUCB} principle.
% Therefore, we would like to ensure that all the (potentially optimal) actions are taken the same number of times at the point that the affected variables get identified.
% This leads to a two-stage method as described in \cref{algo:UpUCB-GapUp}.

% In the first stage, we perform successive elimination until the uneliminated actions are taken sufficiently many times.
% Here $\vta[\estalt{\reward}][\round]$ is the empirical estimate of the reward associated to action $\arm$ and $\vt[\radiusConf][\round]=\nVariables\sqrt{2\log(1/\alt{\smallproba})/\round}$ is the associated radius of confidence interval.
% %After that, we aggregate variables with close estimates.
% Subsequently, for each variable $\indv\in\variables$ we construct the set
% %
% \begin{equation}
%     \label{eq:setBaseEst}
%     \vv[\setBaseEst]
%     = \setdef{\arm\in\arms}{\exists\thinspace \armalt\in\setexclude{\arms}{\{\arm\}}, \vtav[\intConf][\run_0+1]\intersect\vtav[\intConf][\run_0+1][\armalt]\neq\varnothing},
% \end{equation}
% %
% where $\run_0$ is the number of iterations in the elimination phase and the confidence intervals are defined as in \eqref{eq:UCBs-arm}.
% If \cref{asm:gapUplift-ubl} is verified, then with high probability $\arm\in\vv[\setBaseEst]$ only if $\indv\notin\va[\variables]$.
% Therefore, the observed results from these arms can be used to estimate the baseline payoff of $\indv$.
% The identified variables for action $\arm\in\arms$ are then $\va[\setId]=\setdef{\indv\in\variables}{\arm\notin\vv[\setBaseEst]}$.

% The second stage of the algorithm reuses the idea from \UpUCBwb.
% We define the UCB indices following \eqref{eq:UCBs-arm} for $\arm\in\arms$ and for the baseline estimate we choose among $\vv[\setBaseEst]$ the action that is taken the most frequently whenever this set is non-empty. Otherwise we arbitrarily set it to $0$. That is,
% %
% \begin{equation}
%     \label{eq:UCBs-0-UpUCB-GapUp}
%     \vtav[\UCBindex][\run][0] = \begin{cases}
%     0
%     & \text{if} ~ \vv[\setBaseEst]=\varnothing,
%     \\
%     \vtav[\UCBindex][\run][\vtav[\arm][\run][0]] \text{ where $\vtav[\arm][\run][0]=\argmax_{\arm\in\vv[\setBaseEst]}\vta[\pullcount][\run-1]$} & \text {otherwise}.
%     \end{cases}
% \end{equation}
% %
% The uplifting indices that guide the decision of the algorithm are defined by $\vta[\UPindexSum]=\sum_{\indv\in\vta[\setId]}(\vtav[\UCBindex]-\vtav[\UCBindex][\run][0])$.

% As shown below, the regret of \cref{algo:UpUCB-GapUp} takes roughly the same form as the one in \cref{thm:UpUCB-GapUp-BL-regret}, but as in \cref{thm:UpUCB-regret}, the number of variables that an optimal action affects also plays a crucial role in the regret bound.


% % we form a partition of the remaining arms such that if two arms $\arm, \armalt$ belong to different cells of the partition then the confidence intervals $\vta[\intConf]$ and $\vta[\intConf][\run][\armalt]$ do not overlap.
% % Let us denote by $\vav[\arms]$ the cell that arm $\arm$ belongs to. The aggregated empirical means, pull counts, and UCB indices are defined as:
% % %
% % \begin{equation}
% %     \label{eq:UCBs-gapUplift}
% %     \vtav[\pullcount] = \sum_{\runalt=1}^{\run}\one\{\vt[\arm]\in\vav[\arms]\},
% %     ~~
% %     \vtav[\est{\meanReward}] =
% %     \frac{\sum_{\runalt=1}^{\run}\vtv[\valuev]\one\{\vt[\arm]\in\vav[\arms]\}}{\max(1, \vtav[\pullcount])},
% %     ~~
% %     \vtav[\UCBindex]
% %     = \vtav[\est{\meanReward}]
% %     + \sqrt{\frac{2\log(1/\alt{\smallproba})}{\vtav[\pullcount]}}.
% % \end{equation}
% % %
% % The learner then plays the action with the largest UCB index $\vta[\UCBindex]=\sum_{\indv\in\variables}\vtav[\UCBindex]$.
% % %The whole procedure is described in
% % Notice that if \cref{asm:gapUplift-ubl} is violated, the aggregation of the estimates may incur an additional regret in $\Theta(\nAffected\nRuns\gapUplift)$. 

% % \begin{remark}
% % We do not insist on the use of uplifting index here.
% % Otherwise, another alternative is to compare with some most pulled armed as in \cref{algo:UpUCB-L}.
% % However, we believe aggregating estimates that are close to each other is the most natural thing to do under the assumption that two actions cannot have arbitrarily similar effect on a variable unless they affect the variable in the same way.
% % \end{remark}

% \begin{theorem}
% \label{thm:UpUCB-GapUp-regret}
% Let \cref{asm:gapUplift-ubl} hold and $\alt{\smallproba}=\smallproba/(2\nArms\nVariables\nRuns)$.  Then the regret of \UpUCBDeltawb (\cref{algo:UpUCB-GapUp}), with probability at least $1-\smallproba$, satisfies:
% %
% \begin{equation}
%     \label{eq:UpUCB-GapUp-regret}
%     \vt[\reg][\nRuns] \le
%     \sum_{\arm\in\arms:\va[\gapbandit]>0}
%     \left(\frac{8\thinspace\clip(2\va[\gapbandit]/\gapUplift,\va[\nAffected]+\va[\nAffected][\sol[\arm]],2\nVariables)^2\log(2\nArms\nVariables\nRuns/\smallproba)}{\va[\gapbandit]}+\va[\gapbandit]\right).
% \end{equation}
% \end{theorem}
% \begin{proof}
% We shall again consider the event $\event$ defined in \eqref{eq:UCB-L-event}, which holds with probability $1-\smallproba$ as argued in the proof of \cref{prop:UpUCB-L-BL-regret}. Leveraging the decomposition in \eqref{eq:regret-decomp-apx} it is sufficient to prove that on $\event$ we have
% \begin{equation}
%     \label{eq:UpUCB-GapUp-noBL-pullcount-bound}
%     \vta[\pullcount][\nRuns]
%     \le
%     \max\left(
%     \min\left(
%     \frac{32\log(1/\alt{\smallproba})}{\gapUplift^2},
%     \frac{32\nVariables^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right), \frac{8(\va[\nAffected]+\va[\nAffected][\sol[\arm]])^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right)
%     +1.
% \end{equation}
% %
% We assume $\event$ happens in the rest of the proof.

% Let us first focus on the elimination phase, notice that event $\event$ implies $\abs{\vta[\estalt{\reward}][\round]-\va[\reward]}<\vt[\radiusConf][\round]$ for every $\arm\in\vt[\arms][\round]$.
% % We define the event
% % %
% % \begin{equation}
% %     \notag
% %     \event_1 =
% %     \left\{\forall\round\in\oneto{\pullcount_0},
% %     ~\forall\arm\in\arms,
% %     ~ \abs{\vta[\estalt{\reward}][\round]-\va[\reward]}<\nVariables\sqrt{\frac{2\log(1/\alt{\smallproba})}{\round}}\right\}
% % \end{equation}
% % %
% % Following the proof of \cref{lem:concentration-mean-a} and a union bound over $\arm\in\arms$, we know that $\prob(\event_1)\ge1-2\nArms\pullcount_0\alt{\smallproba}$.
% In this case, the optimal actions never get eliminated.
% In fact, if $\sol[\arm]\in\vt[\arms][\round]$, then for all $\arm\in\vt[\arms][\round]$ it holds that
% %
% \begin{equation}
%     \notag
%     \vta[\estalt{\reward}][\round][\sol[\arm]]
%     +2\vt[\radiusConf][\round]
%     \ge
%     \va[\reward][\sol[\arm]]+\vt[\radiusConf][\round]
%     \ge
%     \va[\reward][\arm]+\vt[\radiusConf][\round]
%     \ge \vta[\estalt{\reward}][\round][\arm],
% \end{equation}
% %
% As a consequence, we also have $\sol[\arm]\in\vt[\arms][\round+1]$ and we conclude by the principle of induction.
% With this we further deduce that all action
% $\arm$ with $\va[\gapbandit]\ge4\vt[\radiusConf][\round]$ gets eliminated
% %\nVariables\sqrt{2\log(1/\alt{\smallproba})/\round}$ 
% after it is taken at most $\round$ times.
% %must be eliminated at the latest in round $\round$. 
% To see this, notice that for such action we have
% %
% \begin{equation}
%     \notag
%     \vta[\estalt{\reward}][\round]+2\vt[\radiusConf][\round]
%     < \va[\reward]+3\vt[\radiusConf][\round]
%     = \va[\reward][\sol[\arm]]-\va[\gapbandit]+3\vt[\radiusConf][\round]
%     < \vta[\estalt{\reward}][\round][\sol[\arm]]
%     -\va[\gapbandit]+4\vt[\radiusConf][\round]
%     \le \vta[\estalt{\reward}][\round][\sol[\arm]].
% \end{equation}
% %
% Therefore, for all $\run$ in phase \rom{1} of the algorithm, it is true that
% %
% \begin{equation}
%     \label{eq:UpUCB-GapUp-noBL-pullcount-bound-I}
%     \vta[\pullcount]\le
%     \min\left(
%     \left\lceil\frac{32\log(1/\alt{\smallproba})}{\gapUplift^2}\right\rceil,
%     \left\lceil\frac{32\nVariables^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right\rceil
%     \right).
% \end{equation}
% %
% This suggests that inequality \eqref{eq:UpUCB-GapUp-noBL-pullcount-bound} holds if the algorithm terminates in the elimination phase.

% Otherwise, the algorithm constructs $\vv[\setBase]$'s, $\va[\setId]$'s, and switches to the \textsc{UpUCB} phase.
% Let us denote by $\vv[\setBase]=\setdef{\arm\in\arms}{\indv\notin\va[\variables]}$ the set of actions that do not affect variable $\indv$
% and let $\arms_{\text{res}}=\vt[\arms][\pullcount_0+1]$ be the actions that remain after phase \rom{1}.
% %$\pullcount_0=\ceil{(32/\gapUplift^2)\log(1/\alt{\smallproba})}$ be the number of times that the uneliminated arms are pulled in the first phase.
% We argue that the sets $\vv[\setBaseEst]$ are constructed such that when $\event$ occurs,
% \begin{enumerate}[\textup(\itshape i\textup)]
%     \item $\vv[\setBaseEst]\subseteq\vv[\setBase]$.
%     \item  If there exist $\arm,\armalt\in\arms_{\text{res}}\intersect\vv[\setBase]$ such that $\arm\neq\armalt$ then we also have $\arm,\armalt\in\vv[\setBaseEst]$.
% \end{enumerate}
% %
% The second point is proved by observing that under $\event$ we must have $\vav[\meanReward][0]\in\vtav[\intConf][\run_0+1]\intersect\vtav[\intConf][\run_0+1][\armalt]$ if $\arm,\armalt\in\arms_{\text{res}}\intersect\vv[\setBase]$.
% To show the first point, notice that after the elimination phase, each of the action in $\arms_{\text{res}}$ is taken exactly $\ceil{(32/\gapUplift^2)\log(1/\alt{\smallproba})}$ times and thus $\vta[\radiusConf][\run_0]\le\gapUplift/4$.
% By \cref{asm:gapUplift-ubl}, if $\arm\notin\vv[\setBase]$, then for all $\armalt\in\setexclude{\arms_{\text{res}}}{\{\arm\}}$ we have $\abs{\vav[\meanReward]-\vav[\meanReward][\alt{\arm}]}\ge\gapUplift$, which along with the definition of $\event$ implies $\vtav[\intConf][\run_0+1]\intersect\vtav[\intConf][\run_0+1][\armalt]=\varnothing$, and therefore $\arm\notin\vv[\setBaseEst]$.

% The rest of the proof follows closely that of \cref{thm:UpUCB-regret}.
% Suppose that a suboptimal action $\arm$ is taken at round $\run$ during phase \rom{2} of the algorithm.
% This means $\vta[\UPindexSum]\ge\vta[\UPindexSum][\run][\sol[\arm]]$ (recall that $\sol[\arm]\in\arms_{\text{res}}$ since $\event$ happens), \ie
% %
% \begin{equation}
%     \notag
%     \sum_{\indv\in\va[\setId]}(\vtav[\UCBindex][\run]-\vtav[\UCBindex][\run][0])
%     \ge
%     \sum_{\indv\in\va[\setId][\sol[\arm]]}
%     (\vtav[\UCBindex][\run][\sol[\arm]]-\vtav[\UCBindex][\run][0]).
% \end{equation}
% %
% Rearranging the terms we get 
% %
% \begin{equation}
%     \notag
%     \sum_{\indv\in\va[\setId]}\vtav[\UCBindex][\run]
%     +\sum_{\indv\in\setexclude{\va[\setId][\sol[\arm]]}{\va[\setId]}}
%     \vtav[\UCBindex][\run][0]
%     \ge
%     \sum_{\indv\in\va[\setId][\sol[\arm]]}
%     \vtav[\UCBindex][\run][\sol[\arm]]
%     +\sum_{\indv\in\setexclude{\va[\setId]}{\va[\setId][\sol[\arm]]}}
%     \vtav[\UCBindex][\run][0].
% \end{equation}
% %
% If $\indv\in\setexclude{\va[\setId][\sol[\arm]]}{\va[\setId]}$ then $\arm\in\vv[\setBaseEst]$.
% In particular, $\vv[\setBaseEst]\neq\varnothing$ so $\armalt=\vtav[\arm][\run][0]=\argmax_{\tilde{\arm}\in\vv[\setBaseEst]}\vta[\pullcount][\run-1][\tilde{\arm}]$ is well-defined and $\vtav[\UCBindex][\run][0]=\vtav[\UCBindex][\run][\armalt]$.
% With $\vv[\setBaseEst]\subseteq\vv[\setBase]$ we know that $\vav[\meanReward][\armalt]=\vav[\meanReward][0]$ and accordingly $\abs{\vtav[\meanReward][\run-1][\armalt]-\vav[\meanReward][0]}\le\vta[\radiusConf][\run-1][\armalt]$ by the fact that $\event$ happens.
% This shows $\vtav[\UCBindex][\run][0]\ge\vav[\meanReward][0]$.
% Moreover, $\vta[\pullcount][\run][\armalt]\ge\vta[\pullcount]$ by the choice of $\armalt$; hence, $\vtav[\UCBindex][\run][0]\le\vav[\meanReward][0]+2\vta[\radiusConf][\run-1][\armalt]\le\vav[\meanReward][0]+2\vta[\radiusConf][\run-1]$.
% The same argument applies to $\indv\in\setexclude{\va[\setId]}{\va[\setId][\sol[\arm]]}$, and the UCB indices of $\arm$ and $\sol[\arm]$ can be bounded from above and below as in previous proofs.
% In summary, we obtain
% %
% \begin{equation}
%     \notag
%     \sum_{\indv\in\va[\setId]}(\vav[\meanReward]+2\vta[\radiusConf][\run-1])
%     +\sum_{\indv\in\setexclude{\va[\setId][\sol[\arm]]}{\va[\setId]}}
%     (\vav[\meanReward][0]+2\vta[\radiusConf][\run-1])
%     \ge
%     \sum_{\indv\in\va[\setId][\sol[\arm]]}
%     \vav[\meanReward][\sol[\arm]]
%     +\sum_{\indv\in\setexclude{\va[\setId]}{\va[\setId][\sol[\arm]]}}
%     \vav[\meanReward][0].
% \end{equation}
% %
% Equivalently,
% %
% \begin{equation}
%     \label{eq:UpUCB-GapUp-radConf-larger-than}
%     2\card\left(\va[\setId]\union\va[\setId][\sol[\arm]]\right)\vta[\radiusConf][\run-1]
%     \ge
%     \sum_{\indv\in\va[\setId]\union\va[\setId][\sol[\arm]]}\vav[\meanReward][\sol[\arm]]
%     -\sum_{\indv\in\va[\setId]\union\va[\setId][\sol[\arm]]}\vav[\meanReward].
% \end{equation}
% %
% To conclude, we claim that
% %
% \begin{equation}
%     \label{eq:VV-equal}
%     \va[\setId]\union\va[\setId][\sol[\arm]]=\va[\variables]\union\va[\variables][\sol[\arm]].
% \end{equation}
% %
% Let us first show $\va[\variables]\subseteq\va[\setId]\subseteq\va[\variables]\union\va[\variables][\sol[\arm]]$.
% The first inclusion is a consequence of $\vv[\setBaseEst]\subseteq\vv[\setBase]$:
% %
% \begin{equation}
%     \notag
%     \indv\in\va[\variables] \implies
%     \arm\notin\vv[\setBase] \implies
%     \arm\not\in\vv[\setBaseEst] \implies
%     \indv\in\va[\setId].
% \end{equation}
% %
% As for the second inclusion we prove it's contrapositive:
% %
% \begin{equation}
%     \notag
%     \indv\notin\va[\variables]\union\va[\variables][\sol[\arm]] \implies
%     \arm,\sol[\arm]\in\arms_{\text{res}}\intersect\vv[\setBase] \implies
%     \arm,\sol[\arm]\in\vv[\setBaseEst] \implies
%     \indv\notin\va[\setId]
% \end{equation}
% %
% Notice that the second implication holds because $\arm$ is suboptimal and in particular $\arm\neq\sol[\arm]$.
% The inclusion $\va[\variables][\sol[\arm]]\subseteq\va[\setId][\sol[\arm]]\subseteq\va[\variables]\union\va[\variables][\sol[\arm]]$ can be proved in a similar way, and combining these results gives \eqref{eq:VV-equal}.
% Therefore, the \acl{RHS} of \eqref{eq:UpUCB-GapUp-radConf-larger-than} is exactly $\va[\gapbandit]$ while the \acl{LHS} of \eqref{eq:UpUCB-GapUp-radConf-larger-than} is bounded from above by $2(\va[\nAffected]+\va[\nAffected][\sol[\arm]])\vta[\radiusConf][\run-1]$.
% In consequence,
% %
% \begin{equation}
%     \notag
%     \vta[\pullcount][\run-1]
%     \le \frac{8(\va[\nAffected]+\va[\nAffected][\sol[\arm]])^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}.
% \end{equation}
% %
% Therefore, any suboptimal action that gets taken in the \textsc{UpUCB} phase satisfies
% %
% \begin{equation}
%     \notag
%     \vta[\pullcount][\nRuns]
%     \le \frac{8(\va[\nAffected]+\va[\nAffected][\sol[\arm]])^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}+1.
% \end{equation}
% %
% On the other hand, if an suboptimal action is not taken in the \textsc{UpUCB} phase then \eqref{eq:UpUCB-GapUp-noBL-pullcount-bound-I} applies, so in either case \eqref{eq:UpUCB-GapUp-noBL-pullcount-bound} is verified, which concludes the proof.
% \end{proof}

% \vspace{0.4em}
% \begin{remark}
% A natural candidate for $\vtav[\UCBindex][\run][0]$ is the one that uses aggregated information as in \eqref{eq:mean-estimate-0}.
% The problem of this choice is that how we aggregate the observations collected in the first phase are only determined at the end of the the phase, while this choice itself depends on these observations.
% Mathematically, this prevents us from defining a suitable martingale difference sequence for which we establish concentration bound.
% An easy fix is to only aggregate observations from the second phase, while the use of the observations from the first phase should be limited to those coming from just one arm.
% %in $\vv[\setBaseEst]$.
% \end{remark}

==> Figures/Exp-figure-targeted.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}{0.9\linewidth}
    \includegraphics[width=\linewidth]{Figures/averaged-uplift-with-true-data-stderr.pdf}
    \end{subfigure}
    \caption{Experimental results for the contextual combinatorial model.
    All the curves are averaged over $100$ runs and the shaded areas represent the standard errors.}
    \label{fig:exp-c2}
    %\vspace{-2ex}
    \vspace{-1em}
\end{figure*}

==> Sections/Checklist.tex <==



\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{We have discussed potential extensions, which reflects the limitation of the current work.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Provided in the supplmental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See \cref{sec:exp,apx:exp-c2,apx:exp-detail,apx:exp-add}.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See \cref{apx:exp-detail}}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{See \cref{apx:exp-detail}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> Sections/Lower-bounds.tex <==
This section presents lower bounds that justify our key modeling assumptions. In particular, we show that there would be a higher regret in absence of any of the following: \begin{enumerate*}[\textup(\itshape i\textup)]
\item Limited number of affected variables,
\item Side information about variables beyond just reward, and
\item Some prior knowledge on how the variables are affected.
\end{enumerate*}
The third point sets ground for \cref{sec:unknown-affected}, by showing that the learner needs some prior knowledge to exploit our problem structure.


%Subsequently, in \cref{subsec:lower-bound-information}, we introduce a general information-theoretic lower bounds for bandit problems with similar design, which serve as the main tool for proving the results in \cref{subsec:lower-bound-uplift}. Missing proofs are in~\cref{apx:lower-bound}.

% \todosk{Throughout the paper, we use "impact/impacted" and also "affect/affected". Are they the same, if so let us use the same words.}
% \todoyg{I think we only use impact as nouns and affect as verbs.}

%\subsection{Lower Bound for Uplifting Bandits}
%\label{subsec:lower-bound-uplift}

% For the sake of conciseness, in the following we say that an uplifting bandit has parameters $(\nArms,\nVariables,(\va[\gapbandit],\va[\nAffected])_{\arm\in\arms})$ if the number of actions, the number of variables, the suboptimality gaps, and the number of affected variables of this instance are respectively $\nArms$, $\nVariables$, $(\va[\gapbandit])_{\arm\in\arms}$, and $(\va[\nAffected])_{\arm\in\arms}$.
%refer to any instance of the uplifting bandit problem as described in \cref{sec:model} with $\nArms$ arms, $\nVariables$ variables, suboptimality gaps $(\va[\gapbandit])_{\arm\in\arms}$, and numbers of affected variables $(\va[\nAffected])_{\arm\in\arms}$ noise as a $1$-sub-Gaussian $(\nArms,\nVariables,(\va[\gapbandit],\va[\nAffected])_{\arm\in\arms})$ uplifting bandit instance.
In particular, these lower bounds show that there would be a higher regret in absence of any of the following: \begin{enumerate*}[\textup(\itshape i\textup)]
\item Limited number of affected variables,
\item Side information about variables beyond just reward, and
\item Some prior knowledge on how the variables are affected.
\end{enumerate*}
Moreover, we also derive matching lower bounds for \cref{prop:UpUCB-BL-regret}.
We discuss these results in \cref{apx:lower-bound-statement}.
Subsequently, we introduce a general information-theoretic lower bounds for bandit problems with similar design in \cref{apx:lower-bound-information}, based on which we prove the lower bounds in \cref{apx:proof-lower-bound}.


We focus on instance-dependent lower-bounds and assume that the learner has full knowledge of the baseline distribution.\footnote{%
Of course, the problem only becomes more challenging if the learner actually does not know the baseline distribution.}
These lower bounds are derived for the algorithms that are {\em consistent} \citep{LR85} over the class of $1$-sub-Gaussian uplifting bandits, which means the induced regret of the algorithm on any uplifting bandit with $1$-sub-Gaussian noise satisfies $\vt[\reg]=\smalloh(\run^p)$ for all $p>0$.
%We refer to such algorithms as {\em consistent algorithms}.
%for any instance of such problem, the induced regret of the algorithm on this instance satisfies $\vt[\reg]=\smalloh(\run^p)$ for all $p>0$.

% \begin{proof}
% The proof is deferred to \cref{apx:lower-bound} is based on the general lower bound \cref{lem:lower-bound-instance-dependent} introduced in \cref{subsec:lower-bound-information}.
% \end{proof}
\begin{proposition}[Informal]
\label{prop:lower-bound}
Let $\policy$ be a consistent algorithm over the class of $1$-sub-Gaussian uplifting bandits.
%that at most uses knowledge of $\va[\distribution][0]$, $(\va[\variables])_{\arm\in\arms}$, and the fact that the noise is $1$-sub-Gaussian.
If 
\begin{enumerate}[(a)]
    \item all the variables are affected by all the actions;
    \label{low-cond:affected}
    \item only the reward is observed; or
    \label{low-cond:observed}
    \item $\policy$ has no knowledge about $(\va[\meanReward])_{\arm\in\arms}$ (in particular, $(\va[\variables])_{\arm\in\arms}$ is not known),
    \label{low-cond:knowledge}
\end{enumerate}
Then, for any $\nArms,\nVariables>0$ and sequence $(\va[\nAffected],\va[\gapbandit])_{1\le\arm\le\nArms}\in(\oneto{\nVariables}\times\R_+)^{\nArms}$
%with $\va[\nAffected]\in\oneto{\nVariables}, \va[\nAffected][1]>\va[\gapbandit]\ge\max(0,\va[\nAffected][1]-\va[\nAffected])$ for all $\arm$ 
with $\va[\gapbandit][1]=0$, there exists a $1$-sub-Gaussian uplifting bandit 
whose number of actions, number of variables, suboptimality gaps, and numbers of affected variables are respectively $\nArms$, $\nVariables$, $(\va[\gapbandit])_{\arm\in\arms}$, and $(\va[\nAffected])_{\arm\in\arms}$,
%with parameters $(\nArms,\nVariables,(\va[\gapbandit],\va[\nAffected])_{\arm\in\arms})$
%a $1$-sub-Gaussian uplifting bandit instance with $\nArms$ arms, $\nVariables$ variables, suboptimality gaps $(\va[\gapbandit])_{\arm\in\arms}$, and numbers of affected variables $(\va[\nAffected])_{\arm\in\arms}$ 
such that the regret induced by $\policy$ on it satisfies
%
\begin{equation}
    %\label{eq:lower-bound-m}
    \notag
    \liminf_{\toinf[\nRuns]} \frac{\ex[\vt[\reg][\nRuns]]}{\log\nRuns} \ge \sum_{\arm\in\arms:\va[\gapbandit]>0}\frac{2\nVariables^2}{\va[\gapbandit]}.
\end{equation}
%
% Now, provided that the payoff vector $\vt[\valuev]$ is observed and that $(\va[\variables])_{\arm\in\arms}$ is known by the algorithm, there exists a $1$-sub-Gaussian uplifting bandit with the same parameters
% %
% \begin{equation}
%     \label{eq:lower-bound-L}
%     \liminf_{\toinf[\nRuns]} \frac{\ex[\vt[\reg][\nRuns]]}{\log\nRuns} \ge \sum_{\arm\in\arms:\va[\gapbandit]>0}\frac{2(\va[\nAffected])^2}{\va[\gapbandit]}.
% \end{equation} 
% \todob{Write ${L^a}^2$ as $(L^a)^2$.}
%
% Moreover, if $\policy$ can be implemented under either of the following conditions
% \begin{enumerate}[(a)]
%     \item Only the reward is observed.
%     \item The learner has no knowledge about $(\va[\meanReward])_{\arm\in\arms}$ (in particular, the learner does not know $(\va[\variables])_{\arm\in\arms}$).
%     %The learner cannot distinguish between any two bandits with the same baseline and noise distributions (in particular, the learner does not know $(\va[\variables])_{\arm\in\arms}$).
%     %The prior knowledge of the learner on the distributions is further restricted to the point that it does not enable the learner to distinguish between any two instances with the same baseline and noise distributions (in particular, the learner does not know $(\va[\variables])_{\arm\in\arms}$).
%     %does not encode any information about the means of the arms
%     %only encodes information about the baseline and the noise distributions.
%     %does not allow the leaner to know anything more than the baseline distribution and the covariance of the noise.
%     %is that the noise is $1$-sub-Gaussian, \ie $\priorknow(\va[\distribution][0],\va[\distribution][1],\ldots,\va[\distribution][\nArms])=\priorknow(\va[\distribution][0],\va[\distributionalt][1],\ldots,\va[\distributionalt][\nArms])$ as long as $\va[\distribution]$'s and $\va[\distributionalt]$'s satisfy \cref{asm:noise}.
%     %The learner has no prior knowledge on how the variables are affected.\footnote{Formally, as we will see in the proof, this means that for a fixed baseline distribution, the prior knowledge of the learner does not allow they to distinguish between two instances whose mean values $(\va[\meanReward])_{\arm\in\arms}$ are arbitrarily different.}
% \end{enumerate}
% Then, there exists a $1$-sub-Gaussian uplifting bandit with parameters $(\nArms,\nVariables,(\va[\gapbandit],\va[\nAffected])_{\arm\in\arms})$ where the regret of $\policy$ is
% \begin{equation}
%     \label{eq:lower-bound-m}
%     \liminf_{\toinf[\nRuns]} \frac{\ex[\vt[\reg][\nRuns]]}{\log\nRuns} \ge \sum_{\arm\in\arms:\va[\gapbandit]>0}\frac{2\nVariables^2}{\va[\gapbandit]}.
% \end{equation}
\end{proposition}
%



The proof of \cref{prop:lower-bound} is deferred to \cref{apx:lower-bound}, where we also present an alternative statement of the proposition that implies the optimality of \cref{prop:UpUCB-BL-regret} and 
%\cref{apx:proof-lower-bound}.
a general information-theoretic lower bound for bandit problems with similar design based on which \cref{prop:lower-bound} is established.
%The key idea is to find a class of bandits that is indistinguishable to the learner under their prior knowledge, and for a specific instance of this class show that each suboptimal action necessarily gets taken a certain number of times because some other instances of the class can provide very similar feedback.
%two instances of this class can provide similar feedback so that each suboptimal arm needs to be pulled a certain number of times 
%\todobmargin{I am not 100\% sold on how the lower bounds are presented. It seems that \eqref{eq:lower-bound-m} should go first, because it shows that the world is hard if nothing is known. \eqref{eq:lower-bound-L} shows that $\Omega(L^2)$ regret is needed under reasonable assumptions, which we match starting with Algorithm 1. The lower should perhaps go even before Section 3.}

%We will consider models with $1$-sub-Gaussian noise and mean values $\vav[\meanReward]\in[0,1]$.
%For ease of presentation, this will not be mentioned explicitly in the problem statements but whenever we mention an uplifting bandit instance one should keep in mind that it is an uplifting bandit instance satisfying these assumptions.

As promised, \cref{prop:lower-bound} justifies the importance of the three crucial components of our model.
The intuition behind the lower bounds under conditions \ref{low-cond:affected} and \ref{low-cond:observed} is that smaller regret can only be achieved when the noise in the effect of an action is small, and when the observation of the learner of this effect is not deteriorated by the noise.
%Finally, Condition (b) in~\cref{prop:lower-bound} along with inequality \eqref{eq:lower-bound-m} indicates that the structure of the problem and the side information can only be exploited when the learner is equipped with some knowledge about $(\va[\meanReward])_{\arm\in\arms}$.
%For example, if the learner knows $(\va[\variables])_{\arm\in\arms}$, they can infer that $\vav[\meanReward]=\vav[\meanReward][0]$ whenever $\indv\notin\va[\variables]$.
To understand the lower bound under condition \ref{low-cond:knowledge}, we notice that with finite observations, two problem instances with different structures (\eg different $(\va[\variables])_{\arm\in\arms}$) can provide arbitrary close information to the learner, and thus the learner is doomed to treat them equally if they are not equipped with any prior knowledge that enables them to distinguish between the two problems.
Accordingly, the learner is not able to take advantage of the underlying structure, and no improvement of the performance can be achieved.
%In this regard, the knowledge on $(\va[\meanReward])_{\arm\in\arms}$ actually allows the learner to distinguish between two such instances and treat them differently, which results in an improvement of the regret.


%First, inequality \eqref{eq:lower-bound-L} shows that the regret of the algorithm must scale with $\va[\nAffected]$, the number of variables each action affects.
%Therefore, no improvement can be achieved if the limited number of affected assumption is violated.
%
%Next, condition (a) along with inequality \eqref{eq:lower-bound-m} reveals the necessity of having additional observations.
%Observing the reward itself is not sufficient for getting rid of the dependence on $\nVariables$.
%The intuition behind these two lower bounds is that smaller regret can only be achieved when the noise in the effect of an action is small, and when the observation of the learner of this effect is not deteriorated by the noise.
%\todosk{we say that we need "additional observations" but that does not imply that all variables be observed, if so should we clarify?}

% Finally, Condition (b) in~\cref{prop:lower-bound} along with inequality \eqref{eq:lower-bound-m} indicates that the structure of the problem and the side information can only be exploited when the learner is equipped with some knowledge about $(\va[\meanReward])_{\arm\in\arms}$.
% For example, if the learner knows $(\va[\variables])_{\arm\in\arms}$, they can infer that $\vav[\meanReward]=\vav[\meanReward][0]$ whenever $\indv\notin\va[\variables]$.
% To see why such knowledge is required, we notice that with finite observations, two problem instances with different structures (\eg different $(\va[\variables])_{\arm\in\arms}$) can provide arbitrary close information to the learner, and thus the learner is doomed to treat them equally. This prevents the learner from taking advantage of the underlying structure of the problem.
% In this regard, the knowledge on $(\va[\meanReward])_{\arm\in\arms}$ actually allows the learner to distinguish between two such instances and treat them differently, which results in an improvement of the regret.
%Further examples of such knowledge are provided in \cref{sec:unknown-affected}.


==> Tables/RegretsCopy.tex <==
\begin{table*}[!ht]
\renewcommand{\arraystretch}{1.2}
\hspace*{-.2in}
\begin{center}
\begin{small}
\begin{tabularx}{0.97\textwidth}{c|a|cc|cc|cc}
\toprule
%\multirow{2}{*}{Algorithm} & Standard & \UpU & \UpU &  \UpU & \UpU & \UpU & \UpU \\  
% & UCB & \textup{(b)} & & -\textup{nAff\,(b)} & -\textup{nAff} & -iLift\,\textup{(b)} & -iLift \\ \midrule%\hline
Algorithm & UCB & \UpUCB & \UpUCBwb & \UpUCBL & \UpUCBLwb & \UpUCBDelta & \UpUCBDeltawb     \\ \hline \hline
%Affected variables & & & & & & & \\
Affected variables known & No & Yes & Yes & No & No & No & No \\ %\hline
%Baseline payoffs & & & & & & & \\
Baseline payoffs known & No & Yes & No & Yes & No & Yes & No \\[2pt] %\hline
\hline
\rule{0pt}{2.6ex} Regret Bound & $\nArms\nVariables^2/\gapbandit$ & 
\multicolumn{2}{c|}{ $\nArms\nAffected^2/\gapbandit$} & 
\multicolumn{2}{c|}{ $\nArms\nAffected^2/\gapbandit$} & 
\multicolumn{2}{c}{$\nArms\min(\max(\gapbandit/\gapUplift,\nAffected),\nVariables)^2/\gapbandit$}  \\ \bottomrule
\end{tabularx}
\caption{Summary of our regret bounds for uplifting bandits. Constant and logarithmic factors are ignored throughout.
%$\nArms$ and $\nVariables$ are respectively the number of arms and the number of variables.
For simplicity, we assume here all the actions affect exactly $\nAffected$ of the $\nVariables$ variables and all the suboptimal actions have the same suboptimality gap $\gapbandit$.
\todosk{define $K$,$L$,$M$}}
%$\clip$ denotes the clipping function that restricts the value of its first variable to the range defined by its second and third variable, \ie $\clip(x,\alpha,\beta)=\max(\alpha,\min(\beta,x))$.
%\todob{It does not seem that we ever refer to this table. We should, since we state it upfront.}}
%\vspace{0.4em}
\label{tab:summary}
\end{small}
\end{center}
\vspace{-1em}
\end{table*}

==> Uplifting bandits - arxiv/Algorithms/C2UpUCB.tex <==
\begin{algorithm}[t]
    \caption{\CUpUCB} 
    %for $\arms=\setdef{\arm\in\intinterval{0}{\nTreatments}^\nVariables}{\norm{\arm}_0\le\nAffected}$}
    \label{algo:C2UpUCB}
\begin{algorithmic}[1]
    \STATE {\bfseries Input:} Budget constraint $\nAffected$, Parameters for computing the UCBs indices
    \FOR{$\run = 1, \ldots, \nRuns$}
    %\FOR{$\indtreat\in\treatments\union\{0\}$ and $\indv\in\variables$}
    \FOR{$\indv\in\variables$}
    \STATE Compute UCB indices $(\vtav[\UCBindex][\run][\indtreat])_{\indtreat\in\{0, 1\}}$
    %for $\va[\objalt][\indtreat](\vtv[\feature])$
    \STATE Compute uplifting index $\vtv[\UPindex][\run]$
    \hfill
    \COMMENT{$\vtv[\UPindex][\run]=\vtav[\UCBindex][\run][1]-\vtav[\UCBindex][\run][0]$}~~
    %\ENDFOR
    % \STATE $\vtv[\indtreat] = \argmax_{\indtreat\in\treatments_0}\vtav[\UPindex][\run][\indtreat]$
    % \STATE $\vtv[\UPindex]
    % = \max_{\indtreat\in\treatments_0}\vtav[\UPindex][\run][\indtreat]$
    \ENDFOR
    %\STATE For all $\indv\in\arms$, compute maximum uplifting treatment $\vtv[\indtreat]$ and uplifting index $\vtv[\UPindex]$ as in \eqref{eq:uplifting-treatment-customer}
    %\STATE Let $\vt[\variables]$ be the set of the $\nAffected$ customers with largest $\vtv[\UPindex]$
    \STATE Set $\vt[\variables]\subs\argmax_{\set\subset\variables,\card(\set)\le\nAffected}\sum_{\indv\in\set}\vtv[\UPindex]$
    \STATE Select action $\vt[\arm]=(\one\{\indv\in\vt[\variables]\})_{\allvariables}$
    \hfill
    \COMMENT{this defines the set of treated customers}~~%with $\vtv[\arm]=\vtv[\indtreat]$ if $\indv\in\vt[\variables]$ and $\vtv[\arm]=0$ otherwise
    \ENDFOR
\end{algorithmic}
\end{algorithm}

==> Uplifting bandits - arxiv/Algorithms/C2UpUCB_MT.tex <==
\begin{algorithm}[tb]
    \caption{\CUpUCBMwb}
    \label{algo:C2UpUCB-mt}
\begin{algorithmic}[1]
    \STATE {\bfseries Input:} Budget constraint $\nAffected$, 
    Parameters for computing the UCBs indices, Treatment set $\treatments_0$
    %Error probability $\smallproba$,
    %Regularization parameter $\regpar$
    %\STATE {\bfseries Initialization:} Serve each customer with each treatment once and update the UCBs as in \eqref{eq:UCBs-treatment}
    \FOR{$\run = 1, \ldots, \nRuns$}
    \FOR{$\indv\in\variables$}
    \STATE Compute UCB indices $(\vtav[\UCBindex][\run][\indtreat])_{\indtreat\in\treatments_0}$ for $(\va[\objalt][\indtreat](\vtv[\feature]))_{\indtreat\in\treatments_0}$
    \hfill
    \COMMENT{use \eqref{eq:UCBs-treatment-contextual} for linear payoffs}~~
    %$\vtav[\UCBindex][\run][\vtv[\arm]]$ for $\indv\in\vt[\variables]$ and $\vtav[\UCBindex][\run][0]$ for $\indv\in\setcomplement{\vt[\variables]}$ as in \eqref{eq:UCBs-treatment}
    \STATE Compute uplifting indices $(\vtav[\UPindex][\run][\indtreat])_{\indtreat\in\treatments}$ %defined by
    \hfill
    \COMMENT{$\vtav[\UPindex][\run][\indtreat]=\vtav[\UCBindex][\run][\indtreat]-\vtav[\UCBindex][\run][0]$}~~
    \STATE Compute presumed optimal treatment $\vtv[\indtreat]$ and uplifting index $\vtv[\UPindex]$ 
    \hfill
    \COMMENT{use \eqref{eq:uplifting-treatment-customer}}~~
    \ENDFOR
    %\STATE Let $\vt[\variables]$ be the set of the $\nAffected$ customers with largest $\vtv[\UPindex]$
    \STATE Set $\vt[\variables]\subs\argmax_{\set\subset\variables,\card(\set)\le\nAffected}\sum_{\indv\in\set}\vtv[\UPindex]$
    \hfill
    \COMMENT{this defines the set of treated customers}~~
    \STATE Select action $\vt[\arm]\subs(\vtv[\indtreat]\one\{\indv\in\vt[\variables]\})_{\allvariables}$
    \hfill
    \COMMENT{$\vtv[\arm]=\vtv[\indtreat]$ if $\indv\in\vt[\variables]$; $\vtv[\arm]=0$ otherwise}~~
    \ENDFOR
\end{algorithmic}
\end{algorithm}

==> Uplifting bandits - arxiv/Algorithms/UpUCB_BL.tex <==

%\setcounter{algorithm}{-1}
\begin{algorithm}[t!]
    \caption{\UpUCB} %: known affected variables, unknown baseline payoffs}
    \label{algo:UpUCB-BL}
\begin{algorithmic}[1]
    \STATE {\bfseries Input:} Error probability $\alt{\smallproba}$, Baseline payoffs $\va[\meanReward][0]$, Sets of affected variables $\setdef{\va[\variables]}{\arm\in\arms}$ 
    \STATE {\bfseries Initialization:} Take each action once
    %and compute the UCB indices as in \eqref{eq:UCBs}
    \FOR{$\run = \nArms+1, \ldots, \nRuns$}
    \STATE Compute the statistics following \eqref{eq:mean-estimate-a}
    \STATE For $\arm\in\arms$, compute uplifting index $\vta[\UPindexSum]\subs\sum_{\indv\in\va[\variables]}(\vtav[\est{\meanReward}][\run-1]+\vta[\radiusConf][\run-1]-\vav[\meanReward][0])$
    %\vfill
    %\COMMENT{$\vtav[\est{\meanReward}][\run-1] + \vta[\radiusConf][\run-1]$}
    %\STATE \COMMENT{Compuation of uplifting indices}
    %\STATE For $\arm\in\arms$, set $\vta[\UPindexSum]\subs\sum_{\indv\in\va[\variables]}(\vtav[\UCBindex]-\vtav[\UCBindex][\run][0])$
    \STATE Select action $\vt[\arm]\in\argmax_{\arm\in\arms}\vta[\UPindexSum]$
    %\STATE Update the UCB indices following \eqref{eq:UCBs}
    \ENDFOR
\end{algorithmic}
\end{algorithm}


==> Uplifting bandits - arxiv/Algorithms/UpUCB_GapUp.tex <==
\begin{algorithm}[tb]
    \caption{\UpUCBDeltawb} %: unknown affected variables, unknown baseline payoffs}
    \label{algo:UpUCB-GapUp}
\begin{algorithmic}[1]
    \STATE {\bfseries Input:} Error probability $\alt{\smallproba}$, Lower bound on effect gap $\gapUplift$
    \vskip 0.1em
    \STATE {\bfseries Initialization:}
    Set $\run\subs0$,  $\vt[\arms][1]\subs\arms$, and $\pullcount_0\subs\ceil{(32/\gapUplift^2)\log(1/\alt{\smallproba})}$
    \STATE \texttt{\underline{Phase \rom{1}: Successive elimination}}
    \vskip 0.3em
    \FOR{$\round = 1, \ldots, \pullcount_0$}
    \IF{$\nRuns-\run\ge\card(\vt[\arms][\round])$}
    \STATE Take each action $\arm\in\vt[\arms][\round]$ once
    \STATE Set $\run\subs\run+\card(\vt[\arms][\round])$
    
    \STATE Compute the empirical estimates $\vta[\estalt{\reward}][\round]$ for $\arm\in\vt[\arms][\round]$ and the radius of confidence interval $\vt[\radiusConf][\round]$
    \STATE Update active set
    $\vt[\arms][\round+1]\subs\setdef{\arm\in\vt[\arms][\round]}{
    \vta[\estalt{\reward}][\round]+2\vt[\radiusConf][\round]\ge
    \max_{\armalt}\vta[\estalt{\reward}][\round][\armalt] }$
    \ELSE
    \STATE Take $\nRuns-\run$ actions from $\vt[\arms][\round]$ and terminate the algorithm
    \ENDIF
    \ENDFOR
    %\STATE \texttt{\underline{Estimate aggregation}}
    \vskip 0.1em
    \STATE \texttt{\underline{Phase \rom{2}: UpUCB}}
    \vskip 0.3em
    %\STATE Set $\run_0\subs\run$ and $\radiusConf\subs\sqrt{\frac{2\log(1/\alt{\smallproba})}{\round}}$
    %\STATE FOR each $\indv\in\variables$, FORm a partition
    %$\{\set_1(\indv),\ldots,\set_{q(\indv)}(\indv)\}$
    %of $\vt[\arms][\round]$ such that if two actions $\arm, \armalt$ belong to different cells of the partition then $\abs{\vtav[\est{\meanReward}]-\vtav[\est{\meanReward}][\run][\armalt]}\ge\gapUplift$
    \STATE Construct the sets $\vv[\setBaseEst]$ as in \eqref{eq:setBaseEst} and $\va[\setId]\subs\setdef{\indv\in\variables}{\arm\notin\vv[\setBaseEst]}$
    \FOR{$\run = \run+1, \ldots, \nRuns$}
    \STATE Compute the UCB indices following \eqref{eq:UCBs-arm},\eqref{eq:UCBs-0-UpUCB-GapUp}
    \STATE For $\arm\in\vt[\arms][\pullcount_0+1]$, compute uplifting index $\vta[\UPindexSum]\subs\sum_{\indv\in\va[\setId]}(\vtav[\UCBindex]-\vtav[\UCBindex][\run][0])$
    \STATE Select action $\vt[\arm]\in\argmax_{\arm\in\vt[\arms][\round]}\vta[\UPindexSum]$
    \ENDFOR
\end{algorithmic}
\end{algorithm}

==> Uplifting bandits - arxiv/Algorithms/UpUCB_GapUp_BL.tex <==
\begin{algorithm}[tb]
    \caption{\UpUCBDelta} %: unknown affected variables, known baseline payoffs}
    \label{algo:UpUCB-GapUp-BL}
\begin{algorithmic}[1]
    \STATE {\bfseries Input:} Error probability $\alt{\smallproba}$, Baseline payoffs $\va[\meanReward][0]$, Lower bound on individual uplift $\gapUplift$
    \STATE {\bfseries Initialization:} Take each action once;
    Set $\pullcount_0\subs\ceil{(8/\gapUplift^2)\log(1/\alt{\smallproba})}$ and $\va[\setId]\subs\variables$
    \FOR{$\run = \nArms+1, \ldots, \nRuns$}
    \STATE Compute the UCB indices following \eqref{eq:UCBs-arm}
    \STATE For $\arm\in\arms$, compute uplifting index $\vta[\UPindexSum]\subs\sum_{\indv\in\va[\setId]}(\vtav[\UCBindex]-\vav[\meanReward][0])$
    \STATE Select action $\vt[\arm]\in\argmax_{\arm\in\arms}\vta[\UPindexSum]$
    \IF{$\vta[\pullcount][\run][\vt[\arm]]\ge\pullcount_0$}
        \STATE Set $\va[\setId][\vt[\arm]]\subs\setdef{\indv\in\variables}{\abs{\vtav[\est{\meanReward}][\run][\vt[\arm]]-\vav[\meanReward][0]}>\gapUplift/2}$
    \ENDIF
    \ENDFOR
\end{algorithmic}
\end{algorithm}

==> Uplifting bandits - arxiv/Algorithms/UpUCB_L_BL.tex <==
\begin{algorithm}[tb]
    \caption{\UpUCBL} %: unknown affected variables; known baseline payoffs}
    \label{algo:UpUCB-L-BL}
\begin{algorithmic}[1]
    \STATE {\bfseries Input:} Error probability $\alt{\smallproba}$, Baseline payoffs $\va[\meanReward][0]$, Upper bound $\nAffected$ on the number of affected variables
    \STATE {\bfseries Initialization:} Take each action once
    \FOR{$\run = \nArms+1, \ldots, \nRuns$}
    \FOR{$\arm\in\arms$}
        \STATE Compute UCBs, uplifting indices,
        %$(\vtav[\UCBindex])_{\allvariables}$, $(\vtav[\UPindex])_{\allvariables}$ 
        and confidence intervals 
        %$(\vtav[\intConf])_{\allvariables}$ 
        following \eqref{eq:UCBs-arm}
        %$\vtav[\UCBindex]$ and $\vtav[\intConf]$ following \eqref{eq:UCBs-arm}
        %\STATE For all $\indv\in\variables$, compute $\vtav[\UPindex]=\vtav[\UCBindex]-\vav[\meanReward][0]$
        %\STATE \COMMENT{\textit{Identify affected variables}}
        \STATE Set $\vta[\setId] \subs \setdef{\indv\in\variables}{\vav[\meanReward][0]\notin\vtav[\intConf]}$
        %\label{algline: identification}
        %\IF{$\card(\vta[\setId])<\nAffected$}
        %\STATE \COMMENT{\textit{Pad with variables with highest UCBs on uplifts}}
        %\STATE $\vta[\setLargeUp]\subs\argmax\setdef{\sum_{\indv\in\setLargeUp}\vtav[\UPindex]}
        %{\setLargeUp\subseteq\setexclude{\variables}{\vta[\setId]},
        %\card(\setLargeUp)=\max(0, \nAffected-\card(\vta[\setId]))}$ %\ref{algline: identification}
        \STATE Set $\vta[{\nAffected}] \subs \max(0, \nAffected-\card(\vta[\setId]))$
        \STATE Set $\displaystyle \vta[\setLargeUp] \subs
            \argmax_{\substack{\setLargeUp\subseteq\setexclude{\variables}{\vta[\setId]}\\
            \card(\setLargeUp)=\vta[{\nAffected}]}}
            \sum_{\indv\in\setLargeUp}\vtav[\UPindex]$
        %\ELSE
        %\todob{I wonder why this is needed. $\card(\vta[\setId]) \geq \nAffected$ does not happen with a high probability, right? Can we simplify the algorithm? I would think that computing the UCB on the uplift from top $L$ variables under each action would work.}
        %\todoyg{Taking $\card(\setLargeUp)=\nAffected$ results in a regret of the same order, but we lose a multiplicative constant. (negative lift)}
        %\STATE $\vta[\setLargeUp]\subs\varnothing$
        %\ENDIF
        \STATE Compute uplifting index $\vta[\UPindexSum]\subs\sum_{\indv\in\vta[\setId]\union\vta[\setLargeUp]}\vtav[\UPindex]$ %\todob{Ambiguous notation, since $\rho_t^a$ is also a vector of UCBs on each lift.}
    \ENDFOR
    \STATE Select action $\vt[\arm]\in\argmax_{\arm\in\arms}\vta[\UPindexSum]$
    %\STATE Update the UCB indices and the confidence intervals following \cref{eq:UCBs-arm}
    \ENDFOR
\end{algorithmic}
\end{algorithm}

==> Uplifting bandits - arxiv/Algorithms/UpUCB_L_WB.tex <==
\begin{algorithm}[tb]
    \caption{\UpUCBLwb} %: unknown affected variables; unknown baseline payoffs}
    \label{algo:UpUCB-L}
\begin{algorithmic}[1]
    \STATE {\bfseries Input:} Error probability $\alt{\smallproba}$, Upper bound $\nAffected$ on the number of variables that each action affects 
    \STATE {\bfseries Initialization:} Take each action once
    \FOR{$\run = \nArms+1, \ldots, \nRuns$}
    \STATE Choose $\vt[\mostpullarm]\in\argmax_{\arm\in\arms}\vta[\pullcount][\run-1]$
    and compute UCBs and confidence intervals using \eqref{eq:UCBs-arm}
    \FOR{$\arm\in\arms$}
        %\STATE \COMMENT{Identify affected variables}
        \STATE Set $\vta[\setId]\subs\setdef{\indv\in\variables}
        {\vtav[\intConf]\intersect\vtav[\intConf][\run][\vt[\mostpullarm]]=\varnothing}$
        \STATE For $\indv\in\variables$, compute $\vtav[\UPindex]\subs\vtav[\UCBindex]-\vtav[\UCBindex][\run][\vt[\mostpullarm]]$
        \STATE Set $\vta[{\nAffected}] \subs \max(0, 2\nAffected-\card(\vta[\setId]))$
        \STATE Set
        $\displaystyle \vta[\setLargeUp] \subs
        \argmax_{\substack{\setLargeUp\subseteq\setexclude{\variables}{\vta[\setId]},\\
        \card(\setLargeUp)\le\vta[{\nAffected}]}}
        \sum_{\indv\in\setLargeUp}\vtav[\UPindex]$
         \STATE Compute uplifting index $\vta[\UPindexSum]\subs\sum_{\indv\in\vta[\setId]\union\vta[\setLargeUp]}\vtav[\UPindex]$
    \ENDFOR
    \STATE Select action $\vt[\arm]\in\argmax_{\arm\in\arms}\vta[\UPindexSum]$
    \ENDFOR
\end{algorithmic}
\end{algorithm}
%\vspace{-1em}

==> Uplifting bandits - arxiv/Algorithms/UpUCB_WB.tex <==
\begin{algorithm}[tb]
    \caption{\UpUCBwb} %: known affected variables, unknown baseline payoffs}
    \label{algo:UpUCB}
\begin{algorithmic}[1]
    \STATE {\bfseries Input:} Error probability $\alt{\smallproba}$, the sets of variables each action affects $\setdef{\va[\variables]}{\arm\in\arms}$ 
    \STATE {\bfseries Initialization:} Take each action once 
    %and compute the UCB indices as in \eqref{eq:UCBs}
    \FOR{$\run = \nArms+1, \ldots, \nRuns$}
    \STATE Compute the UCB indices following \eqref{eq:UCBs}
    %\STATE \COMMENT{Compuation of uplifting indices}
    \STATE For $\arm\in\arms$, set $\vta[\UPindexSum]\subs\sum_{\indv\in\va[\variables]}(\vtav[\UCBindex]-\vtav[\UCBindex][\run][0])$
    \STATE Select action $\vt[\arm]\in\argmax_{\arm\in\arms}\vta[\UPindexSum]$
    %\STATE Update the UCB indices following \eqref{eq:UCBs}
    \ENDFOR
\end{algorithmic}
\end{algorithm}

==> Uplifting bandits - arxiv/Appendices/C2UpUCB.tex <==


% In this appendix, we formally introduce the problem of contextual combinatorial uplifting bandit with linear payoffs and provide an analysis thereof.

% % \paragraph{Contextual Combinatorial (C2) Uplifting Bandit\afterhead}
% % \label{subsec:C2UpBandit}
% %\input{Algorithms/C2UpUCB}
% To demonstrate the flexibility of our framework, we consider in this section another contextual extension that tackles the problem of targeted campaign. %(think of a personalized version of example \ref{ex:marketing}). 
% Throughout the section, we refer to the variables as individuals (customers) that we may want to treat (serve) with some treatment (campaign). %$\treatments=\intinterval{1}{\nTreatments}$.
% To improve the overall return on investment, it is often beneficial to treat only a subset of the individuals.
% The bandit problem thus consists of finding the right set of individuals to treat at each round.

In this appendix, we discuss in more detail the problem of contextual combinatorial uplifting bandit that we introduced in \cref{subsec:C2UpBandit}.
We extend the model and the algorithm to the case of multiple treatments in \cref{apx:c2-model}.
Subsequently, we specify the algorithm for the case of linear expected payoffs and present some associated analysis in \cref{apx:c2-linear}.
Numerical experiments conducted with the Criteo Uplift Prediction Dataset are presented in \cref{apx:exp-c2}.

\subsection{Model and Algorithm Template}
\label{apx:c2-model}

Let us consider a pool of $\nVariables$ individuals that may change from round to round, associated with (time-dependent) contexts $(\vtv[\feature])_{\indv\in\variables}$ with $\vtv[\feature]\in\R^\vdim$,
and a set of treatments that can be applied to the individuals.
For convenient, we also write $\treatments_0=\treatments\union\{0\}$, where, as before, $0$ indicates that no treatment is applied to an individual.
%be a set of treatments that can be applied to the individuals and $\treatments_0=\treatments\union\{0\}$ where $0$ indicates that no treatment is applied to an individual.
Following \cref{sec:context},
we consider the action set
%The underlying action set is now 
$\arms=\setdef{\arm\in(\treatments_0)^{\nVariables}}{\norm{\arm}_0\le\nAffected}$,
which encodes the constraint that at most $\nAffected$ individuals can be treated in each run.
Similarly, we associate each treatment with a function $\va[\objalt][\indtreat]$.
The reward and the uplift of choosing action $\arm$ in round $\run$ are given then by
%
\begin{equation}
    \notag
    \va[\reward](\vt[\feature]) = \sum_{\allvariables}\va[\objalt][\vv[\arm]](\vtv[\feature]),
    ~~~
    \va[\up{\reward}](\vt[\feature]) = \sum_{\indv\in\va[\variables]}
    \va[\objalt][\vv[\arm]](\vtv[\feature])-\va[\objalt][0](\vtv[\feature]).
\end{equation}
%
The problem thus consists in finding both the set of customers to treat and the treatments to apply to these customers at each round.
To adapt \CUpUCB to this situation, we define a treatment-dependent uplifting index $\vtav[\UPindex][\run][\indtreat]=\vtav[\UCBindex][\run][\indtreat]-\vtav[\UCBindex][\run][0]$ where $\vtav[\UCBindex][\run][\indtreat]$ and $\vtav[\UCBindex][\run][0]$ are respectively upper confidence bounds on $\va[\objalt][\vv[\arm]](\vtv[\feature])$ and $\va[\objalt][0](\vtv[\feature])$.
Again, if $\va[\objalt][0]$ is known, 
$\vtav[\UCBindex][\run][0]$ can be simply taken as $\va[\objalt][0](\vtv[\feature])$.
%in the definition of $\vtav[\UPindex][\run][\indtreat]$.
Next, at each time step $\run$, we define the presumed optimal treatment for individual $\indv$ and the associated uplifting index as
%
\begin{equation}
    \label{eq:uplifting-treatment-customer}
    \vtv[\indtreat] = \argmax_{\indtreat\in\treatments}\vtav[\UPindex][\run][\indtreat],
    ~~~~~
    \vtv[\UPindex]
    = \vtav[\UPindex][\run][\vtv[\indtreat]]
    = \max_{\indtreat\in\treatments}\vtav[\UPindex][\run][\indtreat].
\end{equation}
%
The adapted \CUpUCB algorithm then chooses the $\nAffected$ customers with the largest uplifting index and for each of these customers chooses their presumed optimal treatment. The resulting algorithm (referred to as \CUpUCBMwb) is summarized in \cref{algo:C2UpUCB-mt} .

\input{Algorithms/C2UpUCB_MT}



\subsection{Linear Expected Payoffs}
\label{apx:c2-linear}

To provide a concrete algorithm and its analysis thereof, let us assume that $\va[\objalt][\indtreat]$ is linear in the feature vector with some unknown coefficient vector $\va[\param][\indtreat]$, \ie $\va[\objalt][\indtreat](\vtv[\feature])=\product{\va[\param][\indtreat]}{\vtv[\feature]}$.
Then, we can construct upper confidence bounds for $\va[\objalt][\indtreat](\vtv[\feature])$ following the ideas of linear UCB \citep{APS11}.
To begin, for each $\indtreat\in\treatments_0$ and $\run\in\intinterval{1}{\nRuns}$, we define
%
\begin{equation}
    \notag
    \vta[\variables][\run][\indtreat]
    = \setdef{\indv\in\variables}{\vtv[\arm]=\indtreat}
    %~~~~~
    %\vta[\points][\run][\indtreat]
    %= \setdef{\vtv[\feature]}{\indv\in\vta[\variables][\run][\indtreat]}
\end{equation}
%
as the set of customers that receive treatment $\indtreat$ in round $\run$.
Fix a regularization parameter $\regpar>0$, we further define the following $\vdim\times\vdim$ matrix and $\vdim$-dimensional vector
%
\begin{equation}
    \label{eq:definition-Vtz}
    \vta[\LSmat][\run][\indtreat] = \regpar\Id + \sum_{\runalt=1}^{\run}\sum_{\indv\in\vta[\variables][\runalt][\indtreat]}
    \vtv[\feature][\runalt]\vtv[\feature][\runalt]^{\top},
    ~~~~~
    \vta[\LSvec][\run][\indtreat]
    = \sum_{\runalt=1}^{\run}\sum_{\indv\in\vta[\variables][\runalt][\indtreat]}
    \vtv[\valuev][\runalt]\vtv[\feature][\runalt].
\end{equation}
%
The regularized least-square estimate of $\va[\param][\indtreat]$ is then given by $\vta[\est{\param}][\run][\indtreat]= (\vta[\LSmat][\run][\indtreat])^{-1}\vta[\LSvec][\run][\indtreat]$.
The UCB index is of the form
%
\begin{equation}
    \label{eq:UCBs-treatment-contextual}
    \vtav[\UCBindex][\run][\indtreat] = \product{\vta[\est{\param}][\run-1][\indtreat]}{\vtv[\feature]}
    +\vt[\radiusEllipConf]\norm{\vtv[\feature]}_{(\vta[\LSmat][\run-1][\indtreat])^{-1}}.
\end{equation}
%
for some $\vt[\radiusEllipConf]$ that is properly chosen.



\paragraph{Regret Guarantee.}
In this part, we provide regret analysis for \cref{algo:C2UpUCB-mt} when
\begin{enumerate*}[\itshape i\upshape)]
\item the baseline payoffs are unknown,
\item the expected payoffs are linear, and
\item the UCB indices are computed following \eqref{eq:UCBs-treatment-contextual}.
\end{enumerate*}
For technical reasons, we will assume the noises $\vtv[\snoise]$ to be mutually independent (here $\vtv[\snoise]=\vtv[\valuev]-\product{\va[\param][\indtreat]}{\vtv[\feature]}$).
We comment on this assumption in \cref{rem:independence-noise}.

The theorem below establishes a high-probability regret bound for \CUpUCBMwb when the above conditions are satisfied.


\begin{theorem}
\label{thm:C2UpUCB-regret}
Assume that $\norm{\vtv[\feature]}\le1$ for all $\run$ and $\indv$ and $(\vtv[\snoise])_{\allvariables}$ are mutually independent and $1$-sub-Gaussian (conditioning on the past).
Let $\parambound>0$ such that $\norm{\va[\param][\indtreat]}\le\parambound$ for all $\indtreat\in\treatments_0$.
Then if \CUpUCBMwb (\cref{algo:C2UpUCB-mt}) is run with the UCB indices defined in \eqref{eq:UCBs-treatment-contextual} under the parameter choices
%
\begin{equation}
    \notag
    \vt[\radiusEllipConf]
    =\sqrt{\regpar}\parambound
    +\sqrt{2\log\left(\frac{\nTreatments+1}{\smallproba}\right)
    +\vdim\log\left(1+\frac{\nVariables\run}{\vdim\regpar}\right)},
\end{equation}
%
and $\regpar\ge\nAffected$, it holds, with probability at least $1-\smallproba$, that
%
\begin{equation}
    \label{eq:C2UpUCB-regret}
    \vt[\reg][\nRuns]
    \le
    4
    \sqrt{
    \vdim\nAffected(\nTreatments+1)\nRuns
    \log\left(1+\frac{\nAffected\nRuns}{\vdim\regpar}\right)
    }
    \left(
    \sqrt{\regpar}\parambound
    +\sqrt{2\log\left(\frac{\nTreatments+1}{\smallproba}\right)
    +\vdim\log\left(1+\frac{\nVariables\nRuns}{\vdim\regpar}\right)}
    \right)
    .
\end{equation}
\end{theorem}

\cref{thm:C2UpUCB-regret} provides a regret bound in $\tbigoh(\sqrt{\max(\vdim,\nAffected)\vdim\nTreatments\nAffected\nRuns})$.
We observe that the dependence on $\nVariables$ is only logarithmic.
In fact, $\nVariables$ plays no role in either the number of parameters to estimate (which is $(\nTreatments+1)\vdim$) or the scale of the noise (which is in $\bigoh(\sqrt{\nAffected})$).
Ideally, we would like to remove completely the dependence on $\nVariables$.
However, we are not able to achieve this in our proof, and we leave whether this is possible or not as an open question.
Finally, due the mutual independence of noises, the regret only scales with $\sqrt{\nAffected}$ as long as $\nAffected\le\vdim$.


\begin{remark}
\label{rem:independence-noise}
The $\log(\nVariables)$ factor appears because $\vta[\est{\param}][\run][0]$ is estimated using feedback from roughly $\nVariables\nRuns$ samples (see \cref{lem:conf-ellip} below).
This is also the reason why we need mutual independence of the noises, since otherwise, this estimation may cause the regret to get $\sqrt{\nVariables}$ larger.
It can be easily verified that the dependence on $\nVariables$ can be completely removed when the baseline payoffs are known and used for computing the uplifting indices.
In this case, we can also show if the noises are not mutually independent, multiplying the second term of $\vt[\radiusEllipConf]$ by $\sqrt{\nAffected}$ still guarantees a regret in $\tbigoh(\vdim\nAffected\sqrt{\nTreatments\nRuns})$.
What is at stake here is \cref{lem:conf-ellip} that we present below, as the size of the confidence ellipsoid varies for different underlying assumptions.
%With the same proof techniques, we can show that when the independence assumption is violated,
%multiplying the second term of the radius of the confidence ellipsoid by respectively $\sqrt{\nAffected}$ and $\sqrt{\nVariables}$ when $\indtreat\in\treatments$ and $\indtreat=0$ recovers the high-probability guarantee.
%This however causes the final regret bound to get $\Theta(\sqrt{\nVariables})$ times larger in the worst case, while we conjecture it is possible to get a regret bound in $\tbigoh(\vdim\nAffected\sqrt{\nTreatments\nRuns})$ for this problem.
\end{remark}


\paragraph{Analysis\afterhead}
To prove \cref{thm:C2UpUCB-regret}, we need to show that $\vtav[\UCBindex]$ as defined in \eqref{eq:UCBs-treatment-contextual} is indeed an upper confidence bound on $\product{\va[\param][\indtreat]}{\vtv[\feature]}$.
This step is based on the following lemma which establishes the confidence ellipsoids of the estimated parameters.
In fact, $\vtav[\UCBindex]$ defined in \eqref{eq:UCBs-treatment-contextual} can be regarded as the largest estimated payoff that one can get from choosing a parameter from the confidence ellipsoid.
%deduced from choosing a parameter from the confidence ellipsoid that gives the largest estimated payoff.

\begin{lemma}
\label{lem:conf-ellip}
Assume that $\norm{\vtv[\feature]}\le1$ for all $\run$ and $\indv$ and $(\vtv[\snoise])_{\allvariables}$ are mutually independent and $1$-sub-Gaussian (conditioning on the past).
For all $\indtreat\in\treatments_0$ and $\alt{\smallproba}\in(0,1)$, with probability at least $1-\alt{\smallproba}$ it holds for all $\run$ that
%
\begin{equation}
    \notag
    \begin{aligned}
    \norm{\va[\param][\indtreat]-\vta[\est{\param}][\run][\indtreat]}_{\vta[\LSmat][\run][\indtreat]}
    &\le
    \sqrt{\regpar}\norm{\va[\param][\indtreat]}
    + \sqrt{2\log\left(\frac{1}{\alt{\smallproba}}\right)
    +\log\left(\frac{\det(\vta[\LSmat][\run][\indtreat])}{\regpar^{\vdim}}\right)}\\
    &\le
    \sqrt{\regpar}\norm{\va[\param][\indtreat]}
    +\sqrt{2\log\left(\frac{1}{\alt{\smallproba}}\right)
    +\vdim\log\left(1+\frac{\nVariables\run}{\vdim\regpar}\right)}.
    \end{aligned}
\end{equation}
\end{lemma}
\begin{proof}
This is an immediate corollary of \cite[Th. 2]{APS11}.
Since $(\vtv[\snoise])_{\allvariables}$ are mutually independent, we can apply this theorem by arranging $(\vtv[\snoise])_{\indv\in\vta[\variables][\run][\indtreat]}$ in some arbitrary order $\vtv[\snoise][\run][\indv_1],\ldots,\vtv[\snoise][\run][\indv_{\card(\vta[\variables][\run][\indtreat])}]$ so that $\vtv[\snoise][\run][\indv_{\indg}]$ is $1$-sub-Gaussian conditioning on $(\bigcup_{\runalt<\run}\setdef{\vtv[\snoise][\runalt]}{\indv\in\vta[\variables][\runalt][\indtreat]})\union\{\vtv[\snoise][\run][\indv_{\indg'}]\}_{1\le \indg'\le \indg}$.

For the second inequality, we notice that $\tr(\vta[\LSmat][\run][\indtreat])\le\vdim\regpar+\sum_{\runalt=1}^{\run}\sum_{\indv\in\vta[\variables][\runalt][\indtreat]}\norm{\vtv[\feature]}^2\le\vdim\regpar+\nVariables\run$.
It thus follows from the AM–GM inequality on the eigenvalues of $\vta[\LSmat][\run][\indtreat]$, $\det(\vta[\LSmat][\run][\indtreat])\le(\tr(\vta[\LSmat][\run][\indtreat])/\vdim)^\vdim$.
\end{proof}

%Before tackling the proof of the theorem, we present another lemma that we will use to bound the sum of the suboptimality gaps.
The lemma below will also be useful for bounding the regret.

\begin{lemma}
\label{lem:Vt-norm-det-bound}
Consider subsets of the variables $\vt[\variables][1],\ldots,\vt[\variables][\nRuns]\subset\variables$ and define $\vt[\LSmat]=\regpar\Id+\sum_{\runalt=1}^{\run}\sum_{\indv\in\vt[\variables][\runalt]}\vtv[\feature][\runalt]\vtv[\feature][\runalt]^{\top}$.
If $\regpar\ge\max_{\run\in\oneto{\nRuns}}\card(\vt[\variables])$ and $\norm{\vtv[\feature]}\le1$ for all $\run$ and $\indv$, it holds that
%
\begin{equation}
    \notag
    \sum_{\run=1}^{\nRuns}
    \sum_{\indv\in\vt[\variables]}\norm{\vtv[\feature]}_{\vt[\LSmat][\run-1]^{-1}}^2
    \le 2\log\left(\frac{\det(\vt[\LSmat][\nRuns])}{\regpar^{\vdim}}\right)
    \le
    2\vdim\log\left(
    1+\frac{\sum_{\run=1}^{\nRuns}\card(\vt[\variables])}{\vdim\regpar}
    \right)
    .
\end{equation}
\end{lemma}
\begin{proof}
For all $\run\ge1$, we have
%
\begin{equation}
    \notag
    \vt[\LSmat][\run]
    =\vt[\LSmat][\run-1]+\sum_{\indv\in\vt[\variables]}\vtv[\feature]\vtv[\feature]^{\top}
    =\vt[\LSmat][\run-1]^{1/2}
    \left(\Id + \sum_{\indv\in\vt[\variables]}\vt[\LSmat][\run-1]^{-1/2}\vtv[\feature]\vtv[\feature]^{\top}\vt[\LSmat][\run-1]^{-1/2}\right)
    \vt[\LSmat][\run-1]^{1/2}
\end{equation}
%
Thus, with $\vtv[\wvec]=\vt[\LSmat][\run-1]^{-1/2}\vtv[\feature]$, we get
%
\begin{equation}
    \label{eq:det-decomp}
    \det(\vt[\LSmat][\run])
    = \det(\vt[\LSmat][\run-1])
    \det\left(\Id+\sum_{\indv\in\vt[\variables]}\vtv[\wvec]\vtv[\wvec]^{\top}\right).
\end{equation}
%
Regarding $\{\vtv[\wvec]\}_{\indv\in\vt[\variables]}$ as column vectors, we denote by their horizontal concatenation as $\wmat\in\R^{\vdim\times\vt[\nVariables]}$, where $\vt[\nVariables]=\card(\vt[\variables])$.
%=(\vtv[\wvec][\run][1] ~ \ldots ~ \vtv[\wvec][\run][\vt[\nVariables]])\in\R^{\vdim\times\vt[\nVariables]}$ where $\vt[\nVariables]=\card(\vt[\variables])$.
We have $\wmat\wmat^{\top}=\sum_{\indv\in\vt[\variables]}\vtv[\wvec]\vtv[\wvec]^{\top}$.
Let the eigenvalues of $\wmat\wmat^{\top}$ be denoted by $\eigv_1,\ldots,\eigv_{\vdim}$, then clearly $\det(\Id+\wmat\wmat^{\top})=\prod_{\indg=1}^{\vdim}(1+\eigv_{\indg})$.
On the other hand, $\sum_{\indg=1}^{\vdim}\eigv_{\indg}=\tr(\wmat\wmat^{\top})=\tr(\wmat^{\top}\wmat)=\sum_{\indv\in\vt[\variables]}\norm{\vtv[\wvec]}^2$. From the non-negativity of the eigenvalues of $\wmat\wmat^{\top}$, we obtain
%
\begin{equation}
    \label{eq:det-inequa}
    \det(\Id+\wmat\wmat^{\top})=\prod_{\indg=1}^{\vdim}(1+\eigv_{\indg})
    \ge 1 + \sum_{\indg=1}^{\vdim}\eigv_{\indg}
    = 1 + \sum_{\indv\in\vt[\variables]}\norm{\vtv[\wvec]}^2
    = 1 + \sum_{\indv\in\vt[\variables]}\norm{\vtv[\feature]}_{\vt[\LSmat][\run-1]^{-1}}^2.
\end{equation}
%
Applying \eqref{eq:det-decomp} and \eqref{eq:det-inequa} recursively leads to
%
\begin{equation}
    \label{eq:det-inequa-recur}
    \det(\vt[\LSmat][\nRuns])
    \ge \det(\regpar\Id)
    \prod_{\run=1}^{\nRuns}
    \left(1 + \sum_{\indv\in\vt[\variables]}\norm{\vtv[\feature]}_{\vt[\LSmat][\run-1]^{-1}}^2\right)
    =
    \regpar^{\vdim}
    \prod_{\run=1}^{\nRuns}
    \left(1 + \sum_{\indv\in\vt[\variables]}\norm{\vtv[\feature]}_{\vt[\LSmat][\run-1]^{-1}}^2\right).
\end{equation}

We now turn back to bound $\sum_{\indv\in\vt[\variables]}\norm{\vtv[\feature]}_{\vt[\LSmat][\run-1]^{-1}}^2$.
Since $\regpar\ge\max_{\run\in\oneto{\nRuns}}\card(\vt[\variables])$ and $\norm{\vtv[\feature]}\le1$, we have
%
\begin{equation}
    \label{eq:sum-log-bound}
    \sum_{\indv\in\vt[\variables]}\norm{\vtv[\feature]}_{\vt[\LSmat][\run-1]^{-1}}^2
    = \min\left(1, \sum_{\indv\in\vt[\variables]}\norm{\vtv[\feature]}_{\vt[\LSmat][\run-1]^{-1}}^2\right)
    \le 2\log\left(1+ \sum_{\indv\in\vt[\variables]}\norm{\vtv[\feature]}_{\vt[\LSmat][\run-1]^{-1}}^2\right).
\end{equation}
%
Combining \eqref{eq:det-inequa-recur} and \eqref{eq:sum-log-bound} we get the first inequality.
The second inequality is proved as in \cref{lem:conf-ellip}.
\end{proof}


We are now ready to prove \cref{thm:C2UpUCB-regret}.
The first part of the proof reuses the trick that we have seen several times before, notably in the proof of \cref{thm:UpUCB-regret}.
We rearrange the UCB indices and show that the suboptimality gaps can be bounded from above by the sum of the radii of certain confidence intervals. The details will be omitted.
Next, we apply \cref{lem:Vt-norm-det-bound} to bound the sum of these upper bounds and conclude.

\begin{proof}[Proof of \cref{thm:C2UpUCB-regret}]
For any $\indtreat\in\treatments_0$,
choosing $\alt{\smallproba}=\smallproba/(\nTreatments+1)$ in \cref{lem:conf-ellip} gives 
\[
\prob\left(\{\exists \run, \norm{\va[\param][\indtreat]-\vta[\est{\param}][\run][\indtreat]}^2_{\vta[\LSmat][\run][\indtreat]}>\vt[\radiusEllipConf]\right)\ge \frac{\smallproba}{\nTreatments+1}.
\]
With a union bound we thus deduce that with probability at least $1-\smallproba$, the inequality $\norm{\va[\param][\indtreat]-\vta[\est{\param}][\run][\indtreat]}^2_{\vta[\LSmat][\run][\indtreat]}\le\vt[\radiusEllipConf]$ holds for all $\run$ and $\indtreat$.
This also implies that for all $\run$ and $\indtreat$, we have
%
\begin{equation}
    \label{eq:contextual-estimate-product-diff}
    \abs{
    \product{\va[\param][\indtreat]}{\vtv[\feature]}
    -\product{\vta[\est{\param}][\run-1][\indtreat]}{\vtv[\feature]}}
    \le \vt[\radiusEllipConf]\norm{\vtv[\feature]}_{(\vta[\LSmat][\run-1][\indtreat])^{-1}}
\end{equation}
%
In the following, we will prove \eqref{eq:C2UpUCB-regret} under the condition that \eqref{eq:contextual-estimate-product-diff} holds, which happens with probability at least $1-\smallproba$ as we just showed.

Let $\run\ge 1$ and $\vt[\sol[\arm]]\in\argmax_{\arm\in\arms} \sum_{\allvariables}\product{\va[\param][\vv[\arm]]}{\vtv[\feature]}$ be an optimal action of this round.
The algorithm chooses $\vt[\arm]$ that maximizes $\vta[\UPindex]=\sum_{\indv\in\va[\variables]}(\vtav[\UCBindex]-\vtav[\UCBindex][\run][0])$, and thus
%
\begin{equation}
    \label{eq:contextual-pf-UCB-diff}
    \sum_{\indv\in\va[\variables][\vt[\arm]]}(\vtav[\UCBindex][\run][\vtv[\arm]]-\vtav[\UCBindex][\run][0])
    \ge\sum_{\indv\in\va[\variables][\vt[\sol[\arm]]]}(\vtav[\UCBindex][\run][\vtv[\sol[\arm]]]-\vtav[\UCBindex][\run][0]).
\end{equation}
%
On the other hand, inequality \eqref{eq:contextual-estimate-product-diff} can be rewritten as
%
\begin{equation}
    \label{eq:contextual-pf-UCB-lu}
    \vtav[\UCBindex][\run][\indtreat]
    -2\vt[\radiusEllipConf]\norm{\vtv[\feature]}_{(\vta[\LSmat][\run-1][\indtreat])^{-1}}
    \le
    \product{\va[\param][\indtreat]}{\vtv[\feature]}
    \le\vtav[\UCBindex][\run][\indtreat].
\end{equation}
%
Combining \eqref{eq:contextual-pf-UCB-diff} and \eqref{eq:contextual-pf-UCB-lu} and rearranging, we get
%
\begin{equation}
    \notag
    \sum_{\indv\in\variables}\product{\va[\param][\vtv[\sol[\arm]]]-\va[\param][\vtv[\arm]]}{\vtv[\feature]}
    =
    \sum_{\indv\in\va[\variables][\vt[\arm]]\union \va[\variables][\vt[\sol[\arm]]]}
    \product{\va[\param][\vtv[\sol[\arm]]]-\va[\param][\vtv[\arm]]}{\vtv[\feature]}
    \le
    \sum_{\indv\in\va[\variables][\vt[\arm]]\union \va[\variables][\vt[\sol[\arm]]]}
    2\vt[\radiusEllipConf]\norm{\vtv[\feature]}_{(\vta[\LSmat][\run-1][\vtv[\arm]])^{-1}}.
    %+ \sum_{\indv\in\setexclude{\va[\variables][\vt[\sol[\arm]]]}{\va[\variables][\vt[\arm]]}}2\vt[\radiusEllipConf]\norm{\vtv[\feature]}_{(\vta[\LSmat][\run-1][0])^{-1}}
\end{equation}
%
Summing the above from $\run=1$ to $\nRuns$ and applying the Cauchy–Schwarz inequality, we obtain
%
\begin{equation}
    \notag
    \begin{aligned}
    \vt[\reg][\nRuns]
    &\le\sum_{\run=1}^{\nRuns}
    \sum_{\indv\in\va[\variables][\vt[\arm]]\union \va[\variables][\vt[\sol[\arm]]]}
    2\vt[\radiusEllipConf]\norm{\vtv[\feature]}_{(\vta[\LSmat][\run-1][\vtv[\arm]])^{-1}}\\
    &\le
    2\vt[\radiusEllipConf][\nRuns]
    \sqrt{
    \left(\sum_{\run=1}^{\nRuns}
    \card(\va[\variables][\vt[\arm]]\union \va[\variables][\vt[\sol[\arm]]])\right)
    \left(\sum_{\run=1}^{\nRuns}
    \sum_{\indv\in\va[\variables][\vt[\arm]]\union \va[\variables][\vt[\sol[\arm]]]}
    \norm{\vtv[\feature]}_{(\vta[\LSmat][\run-1][\vtv[\arm]])^{-1}}^2\right)
    }
    \\
    &\le
    2\vt[\radiusEllipConf][\nRuns]
    \sqrt{2\nAffected\nRuns
    \sum_{\run=1}^{\nRuns}
    \left(
    \sum_{\indtreat\in\treatments}\sum_{\indv\in\vta[\variables][\run][\indtreat]}
    \norm{\vtv[\feature]}_{(\vta[\LSmat][\run-1][\indtreat])^{-1}}^2
    +
    \sum_{\indv\in\setexclude{\va[\variables][\vt[\sol[\arm]]]}{\va[\variables][\vt[\arm]]}}
    \norm{\vtv[\feature]}_{(\vta[\LSmat][\run-1][0])^{-1}}^2
    \right)}.\\
    \end{aligned}
\end{equation}
%
Since $\regpar\ge\nAffected$, by \cref{lem:Vt-norm-det-bound}, for all $\indtreat\in\treatments$ it holds that
%
\begin{equation}
    \notag
    \sum_{\run=1}^{\nRuns}\sum_{\indv\in\vta[\variables][\run][\indtreat]}
    \norm{\vtv[\feature]}_{(\vta[\LSmat][\run-1][\indtreat])^{-1}}^2
    \le
    2\vdim\log\left(
    1+\frac{\nAffected\nRuns}{\vdim\regpar}\right).
\end{equation}
%
Similarly, let us define $\vta[\widetilde{\LSmat}][\run][0]=\regpar\Id+\sum_{\runalt=1}^{\run}\sum_{\indv\in\setexclude{\va[\variables][\vt[\sol[\arm]]]}{\va[\variables][\vt[\arm]]}}\vtv[\feature][\runalt]\vtv[\feature][\runalt]^{\top}$.
Using $\vta[\widetilde{\LSmat}][\run][0]\mleq\vta[\LSmat][\run][0]$ and invoking \cref{lem:Vt-norm-det-bound} with $\vt[\variables]\subs\setexclude{\va[\variables][\vt[\sol[\arm]]]}{\va[\variables][\vt[\arm]]}$ gives
%
\begin{equation}
    \notag
    \sum_{\run=1}^{\nRuns}
    \sum_{\indv\in\setexclude{\va[\variables][\vt[\sol[\arm]]]}{\va[\variables][\vt[\arm]]}}
    \norm{\vtv[\feature]}_{(\vta[\LSmat][\run-1][0])^{-1}}^2
    \le
    \sum_{\run=1}^{\nRuns}
    \sum_{\indv\in\setexclude{\va[\variables][\vt[\sol[\arm]]]}{\va[\variables][\vt[\arm]]}}
    \norm{\vtv[\feature]}_{(\vta[\widetilde{\LSmat}][\run-1][0])^{-1}}^2
    \le
    2\vdim\log\left(
    1+\frac{\nAffected\nRuns}{\vdim\regpar}\right).
\end{equation}
% 
Putting the above three inequalities together, we get exactly \eqref{eq:C2UpUCB-regret}.
\end{proof}

\subsection{Experiments for Targeted Campaign with Criteo Uplifting Dataset}
\label{apx:exp-c2}
% \input{Figures/Exp-figure-targeted}


% \textbf{Targeted Campaign with Criteo Uplift\afterhead}
% \label{subsec:exp-c2}
%contextual combinatorial
In this section, we provide experiments for the contextual combinatorial uplifting model using the Criteo Uplift dataset.
At each round, $100$ individuals are sampled from the dataset and the problem consists in choosing $10$ of them to treat so that the number of visits over the $100$ individuals is maximized.  Here, we compare our methods based on \CUpUCB (\cref{algo:C2UpUCB}) with approaches based on greedy and $\varepsilon$-greedy (see~\citep{LS20} for a description) that are more appropriate baselines in this setup. 
Again, our results are averaged over $100$ independent runs and the shaded areas of the plots represent the standard errors.
%\todosk{Are the curves are
%averaged here too and the shaded areas
%represent the standard errors?}


% To provide counterfactual feedback, following the original paper~\citep{Diemert2018}, we fit two logistic models for the treated and untreated individuals.
%\footnote{See \needref for more details}
% Then, if the learner decides to treat an individual while the individual is untreated in the dataset,
%we use 
% the logistic model fitted on treated users generates the mean of a Bernoulli distribution from which we sample the feedback, and vice versa.
%to generate the probability that the individual would visit the website if treated and sample the feedback from a Bernoulli distribution with that mean, and vice versa.

%\todoygmargin{I removed C2UCB to avoid confusion, but I will still present it in the appendix.}
%, and C2UCB which aims to maximize the total reward over the selected individuals.
% A detailed description of these algorithms is provided in \cref{apx:exp-c2-detail}.
%and the choices of the parameters are provided in the appendix .



\paragraph{Algorithms\afterhead} 
% Following the original paper~\citep{Diemert2018}, we fit two logistic models for the treated and untreated individuals.
In all the considered algorithms, the learner learns a logistic model based on the feedback they have received from the individuals they select to treat.\!\footnote{Logistic models were also considered in the original Criteo dataset paper \citep{Diemert2018} to compute uplifts.}
If the baseline model is unknown, the learner also learns a baseline logistic model based on the feedback received from the individuals they do not treat.
In the following, we will denote respectively by $\vta[\est{\objalt}][\run][1]$ and $\vta[\est{\objalt}][\run][0]$ the conditional probability functions of the two fitted models using data up to and including round $\run$.
When the baseline model is known, we denote by $\va[\objalt][0]$ its conditional probability function.
%Our methods are compared with greedy and $\varepsilon$-greedy.
The methods that we look into in this experiment mainly differ in how they select individuals in each round $\run$, as we detail below.
As before, we use the suffix (bl) to indicate modification of the respective algorithm to the case where the baseline payoffs are known.
%
\begin{itemize}[leftmargin=*]
    \item \textbf{Greedy\,(bl):} The learner chooses the $10$ individuals with the largest estimated uplifts $\vta[\est{\objalt}][\run-1][1](\feature)-\va[\objalt][0](\feature)$.
    \item $\boldsymbol{\varepsilon}$\textbf{-greedy\,(bl):} The learner reserves a exploration budget $b$ where $b$ is sampled from $B(10, \varepsilon)$ the binomial distribution with parameters $10$ and $\varepsilon$.
    $10-b$ individuals are chosen greedily as in the greedy strategy while the remaining $b$ individuals are randomly sampled from those that have not been selected.
    \item $\boldsymbol{\varepsilon}$\textbf{-greedy:} For the greedy selection part in $\varepsilon$-greedy, the estimated uplifts are computed by $\vta[\est{\objalt}][\run-1][1](\feature)-\vta[\est{\objalt}][\run-1][0](\feature)$.
    \item \textbf{\CUpUCB(bl):} For each individual $\indv$ we define their uplifting index
    $\vtav[\UPindex]=\vta[\est{\objalt}][\run-1][1](\feature)+\expparam\norm{\vtv[\feature]}_{(\vta[\LSmat][\run-1][1])^{-1}}-\va[\objalt][0](\feature)$ where $\vta[\LSmat][\run-1][1]$ is defined following \eqref{eq:definition-Vtz} with $\regpar=1$ and $\expparam$ is a exploration parameter to be tuned.
    The algorithm consists in choosing the $10$ individuals with the largest uplifting indices.
    \item \textbf{\CUpUCB:} It works in the same way as C2UPUCB with baseline knowledge but the uplifting index is now defined by 
    $\vtav[\UPindex]=\vta[\est{\objalt}][\run-1][1](\feature)+\expparam\norm{\vtv[\feature]}_{(\vta[\LSmat][\run-1][1])^{-1}}
    -\vta[\est{\objalt}][\run-1][0](\feature)-\expparam\norm{\vtv[\feature]}_{(\vta[\LSmat][\run-1][0])^{-1}}$;
    that is, it is computed as the difference between two upper confidence bounds.
    \item \textbf{C2UCB:} It works in the same way as \CUpUCB but the baseline is ignored, so $\vtav[\UPindex]=\vta[\est{\objalt}][\run-1][1](\feature)+\expparam\norm{\vtv[\feature]}_{(\vta[\LSmat][\run-1][1])^{-1}}$. The linear variant of this algorithm was introduced in \citep{QCZ14} for contextual combinatorial bandits.
    % Note that we did not report results for this method in \cref{subsec:exp-c2}.
\end{itemize}
% \todosk{Fix the name of the Algos \CUpUCB... above}
Note that as the reward comes from a logistic model, we use a logistic regression for the bandit model based on the idea of GLM-UCB \citep{filippi2010parametric}.
% For the last three algorithms (\CUpUCBMwb,~\CUpUCB, and C2UCB)  our implementation is 
For the results, we select the optimal parameters from $\varepsilon\in\{0.05, 0.1, 0.2, 0.3\}$ and $\expparam\in\{0.5, 1, 2, 3\}$.
More details on the tuning of the parameters are provided in \cref{apx:param-tuning}, and the chosen optimal parameters are reported in \cref{tab:params}.

\paragraph{Data Preprocessing\afterhead}
For this experiment, we normalize the data so that the features are contained in the range $[0, 1]$.
Moreover, we also subsample the dataset to increase the visit rate to $0.25$.
In fact, we found the logistic models to perform very poorly on the original dataset (with a f1-score around $0.4$) due to its small visit rate at $0.04$.


\input{Figures/Exp-figure-more-on-c2}

% In this part, we provide additional results for the targeted campaign experiment described in \cref{subsec:exp-c2}.
\paragraph{Feedback\afterhead}
We consider two ways to use the fitted logistic models
%
\begin{enumerate}
    \item The logistic models are only used to generate the counterfactual outcomes.
    That is, the feedback of an individual is sampled from the Bernoulli distribution with mean predicted by either of the models only if the learner decides to treat the individual while the individual is not treated in the dataset or vice-versa.
    \item The logistic models are used to generate all the outcomes.
\end{enumerate}
% We only presented the first scenario in \cref{subsec:exp-c2}.
%We point out here that logistic models are actually misspecified in the first case. \todosk{Unclear what this means?}

\paragraph{Results\afterhead}
%\label{apx:exp-c2}

In \cref{fig:exp-c2-add} (Right), we plot the uplift averaged over all the individuals that have been treated up to a time horizon by an algorithm.
% \footnote{The uplift is computed using the two fitted logistic models.}
Higher this value is better it is because it means we are selecting the individuals for which the treatment is the most effective.
%fitted on the dataset.}
For comparison, we also indicate the average uplift of random selection and an oracle strategy that always chooses the $10$ individuals with the highest uplifts.
%
%show the average uplift of the dataset ($\smallsim\!.02$) and the average uplift of the $10\%$ of population with the highest uplift ($\smallsim\!.11$).
%Therefore, if treating each individual has a cost and this cost exceeds $0.02$,
%\footnote{%
%This had no physical meaning here, because it's just a difference of probabilities.}
%it would be more beneficial to target the individuals with higher uplift.
%Indeed, the average predicted uplift of the $10\%$ of population with the highest uplift is at $0.11$.
Both \CUpUCB and $\varepsilon$-greedy beat greedy and random selection,
%All the algorithms that we present here
%, except for C2UCB, 
%manage to beat random selection, 
which demonstrates the benefit of considering a bandit model for this problem.
%C2UCB does not perform well because it is not optimizing the right objective.
$\varepsilon$-greedy turns out to be quite competitive, but \CUpUCB still has a slight advantage no matter whether the baseline is known or unknown.

% As for the two lines \textsf{random} and \textsf{best} in \cref{subfig:exp-c2}, we indeed plot the average uplift over the whole dataset and over the 10\% of population with the highest uplifts.


%To compare the algorithms, in addition to the average uplift of the treated individuals, 
For further comparison, we also plot the regret in terms of both the predicted uplifts (Left) and the rewards that the learner actually receives (Middle) in \cref{fig:exp-c2-add}.\footnote{We use occasionally the term predicted uplift here to remind that they are computed using logistic models fitted on the dataset and we do not have access to any type of \emph{ground-truth} uplift.}
For the two regrets, we define the optimal action as the one that selects the $10$ individuals with the highest predicted uplifts.
Then, if the logistic models correctly predict the expected rewards, the regret in terms of the predicted uplifts should be the expectation of the regret in terms of the realized rewards, and thus we should get similar curves after averaging over $100$ runs.
This is indeed the case in \cref{subfig:exp-c2-add-without-true}.
Nonetheless, 
%when the models are misspecified, 
when the outcomes also come from true data,
selecting the samples with higher predicted uplifts does not necessarily result in higher rewards, which explains the discrepancy between \cref{subfig:exp-c2-add-with-true} (Left) and \cref{subfig:exp-c2-add-with-true} (Middle).
\CUpUCB and $\varepsilon$-greedy perform quite similarly here when we look at the realized rewards.
%Due to the misspecifcation of the models, 
Since the ground truth outcomes cannot be perfectly predict by logistic models,
we also observe linear regret of all the algorithms in \cref{subfig:exp-c2-add-with-true} (Left), while in \cref{subfig:exp-c2-add-without-true} (Left), both \CUpUCBMwb and \CUpUCB achieves sublinear regret and performs much better than $\varepsilon$-greedy.

In all the cases, Greedy and C2UCB perform poorly.
This points out the importance of exploration (which is taken into account by bandit algorithms) and uplift modeling in this problem.
Finally, to explain the surprising fact that an algorithm might perform better without knowledge of the baseline, we look into the data and find out that samples with higher baselines often have higher uplifts.
Therefore, when the learner is provided with the baselines of the samples, they may avoid choosing these samples at the beginning, which results a slower exploration and a worse performance.

% As for the two lines \textsf{random} and \textsf{best} in \cref{fig:exp-c2}, we indeed plot the average uplift over the whole dataset and over the 10\% of population with the highest uplifts.
% For the results that we present in \cref{subsec:exp-c2} and \cref{apx:exp-c2}, we select the optimal parameters from $\varepsilon\in\{0.05, 0.1, 0.2, 0.3\}$ and $\expparam\in\{0.5, 1, 2, 3\}$.



%and chooses individuals with the highest predicted uplift, no matter whether the baseline model is known or unknown. % (i.e.,\cref{algo:C2UpUCB}).
% \todosk{Can you say what is C2UCB? Also "but \CUpUCB still..." line is unclear, because is \CUpUCB (Algorithm 4)?}
% \todoyg{C2UCB only focuses on the total reward over the selected individuals. Detailed description is provided in the appendix. Yes Algorithm 4 is \CUpUCB.}

%More experimental details, including a complete description of the used algorithms, and additional experimental results can be found in \cref{apx:exp-c2-detail} and \cref{apx:exp-c2}.





==> Uplifting bandits - arxiv/Appendices/Concentration-deprecated.tex <==
In this section, we formally describe the probability model of the $\nArms$-arm uplifting bandit problem that we build upon for proving the regret upper bounds, before deriving several concentration results that are used throughout our analyses.

Our upper-bound analyses are based on the stack-feedback model.
That is, we have a collection of independent random vectors $(\vta[\valuev][\round])_{\arm\in\arms,\round\in\oneto{\nRuns}}$ such that the law of $\vta[\valuev][\round]$ is $\va[\distribution]$.
Each $(\vta[\valuev][\round])_{\round\in\oneto{\nRuns}}$ forms a stack, and when the learner chooses action $\arm$, they receives the vector from the top of the stack. In other words, the value of $\vta[\valuev][\round]$ is observed when the learner pulls $\arm$ for the $\round$-th time.
By abuse of notation, we will also use $\vta[\valuev][\round]$ to denote the value of the random variable (evaluated at some $\sample\in\samples$ with $\samples$ being the underlying probability space).
In most of our algorithms, we are interested in either of the following estimates
%
\begin{equation}
    \notag
    \vtav[\estalt{\meanReward}][\round]=\frac{\sum_{\runalt=1}^{\round}\vtav[\valuev][\runalt]}{\round},
    ~~~~~~
    \vtav[\est{\meanReward}][\run][0] =
    \frac{\sum_{\runalt=1}^{\run}\vtav[\valuev][\runalt][\vt[\arm][\runalt]]\one\{\indv\notin\va[\variables][\vt[\arm]]\}}{\max(1, \vtav[\pullcount][\run][0])}.
\end{equation}
%
Despite the apparent similarity between these two quantities, the key distinction is that the denominator of $\vtav[\estalt{\meanReward}][\round]$ is a constant while the denominator of $\vtav[\est{\meanReward}][\run][0]$ is also a random variable.
Therefore, deriving a concentration bound for the later will require a more delicate treatment.
We first state a concentration inequality for $\vtav[\estalt{\meanReward}][\round]$.
%
\begin{lemma}
\label{lem:iid-concentration}
Let $\smallproba\in(0,1)$. It holds
%
\begin{equation}
    \notag
    \prob\left(\abs{\vtav[\estalt{\meanReward}][\round]-\vav[\meanReward]}\ge\sqrt{\frac{2\log(1/\smallproba)}{\round}}\right)
    \le 2\smallproba.
\end{equation}
\end{lemma}
\begin{proof}
This is immediate from \eqref{eq:subgaussian-concentration} and the fact that $\vtav[\estalt{\meanReward}][\round]$ is $(1/\sqrt{\round})$-subgaussian.
\end{proof}
%
\cref{lem:iid-concentration} is sufficient for the analysis whenever $\vtav[\est{\meanReward}]$ is defined as in \eqref{eq:mean-estimate-a}.
In fact, in this case $\vtav[\est{\meanReward}]=\vtav[\estalt{\meanReward}][\vta[\pullcount]]$ as long as $\vta[\pullcount]\ge1$.
Therefore, if $\abs{\vtav[\estalt{\meanReward}][\round]-\vav[\meanReward]}\le\sqrt{2\log(1/\alt{\smallproba})/\round}$ for all relevant $\arm$ and $\indv$ we have indeed the desired concentration result.

For the more challenging case where an indicator of the probability event is also involved in the estimator, we will leverage on tools from martingale theory.
Let us first introduce a concentration inequality for martingale difference sequence based on \cite[Lem. 2]{BDHK+08} and \cite[Th. 1.2A]{Victor99}.

\begin{lemma}%[{{\cite[Lem. 2]{BDHK+08}}}]
\label{lem:DLP-ineq}
Let $(\vt[\filter][\runalt])_{\runalt=0}^{\run}$ be a filtration and $(\vt[\rv][\runalt])_{\runalt=1}^{\run}$ be a $(\vt[\filter][\runalt])$-adapted martingale difference sequence.
Suppose that there exists $\rvb>0$ such that $\exof{\vt[\rv][\runalt]^2\given{\vt[\filter][\runalt-1]}}\le\rvb^2$ and that the following conditional Bernstein condition is verified for all $\runalt\in\oneto{\run}$ and $\probmoment\ge2$,
\begin{equation}
    \notag
    \exof{\abs{\vt[\rv][\runalt]}^{\probmoment}\given{\vt[\filter][\runalt-1]}} \le \frac{\probmoment!}{2}\rvb^{\probmoment-2}\exof{\vt[\rv][\runalt]^2\given{\vt[\filter][\runalt-1]}}.
\end{equation}
Then, for any $\smallproba\in(0,1/e)$, it holds
%
\begin{equation}
    \notag
    \prob\left(\sum_{\runalt=1}^{\run}\vt[\rv][\runalt]
    \ge 2\max(2\noisedev,2\rvb\sqrt{\log(1/\smallproba)})\sqrt{\log(1/\smallproba)}
    \right) \le \max(\log_2(\run),1)\frac{\smallproba}{2},
\end{equation}
where $\noisedev=\sqrt{\sum_{\runalt=1}^{\run}\exof{\vt[\rv][\runalt]^2\given{\vt[\filter][\runalt-1]}}}$ is the square root of the sum of the conditional variances of $\vt[\rv][\runalt]$'s.
\end{lemma}
\begin{proof}
The proof of \cite[Lem. 2]{BDHK+08} essentially applies.
We just need to replace the use of Freedman’s inequality by the use of de la Peña's inequality \cite[Th. 1.2A]{Victor99} and define $\alpha_0=2\rvb\sqrt{\log(1/\smallproba)}$.
Also notice with this choice of $\alpha_0$ the condition $\smallproba<1/e$ guarantees $\alpha_0\ge2$ so $\ell\ge\log_2{\sqrt{\run}}-1$ already ensures $2^{\ell}\alpha_0\ge\rvb\sqrt{\run}$.
\end{proof}

In the following, $(\vt[\filter])_{\run}$ will represent the natural filtration associated to $(\vt[\valuev], \vt[\arm][\run+1])_{\run}$ such that both $\vt[\valuev]$ and $\vt[\arm][\run+1]$ are $\vt[\filter]$-measurable.

\begin{lemma}
\label{lem:indicator-concentration}
Let $(\eventalt)_{\runalt=1}^{\run}$ be a sequence of events such that $\vt[\eventalt][\runalt]\in\vt[\filter][\runalt-1]$.
We consider
\begin{equation}
    \notag
    \vta[\pullcount][\run][\eventalt] = \sum_{\runalt=1}^{\run}\one\{\vt[\eventalt][\runalt]\},
    ~~~~~
    \vtav[\est{\meanReward}][\run][\eventalt] =
    \frac{\sum_{\runalt=1}^{\run}\vtav[\valuev][\runalt][\vt[\arm][\runalt]]
    \one\{\vt[\eventalt][\runalt]\}}
    {\max(1, \vta[\pullcount][\run][\eventalt])}.
\end{equation}
%
Suppose that all the noise variables $\vav[\snoise]$ satisfy the Bernstein condition \eqref{eq:Bernstein} with $\noisedev=1$ and have their variance bounded by $1$ (this is automatically verified if the noises are $1$-subgaussian).
Then, we have the following concentration bound for $\vtav[\est{\meanReward}][\run][\eventalt]$
%
\begin{equation}
    \label{eq:indicator-estimate-concentration}
    \prob
    \left(
    \left|\vtav[\est{\meanReward}][\run][\eventalt] - \frac{\sum_{\runalt=1}^{\run}\vav[\meanReward][\vt[\arm][\runalt]]\one\{\vt[\eventalt][\runalt]\}}{ \max(1,\vta[\pullcount][\run][\eventalt])}\right|
    \ge
    4\sqrt{\frac{\log((\log(\run)/\log(2))\smallproba)}
    {\max(1,\vta[\pullcount][\run][\eventalt])}}
    + \frac{4\log((\log(\run)/\log(2))\smallproba)}
    {\max(1,\vta[\pullcount][\run][\eventalt])}
    \right)
    \le \smallproba
\end{equation}
\end{lemma}
\begin{proof}
Let $\vtav[\snoise][\runalt][\vt[\arm][\runalt]]=\vtav[\valuev][\runalt][\vt[\arm][\runalt]]-\vav[\meanReward][\vt[\arm][\runalt]]$.
We apply \cref{lem:DLP-ineq} with $\vt[\rv][\runalt]\subs\vtav[\snoise][\runalt][\vt[\arm][\runalt]]\one\{\vt[\eventalt][\runalt]\}$ and $\rvb\subs 1$.
The two conditions that involve $\rvb$ in \cref{lem:DLP-ineq} are indeed verified because
$\ex_{\runalt-1}[\abs{\vtav[\snoise][\runalt][\vt[\arm][\runalt]]\one\{\vt[\eventalt][\runalt]\}}^{\probmoment}]=\ex[\abs{\vav[\snoise][\vt[\arm][\runalt]]}^{\probmoment}]\one\{\vt[\eventalt][\runalt]\}$ for all $\probmoment\in\R$.
The equality with $\probmoment=2$ also shows that $\ex_{\runalt-1}[\vt[\rv][\runalt]^2]\le\one\{\vt[\eventalt][\runalt]\}$ and thus $\sum_{\runalt=1}^{\run}\ex_{\runalt-1}[\vt[\rv][\runalt]^2]\le\vta[\pullcount][\run][\eventalt]$.
\cref{lem:DLP-ineq} then ensures that for all $\alt{\smallproba}\in(0,1/e)$, it holds
%
\begin{equation}
    \notag
    \prob\left(\sum_{\runalt=1}^{\run}
    (\vtav[\valuev][\runalt][\vt[\arm][\runalt]]-\vav[\meanReward][\vt[\arm][\runalt]])\one\{\vt[\eventalt][\runalt]\}
    \ge 4\sqrt{\vta[\pullcount][\run][\eventalt]\log(1/\alt{\smallproba})}
    + 4\log(1/\alt{\smallproba})
    \right) \le \frac{\log(\run)\alt{\smallproba}}{2\log(2)}.
    %\le \log(\run)\alt{\smallproba}.
\end{equation}
%
Applying the same procedure to $\vt[\rv][\runalt]\subs-\vtav[\snoise][\runalt][\vt[\arm][\runalt]]\one\{\vt[\eventalt][\runalt]\}$ and using a union bound we get
%
\begin{equation}
    \notag
    \prob\left(\sum_{\runalt=1}^{\run}
    \abs{(\vtav[\valuev][\runalt][\vt[\arm][\runalt]]-\vav[\meanReward][\vt[\arm][\runalt]])\one\{\vt[\eventalt][\runalt]\}}
    \ge 4\sqrt{\vta[\pullcount][\run][\eventalt]\log(1/\alt{\smallproba})}
    + 4\log(1/\alt{\smallproba})
    \right) \le  \frac{\log(\run)\alt{\smallproba}}{\log(2)}.
\end{equation}
%
We obtain \eqref{eq:indicator-estimate-concentration} by dividing the inequality in $\prob$ by $\max(1,\vta[\pullcount][\run][\eventalt])$ and choose $\alt{\smallproba}=(\log(2)/\log(\run))\smallproba<1/e$.
\end{proof}

\begin{lemma}
Suppose that $\vav[\snoise][0]$ satisfies the Bernstein condition \eqref{eq:Bernstein} with $\noisedev=1$ and its variance is bounded by $1$.
Let $\smallproba\in(0,1/e)$. It holds
\begin{equation}
    \notag
    \prob
    \left(
    \abs{\vtav[\est{\meanReward}][\run][0] - \vav[\meanReward][0]}
    \ge
    4\sqrt{\frac{\log(2\run/\alt{\smallproba})}{\vtav[\pullcount][\run][0]}}
    + \frac{4\log(2\run/\alt{\smallproba})}{\vtav[\pullcount][\run][0]}
    \right)
    \le \smallproba.
\end{equation}
\end{lemma}
\begin{proof}
The result is immediate from \cref{lem:indicator-concentration} with the choice $\vt[\eventalt][\runalt]=\{\indv\notin\va[\variables][\runalt]\}$.
We also use the inequality $\log(\run)/(\log(2)\max(1,\vtav[\pullcount][\run][0]))\le2\run/\vtav[\pullcount][\run][0]$ and the fact that $\vav[\meanReward][\vt[\arm][\runalt]]\one\{\indv\notin\va[\variables][\runalt]\}=\vav[\meanReward][0]\one\{\indv\notin\va[\variables][\runalt]\}$.
\end{proof}

==> Uplifting bandits - arxiv/Appendices/Concentration.tex <==
To prove the regret upper bounds, we will make use of concentration bounds that apply to quantities defined in \eqref{eq:mean-estimate-a} and \eqref{eq:mean-estimate-0}.
Underlying all these results is the following fundamental concentration inequality for $\noisedev$-sub-Gaussian random variables~\citep{vershynin2018high}
%
\begin{equation}
    \label{eq:sub-Gaussian-concentration}
    \prob(\abs{\rv}\ge\scalar)\le2\exp(-\scalar^2/(2\noisevar)) \text{ for all } \scalar>0.
\end{equation}

However, the estimates in \eqref{eq:mean-estimate-a} and \eqref{eq:mean-estimate-0} aggregate observed values in a way that depend on the decisions that have been made.
%have been been made up to a certain instant.
Therefore, concentration bounds for the sum of independent variables, which can be directly derived from \eqref{eq:sub-Gaussian-concentration}, are not sufficient for our purposes.
%\footnote{It is possible to construct a different probability model for which...}
%would need to be applied to all the possible subsequences, which results in a trivial $\bigoh(\nRuns)$ regret bound.
The standard trick to circumvent this issue in bandit literature is to combine Doob's optional skipping (\citep[Chap.\ 3]{Doob53}, \citep[Chap.\ 9]{Chung01}) with concentration inequality for martingale difference sequence.
The following lemma adapted from \citep[Lem.\ A.1]{SS11} is proved exactly using this technique.

\begin{lemma}
\label{lem:concentration-MDS}
Let $(\vt[\filter])_{\run\in\N}$ be a filtration and let $(\vt[\indevent],\vt[\rv])_{\run\in\N}$ be a sequence of $\{0,1\}\times\R$- valued random variables such that $\vt[\indevent]$ is $\vt[\filter][\run-1]$-measurable, and $\vt[\rv]$ is $\vt[\filter]$-measurable and conditionally $\noisedev$-sub-Gaussian, \ie $\exof{\exp(\scalar\vt[\rv])\given{\vt[\filter][\run-1]}}\le\exp(\scalar^2\noisedev^2/2)$ for all $\scalar\in\R$.
Let $\pullcount>0$ and let $\stoptime=\min\setdef{\run\ge1}{\sum_{\runalt=1}^{\run}\vt[\indevent][\runalt]=\pullcount}$, where we take $\stoptime=+\infty$ when $\sum_{\runalt=1}^{+\infty}\vt[\indevent][\runalt]<\pullcount$.
Then, for any $\smallproba\in(0,1)$,
%
\begin{equation}
    \prob\left(\left|\sum_{\run=1}^{\stoptime}\vt[\indevent]\vt[\rv]\right|
    \ge\noisedev\sqrt{2\pullcount\log(2/\smallproba)}
    \right)\le\smallproba.
\end{equation}
\end{lemma}
\begin{proof}
The proof of \citep[Lem. A.1]{SS11} essentially applies.
We just need to replace the use of Hoeffding-Azuma inequality by the use of concentration inequality for conditionally sub-Gaussian martingale difference sequences, which is itself derived from \eqref{eq:sub-Gaussian-concentration} and the fact that the sum of conditionally sub-Gaussian martingale differences is sub-Gaussian.
\end{proof}

In the following, $(\vt[\filter])_{\run}$ will represent the natural filtration associated to $(\vt[\valuev], \vt[\arm][\run+1])_{\run}$ such that $\vt[\arm]$ is $\vt[\filter][\run-1]$-measurable, and $\vt[\valuev]$ is $\vt[\filter]$-measurable.
Applying \cref{lem:concentration-MDS} to properly defined $(\vt[\indevent],\vt[\rv])_{\run}$ along with the use of a union bound gives the following concentration results that are key to our analyses.

\begin{lemma}
\label{lem:concentration-mean-a}
Let $\arm\in\arms$, $\indv\in\variables$, and let $\vtav[\meanReward]$ be defined as in \eqref{eq:mean-estimate-a}. Then for any $\smallproba\in(0,1)$, it holds
\begin{equation}
    \notag
    \prob
    \left(
    \exists \thinspace \run\in\nRuns, \thinspace
    \abs{\vtav[\est{\meanReward}] - \vav[\meanReward]}
    \ge
    \sqrt{\frac{2\log(2/\smallproba)}{\vta[\pullcount]}}
    \right)
    \le \nRuns\smallproba.
\end{equation}
\end{lemma}
\begin{proof}
For $\pullcount\in\oneto{\nRuns}$, we define the random variables
%
\begin{equation}
    \notag
    \vt[\stoptime][\pullcount]=\min
    \left\{\run\ge1 : \sum_{\runalt=1}^{\run}\one\{\vt[\arm][\runalt]=\arm\}=\pullcount\right\}
    \text{~~~and~~~}
    \vtav[\srvsum][\pullcount]=
    \sum_{\runalt=1}^{\vt[\stoptime][\pullcount]}\vtv[\valuev][\runalt]\one\{\vt[\arm][\runalt]=\arm\}.
\end{equation}
%
We then define the failure events
%
\begin{gather*}
    \vv[\event] =
    \left\{
    \exists \thinspace \run\in\oneto{\nRuns}, \thinspace
    \abs{\vtav[\est{\meanReward}] - \vav[\meanReward]}
    \ge
    \sqrt{\frac{2\log(2/\smallproba)}{\vta[\pullcount]}}
    \right\},\\
    \vv[\widetilde{\event}] =
    \left\{
    \exists \thinspace \pullcount\in\oneto{\nRuns}, \thinspace
    \left|
    \vtav[\srvsum][\pullcount]
    - \vav[\meanReward]
    \left(\sum_{\runalt=1}^{\vt[\stoptime][\pullcount]}\one\{\vt[\arm][\runalt]=\arm\}\right)
    \right|
    \ge
    \sqrt{2\pullcount\log(2/\smallproba)}.
    \right\}
\end{gather*}
%
It holds $\vv[\event]\subseteq\vv[\widetilde{\event}]$.
In fact, if $\vv[\event]$ happens then $\abs{\vtav[\est{\meanReward}] - \vav[\meanReward]} \ge \sqrt{2\log(2/\smallproba)/\vtav[\pullcount]}$ for some $\run$ and this is only possible when $\vtav[\pullcount]\ge 1$.
With the definition $\vtav[\pullcount]=\sum_{\runalt=1}^{\run}\one\{\vt[\arm][\runalt]=\arm\}$, we further see that $\vtav[\pullcount]\le\run\le\nRuns$ and $\vt[\stoptime][\vta[\pullcount]]\le\run<+\infty$.
The latter means that we indeed have $\sum_{\runalt=1}^{\vt[\stoptime][\vta[\pullcount]]}\one\{\vt[\arm][\runalt]=\arm\}=\vta[\pullcount]$. Thus multiplying $\abs{\vtav[\est{\meanReward}] - \vav[\meanReward]} \ge \sqrt{2\log(2/\smallproba)/\vtav[\pullcount]}$ by $\pullcount=\vta[\pullcount]\in\oneto{\nRuns}$ gives exactly
%
\begin{equation}
    \notag
    \left|
    \vtav[\srvsum][\pullcount]
    - \vav[\meanReward]
    \left(\sum_{\runalt=1}^{\vt[\stoptime][\pullcount]}\one\{\vt[\arm][\runalt]=\arm\}\right)
    \right|
    \ge
    \sqrt{2\pullcount\log(2/\smallproba)},
\end{equation}
%
which shows that $\vv[\widetilde{\event}]$ happens as well.
It is thus sufficient to prove that $\prob(\vv[\widetilde{\event}])\le\nRuns\smallproba$.

For $\pullcount\in\oneto{\nRuns}$, we apply \cref{lem:concentration-MDS} to $\vt[\indevent]\subs\one\{\vt[\arm]=\arm\}$ and $\vt[\rv]\subs\vtav[\snoise]=\vtav[\valuev]-\vav[\meanReward][\vt[\arm]]$. Since $\vav[\meanReward][\vt[\arm]]\one\{\vt[\arm]=\arm\}=\vav[\meanReward]\one\{\vt[\arm]=\arm\}$, we recover the exact inequality that appears in the definition of $\vv[\widetilde{\event}]$. We conclude with a union bound taking $\pullcount$ ranging from $1$ to $\nRuns$.
\end{proof}

\begin{lemma}
\label{lem:concentration-mean-0}
Let $\indv\in\variables$, and let $\vtav[\meanReward][\run][0]$ be defined as in \eqref{eq:mean-estimate-0}. Then for any $\smallproba\in(0,1)$, it holds
\begin{equation}
    \notag
    \prob
    \left(
    \exists \thinspace \run\in\nRuns, \thinspace
    \abs{\vtav[\est{\meanReward}][\run][0] - \vav[\meanReward][0]}
    \ge
    \sqrt{\frac{2\log(2/\smallproba)}{\vtav[\pullcount][\run][0]}}
    \right)
    \le \nRuns\smallproba.
\end{equation}
\end{lemma}
\begin{proof}
\cref{lem:concentration-mean-0} is proved in the same way as \cref{lem:concentration-mean-a}.
In particular, we apply \cref{lem:concentration-MDS} to $\vt[\indevent]\subs\one\{\indv\notin\va[\variables][\vt[\arm]]\}$ and $\vt[\rv]\subs\vtav[\snoise][\run][0]$.
\end{proof}

==> Uplifting bandits - arxiv/Appendices/Experiments.tex <==
In this appendix, we present missing experimental details from~\cref{sec:exp}. The code implementation of the proposed methods is attached in supplementary material.
All our experiments are run on amazon m4.xlarge EC2 instances.
The Criteo Uplift Prediction Dataset that we use for our experiments has the `CC0: Public Domain' license.

%This dataset is designed for uplift modeling tasks and contains outcomes for both treated and untreated individuals, which makes it suitable for our simulations.
%around $25$M examples, each one representing a user. Each user is represented with $12$ features, and is associated with a binary treatment indicator and two binary outcome variables indicating their visit and conversion status.
%Such a dataset is suitable for our simulations because it contains outcomes for both treated and untreated individuals, and the untreated individuals are randomly sampled from the population.
%All our experiments are run on amazon m4.xlarge EC2 instances.
%To ensure a fair comparison, we tune all the considered algorithms and report the results for the parameters that yield the best averaged performance.
%More precisely, we conduct $100$ independent runs for each experimental setup described below,
%and in each run, we fix the random seed and test all the candidate algorithms with their parameters chosen from a predefined set.
%In the end, we report results that are averaged over these $100$ runs, with an error bar that indicates the standard deviation of the metric.


\subsection{Choice of Algorithm Parameters}
\label{apx:param-tuning}

As mentioned in the main text, we report the results for the parameters that yield the best average performance.
%over the $100$ runs.
Precisely, we conduct $100$ independent runs for each experimental setup, and in each run, we fix the random seed and test all the candidate algorithms with their parameters chosen from a predefined set.
The performance of a specific parameter choice is then evaluated by the sum of the mean and one standard deviation of the regrets of the final run.
In fact, when the algorithm puts too much weight on exploitation, we may get lower mean regret while the standard deviation gets extremely large because the algorithm fails more frequently. %(as shown in for UpUCB)

Below we explain in detail what are the parameters that we tune in the non-contextual experiments.
%All the relevant details for the contextual combinatorial experiment is deferred to \cref{apx:exp-c2-detail}.
The optimal parameters that we have found are summarized in \cref{tab:params}.

\input{Tables/Parameters}

\paragraph{UCB and \textsc{UpUCB}s\afterhead}
For all UCB-type methods, we tune the exploration parameter $\expparam=1/\alt{\smallproba}$, which plays a crucial role in determining the widths of the confidence intervals-- see \eqref{eq:mean-estimate-a} and \eqref{eq:mean-estimate-0}.
Since $\vta[\radiusConf]$ represents the width of the confidence interval of a single variable's payoff in UpUCB algorithms, we set the widths of the confidence intervals of UCB to $\nVariables\vta[\radiusConf]=\nVariables\sqrt{2\expparam/\vta[\pullcount]}$, \ie the UCB indices in UCB are $\vta[\UCBindex]=\vta[\est{\reward}]+\nVariables\vta[\radiusConf]$, where $\vta[\est{\reward}]$ is the empirical mean of action $\arm$'s reward up to time $\run$.
In this way, we can choose exploration parameters of roughly the same order for different algorithms.
In the Gaussian uplifting bandit experiment (\cref{subsec:exp-gaussian}), we pick $\expparam\in\oneto{10}=\intinterval{1}{10}$.
As for the Bernoulli uplifting bandit experiment with Criteo dataset (\cref{subsec:exp-ber}), we select $\expparam\in\setdef{k\times10^{-\gamma}}{k\in\oneto{10},\gamma\in\{5,6,7\}}$.
The optimal performances are achieved with much smaller exploration parameters here because the noises in the variables are independent.

\paragraph{Thompson Sampling.}
We use Thompson sampling with Gaussian prior and Gaussian noise.
The mean and the variance of the prior are set to the mean and the variance of the actions' rewards.
Therefore, Thompson sampling is actually provided with more information than UCB.
Similar to before, the variance of the noise is set to $\nVariables^2\noisedev^2$ since the noise in the total reward scales with $\nVariables$.
The parameter $\noisedev^2$ plays a similar role as $\expparam$ in UCB.
In the Gaussian and Bernoulli uplifting experiments we respectively choose $\noisedev^2\in\setdef{k\times10^{-\gamma}}{k\in\oneto{10},\gamma\in\{0,1,2\}}$ and $\noisedev^2\in\setdef{k\times10^{-\gamma}}{k\in\oneto{10},\gamma\in\{5,6,7\}}$.

%In UCB, the UCB indices for the arms are set to $\vta[\UCBindex]=\vta[\est{\reward}]+\vta[\radiusConf]$ where $\vta[\est{\reward}]=(\sum_{\runalt=1}^{\run}\vt[\reward][\runalt]\one\{\vt[\arm][\runalt]=\arm\})/\max(1,\vta[\pullcount])$ is the empirical mean of arm $\arm$'s reward up to time $\run$.
%Here $\vta[\radiusConf]$ is the width of the confidence interval of the reward while in UpUCB algorithms (\needref) $\vta[\radiusConf]$ is the width of the confidence interval a single variable's payoff, 

% \paragraph{Gaussian Uplifting Bandit\afterhead}
% For all UCB-type methods, we tune the exploration parameter $\expparam=1/\alt{\smallproba}$, which plays a crucial role in computing the widths of the confidence intervals (see \eqref{eq:mean-estimate-a} and \eqref{eq:mean-estimate-0}).
% Its value is chosen from $\intinterval{1}{10}$, and smaller $\beta$ corresponds to more aggressive exploitation.
% As for Thompson sampling, we fix the mean and the variance of the Gaussian prior to be $50$ and $8$, which are roughly the mean and the variance of the Irwin–Hall distribution with parameter $100$ (the probability distribution obtained by summing $100$ independent random variables uniformly distributed from $0$ to $1$).
% We have verified that we do not get significantly better results by choosing these parameters differently.
% As for the variance of the noise provided to the algorithm, we choose it from $\expparam\in\setdef{k\times10^{\gamma}}{k\in\oneto{10},\gamma\in\{2,3,4\}}$ (we recall that the true variance is around $6400$).
% %(proving the true value does not give the best results).

% \paragraph{Bernoulli Uplifting Bandit with Criteo Uplift\afterhead}
% Since the noises are independent, we find that optimal performance is achieved with much smaller exploration parameter.
% We thus select $\expparam\in\setdef{k\times10^{-\gamma}}{k\in\oneto{10},\gamma\in\{5,6,7\}}$.
%the exploration parameter should be much smaller to achieve optimal performance, and thus for this experiment we select $\expparam\in\setdef{k\times10^{-\gamma}}{k\in\oneto{10},\gamma\in\{5,6,7\}}$.

%\paragraph{Targeted Campaign with Criteo Uplift\afterhead}
%See \cref{apx:exp-c2-detail}.


\subsection{More Details on Bernoulli Uplifting Bandit}
\label{apx:exp-ber}

% To construct the payoffs in the Bernoulli uplifting experiment, we assume that each cluster contains a single type of users that react in the same pattern.
% That is, if a user of a certain type is treated, their payoff is sampled from a Bernoulli distribution with mean corresponding to the visit rate of the treated individuals of that cluster, otherwise their payoff is sampled from another Bernoulli distribution with mean corresponding to the visit rate of the untreated individuals of that cluster.
% The payoffs of the variables are sampled independently.

For sake of completeness, we report below 
%Following the procedure described in \cref{subsec:exp-ber}, we obtain the following 
the visit rate of the treated and the untreated individuals of the clusters (rounded to three decimal places) that we obtained for our experiments
%
\begin{equation}
    \notag
    \begin{aligned}
    \meanReward_{\text{treated}}
    = [&.001 ~.037 ~.003 ~.001 ~.003 ~.377 ~.237 ~.309 ~.071 ~.287 \\
    &~.531 ~.044 ~.007 ~.086 ~.002 ~.019 ~.028 ~.007 ~.265 ~.013]\\
    \meanReward_{\text{untreated}}
    = [&.001 ~.023 ~.002 ~.002 ~.004 ~.289 ~.206 ~.229 ~.073 ~.289 \\
    &~.464 ~.035 ~.004 ~.052 ~.001 ~.011 ~.022 ~.004 ~.165 ~.000].
    \end{aligned}
\end{equation}

\noindent
The sizes of the clusters, which also correspond to $(\va[\nAffected])_{\arm\in\arms}$, are
%
\begin{align}
    \notag
    [&10600 ~2764 ~7222 ~11128 ~6385 ~1630 ~2806 ~1089 ~3018
     ~4594\\
     \notag
     &~594 ~7020 ~12654 ~2186 ~9609 ~5101 ~3714 ~4569
     ~1158 ~2159].
\end{align}


\newcommand{\shortminus}{\scalebox{0.75}[1.0]{\( - \)}}

\noindent
The uplifts of the actions (rounded to one decimal place) are
%
\begin{equation}
    \notag
    \begin{aligned}
    \up{\reward} =
    [&0.6 ~\,39.3 ~\,6.6 ~\,\shortminus5.0 ~\,\shortminus5.7 ~\,143.5 ~\,86.0 ~\,87.1 ~\,\shortminus4.5 ~\,\shortminus6.9 
    \\
    &~\,39.8 ~\,66.3 ~\,34.7 ~\,75.4 ~\,4.0
    ~\,40.3 ~\,21.1 ~\,12.3 ~\,115.7 ~\,28.3].
    \end{aligned}
\end{equation}




%\section{Additional Experimental Results}
%\label{apx:exp-add}

%In this section, we present additional experimental results omitted in~\cref{sec:exp}.


% \section{Ablation Study on Gaussian Uplifting Bandit}
% \label{apx:exp-add}
% %\label{apx:ablation}

% In this appendix, we present additional experimental results omitted in~\cref{sec:exp} that are conducted with the Gaussian uplifting bandit model.
% %presented in \cref{subsec:exp-gaussian}.

% \paragraph{Baseline UCB versus Baseline LCB\afterhead}
% In \cref{algo:UpUCB}, we suggest subtracting the UCBs of the baseline payoffs from the UCBs of the actions.
% This could be counter-intuitive because to get an optimistic estimate of the uplift, we should instead subtract the LCBs of the baseline payoffs.
% However, the latter strategy prevents the learner from learning more about the baselines that are badly estimated, and can thus lead to failure more frequently.
% %with the later strategy, if the baseline payoffs of a set of variables that a suboptimal arm affects are severely underestimated at the beginning, the learner may stick to that suboptimal arm, which results 
% In the following, we refer to the two strategies respectively as \UpUCB-bUCB and \UpUCB-bLCB.

% In \cref{subfig:UCB-LCB} (Left), we illustrate the mean regret of the two designs when their parameters are optimally tuned.
% It turns out there the two strategies perform similarly here.
% We would just like to highlight that to achieve the optimal performance, \UpUCB-bLCB needs to use a larger exploration parameter.
% Therefore, in terms of average performance, it seems that the effect of using LCBs of the baseline is close to 
% a shrinkage of the exploration parameter.

% Next, we further inspect the robustness of the algorithms by plotting the $95$th percentile of the regrets (which roughly corresponds to the $5$th largest regret among those recorded in the $100$ runs).
% The same parameters give the optimal values for this metric.
% However, as shown in \cref{subfig:UCB-LCB} (Right), it turns out that \UpUCB-bLCB achieves a much higher $95$th percentile of regret, which indicates that it indeed fails more frequently.

% \paragraph{Misspecification of $\nAffected$.}
% We also investigate the effect of misspecification of $\nAffected$ on \cref{algo:UpUCB-L-BL}.
% For the bandit instance that we employ here, $\max_{\arm\in\arms}\va[\nAffected]=10$ and thus according to \cref{prop:UpUCB-L-BL-regret}, \cref{algo:UpUCB-L-BL} guarantees sublinear regret as long as it is provided with $\nAffected\ge10$. On the flip side, the algorithm may incur linear regret if $\nAffected$ is underestimated.

% To verify this, we run the algorithm with $\nAffected\in\{5,8,10,15\}$ and plot the averaged regret and the $95$-th percentile of regret for optimally tuned exploration parameters in \cref{subfig:misL}.
% We effectively observe sublinear regret when $\nAffected$ is overspecified, but the regret becomes much larger because the algorithm is more conservative and explores more.
% On the other hand, under severe underspecification of $\nAffected$, the algorithm is doomed to fail whatever the exploration parameter used.
% Finally, it seems that slight underspecification of $\nAffected$ can be compensated by choosing a larger exploration parameter. In fact, in the figure we see that for $\nAffected=8$ choosing $\expparam=6$ gives the smallest regret among the presented curves.



==> Uplifting bandits - arxiv/Appendices/Lower-bound.tex <==
% In this appendix, we prove \cref{prop:lower-bound} that justify our key modeling assumptions. In particular, these lower bounds show that there would be a higher regret in absence of any of the following: \begin{enumerate*}[\textup(\itshape i\textup)]
% \item Limited number of affected variables,
% \item Side information about variables beyond just reward, and
% \item Some prior knowledge on how the variables are affected.
% \end{enumerate*}
% Moreover, we also derive matching lower bounds for \cref{prop:UpUCB-BL-regret}.
% We discuss these results in \cref{apx:lower-bound-statement}.
% Subsequently, we introduce a general information-theoretic lower bounds for bandit problems with similar design in \cref{apx:lower-bound-information}, based on which we prove the lower bounds in \cref{apx:proof-lower-bound}.

% \subsection{Lower Bounds for Uplifting Bandits-- Statements and Discussion}
% \label{apx:lower-bound-statement}

% To begin, we restate \cref{prop:lower-bound} from \cref{sec:lower} and introduce associated notations. 
% For sake of conciseness, in the following we say that an uplifting bandit has parameters $(\nArms,\nVariables,(\va[\gapbandit],\va[\nAffected])_{\arm\in\arms})$ if the number of actions, the number of variables, the suboptimality gaps, and the number of affected variables of this instance are respectively $\nArms$, $\nVariables$, $(\va[\gapbandit])_{\arm\in\arms}$, and $(\va[\nAffected])_{\arm\in\arms}$.
% %refer to any instance of the uplifting bandit problem as described in \cref{sec:model} with $\nArms$ arms, $\nVariables$ variables, suboptimality gaps $(\va[\gapbandit])_{\arm\in\arms}$, and numbers of affected variables $(\va[\nAffected])_{\arm\in\arms}$ noise as a $1$-sub-Gaussian $(\nArms,\nVariables,(\va[\gapbandit],\va[\nAffected])_{\arm\in\arms})$ uplifting bandit instance.
% We focus on instance-dependent lower-bounds and assume that the learner has full knowledge of the baseline distribution.
% %\footnote{%
% %Of course, the problem only becomes more challenging if the learner actually does not know the baseline distribution.}
% We also recall that our lower bounds are derived for the algorithms that are {\em consistent} \citepp{LR85} over the class of $1$-sub-Gaussian uplifting bandits, meaning the induced regret of the algorithm on any uplifting bandit with $1$-sub-Gaussian noise satisfies $\vt[\reg]=\smalloh(\run^p)$ for all $p>0$. 


% {
% \addtocounter{proposition}{-1}
% \renewcommand{\theproposition}{\ref{prop:lower-bound}}
% \begin{proposition}
% Let $\policy$ be a consistent algorithm over the class of $1$-sub-Gaussian uplifting bandits that at most uses knowledge of $\va[\distribution][0]$, $(\va[\variables])_{\arm\in\arms}$, and the fact that the noise is $1$-sub-Gaussian.
% Let $\nArms,\nVariables>0$ and sequence $(\va[\nAffected],\va[\gapbandit])_{1\le\arm\le\nArms}\in(\oneto{\nVariables}\times\R_+)^{\nArms}$ satisfy $\va[\gapbandit][1]=0$.
% %that at most uses knowledge of $\va[\distribution][0]$, $(\va[\variables])_{\arm\in\arms}$, and the fact that the noise is $1$-sub-Gaussian.
% Assume either of the following holds.
% \begin{enumerate}[(a)]
%     \item $\va[\nAffected]=\nVariables$ for all $\arm\in\arms$, so that in the bandits considered below all actions affect all variables.
%     \item Only the reward is observed.
%     %\item The prior knowledge of $\policy$ does not enable it to distinguish between any two bandits with the same baseline and noise distributions.
%     \item The algorithm $\policy$ does not make use of any prior knowledge about the arms' expected payoffs $(\va[\meanReward])_{\arm\in\arms}$ (in particular, the knowledge of $(\va[\variables])_{\allvariables}$ is not used by $\policy$).
% \end{enumerate}
% % Then, for any $\nArms,\nVariables>0$ and sequence $(\va[\nAffected],\va[\gapbandit])_{1\le\arm\le\nArms}\in(\oneto{\nVariables}\times\R_+)^{\nArms}$
% % %with $\va[\nAffected]\in\oneto{\nVariables}, \va[\nAffected][1]>\va[\gapbandit]\ge\max(0,\va[\nAffected][1]-\va[\nAffected])$ for all $\arm$ 
% % with $\va[\gapbandit][1]=0$,\footnote{Necessarily $\va[\nAffected]\equiv\nVariables$ under condition \ref{low-cond:affected}.}
% Then, there exists a $1$-sub-Gaussian uplifting bandit 
% with parameters $(\nArms,\nVariables,(\va[\gapbandit],\va[\nAffected])_{\arm\in\arms})$
% such that the regret induced by $\policy$ on it satisfies: 
% \[
% \liminf_{\toinf[\nRuns]} \frac{\ex[\vt[\reg][\nRuns]]}{\log\nRuns} \ge \sum_{\arm\in\arms:\va[\gapbandit]>0}\frac{2\nVariables^2}{\va[\gapbandit]}.
% \]
% \end{proposition}
% }
% %\LowerBound*
% % 

% % {
% % \renewcommand{\theproposition}{\ref{prop:lower-bound}}
% % \begin{proposition}[Formal]
% % \label{prop:lower-bound-formal}
% % Let $\policy$ be a consistent algorithm over the class of $1$-sub-Gaussian uplifting bandits that at most uses knowledge of $\va[\distribution][0]$, $(\va[\variables])_{\arm\in\arms}$, and the fact that the noise is $1$-sub-Gaussian.
% % Let $\nArms,\nVariables>0$ and sequence $(\va[\nAffected],\va[\gapbandit])_{1\le\arm\le\nArms}\in(\oneto{\nVariables}\times\R_+)^{\nArms}$ satisfy $\va[\gapbandit][1]=0$.
% % %that at most uses knowledge of $\va[\distribution][0]$, $(\va[\variables])_{\arm\in\arms}$, and the fact that the noise is $1$-sub-Gaussian.
% % Assume either of the following holds.
% % \begin{enumerate}[(a)]
% %     \item $\va[\nAffected]=\nVariables$ for all $\arm\in\arms$, so that in the bandits considered below all actions affect all variables.
% %     \label{low-cond:affected}
% %     \item Only the reward is observed.
% %     \label{low-cond:observed}
% %     \item The prior knowledge of $\policy$ does not enable it to distinguish between any two bandits with the same baseline and noise distributions.
% %     \label{low-cond:knowledge}
% % \end{enumerate}
% % % Then, for any $\nArms,\nVariables>0$ and sequence $(\va[\nAffected],\va[\gapbandit])_{1\le\arm\le\nArms}\in(\oneto{\nVariables}\times\R_+)^{\nArms}$
% % % %with $\va[\nAffected]\in\oneto{\nVariables}, \va[\nAffected][1]>\va[\gapbandit]\ge\max(0,\va[\nAffected][1]-\va[\nAffected])$ for all $\arm$ 
% % % with $\va[\gapbandit][1]=0$,\footnote{Necessarily $\va[\nAffected]\equiv\nVariables$ under condition \ref{low-cond:affected}.}
% % Then, there exists a $1$-sub-Gaussian uplifting bandit with parameters $(\nArms,\nVariables,(\va[\gapbandit],\va[\nAffected])_{\arm\in\arms})$
% % such that the regret induced by $\policy$ on it satisfies
% % %
% % \begin{equation}
% %     %\label{eq:lower-bound-m}
% %     \notag
% %     \liminf_{\toinf[\nRuns]} \frac{\ex[\vt[\reg][\nRuns]]}{\log\nRuns} \ge \sum_{\arm\in\arms:\va[\gapbandit]>0}\frac{2\nVariables^2}{\va[\gapbandit]}.
% % \end{equation}
% % \end{proposition}
% % \addtocounter{proposition}{-1}
% % }

% The conditions \ref{low-cond:affected} and \ref{low-cond:observed} echo assumptions \ref{asm:limited} and \ref{asm:observability}.
% Note that, however, the condition \ref{low-cond:observed} does not imply the necessity of observing all the payoffs. For example, observing the aggregated payoff $\sum_{\indv\in\va[\variables][\vt[\arm]]}\vtv[\valuev]$ is sufficient for computing the uplifting indices of \UpUCB.
% Having observation of the entire payoff vector $(\vtv[\valuev])_{\indv\in\variables}$ is particularly helpful for the case of unknown affected variables, as under this condition we can identify the affected variables relatively easily.

% Let us now provide some more intuition on the meaning of \ref{low-cond:knowledge}.
% For this, consider two bandits with exactly the same baseline and noise distributions and very close expected payoffs of the arms.
% Then, with finite observations, they provide very similar feedback which prevents the learner from distinguishing between the two problems.
% However, the two bandits may have completely different structures, and in particular, one of them may have all variables affected by all actions since slight perturbation to the baseline would mean that a variable is affected.
% Therefore, the lower bound from \ref{low-cond:affected} applies to this instance.
% Now, provided that the learner is doomed to treat the two instances equally, the lower bound applies to the other instance as well.
% Of course, one can argue that it is unnatural that the regrets of two similar problems differ significantly even when the learner is provided some prior knowledge.
% We believe this is the drawback of the asymptotic analysis that we look at here, since these differences may indeed be small within a reasonable number of runs. This is exactly related to the problem of misspecified model that we mentioned in \cref{footnote:small-impact}.

% The next proposition refines the lower-bound of \cref{prop:lower-bound}\ref{low-cond:affected} to show the optimality of \cref{prop:UpUCB-BL-regret}.
% %
% \begin{proposition}
% \label{prop:lower-bound-L}
% Let $\policy$ be a consistent algorithm over the class of $1$-sub-Gaussian uplifting bandits that at most uses knowledge of $\va[\distribution][0]$, $(\va[\variables])_{\arm\in\arms}$, and the fact that the noise is $1$-sub-Gaussian.
% Then, for any $\nArms,\nVariables>0$ and sequence $(\va[\nAffected],\va[\gapbandit])_{1\le\arm\le\nArms}\in(\oneto{\nVariables}\times\R_+)^{\nArms}$
% %with $\va[\nAffected]\in\oneto{\nVariables}, \va[\nAffected][1]>\va[\gapbandit]\ge\max(0,\va[\nAffected][1]-\va[\nAffected])$ for all $\arm$ 
% with $\va[\gapbandit][1]=0$, there exists a $1$-sub-Gaussian uplifting bandit $(\nArms,\nVariables,(\va[\gapbandit],\va[\nAffected])_{\arm\in\arms})$
% %a $1$-sub-Gaussian uplifting bandit instance with $\nArms$ arms, $\nVariables$ variables, suboptimality gaps $(\va[\gapbandit])_{\arm\in\arms}$, and numbers of affected variables $(\va[\nAffected])_{\arm\in\arms}$ 
% such that the regret induced by $\policy$ on it satisfies
% %
% \begin{equation}
%     \label{eq:lower-bound-L-1}
%     \liminf_{\toinf[\nRuns]} \frac{\ex[\vt[\reg][\nRuns]]}{\log\nRuns} \ge \sum_{\arm\in\arms:\va[\gapbandit]>0}\frac{2(\va[\nAffected])^2}{\va[\gapbandit]}.
% \end{equation} 
% \end{proposition}
% %
% %Clearly, \cref{prop:lower-bound} under condition \ref{low-cond:affected} is just a corollary of \cref{prop:lower-bound-L}, and 
% \cref{prop:lower-bound-L} essentially posits that the regret must scale with the magnitudes of the noises, and the stated lower bound \eqref{eq:lower-bound-L-1} matches an expected version of \eqref{eq:UpUCB-BL-regret} up to a constant factor.
% One way to argue this lower bound holds is by reducing a carefully designed uplifting bandits with parameters $(\nArms,\nVariables,(\va[\gapbandit],\va[\nAffected])_{\arm\in\arms})$ to a $\nArms$-arms bandit with the corresponding noise scales.
% We will take a different approach below which allows us prove all the lower bounds following the same schema.

% \vspace{0.4em}
% \begin{remark}
% Our lower bound is derived with respect to the worst correlation structure of the noise. It is also possible to obtain lower bounds that depend on the covariance of the noise. % using \cref{lem:lower-bound-instance-dependent}.
% For example, if the variables $(\vav[\valuev])_{\allvariables}$ are independent, the lower bound in \eqref{eq:lower-bound-L-1} only scales linearly with $\va[\nAffected]$.
% \end{remark}

% %two problem instances with different structures (\eg different $(\va[\variables])_{\arm\in\arms}$) can provide arbitrary close information to the learner, and thus the learner is doomed to treat them equally if they are not equipped with any prior knowledge that enables them to distinguish between the two problems.
% %Accordingly, the learner is not able to take advantage of the underlying structure, and no improvement of the performance can be achieved.

To prove our lower bounds, 
we fist establish in \cref{apx:lower-bound-information} a general lemma for deriving instance-dependent lower-bounds for bandit problems with underlying variables, side observations, and prior knowledge on the distribution of the variables.
Subsequently, in \cref{apx:proof-lower-bound} we regard uplifting bandit as a special case of this model and apply the lemma to prove \cref{prop:lower-bound,prop:lower-bound-L}.

\subsection{A General Information-theoretic Lower Bound}
\label{apx:lower-bound-information}



%serve as the main tool for proving the results in \cref{subsec:lower-bound-uplift}. Missing proofs are in~\cref{apx:lower-bound}.

Let $\valuev=(\vv[\valuev][1], \ldots, \vv[\valuev][\nVariables])$ be a random vector of $\nVariables$ variables 
that entirely determines the reward so that we can write $\reward=\rewardfunc(\valuev)$ for some deterministic reward function $\rewardfunc\from\R^{\nVariables}\to\R$.
%=\rewardfunc(\vv[\valuev][1], \ldots, \vv[\valuev][\nVariables])$.
Let $\va[\distribution]$ be the distribution of action $\arm$ on the underlying variables and $\va[\distribution][0]$ be the baseline distribution on these variables.
%Moreover, we will consider the general case where
At each round after taking an action, the learner observes a vector in $\R^{\vdim}$ that is itself a function of the variables, written as $\obs(\valuev)$ where $\obs\from\R^{\nVariables}\to\R^{\vdim}$ is the observation function.
%$\obs(\vv[\valuev][1], \ldots, \vv[\valuev][\nVariables])$.
The decision of which action to take can then only be based on the interaction history $(\vt[\arm][1],\obs(\vt[\valuev][1]),\ldots,\vt[\arm][\run-1],\obs(\vt[\valuev][\run-1]))$ and some prior knowledge of the learner about the distributions of the variables $\priorknow(\va[\distribution][0],\ldots,\va[\distribution][\nArms])$.\footnote{For our purpose, we can regard this as a partition of the set of all bandit instances that the learner may encounter.}

A class of action distributions is defined as $\banditclass=\va[\setDist][0]\times\cdots\times\va[\setDist][\nArms]$ where each $\va[\setDist]$ is a set of distributions on $\R^{\nVariables}$. 
We say that $\banditclass$ is indistinguishable under $\priorknow$ if for all $\distribution_{\ast}=(\va[\distribution])_{\arm\in\arms_0},\distributionalt_{\ast}=(\va[\distributionalt])_{\arm\in\arms_0}\in\banditclass$ we have $\priorknow(\va[\distribution][0],\ldots,\va[\distribution][\nArms])=\priorknow(\va[\distributionalt][0],\ldots,\va[\distributionalt][\nArms])$.
A bandit problem with underlying variables, side observations, and prior knowledge on the variable distribution is thus defined by the quadruple $(\banditclass,\rewardfunc,\obs,\priorknow)$.
A policy $\policy$ is said to be \emph{consistent} over $(\banditclass,\rewardfunc)$ if for all $p>0$ and all instance of $(\banditclass,\rewardfunc)$, the regret of $\policy$ on the instance satisfies $\vt[\reg][\run]=\smalloh(\run^{p})$.
A policy $\policy$ is compatible with observation $\obs$ and prior knowledge $\priorknow$ if it can be implemented by a learner that observes $\obs(\valuev)$ and has prior knowledge $\priorknow(\va[\distribution][0],\ldots,\va[\distribution][\nArms])$.

By abuse of notation, for any distributions $\distribution$ on $\R^{\nVariables}$ we will write $\rewardfunc(\distribution)=\ex_{\valuev\sim\distribution}(\rewardfunc(\valuev))$ as the expected reward when the variables follow distribution $\distribution$ whenever this quantity is defined.
We also write $\distribution_{\obs}$ as the pushforward of $\distribution$ along $\obs$.
Let $\setDist$ be a set of distributions such that $\rewardfunc(\distribution)$ is well-defined for any $\distribution\in\setDist$.
Let $\sol[\reward]\in\R$ and $\distribution\in\setDist$ such that $\rewardfunc(\distribution)<\sol[\reward]$.
The following quantity is crucial to the analysis
%
\begin{equation}
    \notag
    \infkl(\distribution,\setDist,\sol[\reward],\rewardfunc,\obs)=\inf_{\distributionalt\in\setDist}\setdef{\dkl(\distribution_{\obs},\distributionalt_{\obs})}{\rewardfunc(\distributionalt)>\sol[\reward]},
\end{equation}
%
where $\dkl(\distribution_{\obs},\distributionalt_{\obs})$ denotes the KL divergence of $\distribution_{\obs}$ from $\distributionalt_{\obs}$.
Intuitively, it quantities how difficult it is to learn that the expected reward $\rewardfunc(\distribution)$ is smaller than $\sol[\reward]$ (smaller the value of $\infkl$ the more difficult it is).
The next lemma is a straightforward adaptation of \citep[Th. 1]{BK96},\citep[Th. 16.2]{LS20} to our model.
It provides a lower bound on the asymptotic regret 

%, assumed to be known by the learner.
%We denote by $\priorknow((\va[\distribution])_{0\le\arm\le\nArms})$ the prior knowledge that the learner has about the problem.
%We will consider classes of such bandit problems written as $\banditclass=\va[\setDist][0]\times\cdots\times\va[\setDist][\nArms]$ where each $\va[\setDist]$ is a set of distributions.
%We say that $\banditclass$ is indistinguishable under $\priorknow$ if for all $(\va[\distribution])_{0\le\arm\le\nArms},(\va[\distributionalt])_{0\le\arm\le\nArms}\in\banditclass$ we have $\priorknow((\va[\distribution])_{0\le\arm\le\nArms})=\priorknow((\va[\distributionalt])_{0\le\arm\le\nArms})\in\banditclass$.

\begin{lemma}
\label{lem:lower-bound-instance-dependent}
Let $\banditclass=\va[\setDist][0]\times\cdots\times\va[\setDist][\nArms]$ be a class of action distributions and $\rewardfunc$ be the reward function.
Let $\policy$ be a consistent algorithm over $(\banditclass,\rewardfunc)$ that is compatible with prior knowledge function $\priorknow$ and observation function $\obs$. Then, if $\banditclass$ is indistinguishable under $\priorknow$, for all $\distribution_{\ast}\in\banditclass$, it holds that
%
\begin{equation}
    \label{eq:lower-bound-lemma}
    \liminf_{\toinf[\nRuns]} \frac{\ex[\vt[\reg][\nRuns]]}{\log\nRuns}
    \ge 
    \sum_{\arm\in\arms:\va[\gapbandit]>0}
    \frac{\va[\gapbandit]}{\infkl(\va[\distribution],\va[\setDist],\sol[\reward],\rewardfunc,\obs)}.
\end{equation}
\end{lemma}
\begin{proof}
The proof follow closely the one presented in \citep{LS20}.
The key observation is that the same proof still carries out if we have a random vector and our reward and observation depends on this random vector.
In particular, let $\measure(\policy,\distribution_{\ast})$ and $\measure(\policy,\distributionalt_{\ast})$ be the probability measure on the actions and the observations induced by the interaction of the policy with the bandit instances $(\distribution_{\ast},\rewardfunc)$ and $(\distributionalt_{\ast},\rewardfunc)$ for $\distribution_{\ast},\distributionalt_{\ast}\in\banditclass$.
The assumption that $\policy$ is compatible with $\obs$ and $\priorknow$ and that $\banditclass$ is indistinguishable under $\priorknow$ allows us to write 
$q_{\policy,\distribution_{\ast}}(\vt[\arm][1],\vt[\obs][1],\ldots,\vt[\arm][\nRuns],\vt[\obs][\nRuns])=\prod_{\run=1}^{\nRuns}\vt[\policy^{\banditclass}](\vt[\arm]|\vt[\arm][1],\vt[\obs][1],\ldots,\vt[\arm][\run-1],\vt[\obs][\run-1])\va[p_{\obs}][\vt[\arm]](\vt[\obs])$, where $\vt[\obs][1],\ldots,\vt[\obs][\nRuns]$ are the observations of the learner, $q_{\policy,\distribution_{\ast}}$ and $\va[p_{\obs}][\vt[\arm]]$ are respectively the probability density functions of $\measure(\policy,\distribution_{\ast})$ and $\va[\distribution_{\obs}]$, and $\vt[\policy^{\banditclass}]=\vt[\policy][\run,\priorknow(\distribution_{\ast})]=\vt[\policy][\run,\priorknow(\distributionalt_{\ast})]$ is a probability kernel that can be chosen using prior knowledge.\footnote{Many technical details are omitted here. We refer the interested readers to \citep{LS20} for a rigorous treatment of such proof.}
We have a similar decomposition for $q_{\policy,\distributionalt_{\ast}}$.
Then, following the proof of \citep[Lem. 15.1]{LS20} we get immediately
%
\begin{equation}
    \notag
    \dkl(\measure(\policy,\distribution_{\ast}),\measure(\policy,\distributionalt_{\ast}))=\sum_{\arm\in\arms}\ex_{\policy,\distribution}[\vta[\pullcount][\nRuns]]\dkl(\va[\distribution_{\obs}],\va[\distributionalt_{\obs}]).
\end{equation}
%
In the above, $\ex_{\policy,\distribution}$ means that the expectation is taken with respect to $\measure(\policy,\distribution_{\ast})$. The proof can be completed in the same way as done for \citep[Th. 16.2]{LS20}.
\end{proof}


\subsection{Lower Bounds for Uplifting Bandits-- Proof}
\label{apx:proof-lower-bound}

%\LowerBound*
The following proposition includes both \cref{prop:lower-bound} and \cref{prop:lower-bound-L}.

\begin{proposition}%[\cref{prop:lower-bound} Restated]
\label{prop:lower-bound-app}
Let $\policy$ be a consistent algorithm over the class of $1$-sub-Gaussian uplifting bandits that at most uses knowledge of $\va[\distribution][0]$, $(\va[\variables])_{\arm\in\arms}$, and the fact that the noise is $1$-sub-Gaussian.
Then, for any $\nArms,\nVariables>0$ and sequence $(\va[\nAffected],\va[\gapbandit])_{1\le\arm\le\nArms}\in(\oneto{\nVariables}\times\R_+)^{\nArms}$
%with $\va[\nAffected]\in\oneto{\nVariables}, \va[\nAffected][1]>\va[\gapbandit]\ge\max(0,\va[\nAffected][1]-\va[\nAffected])$ for all $\arm$ 
with $\va[\gapbandit][1]=0$, there exists a $1$-sub-Gaussian uplifting bandit with parameters $(\nArms,\nVariables,(\va[\gapbandit],\va[\nAffected])_{\arm\in\arms})$
%a $1$-sub-Gaussian uplifting bandit instance with $\nArms$ arms, $\nVariables$ variables, suboptimality gaps $(\va[\gapbandit])_{\arm\in\arms}$, and numbers of affected variables $(\va[\nAffected])_{\arm\in\arms}$ 
such that the regret induced by $\policy$ on it satisfies
%
\begin{equation}
    \label{eq:lower-bound-L}
    \liminf_{\toinf[\nRuns]} \frac{\ex[\vt[\reg][\nRuns]]}{\log\nRuns} \ge \sum_{\arm\in\arms:\va[\gapbandit]>0}\frac{2(\va[\nAffected])^2}{\va[\gapbandit]}.
\end{equation} 
% \todob{Write ${L^a}^2$ as $(L^a)^2$.}
%
Moreover, if $\policy$ can be implemented under either of the following conditions
\begin{enumerate}[(a)]
    \item Only the reward is observed.
    \item The learner does not have any prior knowledge about the arms' expected payoffs.
    %cannot distinguish between any two bandits with the same baseline and noise distributions.
    %(in particular, the learner does not know $(\va[\variables])_{\arm\in\arms}$).
    %The prior knowledge of the learner on the distributions is further restricted to the point that it does not enable the learner to distinguish between any two instances with the same baseline and noise distributions (in particular, the learner does not know $(\va[\variables])_{\arm\in\arms}$).
    %does not encode any information about the means of the arms
    %only encodes information about the baseline and the noise distributions.
    %does not allow the leaner to know anything more than the baseline distribution and the covariance of the noise.
    %is that the noise is $1$-sub-Gaussian, \ie $\priorknow(\va[\distribution][0],\va[\distribution][1],\ldots,\va[\distribution][\nArms])=\priorknow(\va[\distribution][0],\va[\distributionalt][1],\ldots,\va[\distributionalt][\nArms])$ as long as $\va[\distribution]$'s and $\va[\distributionalt]$'s satisfy \cref{asm:noise}.
    %The learner has no prior knowledge on how the variables are affected.\footnote{Formally, as we will see in the proof, this means that for a fixed baseline distribution, the prior knowledge of the learner does not allow they to distinguish between two instances whose mean values $(\va[\meanReward])_{\arm\in\arms}$ are arbitrarily different.}
\end{enumerate}
Then, there exists a $1$-sub-Gaussian uplifting bandit with parameters $(\nArms,\nVariables,(\va[\gapbandit],\va[\nAffected])_{\arm\in\arms})$ where the regret of $\policy$ is
\begin{equation}
    \label{eq:lower-bound-m}
    \liminf_{\toinf[\nRuns]} \frac{\ex[\vt[\reg][\nRuns]]}{\log\nRuns} \ge \sum_{\arm\in\arms:\va[\gapbandit]>0}\frac{2\nVariables^2}{\va[\gapbandit]}.
\end{equation}
\end{proposition}

\begin{proof}
Let $\sol[\reward]=1+\max_{\arm\in\arms}\va[\gapbandit]>0$.
%(1+\max_{\arm\in\arms}\va[\gapbandit])/2\in(0,1)$.
Throughout the proofs, the lower bound will be shown for problem instances with $\vav[\meanReward][0]\equiv0$ and the following mean values for $\arm\in\arms$
%
\begin{equation}
    \label{eq:lower-bound-proof-mean-value}
    \vav[\meanReward][\arm]=\begin{dcases}
    \frac{\sol[\reward]-\va[\gapbandit]}{\va[\nAffected]} & ~\text{if }  1\le\indv\le\va[\nAffected],\\
    \hfil 0 & ~\text{if } \va[\nAffected]+1\le\indv\le\nVariables.
    \end{dcases}
\end{equation}
%
By construction, we have %effectively $\vav[\meanReward]\in[0,1]$ for all $\arm$ and $\indv$. Moreover, 
$\vav[\meanReward]\neq\vav[\meanReward][0]$ if and only if $1\le\indv\le\va[\nAffected]$ and thus the number of mean-affected variables of $\arm$ is exactly $\va[\nAffected]$.
Clearly, $1$ is an optimal action and the suboptimality gap of action $\arm$ is $\va[\gapbandit]$.

Next, we will need to define the classes of action distributions $\banditclass_1, \banditclass_2, \banditclass_3$ that we will use for proving \eqref{eq:lower-bound-L}, (a)-\eqref{eq:lower-bound-m}, and (b)-\eqref{eq:lower-bound-m}.
To begin, we want these classes to be indistinguishable under a certain prior knowledge function, and since we allow the learner to know the baseline distribution, $\va[\setDist][0]$ must be a singleton.
As for $\va[\setDist]$, it will take the form $\va[\setDist]=\setdef{\gaussian(\meanReward,\va[\covmat])}{\meanReward\in\va[\meanRewards]}$ for some mean vector set $\va[\meanRewards]\subset \R^{\nVariables}$ and covariance matrix $\va[\covmat]\in[0,1]^{\nVariables\times\nVariables}$ to be specified.
This implies that every noise variable $\vav[\snoise]$ is $1$-sub-Gaussian and thus $\policy$ is consistent in each of these classes.
Moreover, the classes will also be defined in such a way that when the mean values are taken as in \eqref{eq:lower-bound-proof-mean-value}, $\va[\distribution][0]$ and $\va[\distribution]$ indeed have the same marginal distribution on all but the first $\va[\nAffected]$ variables.

\paragraph{The Importance of Limited Number of Affected Variables\afterhead}
To prove \eqref{eq:lower-bound-L}, we let the unique element of $\setDist_0$ be the Dirac measure that assigns full weight to the point $(0,\ldots,0)$. For any $\arm\in\arms$, we define $\va[\meanRewards]=(\setexclude{\R}{\{0\}})^{\va[\nAffected]}\times\{0\}^{\va[\nVariables-\nAffected]}$ and block matrix $\va[\covmat]$ such that $\vam[\covmat]=\one\{\max(\indv,\indvalt)\le\va[\nAffected]\}$. In other words, the random variable $\va[\valuev]$ can be written in the following form
%
\begin{equation}
    \notag
    \vav[\valuev][\arm]=\begin{dcases}
    \vav[\meanReward][\arm]+\va[\snoise] & ~\text{if } 1\le\indv\le\va[\nAffected],\\
    \hfil 0 & ~\text{if } \va[\nAffected]+1\le\indv\le\nVariables,
    \end{dcases}
\end{equation}
%
where $\va[\snoise]$ is Gaussian with zero mean and unit variance. Notice that the same noise applies to all the affected variables.
By construction, every $\va[\distribution]\in\va[\setDist]$ has exactly the first $\va[\nAffected]$ variables affected, \ie $\va[\variables]=\{1,\ldots,\va[\nAffected]\}$.
Thus $\banditclass_1$ defined in this way is indistinguishable under prior knowledge on baseline distribution $\va[\distribution][0]$ and the sets of affected variables $(\va[\variables])_{\arm\in\arms}$.
To conclude, we would like to apply \cref{lem:lower-bound-instance-dependent}.
For this, we observe that for any $\va[\distribution],\va[\distributionalt]\in\va[\setDist]$ with means $\va[\meanReward]$ and $\va[\meanRewardalt]$, it holds\footnote{This can for example be proved by applying the chain rule of KL divergence.}
%
\begin{equation}
    \label{eq:dkl-PQ-B1}
    \dkl(\va[\distribution],\va[\distributionalt]  )=\begin{dcases}
    \frac{\gapvariable^2}{2} & ~\text{if } \vav[\meanReward]-\vav[\meanRewardalt]=\gapvariable 
    \text{ for all } \indv\in\intinterval{1}{\va[\nAffected]},\\
    \hfil +\infty & ~\text{otherwise}.
    \end{dcases}
\end{equation}
%
With this we see immediately that for $\va[\distribution]$ with mean values \eqref{eq:lower-bound-proof-mean-value}, we have $\infkl(\va[\distribution],\va[\setDist],\sol[\reward],(+),\Idf)=\va[\gapbandit]/(2(\va[\nAffected])^2)$, where $(+)$ and $\Idf$ are respectively the sum and the identity function that gives the reward and the observations of the learner.
Plugging this into \eqref{eq:lower-bound-lemma} gives exactly \eqref{eq:lower-bound-L}.

\paragraph{The importance of Side Observation\afterhead}
To construct $\banditclass_2$, we draw the same noise for all the variables. In terms of covariance matrix, this means all the entries of $\covmat$ is equal to $1$. 
The baseline distribution is $\va[\distribution][0]=\gaussian(\bb{0},\covmat)$ and for every $\arm$, we set $\va[\covmat]=\covmat$ and choose again $\va[\meanRewards]=(\setexclude{\R}{\{0\}})^{\va[\nAffected]}\times\{0\}^{\va[\nVariables-\nAffected]}$.
This time, only the reward, that is, the sum of the variables, is observed,
and the distribution of the reward at action $\arm$ is $\gaussian(\sol[\reward]-\va[\gapbandit],\nVariables^2)$.
For any two real numbers $\scalar, \alt{\scalar}$, one has $\dkl(\gaussian(\scalar,\nVariables^2),\gaussian(\alt{\scalar},\nVariables^2))=(\scalar-\alt{\scalar})^2/(2\nVariables^2)$.
Therefore $\infkl(\va[\distribution],\va[\setDist],\sol[\reward],(+),(+))=\va[\gapbandit]/(2\nVariables^2)$ for $\va[\distribution]$ with mean values \eqref{eq:lower-bound-proof-mean-value}.
Notice that $\banditclass_2$ is also indistinguishable under prior knowledge on the baseline distribution and on the sets of affected variables $(\va[\variables])_{\arm\in\arms}$, and thus \cref{lem:lower-bound-instance-dependent} can be applied, leading to \eqref{eq:lower-bound-m}.

\paragraph{The Importance of Prior Knowledge on How the Variables are Affected\afterhead}
The class $\banditclass_3$ is defined almost in the same way as $\banditclass_2$ except for the fact that we now set $\va[\meanRewards]=\R^{\nVariables}$ for every $\arm\in\arms$.
Our condition (b) postulates that $\banditclass_3$ is indistinguishable under the prior knowledge of the learner.
Similar to \eqref{eq:dkl-PQ-B1}, for any $\va[\distribution],\va[\distributionalt]\in\va[\setDist]$ with means $\va[\meanReward]$ and $\va[\meanRewardalt]$, we now have
%
\begin{equation}
    \notag
    \dkl(\va[\distribution],\va[\distributionalt])=\begin{dcases}
    \frac{\gapvariable^2}{2} & ~\text{if } \vav[\meanReward]-\vav[\meanRewardalt]=\gapvariable 
    \text{ for all } \indv\in\intinterval{1}{\nVariables},\\
    \hfil +\infty & ~\text{otherwise}.
    \end{dcases}
\end{equation}
%
In particular, if $\va[\meanReward]$ is defined as in \eqref{eq:lower-bound-proof-mean-value} and $\vav[\meanRewardalt]=\vav[\meanReward]+(\va[\gapbandit]+\eps)/\nVariables$ for all $\indv$ for some $\eps\in\R$, we have $\dkl(\va[\distribution],\va[\distributionalt])=(\va[\gapbandit]+\eps)^2/(2\nVariables^2)$.
We deduce immediately $\infkl(\va[\distribution],\va[\setDist],\sol[\reward],(+),\Idf)=\va[\gapbandit]/(2\nVariables^2)$.
Invoking \cref{lem:lower-bound-instance-dependent} completes the proof.
\end{proof}




==> Uplifting bandits - arxiv/Appendices/Missing.tex <==
\input{Tables/Notations}


==> Uplifting bandits - arxiv/Appendices/Related.tex <==
% In this appendix we complete our related work by providing comparison to some other models in the bandit literature.

\paragraph{Causal Bandits\afterhead}
The term causal bandits captures the general idea that in a bandit model the generation of reward may be governed by some causal mechanism while the actions correspond to interventions on the underlying causal graph.
This idea was first formalized in \citep{lattimore2016causal} and subsequently explored in a series of work \cite{lee2018structural,lu2020regret,nair2021budgeted} that cover multiples variants of the problem, including both the minimization of simple and cumulative regrets.
Our problem fits into the causal bandit framework by regarding \cref{fig:model} as a simple causal graph where the variables consist of all the directed causes of the reward and the actions correspond to atomic interventions on the action nodes.
The observability of these direct causes are also key assumptions in many of the aforementioned works.
Moreover, in the unknown affected case our causal graph is in fact partially unknown.
This is an intriguing problem in causal bandits as argued by \citep{LMT21}.
While we have shown improvement of the algorithms for this specific model, a interesting question is whether similar improvement can still be shown in more general causal bandit models under the assumption that each actions only affects a limited number of variables of the causal graph.

\paragraph{Combinatorial Bandits\afterhead}
In combinatorial bandits~\cite{cesa2012combinatorial}, the learner selects at each round a subset of ground items depending on which the reward is computed.
In its simplest form, the reward is just the sum of the payoffs of the selected items.
Of particular relevance to us is the semi-bandit setting~\cite{CWY13,KWAS15}, which assumes that the payoffs of the selected items are also observed.
This structure of the reward and observability of individual payoffs both suggest a strong similarity between our model and semi-bandits.
However, this comes with an important conceptual difference: the set of items, or variables, for which we observe the outcomes are selected in semi-bandits, while for us they are fixed and inherent to the reward generation mechanism.
As an example, in example \ref{ex:movie}, combinatorial bandit models optimize the number of movies that are watched among the recommended ones, while we also consider non-recommended movies.
In fact, as argued in \citep{WLCB20}, a recommendation is only effective if the user actually watches the movie and would not watch it without the recommendation

On the other hand, mathematically, it is possible to fit our model into the stochastic combinatorial semi-bandit framework when the sets of affected variables are known.
For this, consider a semi-bandit problem with $\nVariables+\sum_{\arm\in\arms}\va[\nAffected]$ items that correspond to the random variables $\setdef{\vav[\valuev][0]}{\indv\in\variables}\union\bigcup_{\arm\in\arms}\setdef{\vav[\valuev]}{\indv\in\va[\variables]}$.
At each round, the learner selects $\nVariables$ items that depends on the taken action and observes the payoffs of the selected items.
More precisely, when action $\arm$ is taken, the selected items are $\setdef{\vav[\valuev][0]}{\indv\in\setcomplement{\va[\variables]}}\union\setdef{\vav[\valuev]}{\indv\in\va[\variables]}$.

In terms of algorithm, let us consider the \UpUCBwb algorithm described in \cref{algo:UpUCB}, which is based on selecting the action with the largest uplift index $\vta[\UPindexSum]=\sum_{\indv\in\va[\variables]}(\vtav[\UCBindex]-\vtav[\UCBindex][\run][0])$.
We notice that the quantity $\vta[\UCBindex]=\sum_{\indv\in\variables}\vtav[\UCBindex]=\vta[\UPindexSum]+\sum_{\indv\in\variables}\vtav[\UCBindex][\run][0]$ is indeed an upper confidence bound on the reward of action $\arm$ and \UpUCBwb is equivalent to choosing the action with the largest $\vta[\UCBindex]$ in each round.
This observation indeed reduces \UpUCBwb to CombUCB~\cite{CWY13,KWAS15} on the transformed model.
Nonetheless, the \UpUCBwb formulation has several advantages:
\begin{enumerate}[topsep=2pt, itemsep=1.5pt, parsep=2pt, leftmargin=*]%[\itshape i\upshape)]
    \item It captures the fact that we really care about is the uplifting effect and the variables affected by each action.
    \item The uplifting interpretation facilitates algorithm design in more involved situations as we have shown in \cref{sec:unknown-affected}.
    \item While the general analysis of CombUCB yields a regret in %$\bigoh((\nVariables+\sqrt{\nVariables\nArms\nAffected})\sqrt{\nRuns\log\nRuns})$ and
    $\bigoh((\nVariables^2+\nVariables\nArms\nAffected)\log\nRuns/\gapbandit)$, we have shown in \cref{thm:UpUCB-regret} that the regret of \UpUCBwb is in $\bigoh(\nAffected^2\log\nRuns/\gapbandit)$.
    Our analysis presented in \cref{apx:proof-UpUCBwb} also greatly benefits from the \UpUCBwb formulation of the algorihhm.
    %clearly indicates that the number of variables $\nVariables$ should have no effect in our regret bound, as we demonstrate immediately in the following theorem.
    %this will be discussed in more detail in the next paragraph. %\cref{subsec:UpUCB-regret}.
\end{enumerate}

% \vspace{0.4em}
% \begin{remark}
% With the CombUCB formulation of the algorithm, one can deduce the regret is in $\bigoh((\alt{\nVariables}\nArms\nAffected)\log\nRuns/\gapbandit)$
% %Indeed, it is rather straightforward to improve from $\nVariables$ to $\min(\nArms\nAffected,\nVariables)$
% by arguing that at most $\alt{\nVariables}\defeq\min(\nArms\nAffected,\nVariables)$ items are involved in the learning process.
% Our result further improves this by a factor of $\min(\nArms,\nVariables/\nAffected)$.
% \end{remark}




%The term uplift is borrowed from the field of uplift modeling \citep{radcliffe2007using,gutierrez2017causal}.
% We borrow the term uplift from {\em uplift modeling} \citep{radcliffe2007using,gutierrez2017causal}; the latter refers to a collection of techniques for modelling the incremental effect of an action on an individual's behavior.
% %The goal there is to design algorithms to model the incremental effect of an action on an individual's behavior
% At a high level, both uplifting modeling and \ac{MAB} %have the common goal of finding the optimal strategy
% are important tools for decision making, as they both help select an optimal action.
% Despite this apparent relation between the two concepts, few papers explicitly link them together.
% We believe this is because a combination of the two often just results in a redefinition of the reward, on top of which classic bandit algorithms can be applied. This approach was taken in \citep{sawant2018contextual,berrevoets2019optimising}.
% %Both papers alter the goal of the bandit problems and apply existing bandit algorithms to solve the transformed problem
% Instead, our paper
% %takes a different approach and
% focuses on bandit problems in which estimating the uplifts improves the statistical efficiency of the algorithms and designs algorithms for that purpose.

% To achieve this, we assume the reward to be the sum of a set of observable variables and leverage the \emph{sparsity} of an action's effects on these variables.
% The decomposition of reward and the observability of partial rewards also appear in semi-bandit \citep{CWY13,KWAS15}.
% However, there the reward is the sum of the the selected items while for us the set of variables is fixed for every action.
% On the other hand, understanding the benefit of sparsity in \ac{MAB} has been a research topic of emerging interest.
% Most of these works focus on sparsity of the parameter vectors in linear bandit, which could be of great interest in the high-dimensional setting, see \eg \citep{abbasi2012online,bastani2020online,hao2021information} and references therein.
% A notable exception is \citep{kwon2017sparse}, where the authors study a variant of the classical \ac{MAB} problem in which the sparsity is reflected by that fact that the number of arms with positive reward is small.
% Our work is orthogonal to all of these in that we look at a different form of sparsity. As we will see in \cref{subsec:contextual-linear}, while sparsity in parameter can be a cause of sparsity in action effect, the improvement of regret is established with a different mechanism.

%\citep{abbasi2012online,carpentier2012bandit,bastani2020online,hao2021information}


==> Uplifting bandits - arxiv/Appendices/UpUCB-GapUp-UBL.tex <==
% % \subsection{Known Lower Bound on Individual Uplift} \label{sec:part2}


% % \label{sec:part2}
% % Another type of knowledge that can help the learner exploit the structure is a lower bound on individual uplift.
% % This is defined as $\gapUplift>0$ such that for all $\arm\in\arms$ and $\indv\in\va[\variables]$, $\abs{\vav[\meanReward]-\vav[\meanReward][0]}\ge\gapUplift$.
% % Similar assumption were made by \citet{LMT21} to identify which node in the causal graph affects the reward variable.
% % Indeed, this gives us an indicator on how many times we need to take each action in order to identify all its affected variables.

% % Again in this scenario, we derive regret bounds for both when the baseline payoffs are known or not to the learner. 
% % Our algorithms combine UCB, successive elimination \cite{even2006action}, and the idea that the affected variables can be identified after an action is taken sufficiently many times.
% % Our regret bounds feature the ratio $\va[\gapbandit]/\gapUplift$, suggesting that this knowledge is helpful when $\gapUplift$ is relatively large. 
% % We defer details to~\cref{apx:unknown-affected-2}.

% In this second part of~\cref{sec:unknown-affected}, we assume a lower bound on individual uplift is known.
% This means the learner has access to $\gapUplift>0$ satisfying that for all $\arm\in\arms$ and $\indv\in\va[\variables]$, $\abs{\vav[\meanReward]-\vav[\meanReward][0]}\ge\gapUplift$.
% This gives us an indicator on how many times we need to take each action in order to identify all the affected variables. Similar assumption were made by \citet{LMT21} to identify which node in the causal graph affects the reward variable.

% Again in this scenario, we derive regret bounds for both when the baseline payoffs are known or not to the learner. 
% Our algorithms combine UCB, successive elimination \cite{even2006action}, and the idea that the affected variables can be identified after an action is taken sufficiently many times.
% Our regret bounds feature the ratio $\va[\gapbandit]/\gapUplift$, suggesting that this knowledge is helpful when $\gapUplift$ is relatively large. 

% %Our regret bound will feature the ratio $\va[\gapbandit]/\gapUplift$, suggesting that this information is helpful when $\gapUplift$ is relatively large.
% Hereinafter, for any $x,\alpha,\beta\in\R$ with $\alpha\le\beta$, we use $\clip(x,\alpha,\beta)$ to denote the clipping function that restricts $x$ to the interval $[\alpha,\beta]$, \ie $\clip(x,\alpha,\beta)=\max(\alpha,\min(\beta,x))$.

% \subsection{Known Baseline Payoffs}

% As we have seen in \cref{sec:unknown-affected},
% if the baseline payoffs $\va[\meanReward][0]$ are known, we can directly check whether $\vav[\meanReward][0]$ is in the confidence interval.
% Moreover, with the knowledge $\abs{\vav[\meanReward]-\vav[\meanReward][0]}\ge\gapUplift$ for all $\indv\in\va[\variables]$, we deduce that $\va[\variables]$ can be identified correctly with probability $1-2\nVariables\alt{\smallproba}$ after action $\arm$ is taken $\pullcount_0=\ceil{(8/\gapUplift^2)\log(1/\alt{\smallproba})}$ times.
% In fact, let $\vta[\valuev][1],\ldots,\vta[\valuev][\pullcount_0]$ be $\pullcount_0$ i.i.d. realizations of $\va[\valuev]\sim\va[\distribution]$ and $\vtav[\tilde{\meanReward}][\pullcount_0]=(\sum_{\run=1}^{\pullcount_0}\vtav[\valuev])/\pullcount_0$ be the empirical mean of variable $\indv$.
% %Choosing $\varepsilon\in(0,\gapUplift)$ such that $\pullcount_0=(8/(\gapUplift-\varepsilon)^2)\log(1/\alt{\smallproba})$.\footnote{Such $\varepsilon$ exists (and of course, is unique) because $\pullcount_0>(8/\gapUplift^2)\log(2\nVariables/\alt{\smallproba})$.}
% Applying the sub-Gaussian concentration inequality \eqref{eq:sub-Gaussian-concentration} gives
% %
% \begin{equation}
%     \prob\left(\abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward]}\ge\frac{\gapUplift}{2}\right)
%     \le2
%     \exp\left(-\frac{\pullcount_0\gapUplift^2}{8}\right)
%     \le 2\alt{\smallproba}.
%     %\frac{\alt{\smallproba}}{\nVariables}.
% \end{equation}
% %
% With a union bound we conclude that with probability at least $1-2\nVariables\alt{\smallproba}$ it holds for all $\indv$ that $\abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward]}<\gapUplift/2$.
% We distinguish between the following two situations
% %
% \begin{enumerate}
%     \item $\indv\in\va[\variables]$, then $\displaystyle \abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward][0]}\ge\abs{\vav[\meanReward]-\vav[\meanReward][0]}-\abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward]}>\gapUplift-\frac{\gapUplift}{2}=\frac{\gapUplift}{2}$.
%     \item $\indv\notin\va[\variables]$, then $\displaystyle \abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward][0]}=\abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward]}<\frac{\gapUplift}{2}$.
% \end{enumerate}
% %
% This implies that with the choice
% $\va[\setId] = \setdef{\indv\in\variables}{\abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward][0]}>\gapUplift/2}$, we have effectively $\prob(\va[\setId]=\va[\variables])\ge1-2\nVariables\alt{\smallproba}$.
% One natural algorithm is to thus first pull each arm $\pullcount_0$ times and run \UpUCB (\cref{algo:UpUCB-BL}) %(from~\cref{subsec:UpUCB-BL})
% in the remaining rounds by regarding $\va[\setId]$ as the variables that action $\arm$ affects.
% A direct computation shows that the regret of this algorithm is in
% $\bigoh(\sum_{\arm\in\arms:\va[\gapbandit]>0}(\va[\gapbandit]/\gapUplift+\va[\nAffected])^2\log\nRuns/\va[\gapbandit])$.
% %$\bigoh(\pullcount_0\sum_{\arm\in\arms}\va[\gapbandit]+(\nArms\nAffected^2)\log\nRuns/\gapbandit)$.

% However, $\pullcount_0$ can be arbitrarily large when $\gapUplift$ gets closer to $0$, and taking an action much fewer times is probably sufficient to deduce that action is not optimal (with high probability).
% We thus propose to implement the above idea in a more flexible manner:
% We run \UpUCB with the uplifting indices $\vta[\UPindexSum]=\sum_{\indv\in\vta[\setId]}(\vtav[\UCBindex]-\vav[\meanReward][0])$, where
% %
% \begin{equation}
%     \notag
%     \vta[\setId] =
%     \begin{cases}
%     \variables & \text{if} ~ \vta[\pullcount]<\pullcount_0,\\
%     \setdef{\indv\in\variables}{\abs{\vtav[\est{\meanReward}][\run][\vt[\arm]]-\vav[\meanReward][0]}>\gapUplift/2} & \text{otherwise}.
%     \end{cases}
% \end{equation}
% %
% %known baseline payoffs by assuming that all the actions affect all the variables.
% %Then, for each arm $\arm$, as long as its pull count exceeds $\pullcount_0$, we switch the index by considering $\va[\setId]$ as the affected set.
% This algorithm is summarized in \cref{algo:UpUCB-GapUp-BL} and has the following regret guarantee.

% \input{Algorithms/UpUCB_GapUp_BL}

% \begin{theorem}
% \label{thm:UpUCB-GapUp-BL-regret}
% Let $\alt{\smallproba}=\smallproba/(2\nArms\nVariables\nRuns)$. Then the regret of \UpUCBDelta (\cref{algo:UpUCB-GapUp-BL}), 
% with probability at least $1-\smallproba$, satisfies:
% %
% \begin{equation}
%     \label{eq:UpUCB-GapUp-BL-regret}
%     \vt[\reg][\nRuns] \le
%     \sum_{\arm\in\arms:\va[\gapbandit]>0}
%     \left(\frac{8\thinspace\clip(\va[\gapbandit]/\gapUplift,\va[\nAffected],\nVariables)^2\log(2\nArms\nVariables\nRuns/\smallproba)}{\va[\gapbandit]}+\va[\gapbandit]\right).
% \end{equation}
% \end{theorem}
% \begin{proof}
% As before, we prove \eqref{eq:UpUCB-GapUp-BL-regret} under the condition that $\event$ defined in \eqref{eq:UCB-L-event} occurs. Recall that we have shown in the proof of \cref{prop:UpUCB-L-BL-regret} that $\prob(\event)\ge1-\smallproba$ with our choice of $\alt{\smallproba}$, so this effectively leads to a high-probability regret bound.

% In the following we assume that $\event$ occurs and show that for any suboptimal action $\arm\in\arms$, it holds
% %
% \begin{equation}
%     \label{eq:UpUCB-GapUp-pullcount-bound}
%     \vta[\pullcount][\nRuns]
%     \le
%     \max\left(
%     \min\left(
%     \frac{8\log(1/\alt{\smallproba})}{\gapUplift^2},
%     \frac{8\nVariables^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right), \frac{8(\va[\nAffected])^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right)
%     +1.
% \end{equation}
% %
% The inequality \eqref{eq:UpUCB-GapUp-BL-regret} then follows directly from \eqref{eq:regret-decomp-apx} and a rearrangement of the terms.

% We first claim that for any $\arm\in\arms$ if $\vta[\pullcount]\ge\pullcount_0$ then $\vta[\setId]=\va[\variables]$.
% In fact, by the definition of $\pullcount_0$, $\vta[\pullcount]\ge\pullcount_0$ implies that $\vta[\radiusConf]<\gapUplift/2$.
% Therefore, as argued in the text, $\indv\in\vta[\setId]$ if and only if $\indv\in\va[\variables]$.
% Since $\vtav[\UPindex]\ge\vav[\meanUplift]$ for any $\arm$ and $\indv$, this also proves that $\vta[\UPindex]\ge\va[\uplift]$ always holds (we have either $\vta[\setId]=\variables$ or $\vta[\setId]=\va[\variables]$).

% Let $\run\in\intinterval{\nArms+1}{\nRuns}$ be the last time that a suboptimal action $\arm$ is taken so that $\vta[\pullcount][\nRuns]=\vta[\pullcount][\run-1]+1$.
% This indicates $\vta[\UPindexSum]\ge\vta[\UPindexSum][\run][\sol[\arm]]$, and hence $\vta[\UPindexSum]\ge\va[\uplift][\sol[\arm]]$.
% We distinguish between the following two cases:
% %
% \begin{enumerate}[itemsep=2.5pt,topsep=2.5pt,parsep=2.5pt]
%     \item $\vta[\pullcount][\run-1]<\pullcount_0$:
%     Then $\vta[\setId]=\variables$ so $\vta[\UPindexSum]=\sum_{\indv\in\variables}(\vtav[\UCBindex]-\va[\meanReward][0])
%     \le\va[\uplift]+2\nVariables\vta[\radiusConf][\run-1]$, which in turn leads to $\vta[\radiusConf][\run-1]\ge\va[\gapbandit]/(2\nVariables)$, or equivalently $\vta[\pullcount][\run-1]\le8\nVariables^2\log(1/\alt{\smallproba})/(\va[\gapbandit])^2$.
%     \item $\vta[\pullcount][\run-1]\ge\pullcount_0$:
%     Then $\vta[\setId]=\va[\variables]$ so $\vta[\UPindexSum]=\sum_{\indv\in\va[\variables]}(\vtav[\UCBindex]-\va[\meanReward][0])
%     \le\va[\uplift]+2\va[\nAffected]\vta[\radiusConf][\run-1]$, which in turn leads to $\vta[\radiusConf][\run-1]\ge\va[\gapbandit]/(2\va[\nAffected])$, or equivalently $\vta[\pullcount][\run-1]\le8(\va[\nAffected])^2\log(1/\alt{\smallproba})/(\va[\gapbandit])^2$.
% \end{enumerate}
% %
% Since we also have $\vta[\pullcount][\run-1]<\pullcount_0$ in the first case, the above gives
% %
% \begin{equation}
%     \notag
%     \vta[\pullcount][\run-1]
%     \le
%     \max\left(
%     \min\left(
%     \pullcount_0-1,\frac{8\nVariables^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right), \frac{8(\va[\nAffected])^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right).
% \end{equation}
% %
% Plugging in the definition of $\pullcount_0$ we get immediately \eqref{eq:UpUCB-GapUp-pullcount-bound}.
% \end{proof}

% \cref{thm:UpUCB-GapUp-BL-regret} shows that \cref{algo:UpUCB-GapUp-BL} provides a smooth transition between standard UCB and the strategy that identifies the affected variables of all the actions.
% When $\va[\gapbandit]/\gapUplift\ge\nVariables$, the loss of taking action $\arm$ is so large that UCB prevents it from being taken further even if $\vta[\pullcount]\le\pullcount_0$.
% Otherwise, the affected variables get identified after an action is taken sufficient number of times and the algorithm benefits from this knowledge to improve the estimate of the uplift.
% It is also quite straightforward to combine \cref{algo:UpUCB-L-BL} with \cref{algo:UpUCB-GapUp-BL} when both $\nAffected$ and $\gapUplift$ are known; this results in a regret bound that replaces $\clip(\va[\gapbandit]/\gapUplift,\va[\nAffected],\nVariables)$ by $\clip(\va[\gapbandit]/\gapUplift,\va[\nAffected],\nAffected)$ in \eqref{eq:UpUCB-GapUp-BL-regret}.

% \subsection{Unknown Baseline Payoffs}
% Several additional challenges emerge when we want to adapt the aforementioned strategies to the case where the baseline payoffs are unknown.
% First, without additional assumption, it is impossible to tell whether two arbitrarily close estimates indicate the same effect of two actions on a variable.
% Then, without a proper baseline to compare with, we can never exclude the possibility that all the variables are affected by all the actions.
% We will thus need to make the following much more stringent assumption.

% \begin{assumption}
% \label{asm:gapUplift-ubl}
% The effect of any two actions on a variable differ by at least $\gapUplift$ as long as one of them affects this variable, \ie for all $\arm\in\arms$, $\indv\in\va[\variables]$, and $\alt{\arm}\in\setexclude{\arms}{\{\arm\}}$, it holds $\abs{\vav[\meanReward]-\vav[\meanReward][\alt{\arm}]}\ge\gapUplift$.
% \end{assumption}

% \input{Algorithms/UpUCB_GapUp}

% In other words, $\gapbandit$ is not only a lower bound on individual uplift, but also a lower bound on (individual) effect gap.
% Second, with a UCB-style algorithm, the optimal actions may not be taken sufficiently many times, in which case we can only conservatively assume that they affect all the variables.
% This would incur additional regret in the analysis when $\va[\meanReward][0]$ is unknown. 
% %While this does not pose a problem when $\va[\meanReward][0]$ is known, it can cause extra regret when we apply the \ac{DiffUCB} principle.
% Therefore, we would like to ensure that all the (potentially optimal) actions are taken the same number of times at the point that the affected variables get identified.
% This leads to a two-stage method as described in \cref{algo:UpUCB-GapUp}.

% In the first stage, we perform successive elimination until the uneliminated actions are taken sufficiently many times.
% Here $\vta[\estalt{\reward}][\round]$ is the empirical estimate of the reward associated to action $\arm$ and $\vt[\radiusConf][\round]=\nVariables\sqrt{2\log(1/\alt{\smallproba})/\round}$ is the associated radius of confidence interval.
% %After that, we aggregate variables with close estimates.
% Subsequently, for each variable $\indv\in\variables$ we construct the set
% %
% \begin{equation}
%     \label{eq:setBaseEst}
%     \vv[\setBaseEst]
%     = \setdef{\arm\in\arms}{\exists\thinspace \armalt\in\setexclude{\arms}{\{\arm\}}, \vtav[\intConf][\run_0+1]\intersect\vtav[\intConf][\run_0+1][\armalt]\neq\varnothing},
% \end{equation}
% %
% where $\run_0$ is the number of iterations in the elimination phase and the confidence intervals are defined as in \eqref{eq:UCBs-arm}.
% If \cref{asm:gapUplift-ubl} is verified, then with high probability $\arm\in\vv[\setBaseEst]$ only if $\indv\notin\va[\variables]$.
% Therefore, the observed results from these arms can be used to estimate the baseline payoff of $\indv$.
% The identified variables for action $\arm\in\arms$ are then $\va[\setId]=\setdef{\indv\in\variables}{\arm\notin\vv[\setBaseEst]}$.

% The second stage of the algorithm reuses the idea from \UpUCBwb.
% We define the UCB indices following \eqref{eq:UCBs-arm} for $\arm\in\arms$ and for the baseline estimate we choose among $\vv[\setBaseEst]$ the action that is taken the most frequently whenever this set is non-empty. Otherwise we arbitrarily set it to $0$. That is,
% %
% \begin{equation}
%     \label{eq:UCBs-0-UpUCB-GapUp}
%     \vtav[\UCBindex][\run][0] = \begin{cases}
%     0
%     & \text{if} ~ \vv[\setBaseEst]=\varnothing,
%     \\
%     \vtav[\UCBindex][\run][\vtav[\arm][\run][0]] \text{ where $\vtav[\arm][\run][0]=\argmax_{\arm\in\vv[\setBaseEst]}\vta[\pullcount][\run-1]$} & \text {otherwise}.
%     \end{cases}
% \end{equation}
% %
% The uplifting indices that guide the decision of the algorithm are defined by $\vta[\UPindexSum]=\sum_{\indv\in\vta[\setId]}(\vtav[\UCBindex]-\vtav[\UCBindex][\run][0])$.

% As shown below, the regret of \cref{algo:UpUCB-GapUp} takes roughly the same form as the one in \cref{thm:UpUCB-GapUp-BL-regret}, but as in \cref{thm:UpUCB-regret}, the number of variables that an optimal action affects also plays a crucial role in the regret bound.


% % we form a partition of the remaining arms such that if two arms $\arm, \armalt$ belong to different cells of the partition then the confidence intervals $\vta[\intConf]$ and $\vta[\intConf][\run][\armalt]$ do not overlap.
% % Let us denote by $\vav[\arms]$ the cell that arm $\arm$ belongs to. The aggregated empirical means, pull counts, and UCB indices are defined as:
% % %
% % \begin{equation}
% %     \label{eq:UCBs-gapUplift}
% %     \vtav[\pullcount] = \sum_{\runalt=1}^{\run}\one\{\vt[\arm]\in\vav[\arms]\},
% %     ~~
% %     \vtav[\est{\meanReward}] =
% %     \frac{\sum_{\runalt=1}^{\run}\vtv[\valuev]\one\{\vt[\arm]\in\vav[\arms]\}}{\max(1, \vtav[\pullcount])},
% %     ~~
% %     \vtav[\UCBindex]
% %     = \vtav[\est{\meanReward}]
% %     + \sqrt{\frac{2\log(1/\alt{\smallproba})}{\vtav[\pullcount]}}.
% % \end{equation}
% % %
% % The learner then plays the action with the largest UCB index $\vta[\UCBindex]=\sum_{\indv\in\variables}\vtav[\UCBindex]$.
% % %The whole procedure is described in
% % Notice that if \cref{asm:gapUplift-ubl} is violated, the aggregation of the estimates may incur an additional regret in $\Theta(\nAffected\nRuns\gapUplift)$. 

% % \begin{remark}
% % We do not insist on the use of uplifting index here.
% % Otherwise, another alternative is to compare with some most pulled armed as in \cref{algo:UpUCB-L}.
% % However, we believe aggregating estimates that are close to each other is the most natural thing to do under the assumption that two actions cannot have arbitrarily similar effect on a variable unless they affect the variable in the same way.
% % \end{remark}

% \begin{theorem}
% \label{thm:UpUCB-GapUp-regret}
% Let \cref{asm:gapUplift-ubl} hold and $\alt{\smallproba}=\smallproba/(2\nArms\nVariables\nRuns)$.  Then the regret of \UpUCBDeltawb (\cref{algo:UpUCB-GapUp}), with probability at least $1-\smallproba$, satisfies:
% %
% \begin{equation}
%     \label{eq:UpUCB-GapUp-regret}
%     \vt[\reg][\nRuns] \le
%     \sum_{\arm\in\arms:\va[\gapbandit]>0}
%     \left(\frac{8\thinspace\clip(2\va[\gapbandit]/\gapUplift,\va[\nAffected]+\va[\nAffected][\sol[\arm]],2\nVariables)^2\log(2\nArms\nVariables\nRuns/\smallproba)}{\va[\gapbandit]}+\va[\gapbandit]\right).
% \end{equation}
% \end{theorem}
% \begin{proof}
% We shall again consider the event $\event$ defined in \eqref{eq:UCB-L-event}, which holds with probability $1-\smallproba$ as argued in the proof of \cref{prop:UpUCB-L-BL-regret}. Leveraging the decomposition in \eqref{eq:regret-decomp-apx} it is sufficient to prove that on $\event$ we have
% \begin{equation}
%     \label{eq:UpUCB-GapUp-noBL-pullcount-bound}
%     \vta[\pullcount][\nRuns]
%     \le
%     \max\left(
%     \min\left(
%     \frac{32\log(1/\alt{\smallproba})}{\gapUplift^2},
%     \frac{32\nVariables^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right), \frac{8(\va[\nAffected]+\va[\nAffected][\sol[\arm]])^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right)
%     +1.
% \end{equation}
% %
% We assume $\event$ happens in the rest of the proof.

% Let us first focus on the elimination phase, notice that event $\event$ implies $\abs{\vta[\estalt{\reward}][\round]-\va[\reward]}<\vt[\radiusConf][\round]$ for every $\arm\in\vt[\arms][\round]$.
% % We define the event
% % %
% % \begin{equation}
% %     \notag
% %     \event_1 =
% %     \left\{\forall\round\in\oneto{\pullcount_0},
% %     ~\forall\arm\in\arms,
% %     ~ \abs{\vta[\estalt{\reward}][\round]-\va[\reward]}<\nVariables\sqrt{\frac{2\log(1/\alt{\smallproba})}{\round}}\right\}
% % \end{equation}
% % %
% % Following the proof of \cref{lem:concentration-mean-a} and a union bound over $\arm\in\arms$, we know that $\prob(\event_1)\ge1-2\nArms\pullcount_0\alt{\smallproba}$.
% In this case, the optimal actions never get eliminated.
% In fact, if $\sol[\arm]\in\vt[\arms][\round]$, then for all $\arm\in\vt[\arms][\round]$ it holds that
% %
% \begin{equation}
%     \notag
%     \vta[\estalt{\reward}][\round][\sol[\arm]]
%     +2\vt[\radiusConf][\round]
%     \ge
%     \va[\reward][\sol[\arm]]+\vt[\radiusConf][\round]
%     \ge
%     \va[\reward][\arm]+\vt[\radiusConf][\round]
%     \ge \vta[\estalt{\reward}][\round][\arm],
% \end{equation}
% %
% As a consequence, we also have $\sol[\arm]\in\vt[\arms][\round+1]$ and we conclude by the principle of induction.
% With this we further deduce that all action
% $\arm$ with $\va[\gapbandit]\ge4\vt[\radiusConf][\round]$ gets eliminated
% %\nVariables\sqrt{2\log(1/\alt{\smallproba})/\round}$ 
% after it is taken at most $\round$ times.
% %must be eliminated at the latest in round $\round$. 
% To see this, notice that for such action we have
% %
% \begin{equation}
%     \notag
%     \vta[\estalt{\reward}][\round]+2\vt[\radiusConf][\round]
%     < \va[\reward]+3\vt[\radiusConf][\round]
%     = \va[\reward][\sol[\arm]]-\va[\gapbandit]+3\vt[\radiusConf][\round]
%     < \vta[\estalt{\reward}][\round][\sol[\arm]]
%     -\va[\gapbandit]+4\vt[\radiusConf][\round]
%     \le \vta[\estalt{\reward}][\round][\sol[\arm]].
% \end{equation}
% %
% Therefore, for all $\run$ in phase \rom{1} of the algorithm, it is true that
% %
% \begin{equation}
%     \label{eq:UpUCB-GapUp-noBL-pullcount-bound-I}
%     \vta[\pullcount]\le
%     \min\left(
%     \left\lceil\frac{32\log(1/\alt{\smallproba})}{\gapUplift^2}\right\rceil,
%     \left\lceil\frac{32\nVariables^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right\rceil
%     \right).
% \end{equation}
% %
% This suggests that inequality \eqref{eq:UpUCB-GapUp-noBL-pullcount-bound} holds if the algorithm terminates in the elimination phase.

% Otherwise, the algorithm constructs $\vv[\setBase]$'s, $\va[\setId]$'s, and switches to the \textsc{UpUCB} phase.
% Let us denote by $\vv[\setBase]=\setdef{\arm\in\arms}{\indv\notin\va[\variables]}$ the set of actions that do not affect variable $\indv$
% and let $\arms_{\text{res}}=\vt[\arms][\pullcount_0+1]$ be the actions that remain after phase \rom{1}.
% %$\pullcount_0=\ceil{(32/\gapUplift^2)\log(1/\alt{\smallproba})}$ be the number of times that the uneliminated arms are pulled in the first phase.
% We argue that the sets $\vv[\setBaseEst]$ are constructed such that when $\event$ occurs,
% \begin{enumerate}[\textup(\itshape i\textup)]
%     \item $\vv[\setBaseEst]\subseteq\vv[\setBase]$.
%     \item  If there exist $\arm,\armalt\in\arms_{\text{res}}\intersect\vv[\setBase]$ such that $\arm\neq\armalt$ then we also have $\arm,\armalt\in\vv[\setBaseEst]$.
% \end{enumerate}
% %
% The second point is proved by observing that under $\event$ we must have $\vav[\meanReward][0]\in\vtav[\intConf][\run_0+1]\intersect\vtav[\intConf][\run_0+1][\armalt]$ if $\arm,\armalt\in\arms_{\text{res}}\intersect\vv[\setBase]$.
% To show the first point, notice that after the elimination phase, each of the action in $\arms_{\text{res}}$ is taken exactly $\ceil{(32/\gapUplift^2)\log(1/\alt{\smallproba})}$ times and thus $\vta[\radiusConf][\run_0]\le\gapUplift/4$.
% By \cref{asm:gapUplift-ubl}, if $\arm\notin\vv[\setBase]$, then for all $\armalt\in\setexclude{\arms_{\text{res}}}{\{\arm\}}$ we have $\abs{\vav[\meanReward]-\vav[\meanReward][\alt{\arm}]}\ge\gapUplift$, which along with the definition of $\event$ implies $\vtav[\intConf][\run_0+1]\intersect\vtav[\intConf][\run_0+1][\armalt]=\varnothing$, and therefore $\arm\notin\vv[\setBaseEst]$.

% The rest of the proof follows closely that of \cref{thm:UpUCB-regret}.
% Suppose that a suboptimal action $\arm$ is taken at round $\run$ during phase \rom{2} of the algorithm.
% This means $\vta[\UPindexSum]\ge\vta[\UPindexSum][\run][\sol[\arm]]$ (recall that $\sol[\arm]\in\arms_{\text{res}}$ since $\event$ happens), \ie
% %
% \begin{equation}
%     \notag
%     \sum_{\indv\in\va[\setId]}(\vtav[\UCBindex][\run]-\vtav[\UCBindex][\run][0])
%     \ge
%     \sum_{\indv\in\va[\setId][\sol[\arm]]}
%     (\vtav[\UCBindex][\run][\sol[\arm]]-\vtav[\UCBindex][\run][0]).
% \end{equation}
% %
% Rearranging the terms we get 
% %
% \begin{equation}
%     \notag
%     \sum_{\indv\in\va[\setId]}\vtav[\UCBindex][\run]
%     +\sum_{\indv\in\setexclude{\va[\setId][\sol[\arm]]}{\va[\setId]}}
%     \vtav[\UCBindex][\run][0]
%     \ge
%     \sum_{\indv\in\va[\setId][\sol[\arm]]}
%     \vtav[\UCBindex][\run][\sol[\arm]]
%     +\sum_{\indv\in\setexclude{\va[\setId]}{\va[\setId][\sol[\arm]]}}
%     \vtav[\UCBindex][\run][0].
% \end{equation}
% %
% If $\indv\in\setexclude{\va[\setId][\sol[\arm]]}{\va[\setId]}$ then $\arm\in\vv[\setBaseEst]$.
% In particular, $\vv[\setBaseEst]\neq\varnothing$ so $\armalt=\vtav[\arm][\run][0]=\argmax_{\tilde{\arm}\in\vv[\setBaseEst]}\vta[\pullcount][\run-1][\tilde{\arm}]$ is well-defined and $\vtav[\UCBindex][\run][0]=\vtav[\UCBindex][\run][\armalt]$.
% With $\vv[\setBaseEst]\subseteq\vv[\setBase]$ we know that $\vav[\meanReward][\armalt]=\vav[\meanReward][0]$ and accordingly $\abs{\vtav[\meanReward][\run-1][\armalt]-\vav[\meanReward][0]}\le\vta[\radiusConf][\run-1][\armalt]$ by the fact that $\event$ happens.
% This shows $\vtav[\UCBindex][\run][0]\ge\vav[\meanReward][0]$.
% Moreover, $\vta[\pullcount][\run][\armalt]\ge\vta[\pullcount]$ by the choice of $\armalt$; hence, $\vtav[\UCBindex][\run][0]\le\vav[\meanReward][0]+2\vta[\radiusConf][\run-1][\armalt]\le\vav[\meanReward][0]+2\vta[\radiusConf][\run-1]$.
% The same argument applies to $\indv\in\setexclude{\va[\setId]}{\va[\setId][\sol[\arm]]}$, and the UCB indices of $\arm$ and $\sol[\arm]$ can be bounded from above and below as in previous proofs.
% In summary, we obtain
% %
% \begin{equation}
%     \notag
%     \sum_{\indv\in\va[\setId]}(\vav[\meanReward]+2\vta[\radiusConf][\run-1])
%     +\sum_{\indv\in\setexclude{\va[\setId][\sol[\arm]]}{\va[\setId]}}
%     (\vav[\meanReward][0]+2\vta[\radiusConf][\run-1])
%     \ge
%     \sum_{\indv\in\va[\setId][\sol[\arm]]}
%     \vav[\meanReward][\sol[\arm]]
%     +\sum_{\indv\in\setexclude{\va[\setId]}{\va[\setId][\sol[\arm]]}}
%     \vav[\meanReward][0].
% \end{equation}
% %
% Equivalently,
% %
% \begin{equation}
%     \label{eq:UpUCB-GapUp-radConf-larger-than}
%     2\card\left(\va[\setId]\union\va[\setId][\sol[\arm]]\right)\vta[\radiusConf][\run-1]
%     \ge
%     \sum_{\indv\in\va[\setId]\union\va[\setId][\sol[\arm]]}\vav[\meanReward][\sol[\arm]]
%     -\sum_{\indv\in\va[\setId]\union\va[\setId][\sol[\arm]]}\vav[\meanReward].
% \end{equation}
% %
% To conclude, we claim that
% %
% \begin{equation}
%     \label{eq:VV-equal}
%     \va[\setId]\union\va[\setId][\sol[\arm]]=\va[\variables]\union\va[\variables][\sol[\arm]].
% \end{equation}
% %
% Let us first show $\va[\variables]\subseteq\va[\setId]\subseteq\va[\variables]\union\va[\variables][\sol[\arm]]$.
% The first inclusion is a consequence of $\vv[\setBaseEst]\subseteq\vv[\setBase]$:
% %
% \begin{equation}
%     \notag
%     \indv\in\va[\variables] \implies
%     \arm\notin\vv[\setBase] \implies
%     \arm\not\in\vv[\setBaseEst] \implies
%     \indv\in\va[\setId].
% \end{equation}
% %
% As for the second inclusion we prove it's contrapositive:
% %
% \begin{equation}
%     \notag
%     \indv\notin\va[\variables]\union\va[\variables][\sol[\arm]] \implies
%     \arm,\sol[\arm]\in\arms_{\text{res}}\intersect\vv[\setBase] \implies
%     \arm,\sol[\arm]\in\vv[\setBaseEst] \implies
%     \indv\notin\va[\setId]
% \end{equation}
% %
% Notice that the second implication holds because $\arm$ is suboptimal and in particular $\arm\neq\sol[\arm]$.
% The inclusion $\va[\variables][\sol[\arm]]\subseteq\va[\setId][\sol[\arm]]\subseteq\va[\variables]\union\va[\variables][\sol[\arm]]$ can be proved in a similar way, and combining these results gives \eqref{eq:VV-equal}.
% Therefore, the \acl{RHS} of \eqref{eq:UpUCB-GapUp-radConf-larger-than} is exactly $\va[\gapbandit]$ while the \acl{LHS} of \eqref{eq:UpUCB-GapUp-radConf-larger-than} is bounded from above by $2(\va[\nAffected]+\va[\nAffected][\sol[\arm]])\vta[\radiusConf][\run-1]$.
% In consequence,
% %
% \begin{equation}
%     \notag
%     \vta[\pullcount][\run-1]
%     \le \frac{8(\va[\nAffected]+\va[\nAffected][\sol[\arm]])^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}.
% \end{equation}
% %
% Therefore, any suboptimal action that gets taken in the \textsc{UpUCB} phase satisfies
% %
% \begin{equation}
%     \notag
%     \vta[\pullcount][\nRuns]
%     \le \frac{8(\va[\nAffected]+\va[\nAffected][\sol[\arm]])^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}+1.
% \end{equation}
% %
% On the other hand, if an suboptimal action is not taken in the \textsc{UpUCB} phase then \eqref{eq:UpUCB-GapUp-noBL-pullcount-bound-I} applies, so in either case \eqref{eq:UpUCB-GapUp-noBL-pullcount-bound} is verified, which concludes the proof.
% \end{proof}

% \vspace{0.4em}
% \begin{remark}
% A natural candidate for $\vtav[\UCBindex][\run][0]$ is the one that uses aggregated information as in \eqref{eq:mean-estimate-0}.
% The problem of this choice is that how we aggregate the observations collected in the first phase are only determined at the end of the the phase, while this choice itself depends on these observations.
% Mathematically, this prevents us from defining a suitable martingale difference sequence for which we establish concentration bound.
% An easy fix is to only aggregate observations from the second phase, while the use of the observations from the first phase should be limited to those coming from just one arm.
% %in $\vv[\setBaseEst]$.
% \end{remark}

==> Uplifting bandits - arxiv/Appendices/Upper-bound.tex <==
In this appendix, we provide proofs of the regret bounds from \cref{sec:known-affected,sec:unknown-affected}.
Our proofs have the following structure.

\begin{enumerate}
    \item Leveraging \cref{lem:concentration-mean-a,lem:concentration-mean-0} presented in \cref{apx:concentration}, we define a high-probability event $\event$ on which all the expected payoffs belong to their confidence intervals.
    %\item On this event, we show that the all suboptimal action $\arm$ is taken at most $\bigoh(\nAffected^2\log(1/\smallproba)/(\va[\gapbandit])^2)$ number of times.
    \item %To prove the previous point, we show that a suboptimal action can only be taken when its associated width of confidence interval is sufficiently large.
    %This is the case because in each round we take the action with the largest uplifting index, and in particular the uplifting index of the taken action is larger than that of an optimal action.
    For UCB-like methods, we use the fact that the uplifting index of the taken action is larger than that of any optimal action by design to show that on event $\event$ a suboptimal action can only be taken when its associated width of confidence interval is sufficiently large.
    \item The previous point allows us to bound the number of times that a suboptimal action is taken on $\event$.
    %For example, this by $\tbigoh(\nAffected^2/(\va[\gapbandit])^2)$ on $\event$.
    \item We conclude with the following regret decomposition (which was already stated in \eqref{eq:regret-decomp}).
    \begin{equation}
    \label{eq:regret-decomp-apx}
    \reg_{\nRuns} =
    \sum_{\arm\in\arms}\vta[\pullcount]\va[\gapbandit].
\end{equation}
\end{enumerate}

\subsection{Concentration Bounds}
\label{apx:concentration}
\input{Appendices/Concentration}

\subsection{Unknown Baseline: Proof of \cref{thm:UpUCB-regret}}
\label{apx:proof-UpUCBwb}

\UpUCBRegret*

\begin{proof}
We first notice that while there are $\nVariables$ variables, not all of them are involved in estimating the uplifts.
Therefore, we only need to focus on the set of relevant variables $\alt{\variables}=\bigcup_{\arm\in\arms}\va[\variables]$.
Clearly, $\card(\alt{\variables})\le\nArms\nAffected$.
With this in mind, we define the events
%
\begin{align*}
    \event_1 &=
    \{\forall\run\in\oneto{\nRuns},
    ~\forall\arm\in\arms,
    ~\forall\indv\in\va[\variables],
    ~ \abs{\vtav[\est{\meanReward}]-\vav[\meanReward]}\le\vta[\radiusConf]\},\\
    \event_2 &=
    \{\forall\run\in\oneto{\nRuns}, 
    ~\forall\indv\in\alt{\variables},
    ~ \abs{\vtav[\est{\meanReward}][\run][0]-\vav[\meanReward][0]}\le\vtav[\radiusConf][\run][0]\}.
\end{align*}
%
\cref{lem:concentration-mean-a} and \cref{lem:concentration-mean-0} in \cref{apx:concentration} along with union bounds over $\arm$ and $\indv$ guarantee
%
\begin{equation}
    \notag
    \prob(\event_1\union\event_2)
    \ge1-\left(\sum_{\arm\in\arms}\va[\nAffected]+\card(\alt{\variables})\right)\nRuns(2\alt{\smallproba})
    \ge1-4\nArms\nAffected\nRuns\alt{\smallproba}
    = 1 - \smallproba.
\end{equation}
It is thus sufficient to show that \eqref{eq:UpUCB-regret} holds on $\event_1\union\event_2$.

In the remainder of the proof, we consider an arbitrary realization of $\event_1\union\event_2$ and prove that \eqref{eq:UpUCB-regret} indeed holds for this realization.
From \eqref{eq:regret-decomp-apx} it is clear that we just need to bound $\vta[\pullcount][\nRuns]=\sum_{\run=1}^{\nRuns}\one\{\vt[\arm]=\arm\}$ from above for all suboptimal action $\arm\in\arms$ with $\va[\gapbandit]>0$.
This is done by providing a lower bound on $\vta[\radiusConf]$ for any $\run$ such that $\vt[\arm]=\arm$.
To proceed, suppose that a suboptimal action $\arm$ is taken for the last time at round $\run\in\intinterval{\nArms+1}{\nRuns}$.\footnote{%
If the action is not taken anymore after the first $\nRuns$ runs. We have $\vta[\pullcount][\nRuns]=1$ so the upper bound that we show later trivially holds.
}
This implies $\vta[\UPindexSum][\run]\ge\vta[\UPindexSum][\run][\sol[\arm]]$ and $\vta[\pullcount][\nRuns]=\vta[\pullcount][\run-1]+1$. By the definition of the uplifting indices, we get
%
\begin{equation}
    \notag
    \sum_{\indv\in\va[\variables]}(\vtav[\UCBindex][\run]-\vtav[\UCBindex][\run][0])
    \ge
    \sum_{\indv\in\va[\variables][\sol[\arm]]}
    (\vtav[\UCBindex][\run][\sol[\arm]]-\vtav[\UCBindex][\run][0]).
\end{equation}
%
Rearranging and dropping $\sum_{\indv\in\va[\variables]\intersect\va[\variables][\sol[\arm]]}\vtav[\UCBindex][\run][0]$ from both sides, we get
%
\begin{equation}
    \label{eq:UCB-larger-than-UCB}
    \sum_{\indv\in\va[\variables]}\vtav[\UCBindex][\run]
    +\sum_{\indv\in\setexclude{\va[\variables][\sol[\arm]]}{\va[\variables]}}\vtav[\UCBindex][\run][0]
    \ge
    \sum_{\indv\in\va[\variables][\sol[\arm]]}\vtav[\UCBindex][\run][\sol[\arm]]
    +\sum_{\indv\in\setexclude{\va[\variables]}{\va[\variables][\sol[\arm]]}}\vtav[\UCBindex][\run][0].
\end{equation} %\todob{Say that $\sum_{i \in V^a \cap V^{a^*}} U_{t + 1}^0(i)$ was dropped from both sides.}
%
This is similar to the type of inequality that defines standard UCB.
In fact, the left and the right hand sides of \eqref{eq:UCB-larger-than-UCB} are respectively upper confidence bounds on $\sum_{\indv\in\va[\variables]\union\va[\variables][\sol[\arm]]}\vav[\meanReward]$
and upper confidence bounds on $\sum_{\indv\in\va[\variables]\union\va[\variables][\sol[\arm]]}\vav[\meanReward][\sol[\arm]]$.
We next bound these two quantities respectively from above and from below.
Since both $\event_1$ and $\event_2$ hold, we have the following inequalities for the UCB indices
%by the definition of the UCB index \eqref{eq:UCBs}
%
\begin{gather*}
    \forall\runalt\in\oneto{\nRuns},
    ~\forall\arm\in\arms, 
    ~\forall\indv\in\va[\variables],
    ~\vav[\meanReward] + 2\vta[\radiusConf][\runalt-1]
    \ge \vtav[\UCBindex][\runalt]
    \ge \vav[\meanReward],\\
    \forall\runalt\in\oneto{\nRuns}, 
    ~\forall\indv\in\setexclude{\alt{\variables}}{\bigcap_{\arm\in\arms}\va[\variables]},
    ~\vav[\meanReward][0] + 2\vtav[\radiusConf][\runalt-1][0]
    \ge \vtav[\UCBindex][\runalt][0]
    \ge \vav[\meanReward][0].
\end{gather*}
%
Combining the above, we obtain
%
\begin{equation}
    \notag
    \sum_{\indv\in\va[\variables]}
    (\vav[\meanReward]+2\vta[\radiusConf][\run-1])
    +\sum_{\indv\in\setexclude{\va[\variables][\sol[\arm]]}{\va[\variables]}}
    (\vav[\meanReward][0]+2\vtav[\radiusConf][\run-1][0])
    \ge
    \sum_{\indv\in\va[\variables][\sol[\arm]]}\vav[\meanReward][\sol[\arm]]
    +\sum_{\indv\in\setexclude{\va[\variables]}{\va[\variables][\sol[\arm]]}}\vav[\meanReward][0].
\end{equation}
%
Adding $\sum_{\indv\in\va[\variables]\intersect\va[\variables][\sol[\arm]]}\vav[\meanReward][0]$ to both sides and rearranging leads to
%
\begin{equation}
    \notag
    \sum_{\indv\in\va[\variables][\sol[\arm]]}
    \vav[\meanReward][\sol[\arm]]
    - \sum_{\indv\in\va[\variables]}\vav[\meanReward]
    + \sum_{\indv\in\va[\variables]}\vav[\meanReward][0]
    - \sum_{\indv\in\va[\variables][\sol[\arm]]}\vav[\meanReward][0]
    % \sum_{\indv\in\va[\variables][\sol[\arm]]}
    % \vav[\meanReward][\sol[\arm]]
    % - \sum_{\indv\in\va[\variables]}\vav[\meanReward]
    % + \sum_{\indv\in\setexclude{\va[\variables]}{\va[\variables][\sol[\arm]]}}\vav[\meanReward][0]
    % - \sum_{\indv\in\setexclude{\va[\variables][\sol[\arm]]}{\va[\variables]}}\vav[\meanReward][0]
    \le \sum_{\indv\in\va[\variables]}2\vta[\radiusConf][\run-1]
    + \sum_{\indv\in\setexclude{\va[\variables][\sol[\arm]]}{\va[\variables]}}2\vtav[\radiusConf][\run-1][0].
\end{equation}
%
From this we can derive an inequality between the suboptimal gap $\va[\gapbandit]$ and the the widths of the confidence intervals as follows
%
\begin{equation}
    \label{eq:UpUCB-regret-bound-gap}
    \begin{aligned}[b]
    \va[\gapbandit]
    &= \va[\uplift][\sol[\arm]] - \va[\uplift]\\
    &= \sum_{\indv\in\va[\variables][\sol[\arm]]}
    (\vav[\meanReward][\sol[\arm]]-\vav[\meanReward][0])
    -\sum_{\indv\in\va[\variables]}(\vav[\meanReward]-\vav[\meanReward][0])\\
    &= \sum_{\indv\in\va[\variables][\sol[\arm]]}
    \vav[\meanReward][\sol[\arm]]
    - \sum_{\indv\in\va[\variables]}\vav[\meanReward]
    + \sum_{\indv\in\va[\variables]}\vav[\meanReward][0]
    - \sum_{\indv\in\va[\variables][\sol[\arm]]}\vav[\meanReward][0]\\
    % &= \sum_{\indv\in\va[\variables][\sol[\arm]]}
    % \vav[\meanReward][\sol[\arm]]
    % - \sum_{\indv\in\va[\variables]}\vav[\meanReward]
    % + \sum_{\indv\in\setexclude{\va[\variables]}{\va[\variables][\sol[\arm]]}}\vav[\meanReward][0]
    % - \sum_{\indv\in\setexclude{\va[\variables][\sol[\arm]]}{\va[\variables]}}\vav[\meanReward][0]\\
    &\le 2\va[\nAffected]\vta[\radiusConf][\run-1]
    + \sum_{\indv\in\setexclude{\va[\variables][\sol[\arm]]}{\va[\variables]}}2\vtav[\radiusConf][\run-1][0].
    \end{aligned}
\end{equation}
%
We next argue that for all $\indv\in\setexclude{\va[\variables][\sol[\arm]]}{\va[\variables]}$ we have $\vtav[\pullcount][\run-1][0]\ge\vta[\pullcount][\run-1]$ and hence $\vtav[\radiusConf][\run-1][0]\le\vta[\radiusConf][\run-1]$.
In fact, if $\indv\notin\va[\variables]$, then whenever action $\arm$ is taken, the count of $\vtav[\pullcount][\runalt][0]$ also increases by $1$. Formally,
%
\begin{equation}
    \notag
    \vtav[\pullcount][\run-1][0]
    = \sum_{\runalt=1}^{\run-1}\one\{\indv\notin\va[\variables][\vt[\arm][\runalt]]\}
    \ge \sum_{\runalt=1}^{\run-1}\one\{\vt[\arm][\runalt]=\arm\}\one\{\indv\notin\va[\variables][\vt[\arm][\runalt]]\}
    = \sum_{\runalt=1}^{\run-1}\one\{\vt[\arm][\runalt]=\arm\}
    = \vta[\pullcount][\run-1].
\end{equation}
%
% Plugging in the definition of $\vta[\radiusConf]$ and $\vtav[\radiusConf][\run][0]$ in \eqref{eq:UpUCB-regret-bound-gap} then gives
% %
% \begin{equation}
%     \notag
%     \va[\gapbandit]
%     \le
%     (2\sqrt{2}\va[\nAffected]+8\va[\nAffected][\sol[\arm]])
%     \sqrt{\frac{\log(2\run/\alt{\smallproba})}{\vta[\pullcount]}}
%     + (8\va[\nAffected][\sol[\arm]])\frac{\log(2\run/\alt{\smallproba})}{\vta[\pullcount]}.
% \end{equation}
% %
% Let us distinguish between the following two cases
% %
% \begin{enumerate}[itemsep=3pt,topsep=4.5pt,parsep=3pt]
%     \item $\log(2\run/\alt{\smallproba})/\vta[\pullcount]\le1$: Then $\va[\gapbandit]\le(2\sqrt{2}\va[\nAffected]+16\va[\nAffected][\sol[\arm]])\sqrt{\log(2\run/\alt{\smallproba})/\vta[\pullcount]}$.
%     Equivalently
%     %
%     \begin{equation}
%     \notag
%     \vta[\pullcount]
%     \le \frac{(2\sqrt{2}\va[\nAffected]+16\va[\nAffected][\sol[\arm]])^2\log(2\run/\alt{\smallproba})}{(\va[\gapbandit])^2}.
%     \end{equation}
%     %
%     \item $\log(2\run/\alt{\smallproba})/\vta[\pullcount]>1$: Then $\va[\gapbandit]\le(2\sqrt{2}\va[\nAffected]+16\va[\nAffected][\sol[\arm]])(\log(2\run/\alt{\smallproba})/\vta[\pullcount])$.
%     Equivalently
%     %
%     \begin{equation}
%     \notag
%     \vta[\pullcount]
%     \le \frac{(2\sqrt{2}\va[\nAffected]+16\va[\nAffected][\sol[\arm]])\log(2\run/\alt{\smallproba})}{\va[\gapbandit]}.
%     \end{equation}
% \end{enumerate}
% %
% Taking into account these two possibilities, we get
Therefore, we further deduce $\va[\gapbandit]\le2(\va[\nAffected]+\va[\nAffected][\sol[\arm]])\vta[\radiusConf][\run-1]$. Equivalently,

\begin{equation}
    \notag
    \vta[\pullcount][\run-1]
    \le \frac{8(\va[\nAffected]+\va[\nAffected][\sol[\arm]])^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}.
\end{equation}
%
% \begin{equation}
%     \notag
%     \vta[\pullcount]
%     \le \underbrace{\frac{(2\sqrt{2}\va[\nAffected]+16\va[\nAffected][\sol[\arm]])^2\log(2\run/\alt{\smallproba})}{(\va[\gapbandit])^2}
%     \max\left(
%     1, \frac{\va[\gapbandit]}{2\sqrt{2}\va[\nAffected]+16\va[\nAffected][\sol[\arm]]}
%     \right)}_{\va[\pullcount]}.
% \end{equation}
%
We conclude that action $\arm$ is taken at most
%$\floor{\va[\pullcount]}+1$
$\floor{8(\va[\nAffected]+\va[\nAffected][\sol[\arm]])^2\log(1/\alt{\smallproba})/(\va[\gapbandit])^2}+1$
times during the execution of the algorithm. Plugging this into \eqref{eq:regret-decomp-apx} gives exactly \eqref{eq:UpUCB-regret}.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Unknown Affected Variables: Proof of~\cref{thm:UpUCB-L-regret}}
\label{apx:upper-bound-unknown-affected}

Below we prove \cref{thm:UpUCB-L-regret} separately for \UpUCBL and \UpUCBLwb.

%\UpUCBLBRegret*
\begin{proposition} [Regret of \UpUCBL]
\label{prop:UpUCB-L-BL-regret}
Let $\alt{\smallproba}=\smallproba/(2\nArms\nVariables\nRuns)$. If the learner knows  and an upper bound $\nAffected$ on maximum number of variables an action affects and the baseline payoffs, then \UpUCBL (\cref{algo:UpUCB-L-BL}), with probability at least $1-\smallproba$, has regret bounded by:
%
\begin{gather}
    \label{eq:UpUCB-L-BL-regret}
    \vt[\reg][\nRuns] \le
    \sum_{\arm\in\arms:\va[\gapbandit]>0}
    \left(\frac{32\nAffected^2\log(2\nArms\nVariables\nRuns/ \smallproba)}{\va[\gapbandit]}+\va[\gapbandit]\right).
    \raisetag{0.75em}
\end{gather}
\end{proposition}
\begin{proof}
Let us consider the event
%
\begin{equation}
    \label{eq:UCB-L-event}
    \event =
    \{\forall\run\in\oneto{\nRuns},
    ~\forall\arm\in\arms,
    ~\forall\indv\in\variables,
    ~ \abs{\vtav[\est{\meanReward}]-\vav[\meanReward]}<\vta[\radiusConf]\},
\end{equation}
%
%In other words, $\event$ represents the event every confidence interval that we consider in the algorithm contains the corresponding expected value.
By \cref{lem:concentration-mean-0} and a union bound we get immediately $\prob(\event)\ge1-\nArms\nVariables\nRuns(2\alt{\smallproba})=1-\smallproba$.
In the following, we assume that $\event$ occurs and prove \eqref{eq:UpUCB-L-BL-regret}.

First, by the definition of $\vta[\setId]$ we have clearly $\vta[\setId]\subseteq\va[\variables]$.
In fact, if $\indv\notin\va[\variables]$ then $\vav[\meanReward][0]=\vav[\meanReward]\in\vtav[\intConf]$.
The inclusion $\vta[\setId]\subseteq\va[\variables]$ along with the condition $\card(\va[\variables])\le\nAffected$ imply  $\card(\setexclude{\va[\variables]}{\vta[\setId]})\le\nAffected-\card(\vta[\setId])$;
in particular, $\nAffected-\card(\vta[\setId])\ge0$ and thus $\vta[\nAffected]=\nAffected - \card(\vta[\setId])$.

Next, for any $\indv\in\setexclude{\variables}{\vta[\setId]}$, it holds $\vav[\meanReward][0]\in\vtav[\intConf]$. This implies $\vav[\meanReward][0]\le\vtav[\UCBindex]$, and accordingly $\vtav[\UPindex]\ge0$.
We can then write
%
\begin{equation}
    \notag
    \sum_{\indv\in\setexclude{\va[\variables]}{\vta[\setId]}}\vtav[\UPindex]
    \le
    \max_{\substack{\setLargeUp\subseteq\setexclude{\variables}{\vta[\setId]}\\
    \card(\setLargeUp)=\card(\setexclude{\variables}{\vta[\setId]})}}
    \sum_{\indv\in\setLargeUp}\vtav[\UPindex]
    \le
    \max_{\substack{\setLargeUp\subseteq\setexclude{\variables}{\vta[\setId]}\\
    \card(\setLargeUp)=\nAffected-\card(\vta[\setId])}}
    \sum_{\indv\in\setLargeUp}\vtav[\UPindex]
    =
    \sum_{\indv\in\vta[\setLargeUp]}\vtav[\UPindex].
\end{equation}
%
Since $\vtav[\UCBindex]\ge\vav[\meanReward]$ on $\event$, we have $\vtav[\UPindex]\ge\vav[\meanUplift]$; subsequently
%
\begin{equation}
    \notag
    %\label{eq:UpUCB-L-BL-up-upper}
    \va[\uplift]
    = \sum_{\indv\in\va[\variables]}\vav[\meanUplift]
    =
    \sum_{\indv\in\vta[\setId]}\vav[\meanUplift]
    + \sum_{\indv\in\setexclude{\va[\variables]}{\vta[\setId]}}\vav[\meanUplift]
    \le
    \sum_{\indv\in\vta[\setId]}\vtav[\UPindex]
    + \sum_{\indv\in\vta[\setLargeUp]}\vtav[\UPindex]
    =\vta[\UPindexSum].
\end{equation} 
%
This shows that $\vta[\UPindexSum]$ is effectively an upper bound of $\va[\uplift]$.
With this in mind, we are ready to bound the number of times that a suboptimal action is taken.

Let $\arm\in\arms$ with $\va[\gapbandit]>0$ and assume that it is taken at round $\run\in\intinterval{\nArms+1}{\nRuns}$, which means that $\vta[\UPindexSum][\run]\ge\vta[\UPindexSum][\run][\sol[\arm]]$.
We have shown that $\vta[\UPindexSum][\run][\sol[\arm]]\ge\va[\uplift][\sol[\arm]]$.
It remains to provide an upper bound for $\vta[\UPindexSum][\run]$ that involves $\va[\uplift]$.
%
%
% \begin{equation}
%     \label{eq:UpUCB-L-BL-diff-upindex}
%     \vta[\UPindex][\run]-\va[\uplift] \ge \va[\uplift][\sol[\arm]]-\va[\uplift] = \va[\gapbandit].
% \end{equation} \todob{Write out details: $\rho_t^a - r_{up}^a \geq \rho_t^{a^*} - r_{up}^a \geq r_{up}^{a^*} - r_{up}^a$.}
% %
% It remains to bound the \acl{LHS} of \eqref{eq:UpUCB-L-BL-diff-upindex}.
For this, we again use $\vta[\setId]\subseteq\va[\variables]$ and the fact that $\vtav[\UPindex]\ge0$ for all $\indv\in\setexclude{\variables}{\vta[\setId][\run]}$ to decompose
%
\begin{equation}
    \label{eq:UpUCB-L-BL-upindex-decomposition}
    \begin{aligned}
    \vta[\UPindexSum][\run]
    = \sum_{\indv\in\vta[\setId][\run]\union\vta[\setLargeUp][\run]}\vtav[\UPindex][\run]
    \le \sum_{\indv\in\va[\variables]\union\vta[\setLargeUp][\run]}\vtav[\UPindex][\run]
    = \sum_{\indv\in\va[\variables]}\vtav[\UPindex][\run]
    + \sum_{\indv\in\setexclude{\vta[\setLargeUp]}{\va[\variables]}}\vtav[\UPindex][\run].
    \end{aligned}
\end{equation}
%
The summation of the individual uplifting indices over $\indv\in\va[\variables]$ is naturally related to $\va[\uplift]$.
Since $\vav[\meanReward]\ge\vtav[\est{\meanReward}][\run-1]-\vta[\radiusConf][\run-1]$, for all $\indv\in\variables$ it holds
%\todob{Write out details: $\rho_t^a(i) \leq U_t^a(i) - \mu^0(i) \leq \mu^a(i) - \mu^0(i) + 2 c_{t - 1}^a = \mu_{up}^a(i) + 2 c_{t - 1}^a$.}
%
\begin{equation}
    \notag
    \vtav[\UPindex][\run]
    =
    \vtav[\UCBindex] - \vav[\meanReward]
    \le \vav[\meanReward] - \vav[\meanReward][0] +2\vta[\radiusConf][\run-1]
    =\vav[\meanUplift]+2\vta[\radiusConf][\run-1].
\end{equation}
%
In consequence,
%
\begin{equation}
    \label{eq:UpUCB-L-BL-decomp-upper1}
    \sum_{\indv\in\va[\variables]}\vtav[\UPindex][\run]
    \le\sum_{\indv\in\va[\variables]}(\vav[\meanUplift]+2\vta[\radiusConf][\run-1])
    \le\va[\uplift]+2\nAffected\vta[\radiusConf][\run-1].
\end{equation}
%
What we need to show next is that the definition of $\vta[\setId]$ guarantees $\vtav[\UPindex]$ to be small whenever $\indv\notin\vta[\setId]$.
In fact, if $\indv\in\setexclude{\variables}{\vta[\setId][\run]}$, we have $\vav[\meanReward][0]\in\vtav[\intConf][\run]$, and in particular
$\vav[\meanReward][0]\ge\vtav[\est{\meanReward}][\run-1]-\vta[\radiusConf][\run-1]$, implying that
%
\begin{equation}
    \notag
    \vtav[\UPindex][\run]
    =\vtav[\UCBindex][\run]-\vav[\meanReward][0]
    \le (\vtav[\est{\meanReward}][\run-1]+\vta[\radiusConf][\run-1])
    - (\vtav[\est{\meanReward}][\run-1]-\vta[\radiusConf][\run-1])
    = 2\vta[\radiusConf][\run-1].
\end{equation}
%
By definition, $\vta[\setLargeUp]\subseteq\setexclude{\variables}{\vta[\setId][\run]}$, and hence
%
\begin{equation}
    \label{eq:UpUCB-L-BL-decomp-upper2}
    \sum_{\indv\in\setexclude{\vta[\setLargeUp][\run]}{\va[\variables]}}\vtav[\UPindex][\run]
    \le\sum_{\indv\in\setexclude{\vta[\setLargeUp][\run]}{\va[\variables]}}2\vta[\radiusConf][\run-1]
    \le2\nAffected\vta[\radiusConf][\run-1].
\end{equation}
%
Putting \eqref{eq:UpUCB-L-BL-upindex-decomposition}, \eqref{eq:UpUCB-L-BL-decomp-upper1}, and \eqref{eq:UpUCB-L-BL-decomp-upper2} together, we get
%
\begin{equation}
    \notag
    \begin{aligned}
    \vta[\UPindexSum][\run]
    \le \sum_{\indv\in\va[\variables]}\vtav[\UPindex][\run]
    + \sum_{\indv\in\setexclude{\vta[\setLargeUp]}{\va[\variables]}}\vtav[\UPindex][\run]
    \le \va[\uplift] +4\nAffected\vta[\radiusConf][\run-1].
    \end{aligned}
\end{equation}
%
With $\vta[\UPindexSum][\run]\ge\vta[\UPindexSum][\run][\sol[\arm]]\ge\va[\uplift][\sol[\arm]]$ we deduce
%
\begin{equation}
    \notag
    \va[\uplift][\sol[\arm]] \le  \va[\uplift] +4\nAffected\vta[\radiusConf][\run-1].
\end{equation}
%
Therefore, 
$\va[\gapbandit] = \va[\uplift][\sol[\arm]]-\va[\uplift] \le 4\nAffected\vta[\radiusConf][\run-1]$, and equivalently
%
\begin{equation}
    \notag
    \vta[\pullcount][\run-1]
    \le \frac{32\nAffected^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}.
\end{equation} 
%\todob{This result comes completely out of blue. I verified all the math.}
%
Following the argument in the proof of \cref{thm:UpUCB-regret}, this translates into an upper bound on $\vta[\pullcount][\nRuns]$ and
we conclude by %noticing that $\vta[\pullcount][\nRuns]\le\max_{\run\in\oneto{\nRuns-1}}(\vta[])$
invoking the decomposition of \eqref{eq:regret-decomp-apx}.
\end{proof}

%\begin{remark}
We notice that it is quite straightforward to adapt \UpUCBL and its analysis to the setting where the learner knows an action-dependent upper bound $\overline{\va[\nAffected]}\ge\va[\nAffected]$. The only change in \eqref{eq:UpUCB-L-BL-regret} is that $\nAffected$ is replaced by $\overline{\va[\nAffected]}$. Thus we recover \eqref{eq:UpUCB-BL-regret} up to a multiplicative constant when $\overline{\va[\nAffected]}=\Theta(\va[\nAffected])$.
%We complete this section with the proof of the regret bound for \UpUCBLwb.
To derive the regret bound for \UpUCBLwb, we combine idea from the proofs of \cref{thm:UpUCB-regret,prop:UpUCB-L-BL-regret}.
%\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Unknown Baseline Payoffs + Known Upper Bound on Number of Affected Variables}

% \UpUCBLWBRegret*
\begin{proposition}[Regret of \UpUCBLwb] \label{prop:2}
Let $\alt{\smallproba}=\smallproba/(2\nArms\nVariables\nRuns)$. Then the regret of \UpUCBLwb (\cref{algo:UpUCB-L}), with probability at least $1-\smallproba$, satisfies:
%
\begin{equation}
    \label{eq:UpUCB-L-regret}
    \vt[\reg][\nRuns] \le
    \sum_{\arm\in\arms:\va[\gapbandit]>0}
    \left(\frac{512\nAffected^2\log(2\nArms\nVariables\nRuns/\smallproba)}{\va[\gapbandit]}+\va[\gapbandit]\right),
\end{equation}
%
\end{proposition}

\begin{proof}

%This proof combines ideas from the proofs of \cref{thm:UpUCB-regret,prop:UpUCB-L-BL-regret}.
We again place ourselves in the event $\event$ defined in \eqref{eq:UCB-L-event}, and prove \eqref{eq:UpUCB-L-regret} under this condition.
Recall that $\vt[\mostpullarm]\in\argmax_{\arm\in\arms}\vta[\pullcount][\run-1]$ is an action that is taken most frequently during the first $\run-1$ rounds and the associated estimates serve as baselines at round $\run$. We define $\vta[\mostpullvariables]=\va[\variables]\union\va[\variables][\vt[\mostpullarm]]$ as the set of variables that are affected by either action $\arm$ or $\vt[\mostpullarm]$.
Clearly, $\card(\vta[\mostpullvariables])\le2\nAffected$.

We first show that $\vta[\setId]\subseteq\vta[\mostpullvariables]$ whenever $\event$ occurs.
Let $\indv\in\setexclude{\variables}{\vta[\mostpullvariables]}$.
Under $\event$ we have both $\vav[\meanReward][0]=\vav[\meanReward]\in\vtav[\intConf]$ and $\vav[\meanReward][0]=\vav[\meanReward][\vt[\mostpullarm]]\in\vtav[\intConf][\run][\mostpullarm]$.
Therefore, $\vtav[\intConf]\intersect\vtav[\intConf][\run][\vt[\mostpullarm]]\neq\varnothing$; subsequently $\indv\notin\vta[\setId]$. The contrapositive of the above gives exactly $\vta[\setId]\subseteq\vta[\mostpullvariables]$.

We shall now bound $\vta[\pullcount][\nRuns]$ for any suboptimal action $\arm$, from which the proof concludes by applying \eqref{eq:regret-decomp-apx}.
Let $\arm\in\arms$ satisfying $\va[\gapbandit]>0$. If it is taken at round $\run\in\intinterval{\nArms+1}{\nRuns}$, we have $\vta[\UPindexSum]\ge\vta[\UPindexSum][\run][\sol[\arm]]$.
This can be written as
%
% \begin{equation}
%     \label{eq:UpUCB-L-pull-round-larger}
%     \underbrace{\sum_{\indv\in\vta[\setId]}\vtav[\UPindex]
%     +\sum_{\indv\in\vta[\setLargeUp]}\vtav[\UPindex]}_{A}
%     \ge
%     \underbrace{\sum_{\indv\in\vta[\setId][\run][\sol[\arm]]}\vtav[\UPindex][\run][\sol[\arm]]
%     +\sum_{\indv\in\vta[\setLargeUp][\run][\sol[\arm]]}\vtav[\UPindex][\run][\sol[\arm]]}_{B}.
% \end{equation}
\begin{equation}
    \label{eq:UpUCB-L-pull-round-larger}
    \sum_{\indv\in\vta[\setId]}\vtav[\UPindex]
    +\sum_{\indv\in\vta[\setLargeUp]}\vtav[\UPindex]
    \ge
    \sum_{\indv\in\vta[\setId][\run][\sol[\arm]]}\vtav[\UPindex][\run][\sol[\arm]]
    +\sum_{\indv\in\vta[\setLargeUp][\run][\sol[\arm]]}\vtav[\UPindex][\run][\sol[\arm]].
\end{equation}

\paragraph{Decomposition of Suboptimality Gap using the New Baseline.}
Similar to before, we will use \eqref{eq:UpUCB-L-pull-round-larger} to relate the widths of the confidence intervals to the suboptimality gap $\va[\gapbandit]$.
For this, we notice that the suboptimality gap of $\arm$ can be rewritten as
%
\begin{equation}
    \label{eq:proof-UpUCBLWB-gap-decompose}
    \begin{aligned}[b]
    \va[\gapbandit]
    &=\sum_{\indv\in\variables}\vav[\meanReward][\sol[\arm]]
    -\sum_{\indv\in\variables}\vav[\meanReward]\\
    &=\sum_{\indv\in\variables}(\vav[\meanReward][\sol[\arm]]-\vav[\meanReward][\vt[\mostpullarm]])
    -\sum_{\indv\in\variables}(\vav[\meanReward]-\vav[\meanReward][\vt[\mostpullarm]])\\
    %&=\sum_{\indv\in\vta[\mostpullvariables][\run][\sol[\arm]]}\vav[\meanReward][\sol[\arm]]
    %-\sum_{\indv\in\vta[\mostpullvariables]}\vav[\meanReward]\\
    &=\sum_{\indv\in\vta[\mostpullvariables][\run][\sol[\arm]]}(\vav[\meanReward][\sol[\arm]]-\vav[\meanReward][\vt[\mostpullarm]])
    -\sum_{\indv\in\vta[\mostpullvariables]}(\vav[\meanReward]-\vav[\meanReward][\vt[\mostpullarm]])
    \end{aligned}
\end{equation} 
%
The last equality is true because $\vav[\meanReward][\sol[\arm]]=\vav[\meanReward][0]$ outside $\vta[\mostpullvariables][\run][\sol[\arm]]$, and the same holds when we replace $\sol[\arm]$ by $\arm$.
Therefore, our goal is to lower bound the \acl{RHS} of \eqref{eq:UpUCB-L-pull-round-larger} by an expression that contains $\sum_{\indv\in\vta[\mostpullvariables][\run][\sol[\arm]]}(\vav[\meanReward][\sol[\arm]]-\vav[\meanReward][\vt[\mostpullarm]])$
and upper bound the \acl{LHS} of \eqref{eq:UpUCB-L-pull-round-larger} by an expression that contains $\sum_{\indv\in\vta[\mostpullvariables]}(\vav[\meanReward]-\vav[\meanReward][\vt[\mostpullarm]])$.

\paragraph{Lower Bound on RHS of \eqref{eq:UpUCB-L-pull-round-larger}\afterhead}
Since $\sum_{\indv\in\vta[\setLargeUp][\run][\sol[\arm]]}\vtav[\UPindex][\run][\sol[\arm]]$ is the maximum padding, we can lower bound the \acl{RHS} of the inequality by $\sum_{\indv\in\vta[\mostpullvariables][\run][\sol[\arm]]}\vtav[\UPindex][\run][\sol[\arm]]$.
Formally, with $\vta[\setId][\run][\sol[\arm]]\subseteq\vta[\mostpullvariables][\run][\sol[\arm]]$ we have $\card(\setexclude{\vta[\mostpullvariables][\run][\sol[\arm]]}{\vta[\setId][\run][\sol[\arm]]})\le2\nAffected-\card(\vta[\setId][\run][\sol[\arm]])$ and
$\vta[{\nAffected}][\run][\sol[\arm]]=2\nAffected-\card(\vta[\setId][\run][\sol[\arm]])$.
Thus, by definition of $\vta[\setLargeUp][\run][\sol[\arm]]$,
%
\begin{equation}
    \notag
    \sum_{\indv\in\vta[\setLargeUp][\run][\sol[\arm]]}\vtav[\UPindex][\run][\sol[\arm]]
    =
    \max_{\substack{\setLargeUp\subseteq\setexclude{\va[\variables]}{\vta[\setId]}\\
    \card(\setLargeUp)\le2\nAffected-\card(\vta[\setId][\run][\sol[\arm]])}}
    \sum_{\indv\in\setLargeUp}\vtav[\UPindex][\run][\sol[\arm]]
    \ge
    \sum_{\indv\in\setexclude{\vta[\mostpullvariables][\run][\sol[\arm]]}{\vta[\setId][\run][\sol[\arm]]}}\vtav[\UPindex][\run][\sol[\arm]].
\end{equation}
%
To further provide a lower bound on $\sum_{\indv\in\vta[\mostpullvariables][\run][\sol[\arm]]}\vtav[\UPindex][\run][\sol[\arm]]$, we recall that $\vtav[\UPindex][\run][\sol[\arm]]=\vtav[\UCBindex][\run][\sol[\arm]]-\vtav[\UCBindex][\run][\vt[\mostpullarm]]$, so with $\vtav[\UCBindex][\run][\sol[\arm]]\ge\vav[\meanReward][\sol[\arm]]$, $\vtav[\UCBindex][\run][\vt[\mostpullarm]]\le\vav[\meanReward][\vt[\mostpullarm]]+2\vta[\radiusConf][\run-1][\vt[\mostpullarm]]$, and $\card(\vta[\mostpullvariables][\run][\sol[\arm]])\le2\nAffected$, we get
%
\begin{equation}
    \label{eq:UpUCB-L-pull-lower}
    \begin{aligned}[b]
    \sum_{\indv\in\vta[\setId][\run][\sol[\arm]]}\vtav[\UPindex][\run][\sol[\arm]]
    +\sum_{\indv\in\vta[\setLargeUp][\run][\sol[\arm]]}\vtav[\UPindex][\run][\sol[\arm]]
    &\ge
    \sum_{\indv\in\vta[\mostpullvariables][\run][\sol[\arm]]}\vtav[\UPindex][\run][\sol[\arm]]\\
    &\ge \sum_{\indv\in\vta[\mostpullvariables][\run][\sol[\arm]]}
    (\vav[\meanReward][\sol[\arm]] - \vav[\meanReward][\vt[\mostpullarm]] - 2\vta[\radiusConf][\run-1][\vt[\mostpullarm]])\\
    &\ge
    \sum_{\indv\in\vta[\mostpullvariables][\run][\sol[\arm]]}
    (\vav[\meanReward][\sol[\arm]] - \vav[\meanReward][\vt[\mostpullarm]]) - 4\nAffected\vta[\radiusConf][\run-1][\vt[\mostpullarm]].
    \end{aligned}
\end{equation}
%

\paragraph{Upper Bound on LHS of \eqref{eq:UpUCB-L-pull-round-larger}\afterhead}
To make the term $\sum_{\indv\in\vta[\mostpullvariables]}(\vav[\meanReward]-\vav[\meanReward][\vt[\mostpullarm]])$ appear,
we first relate it to the sum of the uplifting indices using $\vtav[\UCBindex]\le\vav[\meanReward]+2\vta[\radiusConf][\run-1]$.
%
\begin{equation}
    \label{eq:proof-UpUCBLWB-LHS-upper1}
    %\label{eq:UpUCB-L-ineq-identified}
    \sum_{\indv\in\vta[\mostpullvariables]}\vtav[\UPindex]
    \le
    \sum_{\indv\in\vta[\mostpullvariables]}(\vav[\meanReward]+2\vta[\radiusConf][\run-1]-\vav[\meanReward][\vt[\mostpullarm]])
    \le \sum_{\indv\in\vta[\mostpullvariables]}(\vav[\meanReward]-\vav[\meanReward][\vt[\mostpullarm]])
    +4\nAffected\vta[\radiusConf][\run-1].
\end{equation}
%
The last inequality uses $\card(\vta[\mostpullvariables])\le2\nAffected$.
Next, to relate $\sum_{\indv\in\vta[\mostpullvariables]}\vtav[\UPindex]$ to the \acl{LHS} of \eqref{eq:UpUCB-L-pull-round-larger}, we want to show
\begin{enumerate*}[\textup(\itshape i\textup)]
    \item $\sum_{\indv\in\vta[\setLargeUp]}\vtav[\UPindex]$ is small, and
    \item We can add additional terms from $\setexclude{\vta[\mostpullvariables]}{\vta[\setId]}$ to the \acl{LHS} of \eqref{eq:UpUCB-L-pull-round-larger}.
\end{enumerate*}
%
These two points correspond respectively to inequalities \eqref{eq:UpUCB-L-BL-decomp-upper2} and \eqref{eq:UpUCB-L-BL-upindex-decomposition} in the proof of \cref{prop:UpUCB-L-BL-regret}.
Again, this can be done by looking at the definition of $\vta[\setId]$.
In fact, if $\indv\in\setexclude{\variables}{\vta[\setId]}$, then by definition $\vtav[\intConf]\intersect\vtav[\intConf][\run][\vt[\mostpullarm]]\neq\varnothing$, implying that
%
\begin{equation}
    %\label{eq:UpUCB-L-ineq-unidentified-indv0}
    \notag
    \begin{aligned}
    \vtav[\est{\meanReward}][\run-1][\vt[\mostpullarm]]+\vta[\radiusConf][\run-1][\vt[\mostpullarm]]
    &\ge\vtav[\est{\meanReward}][\run-1]-\vta[\radiusConf][\run-1],\\
    \vtav[\est{\meanReward}][\run-1]+\vta[\radiusConf][\run-1]
    &\ge\vtav[\est{\meanReward}][\run-1][\vt[\mostpullarm]]-\vta[\radiusConf][\run-1][\vt[\mostpullarm]].
    %0 \le \vtav[\meanReward]-\vav[\meanReward][\vt[\mostpullarm]]+2\vta[\radiusConf][\run-1]+2\vta[\radiusConf][\run-1][\vt[\mostpullarm]].
    \end{aligned}
\end{equation}
%
%since $\vta[\intConf]\intersect\vta[\intConf][\run][\vt[\mostpullarm]]\neq\varnothing$.
The above two inequalities respectively translate into
%
\begin{equation}
    %\label{eq:UpUCB-L-ineq-unidentified-indv}
    \notag
    \begin{aligned}
    \vtav[\UCBindex]-\vtav[\UCBindex][\run][\vt[\mostpullarm]]
    &\le 2\vta[\radiusConf][\run-1],\\
    \vtav[\UCBindex]-\vtav[\UCBindex][\run][\vt[\mostpullarm]]
    &\ge -2\vta[\radiusConf][\run-1][\vt[\mostpullarm]],
    %0 \le \vtav[\meanReward]-\vav[\meanReward][\vt[\mostpullarm]]+2\vta[\radiusConf][\run-1]+2\vta[\radiusConf][\run-1][\vt[\mostpullarm]].
    \end{aligned}
\end{equation}
%
%The second inequality also uses the fact that $\abs{\vtav[\est{\meanReward}][\run-1]-\vav[\meanReward]}\le\vta[\radiusConf][\run-1]$ and $\abs{\vtav[\est{\meanReward}][\run-1][\vt[\mostpullarm]]-\vav[\meanReward][\vt[\mostpullarm]]}\le\vta[\radiusConf][\run-1][\vt[\mostpullarm]]$.
In other words, for any $\indv\in\setexclude{\variables}{\vta[\setId]}$ we have $-2\vta[\radiusConf][\run-1][\vt[\mostpullarm]]\le\vtav[\UPindex]\le2\vta[\radiusConf][\run-1]$.
Subsequently,
%
\begin{align}
    %\begin{aligned}[b]
    \label{eq:UpUCB-L-ineq-unidentified1}
    \sum_{\indv\in\vta[\setLargeUp]}\vtav[\UPindex]
    &\le \sum_{\indv\in\vta[\setLargeUp]}2\vta[\radiusConf][\run-1],\\
    \label{eq:UpUCB-L-ineq-unidentified2}
    \sum_{\indv\in\setexclude{\vta[\mostpullvariables]}{\vta[\setId]}}
    -2\vta[\radiusConf][\run-1][\vt[\mostpullarm]]
    &\le
    \sum_{\indv\in\setexclude{\vta[\mostpullvariables]}{\vta[\setId]}}\vtav[\UPindex].
    %\end{aligned}
\end{align} %\todob{I do not see how the last term on the RHS arises.}
%
Therefore
%
\begin{equation}
    \label{eq:proof-UpUCBLWB-LHS-upper2}
    \begin{aligned}[b]
    \sum_{\indv\in\vta[\setId]}\vtav[\UPindex]
    +\sum_{\indv\in\vta[\setLargeUp]}\vtav[\UPindex]
    &\le
    \sum_{\indv\in\vta[\setId]}\vtav[\UPindex]
    + \sum_{\indv\in\vta[\setLargeUp]}2\vta[\radiusConf][\run-1]
    + \sum_{\indv\in\setexclude{\vta[\mostpullvariables]}{\vta[\setId]}}
    (\vtav[\UPindex]+2\vta[\radiusConf][\run-1][\vt[\mostpullarm]])\\
    &=\sum_{\indv\in\vta[\mostpullvariables]}\vtav[\UPindex]
    + \sum_{\indv\in\vta[\setLargeUp]}2\vta[\radiusConf][\run-1]
    + \sum_{\indv\in\setexclude{\vta[\mostpullvariables]}{\vta[\setId]}}
    2\vta[\radiusConf][\run-1][\vt[\mostpullarm]]\\
    &\le\sum_{\indv\in\vta[\mostpullvariables]}\vtav[\UPindex]
    +4\nAffected\vta[\radiusConf][\run-1]
    +4\nAffected\vta[\radiusConf][\run-1][\vt[\mostpullarm]].
    \end{aligned}
\end{equation}
%
The first inequality makes use of \eqref{eq:UpUCB-L-ineq-unidentified1} and \eqref{eq:UpUCB-L-ineq-unidentified2}, and in particular the last term on the \acl{RHS} is non-negative thanks to \eqref{eq:UpUCB-L-ineq-unidentified2}.
The equality in the second line is true because $\vta[\setId]\subseteq\vta[\mostpullvariables]$.
Finally, for the last inequality we use the fact that $\card(\vta[\setLargeUp])\le2\nAffected$ and $\card(\vta[\mostpullvariables])\le2\nAffected$.
Along with \eqref{eq:proof-UpUCBLWB-LHS-upper2} we get an upper bound on $\sum_{\indv\in\vta[\setId]}\vtav[\UPindex]
    +\sum_{\indv\in\vta[\setLargeUp]}\vtav[\UPindex]$ that involves $\sum_{\indv\in\vta[\mostpullvariables]}(\vav[\meanReward]-\vav[\meanReward][\vt[\mostpullarm]])$.

\paragraph{Conclusion\afterhead}
Combining \eqref{eq:UpUCB-L-pull-round-larger}, \eqref{eq:UpUCB-L-pull-lower}, \eqref{eq:proof-UpUCBLWB-LHS-upper1}, and \eqref{eq:proof-UpUCBLWB-LHS-upper2}, we obtain
%
\begin{equation}
    \notag
    \sum_{\indv\in\vta[\mostpullvariables]}(\vav[\meanReward]-\vav[\meanReward][\vt[\mostpullarm]])
    + 8\nAffected\vta[\radiusConf][\run-1]
    + 4\nAffected\vta[\radiusConf][\run-1][\vt[\mostpullarm]]
    \ge \sum_{\indv\in\vta[\mostpullvariables][\run][\sol[\arm]]}
    (\vav[\meanReward][\sol[\arm]] - \vav[\meanReward][\vt[\mostpullarm]]) - 4\nAffected\vta[\radiusConf][\run-1][\vt[\mostpullarm]].
\end{equation}
%
By the choice of $\vt[\mostpullarm]$ we have $\vta[\radiusConf][\run-1]\ge\vta[\radiusConf][\run-1][\vt[\mostpullarm]]$.
With \eqref{eq:proof-UpUCBLWB-gap-decompose}, it follows that $16\nAffected\vta[\radiusConf][\run-1]\ge\va[\gapbandit]$ and thus
%
\begin{equation}
    \notag
    \vta[\pullcount][\run-1]
    \le \frac{512\nAffected^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}.
\end{equation}
%
Repeating the argument in the proof of \cref{thm:UpUCB-regret} (\ie choose $\run$ to be the last time that action $\arm$ is taken if it is taken more than once and apply decomposition \eqref{eq:regret-decomp-apx}) gives the desired result.
\end{proof}

%\cref{thm:UpUCB-L-regret} is restated below for completeness.

\UpUCBLWBRegret*
\begin{proof}
The proof follows by combining~\cref{prop:UpUCB-L-BL-regret,prop:2}.
\end{proof}


% As before, we prove \eqref{eq:UpUCB-GapUp-BL-regret} under the condition that $\event$ defined in \eqref{eq:UCB-L-event} occurs. Recall that we have shown in the proof of \cref{thm:UpUCB-L-BL-regret} that $\prob(\event)\ge1-\smallproba$ with our choice of $\alt{\smallproba}$, so this effectively leads to a high-probability regret bound.

% In the following we assume that $\event$ occurs and show that for any suboptimal arm $\arm\in\arms$, it holds
% %
% \begin{equation}
%     \label{eq:UpUCB-GapUp-pullcount-bound}
%     \vta[\pullcount][\nRuns]
%     \le
%     \max\left(
%     \min\left(
%     \frac{8\log(1/\alt{\smallproba})}{\gapUplift^2},
%     \frac{8\nVariables^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right), \frac{8(\va[\nAffected])^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right)
%     +1.
% \end{equation}
% %
% The inequality \eqref{eq:UpUCB-GapUp-BL-regret} then follows directly from \eqref{eq:regret-decomp} an a rearrangement of the terms.

% We first claim that for any $\arm\in\arms$ if $\vta[\pullcount]\ge\pullcount_0$ then $\vta[\setId]=\va[\variables]$.
% In fact, by the definition of $\pullcount_0$, $\vta[\pullcount]\ge\pullcount_0$ implies that $\vta[\radiusConf]<\gapUplift/2$.
% Therefore, as argued in the text, $\indv\in\vta[\setId]$ if and only if $\indv\in\va[\variables]$.
% Since $\vtav[\UPindex]\ge\vav[\meanUplift]$ for any $\arm$ and $\indv$, this also proves that $\vta[\UPindex]\ge\va[\uplift]$ always holds (we have either $\vta[\setId]=\variables$ or $\vta[\setId]=\va[\variables]$).

% Let $\run\in\intinterval{\nArms+1}{\nRuns}$ be the last time that a suboptimal arm $\arm$ is pulled so that $\vta[\pullcount][\nRuns]=\vta[\pullcount][\run-1]+1$.
% This indicates $\vta[\UPindex]\ge\vta[\UPindex][\run][\sol[\arm]]$, and hence $\vta[\UPindex]\ge\va[\uplift][\sol[\arm]]$.
% We distinguish between the following two cases:
% %
% \begin{enumerate}[itemsep=2.5pt,topsep=2.5pt,parsep=2.5pt]
%     \item $\vta[\pullcount][\run-1]<\pullcount_0$:
%     Then $\vta[\setId]=\variables$ so $\vta[\UPindex]=\sum_{\indv\in\variables}(\vtav[\UCBindex]-\va[\meanReward][0])
%     \le\va[\uplift]+2\nVariables\vta[\radiusConf][\run-1]$, which in turn leads to $\vta[\radiusConf][\run-1]\ge\va[\gapbandit]/(2\nVariables)$, or equivalently $\vta[\pullcount][\run-1]\le8\nVariables^2\log(1/\alt{\smallproba})/(\va[\gapbandit])^2$.
%     \item $\vta[\pullcount][\run-1]\ge\pullcount_0$:
%     Then $\vta[\setId]=\va[\variables]$ so $\vta[\UPindex]=\sum_{\indv\in\va[\variables]}(\vtav[\UCBindex]-\va[\meanReward][0])
%     \le\va[\uplift]+2\va[\nAffected]\vta[\radiusConf][\run-1]$, which in turn leads to $\vta[\radiusConf][\run-1]\ge\va[\gapbandit]/(2\va[\nAffected])$, or equivalently $\vta[\pullcount][\run-1]\le8(\va[\nAffected])^2\log(1/\alt{\smallproba})/(\va[\gapbandit])^2$.
% \end{enumerate}
% %
% Since we also have $\vta[\pullcount][\run-1]<\pullcount_0$ in the first case, the above gives
% %
% \begin{equation}
%     \notag
%     \vta[\pullcount][\run-1]
%     \le
%     \max\left(
%     \min\left(
%     \pullcount_0-1,\frac{8\nVariables^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right), \frac{8(\va[\nAffected])^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right).
% \end{equation}
% %
% Plugging in the definition of $\pullcount_0$ we get immediately \eqref{eq:UpUCB-GapUp-pullcount-bound}.

% \subsection{Proof of \cref{thm:UpUCB-GapUp-regret}}

% We shall again consider the event $\event$ defined in \eqref{eq:UCB-L-event}, which holds with probability $1-\smallproba$ as argued in the proof of \cref{thm:UpUCB-L-BL-regret}. Leveraging the decomposition in \eqref{eq:regret-decomp} it is sufficient to prove that on $\event$ we have
% \begin{equation}
%     \label{eq:UpUCB-GapUp-noBL-pullcount-bound}
%     \vta[\pullcount][\nRuns]
%     \le
%     \max\left(
%     \min\left(
%     \frac{32\log(1/\alt{\smallproba})}{\gapUplift^2},
%     \frac{32\nVariables^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right), \frac{8(\va[\nAffected]+\va[\nAffected][\sol[\arm]])^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right)
%     +1.
% \end{equation}
% %
% We assume $\event$ happens in the rest of the proof.

% Let us first focus on the elimination phase, notice that event $\event$ implies $\abs{\vta[\estalt{\reward}][\round]-\va[\reward]}<\vt[\radiusConf][\round]$ for every $\arm\in\vt[\arms][\round]$.
% % We define the event
% % %
% % \begin{equation}
% %     \notag
% %     \event_1 =
% %     \left\{\forall\round\in\oneto{\pullcount_0},
% %     ~\forall\arm\in\arms,
% %     ~ \abs{\vta[\estalt{\reward}][\round]-\va[\reward]}<\nVariables\sqrt{\frac{2\log(1/\alt{\smallproba})}{\round}}\right\}
% % \end{equation}
% % %
% % Following the proof of \cref{lem:concentration-mean-a} and a union bound over $\arm\in\arms$, we know that $\prob(\event_1)\ge1-2\nArms\pullcount_0\alt{\smallproba}$.
% In this case, the optimal arms never get eliminated.
% In fact, if $\sol[\arm]\in\vt[\arms][\round]$, then for all $\arm\in\vt[\arms][\round]$ it holds that
% %
% \begin{equation}
%     \notag
%     \vta[\estalt{\reward}][\round][\sol[\arm]]
%     +2\vt[\radiusConf][\round]
%     \ge
%     \va[\reward][\sol[\arm]]+\vt[\radiusConf][\round]
%     \ge
%     \va[\reward][\arm]+\vt[\radiusConf][\round]
%     \ge \vta[\estalt{\reward}][\round][\arm],
% \end{equation}
% %
% As a consequence, we also have $\arm\in\vt[\arms][\round+1]$ and we conclude by the principle of induction.
% With this we further deduce that all arm
% $\arm$ with $\va[\gapbandit]\ge4\vt[\radiusConf][\round]$ gets eliminated
% %\nVariables\sqrt{2\log(1/\alt{\smallproba})/\round}$ 
% after it is pulled at most $\round$ times.
% %must be eliminated at the latest in round $\round$. 
% To see this, notice that for such arm we have
% %
% \begin{equation}
%     \notag
%     \vta[\estalt{\reward}][\round]+2\vt[\radiusConf][\round]
%     < \va[\reward]+3\vt[\radiusConf][\round]
%     = \va[\reward][\sol[\arm]]-\va[\gapbandit]+3\vt[\radiusConf][\round]
%     < \vta[\estalt{\reward}][\round][\sol[\arm]].
% \end{equation}
% %
% Therefore, for all $\run$ in phase \rom{1} of the algorithm, it is true that
% %
% \begin{equation}
%     \label{eq:UpUCB-GapUp-noBL-pullcount-bound-I}
%     \vta[\pullcount]\le
%     \min\left(
%     \left\lceil\frac{32\log(1/\alt{\smallproba})}{\gapUplift^2}\right\rceil,
%     \left\lceil\frac{32\nVariables^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right\rceil
%     \right).
% \end{equation}
% %
% This suggests that inequality \eqref{eq:UpUCB-GapUp-noBL-pullcount-bound} holds if the algorithm terminates in the elimination phase.

% Otherwise, the algorithm constructs $\vv[\setBase]$'s, $\va[\setId]$'s, and switches to the UpUCB phase.
% Let us denote by $\vv[\setBase]=\setdef{\arm\in\arms}{\indv\notin\va[\variables]}$ the set of actions that do not affect variable $\indv$
% and let $\arms_{\text{res}}$ be the arms that remain after phase \rom{1}.
% %$\pullcount_0=\ceil{(32/\gapUplift^2)\log(1/\alt{\smallproba})}$ be the number of times that the uneliminated arms are pulled in the first phase.
% We argue that the sets $\vv[\setBaseEst]$ are constructed such that when $\event$ occurs, $\vv[\setBaseEst]\subseteq\vv[\setBase]$ and if there exist $\arm,\armalt\in\arms_{\text{res}}\intersect\vv[\setBase]$ such that $\arm\neq\armalt$ then we also have $\arm,\armalt\in\vv[\setBaseEst]$.
% The latter is proved by observing that under $\event$ we must have $\vav[\meanReward][0]\in\vtav[\intConf][\run_0+1]\intersect\vtav[\intConf][\run_0+1][\armalt]$ if $\arm,\armalt\in\arms_{\text{res}}\intersect\vv[\setBase]$.
% To show the former, notice that after the elimination phase, each of the arm in $\arms_{\text{res}}$ is pulled exactly $\ceil{(32/\gapUplift^2)\log(1/\alt{\smallproba})}$ times and thus $\vta[\radiusConf][\run_0]\le\gapUplift/4$.
% By \cref{asm:gapUplift-ubl}, if $\arm\notin\vv[\setBase]$, then for all $\armalt\in\setexclude{\arms_{\text{res}}}{\{\arm\}}$ we have $\abs{\vav[\meanReward]-\vav[\meanReward][\alt{\arm}]}\ge\gapUplift$, which along with the definition of $\event$ implies $\vtav[\intConf][\run_0+1]\intersect\vtav[\intConf][\run_0+1][\armalt]=\varnothing$, and therefore $\arm\notin\vv[\setBaseEst]$.

% The rest of the proof follows closely that of \cref{thm:UpUCB-regret}.
% Suppose that a suboptimal arm $\arm$ is pulled at round $\run$ during phase \rom{2} of the algorithm.
% This means $\vta[\UPindex]\ge\vta[\UPindex][\run][\sol[\arm]]$ (recall that $\sol[\arm]\in\arms_{\text{res}}$ since $\event$ happens), \ie
% %
% \begin{equation}
%     \notag
%     \sum_{\indv\in\va[\setId]}(\vtav[\UCBindex][\run]-\vtav[\UCBindex][\run][0])
%     \ge
%     \sum_{\indv\in\va[\setId][\sol[\arm]]}
%     (\vtav[\UCBindex][\run][\sol[\arm]]-\vtav[\UCBindex][\run][0]).
% \end{equation}
% %
% Rearranging the terms we get 
% %
% \begin{equation}
%     \notag
%     \sum_{\indv\in\va[\setId]}\vtav[\UCBindex][\run]
%     +\sum_{\indv\in\setexclude{\va[\setId][\sol[\arm]]}{\va[\setId]}}
%     \vtav[\UCBindex][\run][0]
%     \ge
%     \sum_{\indv\in\va[\setId][\sol[\arm]]}
%     \vtav[\UCBindex][\run][\sol[\arm]]
%     +\sum_{\indv\in\setexclude{\va[\setId]}{\va[\setId][\sol[\arm]]}}
%     \vtav[\UCBindex][\run][0].
% \end{equation}
% %
% If $\indv\in\setexclude{\va[\setId][\sol[\arm]]}{\va[\setId]}$ then $\arm\in\vv[\setBaseEst]$.
% In particular, $\vv[\setBaseEst]\neq\varnothing$ so $\armalt=\vtav[\arm][\run][0]=\argmax_{\tilde{\arm}\in\vv[\setBaseEst]}\vta[\pullcount][\run-1][\tilde{\arm}]$ is well-defined and $\vtav[\UCBindex][\run][0]=\vtav[\UCBindex][\run][\armalt]$.
% With $\vv[\setBaseEst]\subseteq\vv[\setBase]$ we know that $\vav[\meanReward][\armalt]=\vav[\meanReward][0]$ and accordingly $\abs{\vtav[\meanReward][\run-1][\armalt]-\vav[\meanReward][0]}\le\vta[\radiusConf][\run-1][\armalt]$ by the fact that $\event$ happens.
% This shows $\vtav[\UCBindex][\run][0]\ge\vav[\meanReward][0]$.
% Moreover, $\vta[\pullcount][\run][\armalt]\ge\vta[\pullcount]$ by the choice of $\armalt$; hence, $\vtav[\UCBindex]\le\vav[\meanReward][0]+2\vta[\radiusConf][\run-1][\armalt]\le\vav[\meanReward][0]+2\vta[\radiusConf][\run-1]$.
% The same argument applies to $\indv\in\setexclude{\va[\setId]}{\va[\setId][\sol[\arm]]}$, and the UCB indices of $\arm$ and $\sol[\arm]$ can be bounded from above and below as in previous proofs.
% In summary, we obtain
% %
% \begin{equation}
%     \notag
%     \sum_{\indv\in\va[\setId]}(\vav[\meanReward]+2\vta[\radiusConf][\run-1])
%     +\sum_{\indv\in\setexclude{\va[\setId][\sol[\arm]]}{\va[\setId]}}
%     (\vav[\meanReward][0]+2\vta[\radiusConf][\run-1])
%     \ge
%     \sum_{\indv\in\va[\setId][\sol[\arm]]}
%     \vav[\meanReward][\sol[\arm]]
%     +\sum_{\indv\in\setexclude{\va[\setId]}{\va[\setId][\sol[\arm]]}}
%     \vav[\meanReward][0].
% \end{equation}
% %
% Equivalently,
% %
% \begin{equation}
%     \label{eq:UpUCB-GapUp-radConf-larger-than}
%     2\card\left(\va[\setId]\union\va[\setId][\sol[\arm]]\right)\vta[\radiusConf][\run-1]
%     \ge
%     \sum_{\indv\in\va[\setId]\union\va[\setId][\sol[\arm]]}\vav[\meanReward][\sol[\arm]]
%     -\sum_{\indv\in\va[\setId]\union\va[\setId][\sol[\arm]]}\vav[\meanReward].
% \end{equation}
% %
% To conclude, we claim that
% %
% \begin{equation}
%     \label{eq:VV-equal}
%     \va[\setId]\union\va[\setId][\sol[\arm]]=\va[\variables]\union\va[\variables][\sol[\arm]].
% \end{equation}
% %
% Let us first show $\va[\variables]\subseteq\va[\setId]\subseteq\va[\variables]\union\va[\variables][\sol[\arm]]$.
% The first inclusion is a consequence of $\vv[\setBaseEst]\subseteq\vv[\setBase]$:
% %
% \begin{equation}
%     \notag
%     \indv\in\va[\variables] \implies
%     \arm\notin\vv[\setBase] \implies
%     \arm\not\in\vv[\setBaseEst] \implies
%     \indv\in\va[\setId].
% \end{equation}
% %
% As for the second inclusion we prove it's contrapositive:
% %
% \begin{equation}
%     \notag
%     \indv\notin\va[\variables]\union\va[\variables][\sol[\arm]] \implies
%     \arm,\sol[\arm]\in\arms_{\text{res}}\intersect\vv[\setBase] \implies
%     \arm,\sol[\arm]\in\vv[\setBaseEst] \implies
%     \indv\notin\va[\setId]
% \end{equation}
% %
% Notice that the second implication holds because $\arm$ is suboptimal and in particular $\arm\neq\sol[\arm]$.
% The inclusion $\va[\variables][\sol[\arm]]\subseteq\va[\setId][\sol[\arm]]\subseteq\va[\variables]\union\va[\variables][\sol[\arm]]$ can be proved in a similar way, and combining these results gives \eqref{eq:VV-equal}.
% Therefore, the \acl{RHS} of \eqref{eq:UpUCB-GapUp-radConf-larger-than} is exactly $\va[\gapbandit]$ while the \acl{LHS} of \eqref{eq:UpUCB-GapUp-radConf-larger-than} is bounded from above by $2(\va[\nAffected]+\va[\nAffected][\sol[\arm]])\vta[\radiusConf][\run-1]$.
% In consequence,
% %
% \begin{equation}
%     \notag
%     \vta[\pullcount][\run-1]
%     \le \frac{8(\va[\nAffected]+\va[\nAffected][\sol[\arm]])^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}.
% \end{equation}
% %
% Therefore, any suboptimal arm that gets pulled in the UpUCB phase satisfies
% %
% \begin{equation}
%     \notag
%     \vta[\pullcount][\nRuns]
%     \le \frac{8(\va[\nAffected]+\va[\nAffected][\sol[\arm]])^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}+1.
% \end{equation}
% %
% On the other hand, if an suboptimal arm is not pulled in the UpUCB phase then \eqref{eq:UpUCB-GapUp-noBL-pullcount-bound-I} applies, so in either case \eqref{eq:UpUCB-GapUp-noBL-pullcount-bound} is verified, which concludes the proof.

\subsection{Unknown Affected Variables: Proofs of \cref{thm:UpUCB-GapUp-BL-regret,thm:UpUCB-GapUp-regret}}
\label{apx:lower-bound-unknown-affected}
\UpUCBGapUpBL*
\begin{proof}
As before, we prove \eqref{eq:UpUCB-GapUp-BL-regret} under the condition that $\event$ defined in \eqref{eq:UCB-L-event} occurs. Recall that we have shown in the proof of \cref{prop:UpUCB-L-BL-regret} that $\prob(\event)\ge1-\smallproba$ with our choice of $\alt{\smallproba}$, so this effectively leads to a high-probability regret bound.

In the following we assume that $\event$ occurs and show that for any suboptimal action $\arm\in\arms$, it holds
%
\begin{equation}
    \label{eq:UpUCB-GapUp-pullcount-bound}
    \vta[\pullcount][\nRuns]
    \le
    \max\left(
    \min\left(
    \frac{8\log(1/\alt{\smallproba})}{\gapUplift^2},
    \frac{8\nVariables^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right), \frac{8(\va[\nAffected])^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right)
    +1.
\end{equation}
%
The inequality \eqref{eq:UpUCB-GapUp-BL-regret} then follows directly from \eqref{eq:regret-decomp-apx} and a rearrangement of the terms.

We first claim that for any $\arm\in\arms$ if $\vta[\pullcount]\ge\pullcount_0$ then $\vta[\setId]=\va[\variables]$.
In fact, by the definition of $\pullcount_0$, $\vta[\pullcount]\ge\pullcount_0$ implies that $\vta[\radiusConf]<\gapUplift/2$.
Therefore, as argued in the text, $\indv\in\vta[\setId]$ if and only if $\indv\in\va[\variables]$.
Since $\vtav[\UPindex]\ge\vav[\meanUplift]$ for any $\arm$ and $\indv$, this also proves that $\vta[\UPindex]\ge\va[\uplift]$ always holds (we have either $\vta[\setId]=\variables$ or $\vta[\setId]=\va[\variables]$).

Let $\run\in\intinterval{\nArms+1}{\nRuns}$ be the last time that a suboptimal action $\arm$ is taken so that $\vta[\pullcount][\nRuns]=\vta[\pullcount][\run-1]+1$.
This indicates $\vta[\UPindexSum]\ge\vta[\UPindexSum][\run][\sol[\arm]]$, and hence $\vta[\UPindexSum]\ge\va[\uplift][\sol[\arm]]$.
We distinguish between the following two cases:
%
\begin{enumerate}[itemsep=2.5pt,topsep=2.5pt,parsep=2.5pt]
    \item $\vta[\pullcount][\run-1]<\pullcount_0$:
    Then $\vta[\setId]=\variables$ so $\vta[\UPindexSum]=\sum_{\indv\in\variables}(\vtav[\UCBindex]-\va[\meanReward][0])
    \le\va[\uplift]+2\nVariables\vta[\radiusConf][\run-1]$, which in turn leads to $\vta[\radiusConf][\run-1]\ge\va[\gapbandit]/(2\nVariables)$, or equivalently $\vta[\pullcount][\run-1]\le8\nVariables^2\log(1/\alt{\smallproba})/(\va[\gapbandit])^2$.
    \item $\vta[\pullcount][\run-1]\ge\pullcount_0$:
    Then $\vta[\setId]=\va[\variables]$ so $\vta[\UPindexSum]=\sum_{\indv\in\va[\variables]}(\vtav[\UCBindex]-\va[\meanReward][0])
    \le\va[\uplift]+2\va[\nAffected]\vta[\radiusConf][\run-1]$, which in turn leads to $\vta[\radiusConf][\run-1]\ge\va[\gapbandit]/(2\va[\nAffected])$, or equivalently $\vta[\pullcount][\run-1]\le8(\va[\nAffected])^2\log(1/\alt{\smallproba})/(\va[\gapbandit])^2$.
\end{enumerate}
%
Since we also have $\vta[\pullcount][\run-1]<\pullcount_0$ in the first case, the above gives
%
\begin{equation}
    \notag
    \vta[\pullcount][\run-1]
    \le
    \max\left(
    \min\left(
    \pullcount_0-1,\frac{8\nVariables^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right), \frac{8(\va[\nAffected])^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right).
\end{equation}
%
Plugging in the definition of $\pullcount_0$ we get immediately \eqref{eq:UpUCB-GapUp-pullcount-bound}.
\end{proof}

\UpUCBGapUpregret*
\begin{proof}
We shall again consider the event $\event$ defined in \eqref{eq:UCB-L-event}, which holds with probability $1-\smallproba$ as argued in the proof of \cref{prop:UpUCB-L-BL-regret}. Leveraging the decomposition in \eqref{eq:regret-decomp-apx} it is sufficient to prove that on $\event$ we have
\begin{equation}
    \label{eq:UpUCB-GapUp-noBL-pullcount-bound}
    \vta[\pullcount][\nRuns]
    \le
    \max\left(
    \min\left(
    \frac{32\log(1/\alt{\smallproba})}{\gapUplift^2},
    \frac{32\nVariables^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right), \frac{8(\va[\nAffected]+\va[\nAffected][\sol[\arm]])^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right)
    +1.
\end{equation}
%
We assume $\event$ happens in the rest of the proof.

Let us first focus on the elimination phase, notice that event $\event$ implies $\abs{\vta[\estalt{\reward}][\round]-\va[\reward]}<\vt[\radiusConf][\round]$ for every $\arm\in\vt[\arms][\round]$.
% We define the event
% %
% \begin{equation}
%     \notag
%     \event_1 =
%     \left\{\forall\round\in\oneto{\pullcount_0},
%     ~\forall\arm\in\arms,
%     ~ \abs{\vta[\estalt{\reward}][\round]-\va[\reward]}<\nVariables\sqrt{\frac{2\log(1/\alt{\smallproba})}{\round}}\right\}
% \end{equation}
% %
% Following the proof of \cref{lem:concentration-mean-a} and a union bound over $\arm\in\arms$, we know that $\prob(\event_1)\ge1-2\nArms\pullcount_0\alt{\smallproba}$.
In this case, the optimal actions never get eliminated.
In fact, if $\sol[\arm]\in\vt[\arms][\round]$, then for all $\arm\in\vt[\arms][\round]$ it holds that
%
\begin{equation}
    \notag
    \vta[\estalt{\reward}][\round][\sol[\arm]]
    +2\vt[\radiusConf][\round]
    \ge
    \va[\reward][\sol[\arm]]+\vt[\radiusConf][\round]
    \ge
    \va[\reward][\arm]+\vt[\radiusConf][\round]
    \ge \vta[\estalt{\reward}][\round][\arm],
\end{equation}
%
As a consequence, we also have $\sol[\arm]\in\vt[\arms][\round+1]$ and we conclude by the principle of induction.
With this we further deduce that all action
$\arm$ with $\va[\gapbandit]\ge4\vt[\radiusConf][\round]$ gets eliminated
%\nVariables\sqrt{2\log(1/\alt{\smallproba})/\round}$ 
after it is taken at most $\round$ times.
%must be eliminated at the latest in round $\round$. 
To see this, notice that for such action we have
%
\begin{equation}
    \notag
    \vta[\estalt{\reward}][\round]+2\vt[\radiusConf][\round]
    < \va[\reward]+3\vt[\radiusConf][\round]
    = \va[\reward][\sol[\arm]]-\va[\gapbandit]+3\vt[\radiusConf][\round]
    < \vta[\estalt{\reward}][\round][\sol[\arm]]
    -\va[\gapbandit]+4\vt[\radiusConf][\round]
    \le \vta[\estalt{\reward}][\round][\sol[\arm]].
\end{equation}
%
Therefore, for all $\run$ in phase \rom{1} of the algorithm, it is true that
%
\begin{equation}
    \label{eq:UpUCB-GapUp-noBL-pullcount-bound-I}
    \vta[\pullcount]\le
    \min\left(
    \left\lceil\frac{32\log(1/\alt{\smallproba})}{\gapUplift^2}\right\rceil,
    \left\lceil\frac{32\nVariables^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}\right\rceil
    \right).
\end{equation}
%
This suggests that inequality \eqref{eq:UpUCB-GapUp-noBL-pullcount-bound} holds if the algorithm terminates in the elimination phase.

Otherwise, the algorithm constructs $\vv[\setBase]$'s, $\va[\setId]$'s, and switches to the \textsc{UpUCB} phase.
Let us denote by $\vv[\setBase]=\setdef{\arm\in\arms}{\indv\notin\va[\variables]}$ the set of actions that do not affect variable $\indv$
and let $\arms_{\text{res}}=\vt[\arms][\pullcount_0+1]$ be the actions that remain after phase \rom{1}.
%$\pullcount_0=\ceil{(32/\gapUplift^2)\log(1/\alt{\smallproba})}$ be the number of times that the uneliminated arms are pulled in the first phase.
We argue that the sets $\vv[\setBaseEst]$ are constructed such that when $\event$ occurs,
\begin{enumerate}[\textup(\itshape i\textup)]
    \item $\vv[\setBaseEst]\subseteq\vv[\setBase]$.
    \item  If there exist $\arm,\armalt\in\arms_{\text{res}}\intersect\vv[\setBase]$ such that $\arm\neq\armalt$ then we also have $\arm,\armalt\in\vv[\setBaseEst]$.
\end{enumerate}
%
The second point is proved by observing that under $\event$ we must have $\vav[\meanReward][0]\in\vtav[\intConf][\run_0+1]\intersect\vtav[\intConf][\run_0+1][\armalt]$ if $\arm,\armalt\in\arms_{\text{res}}\intersect\vv[\setBase]$.
To show the first point, notice that after the elimination phase, each of the action in $\arms_{\text{res}}$ is taken exactly $\ceil{(32/\gapUplift^2)\log(1/\alt{\smallproba})}$ times and thus $\vta[\radiusConf][\run_0]\le\gapUplift/4$.
By \cref{asm:gapUplift-ubl}, if $\arm\notin\vv[\setBase]$, then for all $\armalt\in\setexclude{\arms_{\text{res}}}{\{\arm\}}$ we have $\abs{\vav[\meanReward]-\vav[\meanReward][\alt{\arm}]}\ge\gapUplift$, which along with the definition of $\event$ implies $\vtav[\intConf][\run_0+1]\intersect\vtav[\intConf][\run_0+1][\armalt]=\varnothing$, and therefore $\arm\notin\vv[\setBaseEst]$.

The rest of the proof follows closely that of \cref{thm:UpUCB-regret}.
Suppose that a suboptimal action $\arm$ is taken at round $\run$ during phase \rom{2} of the algorithm.
This means $\vta[\UPindexSum]\ge\vta[\UPindexSum][\run][\sol[\arm]]$ (recall that $\sol[\arm]\in\arms_{\text{res}}$ since $\event$ happens), \ie
%
\begin{equation}
    \notag
    \sum_{\indv\in\va[\setId]}(\vtav[\UCBindex][\run]-\vtav[\UCBindex][\run][0])
    \ge
    \sum_{\indv\in\va[\setId][\sol[\arm]]}
    (\vtav[\UCBindex][\run][\sol[\arm]]-\vtav[\UCBindex][\run][0]).
\end{equation}
%
Rearranging the terms we get 
%
\begin{equation}
    \notag
    \sum_{\indv\in\va[\setId]}\vtav[\UCBindex][\run]
    +\sum_{\indv\in\setexclude{\va[\setId][\sol[\arm]]}{\va[\setId]}}
    \vtav[\UCBindex][\run][0]
    \ge
    \sum_{\indv\in\va[\setId][\sol[\arm]]}
    \vtav[\UCBindex][\run][\sol[\arm]]
    +\sum_{\indv\in\setexclude{\va[\setId]}{\va[\setId][\sol[\arm]]}}
    \vtav[\UCBindex][\run][0].
\end{equation}
%
If $\indv\in\setexclude{\va[\setId][\sol[\arm]]}{\va[\setId]}$ then $\arm\in\vv[\setBaseEst]$.
In particular, $\vv[\setBaseEst]\neq\varnothing$ so $\armalt=\vtav[\arm][\run][0]=\argmax_{\tilde{\arm}\in\vv[\setBaseEst]}\vta[\pullcount][\run-1][\tilde{\arm}]$ is well-defined and $\vtav[\UCBindex][\run][0]=\vtav[\UCBindex][\run][\armalt]$.
With $\vv[\setBaseEst]\subseteq\vv[\setBase]$ we know that $\vav[\meanReward][\armalt]=\vav[\meanReward][0]$ and accordingly $\abs{\vtav[\meanReward][\run-1][\armalt]-\vav[\meanReward][0]}\le\vta[\radiusConf][\run-1][\armalt]$ by the fact that $\event$ happens.
This shows $\vtav[\UCBindex][\run][0]\ge\vav[\meanReward][0]$.
Moreover, $\vta[\pullcount][\run][\armalt]\ge\vta[\pullcount]$ by the choice of $\armalt$; hence, $\vtav[\UCBindex][\run][0]\le\vav[\meanReward][0]+2\vta[\radiusConf][\run-1][\armalt]\le\vav[\meanReward][0]+2\vta[\radiusConf][\run-1]$.
The same argument applies to $\indv\in\setexclude{\va[\setId]}{\va[\setId][\sol[\arm]]}$, and the UCB indices of $\arm$ and $\sol[\arm]$ can be bounded from above and below as in previous proofs.
In summary, we obtain
%
\begin{equation}
    \notag
    \sum_{\indv\in\va[\setId]}(\vav[\meanReward]+2\vta[\radiusConf][\run-1])
    +\sum_{\indv\in\setexclude{\va[\setId][\sol[\arm]]}{\va[\setId]}}
    (\vav[\meanReward][0]+2\vta[\radiusConf][\run-1])
    \ge
    \sum_{\indv\in\va[\setId][\sol[\arm]]}
    \vav[\meanReward][\sol[\arm]]
    +\sum_{\indv\in\setexclude{\va[\setId]}{\va[\setId][\sol[\arm]]}}
    \vav[\meanReward][0].
\end{equation}
%
Equivalently,
%
\begin{equation}
    \label{eq:UpUCB-GapUp-radConf-larger-than}
    2\card\left(\va[\setId]\union\va[\setId][\sol[\arm]]\right)\vta[\radiusConf][\run-1]
    \ge
    \sum_{\indv\in\va[\setId]\union\va[\setId][\sol[\arm]]}\vav[\meanReward][\sol[\arm]]
    -\sum_{\indv\in\va[\setId]\union\va[\setId][\sol[\arm]]}\vav[\meanReward].
\end{equation}
%
To conclude, we claim that
%
\begin{equation}
    \label{eq:VV-equal}
    \va[\setId]\union\va[\setId][\sol[\arm]]=\va[\variables]\union\va[\variables][\sol[\arm]].
\end{equation}
%
Let us first show $\va[\variables]\subseteq\va[\setId]\subseteq\va[\variables]\union\va[\variables][\sol[\arm]]$.
The first inclusion is a consequence of $\vv[\setBaseEst]\subseteq\vv[\setBase]$:
%
\begin{equation}
    \notag
    \indv\in\va[\variables] \implies
    \arm\notin\vv[\setBase] \implies
    \arm\not\in\vv[\setBaseEst] \implies
    \indv\in\va[\setId].
\end{equation}
%
As for the second inclusion we prove it's contrapositive:
%
\begin{equation}
    \notag
    \indv\notin\va[\variables]\union\va[\variables][\sol[\arm]] \implies
    \arm,\sol[\arm]\in\arms_{\text{res}}\intersect\vv[\setBase] \implies
    \arm,\sol[\arm]\in\vv[\setBaseEst] \implies
    \indv\notin\va[\setId]
\end{equation}
%
Notice that the second implication holds because $\arm$ is suboptimal and in particular $\arm\neq\sol[\arm]$.
The inclusion $\va[\variables][\sol[\arm]]\subseteq\va[\setId][\sol[\arm]]\subseteq\va[\variables]\union\va[\variables][\sol[\arm]]$ can be proved in a similar way, and combining these results gives \eqref{eq:VV-equal}.
Therefore, the \acl{RHS} of \eqref{eq:UpUCB-GapUp-radConf-larger-than} is exactly $\va[\gapbandit]$ while the \acl{LHS} of \eqref{eq:UpUCB-GapUp-radConf-larger-than} is bounded from above by $2(\va[\nAffected]+\va[\nAffected][\sol[\arm]])\vta[\radiusConf][\run-1]$.
In consequence,
%
\begin{equation}
    \notag
    \vta[\pullcount][\run-1]
    \le \frac{8(\va[\nAffected]+\va[\nAffected][\sol[\arm]])^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}.
\end{equation}
%
Therefore, any suboptimal action that gets taken in the \textsc{UpUCB} phase satisfies
%
\begin{equation}
    \notag
    \vta[\pullcount][\nRuns]
    \le \frac{8(\va[\nAffected]+\va[\nAffected][\sol[\arm]])^2\log(1/\alt{\smallproba})}{(\va[\gapbandit])^2}+1.
\end{equation}
%
On the other hand, if an suboptimal action is not taken in the \textsc{UpUCB} phase then \eqref{eq:UpUCB-GapUp-noBL-pullcount-bound-I} applies, so in either case \eqref{eq:UpUCB-GapUp-noBL-pullcount-bound} is verified, which concludes the proof.
\end{proof}


==> Uplifting bandits - arxiv/Content.tex <==
%\doparttoc % Tell to minitoc to generate a toc for the parts
%\faketableofcontents % Run a fake tableofcontents command for the partocs

% \part{} % Start the document part
% \parttoc % Insert the document TOC

\begin{abstract}
\input{Sections/Abstract}
\end{abstract}

\newpage
\begin{spacing}{0.85}
\tableofcontents
\end{spacing}
\newpage

\section{Introduction}
\label{sec:intro}
\input{Sections/Introduction}

\section{Problem Description}
\label{sec:model}
\input{Sections/UpBandit}


%\section{Uplifting Bandit: Case of Known Affected}
\section{Case of Unknown Baseline}
\label{sec:known-affected}
\input{Sections/UpUCB}

% \section{Lower Bounds}
% \label{sec:lower}
% \input{Sections/Lower-bounds}

\section{Case of Unknown Affected Variables}
\label{sec:unknown-affected}
\input{Sections/Unknown-affected}




\input{Figures/Exp-figure-main}
\section{Numerical Experiments}
\label{sec:exp}
\input{Sections/Experiments}

\section{Contextual Extensions}
\label{sec:context}
\input{Sections/Contextual}

\section{Related Work}
\label{sec:related}
\input{Sections/Related}


\section{Concluding Remarks}
\label{sec:conc}
\input{Sections/Conclusion}

\input{Tables/Notations}

\bibliography{references}
\bibliographystyle{plainnat}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newpage
\appendix

% \noindent\rule{\textwidth}{1pt}
% \begin{center}
% \vspace{7pt}
% {\Large  Appendix for ``Uplifting Bandits''}
% \end{center}
% \noindent\rule{\textwidth}{1pt}
%\appendixpage
% \section*{Table of Contents}
% \startcontents[sections]
% \printcontents[sections]{l}{1}{\setcounter{tocdepth}{2}}
%\tableofcontents


% \section{Notation Table}
% \label{apx:missing}
% \input{Appendices/Missing}

% \newpage
% \section{Additional Related Work}
% \label{apx:related}
% \input{Appendices/Related}

%\section{More on \textsc{UpUCB}}
%\label{apx:UpUCB}
%\input{Appendices/UpUCB-more}

% \section{Concentration bounds}
% \label{apx:concentration}
% \input{Appendices/Concentration}

\section{Proofs for Upper Bound Results}
\label{apx:upper-bound}
\input{Appendices/Upper-bound}

\section{Lower Bounds}
\label{apx:lower-bound}
\input{Appendices/Lower-bound}

% \section{Case of Unknown Affected Variables: Scenario 2}
% \label{apx:unknown-affected-2}
% \input{Appendices/UpUCB-GapUp-UBL}

\section{Contextual Combinatorial Uplifting Bandits}
\label{apx:C2UpUCB}
\input{Appendices/C2UpUCB}

\section{Additional Experimental Details}
\label{apx:exp-detail}
\input{Appendices/Experiments}


==> Uplifting bandits - arxiv/Figures/Exp-figure-ablation.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=0.49\linewidth]{Figures/UpUCB-UCBLCB-mean.pdf}
    \includegraphics[width=0.49\linewidth]{Figures/UpUCB-UCBLCB-95.pdf}
    \caption{Baseline UCB versus Baseline LCB}
    \label{subfig:UCB-LCB}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=0.49\linewidth]{Figures/UpUCB-L-mean.pdf}
    \includegraphics[width=0.49\linewidth]{Figures/UpUCB-L-95.pdf}
    \caption{Consequence of misspecification of $\nAffected$}
    \label{subfig:misL}
    \end{subfigure}
    %\captionsetup{labelsep=space}
    \caption{Ablation study on Gaussian uplifting bandit to investigate two aspects of our algorithms. Besides mean regret with standard error, we also plot the $95$-th percentile of the regrets as an indicator for the robustness of a method.}
    \vspace{-1em}
\end{figure*}

==> Uplifting bandits - arxiv/Figures/Exp-figure-main.tex <==
\begin{figure*}[t!]
%\begin{wrapfigure}[24]{r}{0.4\textwidth}
    \centering
    \vspace{-2em}
    \begin{subfigure}{0.45\linewidth}
    \includegraphics[width=\linewidth]{Figures/Gaussian-main-stderr.pdf}
    \caption{Gaussian uplifting bandit}
    \label{subfig:exp-gau}
    \end{subfigure}
    \hspace{1em}
    \begin{subfigure}{0.45\linewidth}
    \includegraphics[width=\linewidth]{Figures/Bernoulli-main-stderr.pdf}
    \caption{Bernoulli uplifting bandit}
    \label{subfig:exp-ber}
    \end{subfigure}
    % \begin{subfigure}{0.325\linewidth}
    % \includegraphics[width=\linewidth]{Figures/averaged-uplift-with-true-data-stderr.pdf}
    % \caption{Targeted campaign}
    % \label{subfig:exp-c2}
    % \end{subfigure}
    \captionsetup{labelsep=space}
    \caption{Experimental results on a synthetic and real-world dataset.
    All the curves are averaged over $100$ runs and the shaded areas represent the standard errors.}
    %\caption{\textbf{- [Illustrative experiments]:} The realized actions (top, each line representing a coordinate of $\vwt[\action]$) and the individual regret (bottom) of a subset of players in a finite two-player zero-sum game (left), a resource allocation auction (middle), and a three-player matching-pennies game \cite{Jordan93} (right).}
    \label{fig:exp-main}
    %\vspace{-2em}
%\end{wrapfigure}
\end{figure*}

==> Uplifting bandits - arxiv/Figures/Exp-figure-more-on-c2.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{\linewidth}
    \centering
    \includegraphics[width=0.325\linewidth]{Figures/regret-with-true-data.pdf}
    \includegraphics[width=0.325\linewidth]{Figures/regret-realized-with-true-data.pdf}
    \includegraphics[width=0.325\linewidth]{Figures/averaged-uplift-with-true-data-apx.pdf}
    \caption{Logistic models only used to generate counterfactual outcomes.}
    \label{subfig:exp-c2-add-with-true}
    \end{subfigure}\\
    \vspace*{0.6em}
    \begin{subfigure}[b]{\linewidth}
    \centering
    \includegraphics[width=0.325\linewidth]{Figures/regret-without-true-data.pdf}
    \includegraphics[width=0.325\linewidth]{Figures/regret-realized-without-true-data.pdf}
    \includegraphics[width=0.325\linewidth]{Figures/averaged-uplift-without-true-data-apx.pdf}
    \caption{Logistic models used to generate all the outcomes.}
    \label{subfig:exp-c2-add-without-true}
    \end{subfigure}
    %\captionsetup{labelsep=space}
    \caption{Results on the targeted campaign experiment. For the top row  the logistic models are only used to generate counterfactual outcomes, and in the bottom row all the outcomes are generated using the predicted conditional probabilities of the logistic models. We plot regret computed using the predicted uplifts and the realized rewards, and the predicted uplift averaged over all the treated individuals.}
    %\vspace{-2ex}
    \label{fig:exp-c2-add}
    \vspace{-1em}
\end{figure}

==> Uplifting bandits - arxiv/Figures/Exp-figure-targeted.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}{0.9\linewidth}
    \includegraphics[width=\linewidth]{Figures/averaged-uplift-with-true-data-stderr.pdf}
    \end{subfigure}
    \caption{Experimental results for the contextual combinatorial model.
    All the curves are averaged over $100$ runs and the shaded areas represent the standard errors.}
    \label{fig:exp-c2}
    %\vspace{-2ex}
    \vspace{-1em}
\end{figure*}

==> Uplifting bandits - arxiv/Figures/Illustration.tex <==
% 0.34 0.63
\begin{figure*}[t]
\centering
\begin{minipage}[b]{.31\textwidth}
  \centering
   \includegraphics[width=0.94\textwidth]{Figures/UpBandit-Model.pdf}
  \captionof{figure}{Illustration of the uplifting bandit model. This example has $\nArms=3$ arms, $\nVariables=5$ variables and each action affects  $\va[\nAffected]=2$ variables.
  Dash lines indicate the variables' payoffs follow the baseline distribution $\va[\distribution][0]$ by default.} %when not affected.}
  %\todob{We can also try to explain notation here.}}
  \label{fig:model}
\end{minipage}
\hfill
\begin{minipage}[b]{.66\textwidth}
  \centering
  \begin{subfigure}{0.475\textwidth}
  \centering
  \includegraphics[width=0.86\textwidth]{Figures/UpUCB.pdf}
  \vskip 5pt
  \caption{\UpUCBwb: After suboptimal action $\vt[\arm]$ is taken, the confidence intervals of $(\vav[\meanReward])_{\indv\in\va[\variables][\vt[\arm]]}$ and $(\vav[\meanReward][0])_{\indv\in\setexclude{\va[\variables][\sol[\arm]]}{\va[\variables][\vt[\arm]]}}$ shrink (from purple to pink). Hence the uplifting index of $\vt[\arm]$ decreases while that of $\sol[\arm]$ increases (from dash to solid).}
  %\todob{Explain colors.}}
  \label{subfig:UpUCBwb}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.475\textwidth}
  \centering
  \includegraphics[width=0.86\textwidth]{Figures/UpUCB-nAff-b.pdf}
  \vskip 5pt
  \caption{\UpUCBL: To compute the uplifting index of an action, we identify a set of variables whose associated confidence intervals do not contain the baseline payoff and pad it with the variables with the largest UCBs on uplifts.}
  \label{subfig:UpUCBL}
  \end{subfigure}
  \addtocounter{figure}{-1}
  %of the working principles of
  \captionof{figure}{Explanation about \UpUCBwb and \UpUCBL using the model illustrated in \cref{fig:model}.}
  %\todosk{If Fig.2 is on the model from Fig.1, then that point is not coming across.}}
  \label{fig:algorithms}
\end{minipage}
\vspace{-0.6em}
\end{figure*}

==> Uplifting bandits - arxiv/Sections/Abstract.tex <==
We introduce a multi-armed bandit model where the reward is a sum of multiple random variables, and each action only alters the distributions of some of them. After each action, the agent observes the realizations of all the variables. This model is motivated by marketing campaigns and recommender systems, where the variables represent outcomes on individual customers, such as clicks. We propose UCB-style algorithms that estimate the \emph{uplifts} of the actions over a baseline. We study multiple variants of the problem, including when the baseline and affected variables are unknown, and prove sublinear regret bounds for all of these. We also provide lower bounds that justify the necessity of our modeling assumptions. Experiments on synthetic and real-world datasets show the benefit of methods that estimate the uplifts over policies that do not use this structure.


==> Uplifting bandits - arxiv/Sections/Checklist.tex <==



\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{We have discussed potential extensions, which reflects the limitation of the current work.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Provided in the supplmental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See \cref{sec:exp,apx:exp-c2,apx:exp-detail,apx:exp-add}.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See \cref{apx:exp-detail}}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{See \cref{apx:exp-detail}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> Uplifting bandits - arxiv/Sections/Conclusion.tex <==
%\section{Concluding Remarks}

This paper addresses \acl{MAB} problems whose rewards can be written as a sum of some observable variables.
We showed that when each of the action only affects a limited number of these variables, much smaller regret can be achieved, and we developed algorithms with such guarantee under different variations of knowledge the learner possesses. While the focus of this paper is on \ac{UCB}s for stochastic bandits, we believe understanding how similar problem structure can be exploited for other algorithms
%and problem settings 
such as Thompson sampling, information directed sampling, or even methods for adversarial bandits is also important.

% Our work paves the way for several interesting future lines of research.
% First, we have discussed contextual extensions in \cref{sec:context}, but further investigation will be required to concertize our statements.
% Moreover, while the impact of an action may be concentrated on a few variables, assuming zero impact on the remaining ones is still a strict assumption.
% Designing theoretical-grounded algorithms for both the contextual and the misspecified regime will without doubt make our results much more practically relevant.
% Finally, while the focus of the paper is on \ac{UCB}s for stochastic bandits, how other algorithms and problem setting such as Thompson sampling, information directed sampling, or even algorithms for adversarial bandits can benefit from a similar problem structure is also an intriguing question.

==> Uplifting bandits - arxiv/Sections/Contextual.tex <==


In this section, we briefly discuss potential contextual extensions of our model.
As in contextual bandits, 
context is a side information that helps the learner to make a more informed decision, which results in a higher reward. To incorporate context, one possibility is to associate each variable with a feature vector $\vtv[\feature]\in\R^\vdim$.
The subscript $\run$ indicates that the context can change from one round to another.
We also associate each action with a function $\va[\obj]$ so that the expected payoff of action $\arm$ acting on a variable with feature $\vtv[\feature]$ is $\va[\obj](\vtv[\feature])$.
The expected reward of choosing $\arm$ at round $\run$ is then $\va[\reward](\vt[\feature])=\sum_{\allvariables}\va[\obj](\vtv[\feature])$.
The optimal action of round $\run$ is $\vt[\sol[\arm]]=\argmax_{\arm\in\arms}\va[\reward](\vt[\feature])$ and the regret of a learner that takes the actions $(\vt[\arm])_{\run\in\oneto{\nRuns}}$ is given by
%
\[
\vt[\reg][\nRuns]
    = \sum_{\run=1}^{\nRuns}\sum_{\indv\in\variables}
    (\va[\obj][\vt[\sol[\arm]]](\vtv[\feature]) - \va[\obj][\vt[\arm]](\vtv[\feature])).
\]
%
As in \cref{sec:model}, upon taking an action, the learner observes the noisy payoffs of all the variables.
The key structure in our model is there exists a baseline payoff vector $\va[\meanReward][0]$ such that for any given action $\arm$, the equality $\vav[\meanReward]=\vav[\meanReward][0]$ holds for most $\indv\in\variables$.
Given context, this can be translated into the existence of a baseline function $\va[\obj][0]$ such that for any given $\arm$ and $\run$, the equality $\va[\obj](\vtv[\feature])=\va[\obj][0](\vtv[\feature])$ holds for most $\indv\in\variables$.
The uplift of action $\arm$ is defined as \[\va[\up{\reward}](\vt[\feature])=\sum_{\allvariables}\va[\obj](\vtv[\feature])-\va[\obj][0](\vtv[\feature]).\]
We provide two concrete examples of the contextual extension below.
%We will focus on the situation where the feature vectors $(\vtv[\feature])_{\allvariables}$ are revealed to the learner at the beginning of each round. \todobmargin{Why the last sentence? This setting is standard.}

\medskip
\paragraph{Contextual Uplifting Bandit with Linear Payoffs\afterhead}
\label{subsec:contextual-linear}
%For concreteness, let us consider a model with linear payoffs. Then
In this model, each action is associated with an unknown parameter $\va[\param]$ and the expected payoff is the scalar product of $\va[\param]$ and the feature of the variable, \ie $\va[\obj](\vtv[\feature])=\product{\va[\param]}{\vtv[\feature]}$.
We also assume the aforementioned equality to hold for the baseline function $\va[\obj][0]$
and we use 
\[\vta[\variables]=\setdef{\indv\in\variables}{\product{\va[\param]}{\vtv[\feature]}\neq\product{\va[\param][0]}{\vtv[\feature]}}\]
for the variables affected by action $\arm$ at round $\run$.
One sufficient condition for $\vta[\variables]$ to be small is sparsity in both the parameter difference $\va[\up{\param}]=\va[\param]-\va[\param][0]$ and the context vector $\vtv[\feature]$.
In fact, $\product{\va[\param]}{\vtv[\feature]}=\product{\va[\param][0]}{\vtv[\feature]}$ as long as the supports of $\va[\up{\param}]$ and $\vtv[\feature]$ are disjoint.
%, \ie $\supp(\va[\up{\param}])\intersect\supp(\vta[\feature])=\varnothing$.
In the sequel, we assume $\card(\vta[\variables])$ is uniformly bounded by $\nAffected$.

Clearly, our algorithms can be directly applied as long as we can construct a \ac{UCB} on $\product{\va[\param]}{\vtv[\feature]}$.
This can for example be done using the construction of Linear UCB~\citep{APS11}.
In this way, the decision of the learner is again based on the uncertain estimates of at most $\bigoh(\nAffected)$ variables, and we thus expect the improvements that we have shown in our theorems would persist.
As an example, when both $\va[\param][0]$ and $\vta[\variables]$ are known, \UpUCB adapted to this situation constructs \ac{UCB} for $\sum_{\indv\in\vta[\variables]}\product{\va[\up{\param}]}{\vtv[\feature]}$, and it is straightforward to show that the regret of such algorithm can be as small as $\bigoh(\nAffected\vdim\sqrt{\nArms\nRuns})$.\footnote{As in the previous sections, this bounds applies to the case where the noises are not necessarily independent.}
In contrast, if the learner works directly with the total reward, the regret is in $\bigoh(\nVariables\vdim\sqrt{\nArms\nRuns})$.

% If both $\va[\param][0]$ and $\vta[\variables]$ are known by the learner, it only needs to learn $\va[\up{\param}]=\va[\param]-\va[\param][0]$ based on feedback received from $\vta[\variables]$, and computes an upper confidence bound on $\sum_{\indv\in\vta[\variables]}\product{\va[\up{\param}]}{\vtv[\feature]}$ to select actions.
% Following the standard analysis of linear UCB~\citep{APS11}, it is straightforward to show that the regret is $\bigoh(\nAffected\vdim\sqrt{\nArms\nRuns})$ when $\card(\vta[\variables])$ is uniformly bounded by $\nAffected$.
% In contrast, if the learner works directly with the total reward, the regret would be $\bigoh(\nVariables\vdim\sqrt{\nArms\nRuns})$. \todobmargin{Did we confirm this? We had some argument here.} %$\sum_{\allvariables}\product{\va[\param]}{\vtv[\feature]}$, the 

% %\todobmargin{I would make this discussion even more high level. If you think about it, our algorithms can be easily applied to structured problems, by replacing their UCBs with those for structured problems. The only thing that is not clear is what the regret bound would be. Make this clear.}


% If the baseline is unknown, inspired by \cref{algo:UpUCB}, we believe that the learner can compute the differences between two upper confidence bounds, on $\sum_{\indv\in\vta[\variables]}\product{\va[\param]}{\vtv[\feature]}$ and $\sum_{\indv\in\vta[\variables]}\product{\va[\param][0]}{\vtv[\feature]}$. 
% Finally, a strategy in the spirit of \cref{algo:UpUCB-GapUp-BL} might work when $\vta[\variables]$ is unknown.

% \todobmargin{Integrate this remark with the earlier paragraph.}

% Let us consider a model where each action is associated to a parameter $\va[\param]$ and there exists $\va[\param][0]$ such that $\va[\up{\param}]=\va[\param]-\va[\param][0]$ is sparse.
% We denote by $\va[\setSupp]=\supp(\va[\param]-\va[\param][0])$ as the support of the difference vector.
% The feature vectors of the individuals $(\vtv[\feature])_{\allvariables}$ can change over time and are revealed at the beginning of each round. The expected payoffs are the scalar products between the action parameter and the context features. The noise are assumed to be independent and conditionally $1$-subgaussian.
% We shall also assume that at each round $\run$, for every action $\arm$, $\product{\va[\param]}{\vtv[\feature]}=\product{\va[\param][0]}{\vtv[\feature]}$ for most of $\indv\in\variables$.
% A sufficient condition for $\product{\va[\param]}{\vtv[\feature]}=\product{\va[\param][0]}{\vtv[\feature]}$ is of of course $\supp(\va[\up{\param}])\intersect\supp(\vta[\feature])=\varnothing$.
% Similar to before, we define $\vta[\variables]=\setdef{\indv\in\variables}{\product{\va[\param]}{\vtv[\feature]}\neq\product{\va[\param][0]}{\vtv[\feature]}}$.
% Our algorithm operates with the knowledge of both $\va[\setSupp]$ and $\vta[\variables]$ (of course, the supersets of these sets suffice).
% We write $\sparsity=\max_{\arm\in\arms}\card(\va[\setSupp])$ and $\nAffected=\max_{\arm\in\arms,\run\in\oneto{\nRuns}}\card(\vta[\variables])$.

% Let $\extendvdim=\vdim+\sum_{\arm\in\arms}\card(\va[\setSupp])$ and $\va[\setRes]=\intinterval{\vdim+\sum_{\armalt=1}^{\arm-1}\card(\va[\setSupp][\armalt])+1}{\vdim+\sum_{\armalt=1}^{\arm}\card(\va[\setSupp][\armalt])}$.
% As for the algorithm, we define $\param=(\va[\param][0],\va[\restr{\param}{\va[\setSupp][1]}][1],\ldots,\va[\restr{\param}{\va[\setSupp][\nArms]}][\nArms])\in\R^{\extendvdim}$ as the concatenation of all relevant parameters.
% The extended features $\vtav[\extendfeature]\in\R^{\extendvdim}$ are constructed such that $\supp(\vtav[\extendfeature])\subset\setcomplement{\va[\setSupp]}\union\va[\setRes]$, $\restr{\vtav[\extendfeature]}{\va[\setRes]}=\restr{\vtv[\feature]}{\va[\setSupp]}$ and $\restr{\vtav[\extendfeature]}{\setcomplement{\va[\setSupp]}}=\restr{\vtv[\feature]}{\setcomplement{\va[\setSupp]}}$ (where $\setcomplement{\va[\setSupp]}=\setexclude{\oneto{\vdim}}{\va[\setSupp]}$). In the following we will abbreviate $\vtv[\extendfeature]=\vtav[\extendfeature][\run][\vt[\arm]]$.
% Clearly, it holds $\product{\param}{\vtv[\extendfeature]}=\product{\va[\param][\vt[\arm]]}{\vtv[\feature]}$.




%\todobmargin{This subsection is hard to follow. BTW what is the observation model? Do we still observe all variables?}

% Here, we make a practical {\em no interference} assumption, that the payoff of each individual only depends on whether they are treated or not (i.e., independent of others). 
% %the treatment they receive.
% We can thus define functions $\va[\objalt][\indtreat]$ for $\indtreat\in\{0,1\}$ so that $\va[\obj](\vtv[\feature])=\va[\objalt][\vv[\arm]](\vtv[\feature])$.\footnote{%
% Strictly speaking, $\va[\obj]$ is a function of $(\vtv[\feature], \indv)$ here.}
% Considering the action of not treating any individual as the baseline,
% the uplift of action $\arm$ in round $\run$ is given by $\va[\up{\reward}](\vt[\feature])=\sum_{\indv\in\va[\variables]}\va[\objalt][\vv[\arm]](\vtv[\feature])-\va[\objalt][0](\vtv[\feature])$,
% where $\va[\variables]$ is the set of individuals treated by action $\arm$.
% For UCB-type methods, we should thus provide upper confidence bounds $\vtav[\UCBindex][\run][\indtreat]$ for $\va[\objalt][\indtreat](\vtv[\feature])$.
% Depending on whether the baseline function is known or not, we may subtract $\va[\objalt][0](\vtv[\feature])$ or $\vtav[\UCBindex][\run][0]$ from $\vtav[\UCBindex][\run][1]$ to compute the uplifting indices for each individual.
% The algorithm then chooses the $\nAffected$ individuals with the highest uplifting indices.
    % We refer to the resulting algorithm as \CUpUCB and provide its pseudo code in \cref{apx:missing}.
% %This algorithm, which we refer to as \CUpUCB, is outlined in \cref{algo:C2UpUCB}.
% In \cref{apx:C2UpUCB}, we further present a generalization of the algorithm to the case of multiple treatments and a theoretical analysis thereof for linear expected payoffs.

%For simplicity, we again assume the expected payoff to be linear in the feature vector.

%The form of $\va[\obj]$ may also encode some information about the action.
%A prominent example is when the action has a combinatorial nature
%To illustrate this idea, we present a very different model inspired by applications in targeted campaign.

\paragraph{Contextual Combinatorial Uplifting Bandit\afterhead}
\label{subsec:C2UpBandit}

\input{Algorithms/C2UpUCB}

To demonstrate the flexibility of our framework, we also consider a different model that tackles the problem of targeted campaign. %(think of a personalized version of example \ref{ex:marketing}). 
Here, we refer to the variables as individuals (customers) that we may want to treat (serve) with some treatment (campaign). %$\treatments=\intinterval{1}{\nTreatments}$.
To improve the overall return on investment, it is often beneficial to treat only a subset of the individuals.
The bandit problem thus consists of finding the right set of individuals to treat at each round.
Concretely, if the learner selects at most $\nAffected$ individuals to treat in a round, 
the action set can be written as $\arms=\setdef{\arm\in\{0,1\}^{\nVariables}}{\norm{\arm}_0\le\nAffected}$, where $\norm{\arm}_0$ is the number of non-zero coordinates of $\arm$.
In this form, the $\indv$-th coordinate of $\arm$ is $1$ if and only if individual $\indv$ receives the treatment.
%non-zero only if the individual $\indv$ receives some treatment, in which case its value indicates the treatment the individual receives.
Similar to before, we observe the payoffs of all the individuals after treatments are applied.

%\todobmargin{This subsection is hard to follow. BTW what is the observation model? Do we still observe all variables?}

Here, we make a practical {\em no interference} assumption, that the payoff of each individual only depends on whether they are treated or not (i.e., independent of others). 
%the treatment they receive.
We can thus define functions $\va[\objalt][\indtreat]$ for $\indtreat\in\{0,1\}$ so that $\va[\obj](\vtv[\feature])=\va[\objalt][\vv[\arm]](\vtv[\feature])$.\footnote{%
Strictly speaking, $\va[\obj]$ is a function of $(\vtv[\feature], \indv)$ here.}
Considering the action of not treating any individual as the baseline,
the uplift of action $\arm$ in round $\run$ is given by \[\va[\up{\reward}](\vt[\feature])=\sum_{\indv\in\va[\variables]}\va[\objalt][\vv[\arm]](\vtv[\feature])-\va[\objalt][0](\vtv[\feature]),\]
where $\va[\variables]$ is the set of individuals treated by action $\arm$.
For UCB-type methods, we should thus provide upper confidence bounds $\vtav[\UCBindex][\run][\indtreat]$ for $\va[\objalt][\indtreat](\vtv[\feature])$.
Depending on whether the baseline function is known or not, we may subtract $\va[\objalt][0](\vtv[\feature])$ or $\vtav[\UCBindex][\run][0]$ from $\vtav[\UCBindex][\run][1]$ to compute the uplifting indices for each individual.
The algorithm then chooses the $\nAffected$ individuals with the highest uplifting indices.
We refer to the resulting algorithm as \CUpUCB, where C2 is the abbreviation of ``contextual combinatorial''.
We provide its pseudo code in \cref{algo:C2UpUCB} (where we suppose the baseline is unknown).
%This algorithm, which we refer to as \CUpUCB, is outlined in \cref{algo:C2UpUCB}.

In \cref{apx:C2UpUCB}, we further present a generalization of the algorithm to the case of multiple treatments, a theoretical analysis thereof for linear payoffs, and accompanying numerical experiments.


==> Uplifting bandits - arxiv/Sections/Experiments.tex <==
% Our numerical experiments cover the main model described in \cref{sec:model} and the contextual combinatorial uplifting model introduced in~\cref{subsec:C2UpBandit}.
% Besides a toy problem that we create from scratch, 

% around $25$M examples, each one representing a user. Each user is represented with $12$ features, and is associated with a binary treatment indicator and two binary outcome variables indicating their visit and conversion status.
% Such a dataset is suitable for our simulations because it contains outcomes for both treated and untreated individuals, and the untreated individuals are randomly sampled from the population.
% All our experiments are run on amazon m4.xlarge EC2 instances.

%More precisely, we conduct $100$ independent runs for each experimental setup described below,
%and in each run, we fix the random seed and test all the candidate algorithms with their parameters chosen from a predefined set.
%In the end, we report results that are averaged over these $100$ runs, with an error bar that indicates the standard deviation of the metric.

%More experimental details, including the sets from which the parameters are chosen, and additional experimental results can be found in \cref{apx:exp-detail,apx:exp-add} 

In this section, we present numerical experiments to demonstrate the benefit of estimating uplifts in our model.
We compare
%our methods introduced in \cref{sec:UpUCB-BL,sec:known-affected,sec:unknown-affected} 
\UpUCB, \UpUCBwb, \UpUCBL, and \UpUCBLwb
(\cref{algo:UpUCB-BL,algo:UpUCB,algo:UpUCB-L-BL,algo:UpUCB-L})
against UCB and Thompson sampling with Gaussian prior and Gaussian noise that only use the observed rewards $(\vt[\reward])_{\run\in\oneto{\nRuns}}$.
%\todoyg{Not sure if we need to justify the use of Gaussian prior and Gaussian noise for the Bernoulli experiment.}
To ensure a fair comparison, we tune all the considered algorithms and report the results for the parameters that yield the best averaged performance.
The experimental setup details are provided in \cref{apx:exp-detail}. The experiments for the contextual combinatorial uplifting model introduced in~\cref{subsec:C2UpBandit} are presented in \cref{apx:exp-c2}.
%The first two experiments concern our main model as described in \needref, while the third experiment addresses the combinatorial contextual uplifting model introduced in \needref.

%All the curves are averaged $100$ independent runs

\paragraph{Gaussian Uplifting Bandit\afterhead}
\label{subsec:exp-gaussian}
We first study our algorithms %(\cref{algo:UpUCB,algo:UpUCB-L-BL,algo:UpUCB-L,algo:UpUCB-GapUp-BL}) 
%\ie each action affects $10$ variables.\
in a Gaussian uplifting bandit,
\ie the noise vectors $(\va[\snoise])_{\arm\in\arms}$ are Gaussian,
with $\nArms = 10$ actions, $\nVariables = 100$ variables, and  $\va[\nAffected] \equiv 10$ meaning that each action affects $10$ variables.
%\footnote{%
%By Gaussian uplifting bandit we mean that the noise vectors $(\va[\snoise])_{\arm\in\arms}$ are Gaussian.}
The expected payoffs are contained in $[0,1]$,
%$(\vav[\meanReward][0])_{\allvariables}, (\vav[\meanReward][\arm][\indv])_{\arm\in\arms, \indv\in\va[\variables]}\in[0,1]$
%while ensuring a minimum individual uplift of $\gapUplift=0.1$
and the covariance matrix of the noise is taken the same for all the actions.
%, which we take the same for all the actions, are randomly generated.
The suboptimality gap of the created problem is around $0.2$, and the variance of the total noise $\sum_{\allvariables}\vav[\snoise]$ is around $80$.

\paragraph{Bernoulli Uplifting Bandit with Criteo Uplift\afterhead}
\label{subsec:exp-ber}
We use the Criteo Uplift Prediction Dataset~\citep{Diemert2018} 
%(abbreviated as Criteo Uplift in the following)
with `visit' as the outcome variable to build a Bernoulli uplifting bandit, where the payoff of each variable has a Bernoulli distribution.
This dataset is designed for uplift modeling, and has outcomes for both treated and untreated individuals.
Thus it is suitable for our simulations.
To build the model, we sample $10^5$ examples from the dataset, and use K-means to partition these samples into $20$ clusters of various sizes.
The $10^5$ examples are taken as our variables.
We consider $20$ actions that correspond to treating individuals of each cluster.
%, and construct independent Bernoulli payoffs using the visit rates of the treated/untreated individuals of the clusters following a procedure detailed in \cref{apx:exp-ber}.
Assuming that each cluster contains a single type of users that react in the same pattern,
we sample the payoffs $(\vtv[\valuev])_{\allvariables}$ from independent Bernoulli distributions with means that equal the average visit rates of the treated or untreated individuals of the clusters, depending on which action is chosen.
Here, $\nAffected=12654$ and $\gapbandit$ is around~$30$.

\paragraph{Results\afterhead}
\cref{fig:exp-main} confirms that we can effectively achieve much smaller regret by restricting our attention to the uplift.
Moreover, when the sets of affected are known, the loss of not knowing the baseline payoffs seems to be minimal.
Not knowing the affected variables has a more severe effect, and in particular causes much larger regret in the second experiment.
In fact, the design of \UpUCBLwb and \UpUCBL heavily rely on the additive structure of the uplifting index, and can thus hardly benefit from the payoff independence which allows the other four algorithms to achieve smaller regret in this case.


%In \cref{apx:ablation}, we further present an ablation study that looks into the consequence of using baseline lower confidence bounds in \cref{algo:UpUCB}, and the impact of misspecification of $\nAffected$ in \cref{algo:UpUCB-L}.

%As we provide \UpUCBL and \UpUCBDelta with the ground truth values of $\nAffected$ and $\gapUplift$, the only parameter to tune is $\expparam=1/\alt{\smallproba}$. We choose it from from $\intinterval{1}{10}$.
%To ensure a fair comparison between the algorithms, we tune the exploration parameter $\expparam=1/\alt{\smallproba}$ for each algorithm and report the curve with the best $\expparam$ chosen from $\intinterval{1}{10}$.


%\UpUCBL (which is provided with the optimal $\nAffected=10$ here) also performs much better than algorithms that ignore the structure of the problem, even in the case where both the baseline and the sets of affected are unknown.
%Finally, as expected, \UpUCBDelta exhibits a quite different behavior.
%In the early stage of the algorithm, it performs exactly as UCB and the regret curve only flattens after a tipping point, which corresponds to the moment that the set $\va[\variables]$ of all the relevant arms are identified.



% For each cluster, we compute the average visit rate of the treated and untreated individuals
% and $20$ clusters correspond respectively to the variables and the actions of our model.
% To construct the feedback, we assume that each cluster contains a single type of users that react in the same pattern.
% That is, if a user of a certain type is treated, their feedback is sampled from a Bernoulli distribution with mean computed using all treated individuals from the corresponding cluster; otherwise their feedback is sampled from another Bernoulli distribution with mean computed using all untreated individuals from that cluster. %\footnote{The obtained mean values and cluster sizes are reported in \cref{apx:exp-ber}.}
% The actions are then defined as applying treatment to a specific type of individuals, and the feedback of the users are sampled independently.
% In the created problem, $\nAffected=12654$ and $\gapbandit\sim30$.
% % The $10^5$ examples and $20$ clusters correspond respectively to the variables and the actions of our model.
% % To construct the feedback, we assume that each cluster contains a single type of users that react in the same pattern.
% % That is, if a user of a certain type is treated, their feedback is sampled from a Bernoulli distribution with mean computed using all treated individuals from the corresponding cluster; otherwise their feedback is sampled from another Bernoulli distribution with mean computed using all untreated individuals from that cluster. %\footnote{The obtained mean values and cluster sizes are reported in \cref{apx:exp-ber}.}
% % The actions are then defined as applying treatment to a specific type of individuals, and the feedback of the users are sampled independently.
% % In the created problem, $\nAffected=12654$ and $\gapbandit\sim30$.

% As before, we compare \UpUCB and \UpUCBwb against UCB and Thompson sampling that only use observed rewards.
% %The results are reported in
% From \cref{subfig:exp-ber} we see again that focusing on the uplift helps significantly in reducing the regret.
%Moreover, we also find both UpUCB with known and unknown baselines to be much more robust to the choice of $\expparam$.

\input{Figures/Exp-figure-ablation}
\subsection{Ablation Study on Gaussian Uplifting Bandit}
 \label{sec:abalation}
% \label{apx:exp-add}
%\label{apx:ablation}

Below we further present ablation studies on  the Gaussian uplifting bandit model.
%presented in \cref{subsec:exp-gaussian}.

\paragraph{Baseline UCB versus Baseline LCB\afterhead}
In \cref{algo:UpUCB}, we suggest subtracting the UCBs of the baseline payoffs from the UCBs of the actions.
This could be counter-intuitive because to get an optimistic estimate of the uplift, we should instead subtract the LCBs of the baseline payoffs.
However, the latter strategy prevents the learner from learning more about the baselines that are badly estimated, and can thus lead to failure more frequently.
%with the later strategy, if the baseline payoffs of a set of variables that a suboptimal arm affects are severely underestimated at the beginning, the learner may stick to that suboptimal arm, which results 
In the following, we refer to the two strategies respectively as \UpUCB-bUCB and \UpUCB-bLCB.

In \cref{subfig:UCB-LCB} (Left), we illustrate the mean regret of the two designs when their parameters are optimally tuned.
It turns out there the two strategies perform similarly here.
We would just like to highlight that to achieve the optimal performance, \UpUCB-bLCB needs to use a larger exploration parameter.
Therefore, in terms of average performance, it seems that the effect of using LCBs of the baseline is close to 
a shrinkage of the exploration parameter.

Next, we further inspect the robustness of the algorithms by plotting the $95$th percentile of the regrets (which roughly corresponds to the $5$th largest regret among those recorded in the $100$ runs).
The same parameters give the optimal values for this metric.
However, as shown in \cref{subfig:UCB-LCB} (Right), it turns out that \UpUCB-bLCB achieves a much higher $95$th percentile of regret, which indicates that it indeed fails more frequently.

\paragraph{Misspecification of $\nAffected$.}
We also investigate the effect of misspecification of $\nAffected$ on \cref{algo:UpUCB-L-BL}.
For the bandit instance that we employ here, $\max_{\arm\in\arms}\va[\nAffected]=10$ and thus according to \cref{prop:UpUCB-L-BL-regret}, \cref{algo:UpUCB-L-BL} guarantees sublinear regret as long as it is provided with $\nAffected\ge10$. On the flip side, the algorithm may incur linear regret if $\nAffected$ is underestimated.

To verify this, we run the algorithm with $\nAffected\in\{5,8,10,15\}$ and plot the averaged regret and the $95$-th percentile of regret for optimally tuned exploration parameters in \cref{subfig:misL}.
We effectively observe sublinear regret when $\nAffected$ is overspecified, but the regret becomes much larger because the algorithm is more conservative and explores more.
On the other hand, under severe underspecification of $\nAffected$, the algorithm is doomed to fail whatever the exploration parameter used.
Finally, it seems that slight underspecification of $\nAffected$ can be compensated by choosing a larger exploration parameter. In fact, in the figure we see that for $\nAffected=8$ choosing $\expparam=6$ gives the smallest regret among the presented curves.



==> Uplifting bandits - arxiv/Sections/Introduction.tex <==
%\todob{I thought that we agreed to refer to "arms" as "actions". There are many occurrences of "arm" in this section.} \todob{I find it strange that we start with an algorithm. Instead, say in a few sentences what a stochastic bandit is.}

\Ac{MAB} is an important framework for sequential decision making under uncertainty~\citep{LR85,bubeck2012regret,LS20}. In this problem, a learner repeatedly takes action and receives their rewards, while the outcomes of the other actions are unobserved. The goal of the learner is to maximize their cumulative reward over time by balancing exploration (select actions with uncertain reward estimates) and exploitation (select actions with high reward estimates). \ac{MAB} has applications in online advertisement, recommender systems, portfolio management, and dynamic channel selection in wireless networks.
%~\citep{LS20}. 

One prominent question in the \ac{MAB} literature is how the dependencies between the actions can be exploited to improve statistical efficiency. Popular examples working toward this goal include {\em linear bandits}~\citep{dani2008stochastic} and {\em combinatorial bandits}~\citep{cesa2012combinatorial}.
In this work, we study a different structured bandit problem with the following three features:
%\todoygmargin{I still found the first sentence to be weird so I tried to modify it. I think the problem is that when we say observable payoffs of the variables it feel like there can also be unobservable ones.
%The original sentence is commented out.}
\begin{enumerate*}[\textup(\itshape i\textup)]
    %\item the reward is a sum of observable payoffs of a fixed set of variables, and
    \item the reward is the sum of the payoffs of a fixed set of variables; 
    \item these payoffs are observed; and
    %the reward is obtained by summing observable payoffs of a fixed set of variables, and
    \item each action only affects a small subset of the variables.
\end{enumerate*}
This structure arises in many applications, as discussed below.
%
% Our main result shows, under a minor assumption,  even without the knowledge of the impacted variables or the baseline distribution, a learner can achieve strong regret bounds.   
%At a high level, our model is motivated by the general idea that while the final quantity of interest, \ie the reward, may be generated through a complicated mechanism that involves many factors, each single action might only have impact on a few of these factors. In this work, we focus on the special case where the reward can be described as the sum of a set of variables.
%
% \textbf{Motivating Examples.} 
% % In fact, this particular model already finds applications in various problems.
% As the name suggests, our model relevant to many of the problems that involve uplift modeling / treatment effect estimation. \todob{Cite.} We provide some examples below for the sake of concreteness.
\begin{enumerate}[label=\textbf{(\alph*)}, wide=0pt]
% \item \textbf{Product discount.}
% Consider a company that wants to use discounting to increase their sales. It is common to design discount strategies that only apply to a small subset of products. In this case, we can view the sales of each product as a variable and each discount strategy as an arm. We can then assume that each arm only has a significant impact on the sales of those products discounted by this arm (i.e., the cumulative impact on other products is negligible). 
% on some of their products in order to increase their total revenue. In this case, each arm is a promotional discount  
% This would typically only have major impact on the sales of these discounted products.
% Therefore, if we view the revenue generated by each product as a variable, each action of the company only affects a limited number of these variables.

\item \textbf{Online Marketing.}
\label{ex:marketing}
An ecommerce platform can opt among several marketing strategies (actions) to encourage customers to make more purchases on their website.
% This includes for example email campaign, cashback promotion, and influencer marketing.
% \todoygmargin{Maybe this sentence can be removed?}
As different customers can be sensitive to a different marketing strategy, regarding each of them as a variable, it is natural to expect that each action would likely affect only a subset of the variables. 
The payoff associated to a customer can be for example the revenue generated by that customer; then the reward is just the total revenue received by the platform.
%is just the sum of the revenues from all the customers.
%However, one may not know which variables are actually affected. We attempt to address this challenge in \cref{sec:unknown-affected}.
%On the other hand, the platform may want to personalize the campaigns to some targeted audience. This motivates the study of the model introduced in \cref{sec:context}. 

\item\textbf{Product Discount.} 
\label{ex:product}
Consider a company that uses discount strategies to increase their sales. It is common to design discount strategies that only apply to a small subset of products. In this case, we can view the sales of each product as a variable and each discount strategy as an action, and assume that each action only has a significant impact on the sales of those products discounted by this action.
%\todob{"arm" should be an "action". Let's be consistent?}
% on some of their products in order to increase their total revenue. In this case, each arm is a promotional discount  
% This would typically only have major impact on the sales of these discounted products.
% Therefore, if we view the revenue generated by each product as a variable, each action of the company only affects a limited number of these variables.

\item \textbf{Movie Recommendation.}
\label{ex:movie}
Consider a bandit model for movie recommendation where actions correspond to different recommendation algorithms, and the variables are all the movies in the catalog. For each user, define a set of binary payoffs that indicate whether the user watches a movie in the catalog, and the reward is the number of movies from the catalog that this user watches. Since a recommendation (action) for this user contains (promotes) only a subset of movies, it is reasonable to assume that only their associated payoffs are affected by the action.
% A notable difference with the combinatorial bandit model is that we also consider non-recommended movies here.
% In fact, as argued in \citep{WLCB20}, a recommendation is only effective if the user actually watches the movie and would not watch it without the recommendation.

% \item \textbf{Movie Recommendation.}
% \label{ex:movie}
% Let us consider a bandit model for movie recommendation in which actions correspond to different recommendation algorithms and the reward is the number of movies from the catalog that a user watches.
% We define for each user a set of binary payoffs that indicate whether the user watches a movie or not after the recommendation. 
% The reward can then be represented as the sum of these payoffs, and since each recommendation only contains a set of movies, it is reasonable to assume that only the associated payoffs are affected by the recommendation.
% A notable difference with the combinatorial bandit model is that we also consider non-recommended movies here.
% In fact, as argued in \citep{WLCB20}, a recommendation is only effective if the user actually watches the movie and would not watch it without the recommendation.
%The actions represent various recommendation systems. The reward, defined as the sum of these variables, is then the number of watched movies.
%If we assume that the probability of watching a movie changes only if is recommended, each arm only impacts the recommended variables (movies).\footnote{Instead of the watch/no watch binary variables, we can also generalize this setup to include movie ratings.} \todob{No need for the footnote. This is an example and it can be anything that we want.}

% \item \textbf{Movie recommendation.}
% As argued in \citep{WLCB20}, \todob{Use CITET for in-text citations.} a recommendation system should not only recommend movies, but also affect user behavior. A recommendation is only effective if the user actually watches the movie and would not do it otherwise.
% This problem perfectly fits our framework. Fix a user, and define binary variables for whether the user watched a movie in the catalog. The arms represent various recommendation systems. The reward, defined as the sum of these variables, is then the number of watched movies.
% If we assume that the probability of watching a movie changes only if is recommended, each arm only impacts the recommended variables (movies).\footnote{Instead of the watch/no watch binary variables, we can also generalize this setup to include movie ratings.} \todob{No need for the footnote. This is an example and it can be anything that we want.}
\end{enumerate}


\paragraph{Our Contributions.} To begin with, we formalize an \emph{uplifting bandit} model that captures the aforementioned structure.
%in \cref{sec:model}.
%The model is stochastic, that is the payoffs of the variables follow an unknown distribution that depends on the chosen action. 
The term \emph{uplift} is borrowed from the field of {\em uplift modeling}~\citep{radcliffe2007using,gutierrez2017causal} and indicates that the actions' effects are incremental over a certain baseline.
%The term \emph{uplift} refers to the difference between an action's reward and a certain baseline, and is borrowed from the field of {\em uplift modeling}~\citep{radcliffe2007using,gutierrez2017causal}.
%\todoyg{This information on baseline and uplift is necessary here, but I feel the current phrasing is a bit awkward and cannot find a way to improve it.}
We consider a stochastic model, that is, the payoffs of the variables follow an unknown distribution that depends on the chosen action,
and study this problem under various assumptions on the learners' prior knowledge about
    \begin{enumerate*}[\textup(\bf 1\textup)]
    \item \label{a} the baseline payoff of each variable and\item \label{b} the set of affected variables of each action. 
    \end{enumerate*}
    % \todob{It is not clear what "(one)" refers to.}
    % \todoyg{I changed back to what sounds the most natural to me. Feel free to modify it.}
Our first result (\cref{sec:UpUCB-BL}) shows that when both \ref{a} and \ref{b} are known, a simple modification of the \ac{UCB} algorithm~\citep{auer2002using} (Algorithm~\UpUCB) for estimating the uplifts has a much lower regret than its standard implementation. Roughly speaking, when $\nVariables$ is the number of variables and $\nAffected$ is the number of variables affected by each action, we get a $O(\nAffected^2)$ regret bound instead of $O(\nVariables^2)$. 
%This is due to the ``sparsity'' of the actions' effects.
This results in major regret reduction for $\nAffected \ll \nVariables$, and is a distinguishing feature of all our results.
    
%Our main results are 
Going one step further, we design algorithms that have minimax optimal regret bounds without assuming that either~\ref{a} or~\ref{b} is known 
in \cref{sec:known-affected,sec:unknown-affected}.
%We build towards them in \cref{sec:known-affected,sec:unknown-affected}. 
When ~\ref{a} the baseline payoffs are unknown and \ref{b} the affected variables are known, we compute differences of \ac{UCB}s to estimate the uplifts (Algorithm~\UpUCBwb).
In contrast to standard \ac{UCB} methods, these differences are \emph{not} optimistic; this is because the feedback of the actions also reveals important information about the baseline.
%are related through the baseline payoffs.
%and the feedback of action also reveals important information for other actions. 
When ~\ref{b} the affected variables are  %the affected variables are 
also unknown, we identify them on the fly to maintain suitable estimates of the uplifts. We study two approaches, which differ in what they know about the affected variables. Algorithm~\UpUCBLwb knows an upper bound on number of affected variables, whereas Algorithm~\UpUCBDeltawb knows a lower bound on individual uplift. Our regret bounds are summarized in \cref{tab:summary}.
These results are further completed with lower bounds that justify the need for our modeling assumptions (\cref{sec:lower}).
    
    
% We discuss lower bounds and contextual extensions of our model in \cref{sec:lower} and \cref{sec:context}, which justifies the necessity of our modeling assumptions and demonstrates the generality of the model as well as the algorithmic ideas that we develop in the non-contextual setup.
    
%     Below we summarize our main contributions. 
% \begin{enumerate}[wide=0pt]
% \item Our main focus is on  

% The algorithm of \cref{subsec:UpUCB-BL} makes the strong assumptions that the baseline and the sets of affected variables are known.
%     \cref{sec:known-affected} and \cref{sec:unknown-affected} are dedicated to removing these assumptions.
% \end{enumerate}

\input{Tables/Regrets}



% Comparison with other related lines  of work in bandit literature (e.g., causal, combinatorial) is provided in~\cref{apx:related}.
    %such as {\em causal bandits} and {\em combinatorial bandits} is provided in~\cref{apx:related}.

% \begin{enumerate}[wide=0pt]
    % \item In \cref{sec:model}, we formalize an \emph{uplifting bandit} model that captures the problem structure described in the previous examples.
    % We focus on stochastic bandit problems, in which the payoffs of the variables follow a fixed unknown distribution.
    % The term \emph{uplift} refers to the difference between an action's reward and a certain baseline, and is borrowed from the field of uplift modeling~\citep{radcliffe2007using,gutierrez2017causal}.
    %Uplift modeling refers to a collection of techniques for modelling the incremental effect of an action on an individual's behavior.

    %and designs algorithms for that purpose.
    
    % \item Precisely, we show in \cref{subsec:UpUCB-BL} that thanks to the sparsity of the actions' effects, a simple modification of the \ac{UCB} algorithm~\citep{auer2002using} for estimating the uplifts allows us to achieve much smaller regret.
    %improve significantly in the statistical efficiency of the algorithm.
   
    %In a word, this is because the noise in the estimated quantity becomes much smaller in our algorithm.

% \end{enumerate}


% \paragraph{Related Work}

% We borrow the term uplift from {\em uplift modeling} \citep{radcliffe2007using,gutierrez2017causal}; the latter refers to a collection of techniques for modelling the incremental effect of an action on an individual's behavior.
% At a high level, both uplifting modeling and \ac{MAB}  help select the optimal action.
% Despite this apparent relation between the two concepts, few papers explicitly link them together.
% We believe this is because a combination of the two often just results in a redefinition of the reward, on top of which classic bandit algorithms can be applied. This approach was taken in \citet{sawant2018contextual,berrevoets2019optimising}.
% Instead, our paper
% focuses on bandit problems in which estimating the uplifts improves the statistical efficiency of the algorithms and designs algorithms for that purpose.

% To achieve this, we assume the reward to be the sum of a set of observable variables and leverage the \emph{sparsity} of an action's effects on these variables.
% The decomposition of reward and the observability of partial rewards also appear in semi-bandit \citep{CWY13,KWAS15}.
% However, the reward is the sum of the the selected variables there while for us the set of variables is fixed for every action.
% On the other hand, understanding the benefit of sparsity in \ac{MAB} has been a research topic of emerging interest.
% Most of these works focus on sparsity of the parameter vectors in linear bandit, which could be of great interest in the high-dimensional setting, see \eg \citet{abbasi2012online,bastani2020online,hao2021information} and references therein.
% A notable exception is \citet{kwon2017sparse}, where the authors study a variant of the classical \ac{MAB} problem in which the sparsity is reflected by that fact that the number of arms with positive reward is small.
% Our work is orthogonal to all of these in that we look at a different form of sparsity. As we will see in \cref{subsec:contextual-linear}, while sparsity in parameter can be a cause of sparsity in action effect, the improvement of regret is established with a different mechanism.

\paragraph{Organization.} We introduce our uplifting bandit model along with its various variations in~\cref{sec:model}. Over Sections~\ref{sec:UpUCB-BL},~\ref{sec:known-affected},~\ref{sec:unknown-affected}, we provide regret bounds for these variations. Lower bounds and numerical experiments are presented in~\cref{sec:lower} and \cref{sec:exp}.
%In \cref{sec:exp}, we present numerical experiments that confirm the benefit of our approach.
%We discuss contextual extensions  in~\cref{sec:context} and experimental results in~\cref{sec:exp}. 
To demonstrate the generality of our setup and how our algorithmic ideas extend beyond vanilla multi-armed bandits, we further discuss contextual extensions of our model in \cref{sec:context}.
Comparison to related work is deferred to \cref{sec:related}.
% In~\cref{sec:known-affected}, we handle the simplest setting where learner knows the baseline payoffs and the affected variables which we focus on relaxing in the remaining paper. But first our lower bounds in \cref{sec:lower} shows that improvement regret bounds require some assumptions. 


==> Uplifting bandits - arxiv/Sections/Lower-bounds.tex <==
This section presents lower bounds that justify our key modeling assumptions. In particular, we show that there would be a higher regret in absence of any of the following: \begin{enumerate*}[\textup(\itshape i\textup)]
\item Limited number of affected variables,
\item Side information about variables beyond just reward, and
\item Some prior knowledge on how the variables are affected.
\end{enumerate*}
The third point sets ground for \cref{sec:unknown-affected}, by showing that the learner needs some prior knowledge to exploit our problem structure.


%Subsequently, in \cref{subsec:lower-bound-information}, we introduce a general information-theoretic lower bounds for bandit problems with similar design, which serve as the main tool for proving the results in \cref{subsec:lower-bound-uplift}. Missing proofs are in~\cref{apx:lower-bound}.

% \todosk{Throughout the paper, we use "impact/impacted" and also "affect/affected". Are they the same, if so let us use the same words.}
% \todoyg{I think we only use impact as nouns and affect as verbs.}

%\subsection{Lower Bound for Uplifting Bandits}
%\label{subsec:lower-bound-uplift}

% For the sake of conciseness, in the following we say that an uplifting bandit has parameters $(\nArms,\nVariables,(\va[\gapbandit],\va[\nAffected])_{\arm\in\arms})$ if the number of actions, the number of variables, the suboptimality gaps, and the number of affected variables of this instance are respectively $\nArms$, $\nVariables$, $(\va[\gapbandit])_{\arm\in\arms}$, and $(\va[\nAffected])_{\arm\in\arms}$.
%refer to any instance of the uplifting bandit problem as described in \cref{sec:model} with $\nArms$ arms, $\nVariables$ variables, suboptimality gaps $(\va[\gapbandit])_{\arm\in\arms}$, and numbers of affected variables $(\va[\nAffected])_{\arm\in\arms}$ noise as a $1$-sub-Gaussian $(\nArms,\nVariables,(\va[\gapbandit],\va[\nAffected])_{\arm\in\arms})$ uplifting bandit instance.
In particular, these lower bounds show that there would be a higher regret in absence of any of the following: \begin{enumerate*}[\textup(\itshape i\textup)]
\item Limited number of affected variables,
\item Side information about variables beyond just reward, and
\item Some prior knowledge on how the variables are affected.
\end{enumerate*}
Moreover, we also derive matching lower bounds for \cref{prop:UpUCB-BL-regret}.
We discuss these results in \cref{apx:lower-bound-statement}.
Subsequently, we introduce a general information-theoretic lower bounds for bandit problems with similar design in \cref{apx:lower-bound-information}, based on which we prove the lower bounds in \cref{apx:proof-lower-bound}.


We focus on instance-dependent lower-bounds and assume that the learner has full knowledge of the baseline distribution.\footnote{%
Of course, the problem only becomes more challenging if the learner actually does not know the baseline distribution.}
These lower bounds are derived for the algorithms that are {\em consistent} \citep{LR85} over the class of $1$-sub-Gaussian uplifting bandits, which means the induced regret of the algorithm on any uplifting bandit with $1$-sub-Gaussian noise satisfies $\vt[\reg]=\smalloh(\run^p)$ for all $p>0$.
%We refer to such algorithms as {\em consistent algorithms}.
%for any instance of such problem, the induced regret of the algorithm on this instance satisfies $\vt[\reg]=\smalloh(\run^p)$ for all $p>0$.

% \begin{proof}
% The proof is deferred to \cref{apx:lower-bound} is based on the general lower bound \cref{lem:lower-bound-instance-dependent} introduced in \cref{subsec:lower-bound-information}.
% \end{proof}
\begin{proposition}[Informal]
\label{prop:lower-bound}
Let $\policy$ be a consistent algorithm over the class of $1$-sub-Gaussian uplifting bandits.
%that at most uses knowledge of $\va[\distribution][0]$, $(\va[\variables])_{\arm\in\arms}$, and the fact that the noise is $1$-sub-Gaussian.
If 
\begin{enumerate}[(a)]
    \item all the variables are affected by all the actions;
    \label{low-cond:affected}
    \item only the reward is observed; or
    \label{low-cond:observed}
    \item $\policy$ has no knowledge about $(\va[\meanReward])_{\arm\in\arms}$ (in particular, $(\va[\variables])_{\arm\in\arms}$ is not known),
    \label{low-cond:knowledge}
\end{enumerate}
Then, for any $\nArms,\nVariables>0$ and sequence $(\va[\nAffected],\va[\gapbandit])_{1\le\arm\le\nArms}\in(\oneto{\nVariables}\times\R_+)^{\nArms}$
%with $\va[\nAffected]\in\oneto{\nVariables}, \va[\nAffected][1]>\va[\gapbandit]\ge\max(0,\va[\nAffected][1]-\va[\nAffected])$ for all $\arm$ 
with $\va[\gapbandit][1]=0$, there exists a $1$-sub-Gaussian uplifting bandit 
whose number of actions, number of variables, suboptimality gaps, and numbers of affected variables are respectively $\nArms$, $\nVariables$, $(\va[\gapbandit])_{\arm\in\arms}$, and $(\va[\nAffected])_{\arm\in\arms}$,
%with parameters $(\nArms,\nVariables,(\va[\gapbandit],\va[\nAffected])_{\arm\in\arms})$
%a $1$-sub-Gaussian uplifting bandit instance with $\nArms$ arms, $\nVariables$ variables, suboptimality gaps $(\va[\gapbandit])_{\arm\in\arms}$, and numbers of affected variables $(\va[\nAffected])_{\arm\in\arms}$ 
such that the regret induced by $\policy$ on it satisfies
%
\begin{equation}
    %\label{eq:lower-bound-m}
    \notag
    \liminf_{\toinf[\nRuns]} \frac{\ex[\vt[\reg][\nRuns]]}{\log\nRuns} \ge \sum_{\arm\in\arms:\va[\gapbandit]>0}\frac{2\nVariables^2}{\va[\gapbandit]}.
\end{equation}
%
% Now, provided that the payoff vector $\vt[\valuev]$ is observed and that $(\va[\variables])_{\arm\in\arms}$ is known by the algorithm, there exists a $1$-sub-Gaussian uplifting bandit with the same parameters
% %
% \begin{equation}
%     \label{eq:lower-bound-L}
%     \liminf_{\toinf[\nRuns]} \frac{\ex[\vt[\reg][\nRuns]]}{\log\nRuns} \ge \sum_{\arm\in\arms:\va[\gapbandit]>0}\frac{2(\va[\nAffected])^2}{\va[\gapbandit]}.
% \end{equation} 
% \todob{Write ${L^a}^2$ as $(L^a)^2$.}
%
% Moreover, if $\policy$ can be implemented under either of the following conditions
% \begin{enumerate}[(a)]
%     \item Only the reward is observed.
%     \item The learner has no knowledge about $(\va[\meanReward])_{\arm\in\arms}$ (in particular, the learner does not know $(\va[\variables])_{\arm\in\arms}$).
%     %The learner cannot distinguish between any two bandits with the same baseline and noise distributions (in particular, the learner does not know $(\va[\variables])_{\arm\in\arms}$).
%     %The prior knowledge of the learner on the distributions is further restricted to the point that it does not enable the learner to distinguish between any two instances with the same baseline and noise distributions (in particular, the learner does not know $(\va[\variables])_{\arm\in\arms}$).
%     %does not encode any information about the means of the arms
%     %only encodes information about the baseline and the noise distributions.
%     %does not allow the leaner to know anything more than the baseline distribution and the covariance of the noise.
%     %is that the noise is $1$-sub-Gaussian, \ie $\priorknow(\va[\distribution][0],\va[\distribution][1],\ldots,\va[\distribution][\nArms])=\priorknow(\va[\distribution][0],\va[\distributionalt][1],\ldots,\va[\distributionalt][\nArms])$ as long as $\va[\distribution]$'s and $\va[\distributionalt]$'s satisfy \cref{asm:noise}.
%     %The learner has no prior knowledge on how the variables are affected.\footnote{Formally, as we will see in the proof, this means that for a fixed baseline distribution, the prior knowledge of the learner does not allow they to distinguish between two instances whose mean values $(\va[\meanReward])_{\arm\in\arms}$ are arbitrarily different.}
% \end{enumerate}
% Then, there exists a $1$-sub-Gaussian uplifting bandit with parameters $(\nArms,\nVariables,(\va[\gapbandit],\va[\nAffected])_{\arm\in\arms})$ where the regret of $\policy$ is
% \begin{equation}
%     \label{eq:lower-bound-m}
%     \liminf_{\toinf[\nRuns]} \frac{\ex[\vt[\reg][\nRuns]]}{\log\nRuns} \ge \sum_{\arm\in\arms:\va[\gapbandit]>0}\frac{2\nVariables^2}{\va[\gapbandit]}.
% \end{equation}
\end{proposition}
%



The proof of \cref{prop:lower-bound} is deferred to \cref{apx:lower-bound}, where we also present an alternative statement of the proposition that implies the optimality of \cref{prop:UpUCB-BL-regret} and 
%\cref{apx:proof-lower-bound}.
a general information-theoretic lower bound for bandit problems with similar design based on which \cref{prop:lower-bound} is established.
%The key idea is to find a class of bandits that is indistinguishable to the learner under their prior knowledge, and for a specific instance of this class show that each suboptimal action necessarily gets taken a certain number of times because some other instances of the class can provide very similar feedback.
%two instances of this class can provide similar feedback so that each suboptimal arm needs to be pulled a certain number of times 
%\todobmargin{I am not 100\% sold on how the lower bounds are presented. It seems that \eqref{eq:lower-bound-m} should go first, because it shows that the world is hard if nothing is known. \eqref{eq:lower-bound-L} shows that $\Omega(L^2)$ regret is needed under reasonable assumptions, which we match starting with Algorithm 1. The lower should perhaps go even before Section 3.}

%We will consider models with $1$-sub-Gaussian noise and mean values $\vav[\meanReward]\in[0,1]$.
%For ease of presentation, this will not be mentioned explicitly in the problem statements but whenever we mention an uplifting bandit instance one should keep in mind that it is an uplifting bandit instance satisfying these assumptions.

As promised, \cref{prop:lower-bound} justifies the importance of the three crucial components of our model.
The intuition behind the lower bounds under conditions \ref{low-cond:affected} and \ref{low-cond:observed} is that smaller regret can only be achieved when the noise in the effect of an action is small, and when the observation of the learner of this effect is not deteriorated by the noise.
%Finally, Condition (b) in~\cref{prop:lower-bound} along with inequality \eqref{eq:lower-bound-m} indicates that the structure of the problem and the side information can only be exploited when the learner is equipped with some knowledge about $(\va[\meanReward])_{\arm\in\arms}$.
%For example, if the learner knows $(\va[\variables])_{\arm\in\arms}$, they can infer that $\vav[\meanReward]=\vav[\meanReward][0]$ whenever $\indv\notin\va[\variables]$.
To understand the lower bound under condition \ref{low-cond:knowledge}, we notice that with finite observations, two problem instances with different structures (\eg different $(\va[\variables])_{\arm\in\arms}$) can provide arbitrary close information to the learner, and thus the learner is doomed to treat them equally if they are not equipped with any prior knowledge that enables them to distinguish between the two problems.
Accordingly, the learner is not able to take advantage of the underlying structure, and no improvement of the performance can be achieved.
%In this regard, the knowledge on $(\va[\meanReward])_{\arm\in\arms}$ actually allows the learner to distinguish between two such instances and treat them differently, which results in an improvement of the regret.


%First, inequality \eqref{eq:lower-bound-L} shows that the regret of the algorithm must scale with $\va[\nAffected]$, the number of variables each action affects.
%Therefore, no improvement can be achieved if the limited number of affected assumption is violated.
%
%Next, condition (a) along with inequality \eqref{eq:lower-bound-m} reveals the necessity of having additional observations.
%Observing the reward itself is not sufficient for getting rid of the dependence on $\nVariables$.
%The intuition behind these two lower bounds is that smaller regret can only be achieved when the noise in the effect of an action is small, and when the observation of the learner of this effect is not deteriorated by the noise.
%\todosk{we say that we need "additional observations" but that does not imply that all variables be observed, if so should we clarify?}

% Finally, Condition (b) in~\cref{prop:lower-bound} along with inequality \eqref{eq:lower-bound-m} indicates that the structure of the problem and the side information can only be exploited when the learner is equipped with some knowledge about $(\va[\meanReward])_{\arm\in\arms}$.
% For example, if the learner knows $(\va[\variables])_{\arm\in\arms}$, they can infer that $\vav[\meanReward]=\vav[\meanReward][0]$ whenever $\indv\notin\va[\variables]$.
% To see why such knowledge is required, we notice that with finite observations, two problem instances with different structures (\eg different $(\va[\variables])_{\arm\in\arms}$) can provide arbitrary close information to the learner, and thus the learner is doomed to treat them equally. This prevents the learner from taking advantage of the underlying structure of the problem.
% In this regard, the knowledge on $(\va[\meanReward])_{\arm\in\arms}$ actually allows the learner to distinguish between two such instances and treat them differently, which results in an improvement of the regret.
%Further examples of such knowledge are provided in \cref{sec:unknown-affected}.


==> Uplifting bandits - arxiv/Sections/Related.tex <==
In this section, we link our work to other existing bandit models.
To begin, as suggested by the name, the concept of \emph{uplift} plays a crucial role in our approach.
From a high-level perspective, the goals of both uplifting modeling and \ac{MAB} is to help selecting the optimal action.
The former achieves it by modelling the incremental effect of an action on an individual's behavior.
Despite this apparent connection between the two concepts, few papers explicitly link them together.
We believe that this is because the resulting problem can often be solved by classic bandit algorithms with a redefined reward. This approach was taken in \citep{sawant2018contextual,berrevoets2019optimising}.

Instead, our paper focuses on bandit problems in which estimating the uplifts improves the statistical efficiency of the algorithms, and this is possible thanks to the `sparsity' of the actions' effects.
Prior to our work, sparsity assumptions in bandits primarily concerned the sparsity of the parameter vectors in linear bandits, 
which could be of great interest in high-dimensional settings \citep{abbasi2012online,bastani2020online,hao2021information}.
A notable exception is \citet{kwon2017sparse} who studied a variant of the \ac{MAB} where the sparsity is reflected by the fact that the number of arms with positive reward is small.
Our work is orthogonal to all of these in that we look at a different form of sparsity. As we saw in \cref{sec:context}, while sparsity in parameter can be a cause of sparsity in action effect, the improvement of regret is established with a different mechanism.
In the upcoming paragraphs, we further exhibit how our model is related to causal and combinatorial bandits.

\paragraph{Causal Bandits\afterhead}
The term causal bandits captures the general idea that in a bandit model the generation of reward may be governed by some causal mechanism while the actions correspond to interventions on the underlying causal graph.
This idea was first formalized in \citep{lattimore2016causal} and subsequently explored in a series of work \citep{lee2018structural,lu2020regret,nair2021budgeted} that cover multiples variants of the problem, including both the minimization of simple and cumulative regrets.
Our problem fits into the causal bandit framework by regarding \cref{fig:model} as a simple causal graph where the variables consist of all the directed causes of the reward and the actions correspond to atomic interventions on the action nodes.
The observability of these direct causes are also key assumptions in many of the aforementioned works.
Moreover, in the unknown affected case our causal graph is in fact partially unknown.
This is an intriguing problem in causal bandits as argued by \citep{LMT21}.
While we have shown improvement of the algorithms for this specific model, a interesting question is whether similar improvement can still be shown in more general causal bandit models under the assumption that each actions only affects a limited number of variables of the causal graph.

\paragraph{Combinatorial Bandits\afterhead}
In combinatorial bandits~\citep{cesa2012combinatorial}, the learner selects at each round a subset of ground items depending on which the reward is computed.
In its simplest form, the reward is just the sum of the payoffs of the selected items.
Of particular relevance to us is the semi-bandit setting~\citep{CWY13,KWAS15}, which assumes that the payoffs of the selected items are also observed.
This structure of the reward and observability of individual payoffs both suggest a strong similarity between our model and semi-bandits.
However, this comes with an important conceptual difference: the set of items, or variables, for which we observe the outcomes are selected in semi-bandits, while for us they are fixed and inherent to the reward generation mechanism.
As an example, in example \ref{ex:movie}, combinatorial bandit models optimize the number of movies that are watched among the recommended ones, while we also consider non-recommended movies.
In fact, as argued in \citep{WLCB20}, a recommendation is only effective if the user actually watches the movie and would not watch it without the recommendation

On the other hand, mathematically, it is possible to fit our model into the stochastic combinatorial semi-bandit framework when the sets of affected variables are known.
For this, consider a semi-bandit problem with $\nVariables+\sum_{\arm\in\arms}\va[\nAffected]$ items that correspond to the random variables $\setdef{\vav[\valuev][0]}{\indv\in\variables}\union\bigcup_{\arm\in\arms}\setdef{\vav[\valuev]}{\indv\in\va[\variables]}$.
At each round, the learner selects $\nVariables$ items that depends on the taken action and observes the payoffs of the selected items.
More precisely, when action $\arm$ is taken, the selected items are $\setdef{\vav[\valuev][0]}{\indv\in\setcomplement{\va[\variables]}}\union\setdef{\vav[\valuev]}{\indv\in\va[\variables]}$.

In terms of algorithm, let us consider the \UpUCBwb algorithm described in \cref{algo:UpUCB}, which is based on selecting the action with the largest uplift index $\vta[\UPindexSum]=\sum_{\indv\in\va[\variables]}(\vtav[\UCBindex]-\vtav[\UCBindex][\run][0])$.
We notice that the quantity $\vta[\UCBindex]=\sum_{\indv\in\variables}\vtav[\UCBindex]=\vta[\UPindexSum]+\sum_{\indv\in\variables}\vtav[\UCBindex][\run][0]$ is indeed an upper confidence bound on the reward of action $\arm$ and \UpUCBwb is equivalent to choosing the action with the largest $\vta[\UCBindex]$ in each round.
This observation indeed reduces \UpUCBwb to CombUCB~\citep{CWY13,KWAS15} on the transformed model.
Nonetheless, the \UpUCBwb formulation has several advantages:
\begin{enumerate}[topsep=2pt, itemsep=1.5pt, parsep=2pt, leftmargin=*]%[\itshape i\upshape)]
    \item It captures the fact that we really care about is the uplifting effect and the variables affected by each action.
    \item The uplifting interpretation facilitates algorithm design in more involved situations as we have shown in \cref{sec:unknown-affected}.
    \item While the general analysis of CombUCB yields a regret in %$\bigoh((\nVariables+\sqrt{\nVariables\nArms\nAffected})\sqrt{\nRuns\log\nRuns})$ and
    $\bigoh((\nVariables^2+\nVariables\nArms\nAffected)\log\nRuns/\gapbandit)$, we have shown in \cref{thm:UpUCB-regret} that the regret of \UpUCBwb is in $\bigoh(\nAffected^2\log\nRuns/\gapbandit)$.
    Our analysis presented in \cref{apx:proof-UpUCBwb} also greatly benefits from the \UpUCBwb formulation of the algorihhm.
    %clearly indicates that the number of variables $\nVariables$ should have no effect in our regret bound, as we demonstrate immediately in the following theorem.
    %this will be discussed in more detail in the next paragraph. %\cref{subsec:UpUCB-regret}.
\end{enumerate}

==> Uplifting bandits - arxiv/Sections/Unknown-affected.tex <==
Now we study the more challenging setting where the affected variables $(\va[\variables])_{\arm\in\arms}$ are unknown to the learner.
\cref{prop:lower-bound} states that improvement is impossible if the learner does not possess any prior knowledge that allow them to exploit the structure.
%about the structure of the problem.
%on how the payoffs of each action $(\va[\meanReward])_{\arm\in\arms}$ differ from each other, or how they differ from the baseline payoffs $\va[\meanReward][0]$.
To circumvent this negative result, we study two weak assumptions motivated by practice: the learner has either access to \begin{enumerate*}[\textup(\itshape i\textup)]
\item an upper bound on the number of affected variables or
% , for which we show that $\bigoh((\nArms\nAffected^2)\log\nRuns/\gapbandit)$ regret bounds can be achieved, or
\item a lower bound on individual uplift.
\end{enumerate*}
% To streamline the presentation, we only present the first setting here and defer the discussion of the other to~\cref{apx:unknown-affected-2}.
% We primarily focus on the first scenario here, deferring most of the discussion on the second scenario to~\cref{apx:unknown-affected-2}.
% We also briefly discuss another type of knowledge that can be exploited by the learner in the end of the section, while deferring most of the related content to \cref{apx:unknown-affected-2}.


%we will consider two types of knowledge that the learner might be able to exploit to improve the algorithm: an upper bound $\nAffected$ on the number of variables an arm affects (Section~\ref{sec:part1}), or a lower bound $\gapUplift$ on individual uplifting effect (Section~\ref{sec:part2}). Missing proofs are in~\cref{apx:upper-bound}.

%We have previously assumed the set of affected variables $\va[\variables]$ to be known for every $\arm\in\arms$.
%In this section we focus on the situation where this assumption is violated, and show that under suitable assumptions, we still manage to recover similar regret bounds.
%Unless otherwise stated, all of our algorithms 

\subsection{Known Upper Bound on Number of Affected Variables}
\label{sec:part1}
Here we assume that we have a known upper bound on number of affected variables $\nAffected$ (\ie $\nAffected\ge\max_{\arm\in\arms}\va[\nAffected]$). We design algorithms with $\bigoh(\nArms\nAffected^2\log\nRuns/\gapbandit)$ regret bounds
that takes $\nAffected$ as input. We consider the cases of known and unknown baseline payoffs.
% In this first part, we assume an upper bound $\nAffected$ on the number of variables an arm affects is given.

%%% To be added
% \input{Algorithms/UpUCB_L_BL}
\subsubsection{Known Baseline Payoffs}
\label{subsubsec:UpUCB-L-BL}
To illustrate our ideas, we start by assuming that the baseline payoffs are known.
%the baseline payoffs $\va[\meanReward][0]=(\vav[\meanReward][0])_{\allvariables}$ are known.
We propose an optimistic algorithm that maintains a \ac{UCB} on the total uplift with an overestimate in the order of $\nAffected$.
%by identifying the affected variables on the fly and restricting its focus to at most $\nAffected$ variables in each round.
%The main idea of our method is to identify the affected variables on the fly while maintaining a suitable \ac{UCB} on the total uplifting effect even when the affected variables are not yet fully identified.
Let $\vta[\pullcount]$, $\vta[\radiusConf]$, and $\vtav[\est{\meanReward}]$ be defined as in \eqref{eq:mean-estimate-a}.
%but this time for all $\indv\in\variables$.
The UCB, uplifting indices, and the confidence intervals for each (action, variable) pair $(\arm,\indv)\in\arms\times\variables$ are %given by
%
\begin{equation}
    \label{eq:UCBs-arm}
    \begin{aligned}[b]
    \vtav[\UCBindex] &= \vtav[\est{\meanReward}][\run-1] + \vta[\radiusConf][\run-1],~~
    \vtav[\UPindex] = \vtav[\UCBindex]-\vav[\meanReward][0],\\
    \vtav[\intConf]&=[\vtav[\est{\meanReward}][\run-1]-\vta[\radiusConf][\run-1],\,\vtav[\est{\meanReward}][\run-1]+\vta[\radiusConf][\run-1]].
    \end{aligned}
\end{equation} 
%\todob{$\rho^a_t(i)$ needs to be introduced in text.}
%\todob{I would not use $I$ for confidence sets, because many bandit papers use $I$ for pulled arms. What about $\mathcal{C}$?}
%
% To construct a \ac{UCB} of the total uplifting effect $\va[\uplift]=\sum_{\indv\in\va[\variables]}\vav[\meanUplift]$, we make use of the uplifting indices $\vtav[\UPindex]=\vtav[\UCBindex]-\vav[\meanReward][0]$ which provide high-probability upper bounds on the individual uplifting effects $\va[\meanUplift]=(\vav[\meanUplift])_{\allvariables}$.
% The algorithm presented in \needref suggests summing the uplifting indices over $\indv\in\va[\variables]$, but $\va[\variables]$ is no longer known by the learner.
%With the introduction of these two quantities, we state our algorithm, \UpUCBL (in~\cref{apx:missing}), and illustrate how we build an action's uplifting index in \cref{subfig:UpUCBL}.
In the sequel, we refer to $\vtav[\UPindex]$ as the \emph{individual uplifting index} of the pair $(\arm,\indv)$. It serves as an estimate of the individual uplift $\vav[\meanUplift]$.
%$\vta[\UPindexSum]$ that we defined in \cref{subsec:UpUCB-BL}.
Our algorithm, \UpUCBL, leverages two important procedures to compute an optimistic estimate of the uplift %the total uplift 
$\va[\up{\reward}]$: identification of affected variables, and padding with variables with the highest individual uplifting indices. %Specifically, in line 6,

To begin,  in line 6, \UpUCBL constructs the set of \emph{identified variables} 
%$\vta[\setId]= \setdef{\indv\in\variables}{\vav[\meanReward][0]\notin\vtav[\intConf]}$
%
\begin{equation}
    \notag
    \vta[\setId] = \setdef{\indv\in\variables}{\vav[\meanReward][0]\notin\vtav[\intConf]}.
\end{equation}
%
This set is contained in $\va[\variables]$ with high probability.
In fact, by concentration of measure, with high probability $\vav[\meanReward]\in\vtav[\intConf]$, in which case $\vav[\meanReward][0]\notin\vtav[\intConf]$ indicates $\indv\in\va[\variables]$.
However, $\vta[\setId]$ is not guaranteed to capture all the affected variables, so
%this is not sufficient because to maintain a \ac{UCB} on the total uplifting effect $\va[\uplift]=\sum_{\indv\in\va[\variables]}\vav[\meanUplift]$, we need to account for the identified variables as well as the non-identified ones.
%Under the condition $\vta[\setId]\subseteq\va[\variables]$, it remains to 
we also need to provide an upper bound for $\sum_{\indv\in\setexclude{\va[\variables]}{\vta[\setId]}}\vav[\meanUplift]$, the uplift contributed by the unidentified affected variables.
Since the individual uplifting index $\vtav[\UPindex]$ is in fact a \ac{UCB} on the individual uplift $\vav[\meanUplift]$ here and $\card(\va[\variables])\le\nAffected$, we can simply choose the $\nAffected-\card(\vta[\setId])$ variables in $\setexclude{\variables}{\vta[\setId]}$ with the largest individual uplifting index $\vtav[\UPindex]$, as done in line 8 of \cref{algo:UpUCB-L-BL}.
%individual uplifting indices $\vtav[\UPindex]$. 
We refer to this set as $\vta[\setLargeUp]$.
We then get a proper \ac{UCB} on the uplift of action $\arm$ by computing $\vta[\UPindexSum]=\sum_{\indv\in\vta[\setId]\union\vta[\setLargeUp]}\vtav[\UPindex]$ in line 9.
This process is summarized in \cref{algo:UpUCB-L-BL} and illustrated in \cref{subfig:UpUCBL}.

%By combining these, we get a proper \ac{UCB} on the uplift of action $\arm$ (Line 9).

%We notice that while directly choosing the $\nAffected$ variables with the highest uplifting indices also yields a \ac{UCB} of the arm's uplifting, it may overestimate too much the true uplifting effect in the presence of negative lift 


%that the identification step is important because individual uplift can be negative, in which case choosing the $\nAffected$ variables with the highest $\vtav[\UPindex]$ would overestimate the uplift significantly.
%egret in \cref{thm:UpUCB-L-BL-regret} is comparable to \cref{prop:UpUCB-BL-regret} when $\nAffected \approx \va[\nAffected]$ holds for most $\arm\in\arms$. 
%It is also straightforward to adapt \UpUCBL and its analysis to the setting where the learner knows an action-dependent upper bound $\overline{\va[\nAffected]}\ge\va[\nAffected]$. The only change in \eqref{eq:UpUCB-L-BL-regret} is that $\nAffected$ is replaced by $\overline{\va[\nAffected]}$. Thus we recover \eqref{eq:UpUCB-BL-regret} up to a multiplicative constant when $\overline{\va[\nAffected]}=\Theta(\va[\nAffected])$.
%Finally, we would like to highlight that the identification step is important because individual uplift can be negative, in which case choosing the $\nAffected$ variables with the highest $\vtav[\UPindex]$ would overestimate the uplift significantly.

% This in turns translates into lower regret, as testified by the following theorem.

% It is thus sufficient to construct an upper bound on $\sum_{\indv\in\setexclude{\va[\variables]}{\vta[\setId]}}\vav[\UPindex]$, which can be done leveraging the knowledge of $\nAffected$.
% Let us define
%This procedure can be largely improved with . In fact, to get an upper bound we just need to focus on the $\nAffected$ variables with the largest uplifting indices. Taking into account the fact that some of the affected variables have already been identified, we set
%
%However, we also need to maintain a \ac{UCB} on the uplifting effect $\va[\uplift]=\sum_{\indv\in\va[\variables]}(\vav[\meanReward]-\vav[\meanReward][0])$ even if all the affected variables have not been identified.
%since we never know whether we have identified all the affected variables or not if $\va[\nAffected]<\nAffected$, we also need to maintain an upper confidence
%This is where the knowledge of $\nAffected$ comes into play.
%The knowledge of $\nAffected$ can then help us ensure that the deviation is only in the order of $\nAffected$.
% Let $\vtav[\UPindex]=\vtav[\UCBindex]-\vav[\meanReward][0]$.
% Assume that we have effectively $\vta[\setId]\subseteq\va[\variables]$ and $\vtav[\UPindex]\ge\vav[\meanReward]-\vav[\meanReward][0]$.
% We can then write
% %
% \begin{equation}
%     \notag
%     \begin{aligned}
%     \sum_{\indv\in\va[\variables]}(\vav[\meanReward]-\vav[\meanReward][0])
%     &\le
%     \sum_{\indv\in\va[\variables]}\vtav[\UPindex]\\
%     &=
%     \sum_{\indv\in\vta[\setId]}\vtav[\UPindex]
%     + \sum_{\indv\in\setexclude{\va[\variables]}{\vta[\setId]}}\vtav[\UPindex]\\
%     &\le
%     \sum_{\indv\in\vta[\setId]}\vtav[\UPindex]
%     + \max_{\substack{\setLargeUp\subseteq\setexclude{\variables}{\vta[\setId]}
%     \\\card(\setLargeUp)=\nAffected-\card(\vta[\setId])}}
%     \sum_{\indv\in\setLargeUp}\vtav[\UPindex].
%     \end{aligned}
% \end{equation}
% %
% In the last line, we use the fact that $\vtav[\UPindex]\ge0$ for all $\indv\notin\vta[\setId]$ and the inequality $\card(\setexclude{\va[\variables]}{\vta[\setId]})\le\nAffected-\card(\vta[\setId])$.
% The above gives a valid \ac{UCB} of the uplifting effect of $\arm$.
% Let
%
% \begin{equation}
%     \notag
%     \vta[\setLargeUp]
%     =
%     \argmax_{\substack{\setLargeUp\subseteq\setexclude{\variables}{\vta[\setId]}
%     \\\card(\setLargeUp)=\nAffected-\card(\vta[\setId])}}
%     \sum_{\indv\in\setLargeUp}\vtav[\UPindex]
% \end{equation}
% %
% as the the set of the $\nAffected-\card(\vta[\setId])$ variables in $\setexclude{\variables}{\vta[\setId]}$ with largest $\vtav[\UPindex]$.
% Summing over $\vta[\setLargeUp]$ indeed gives an upper bound on $\sum_{\indv\in\setexclude{\va[\variables]}{\vta[\setId]}}\vav[\UPindex]$ since $\card(\va[\variables])\le\nAffected$, and if $\indv\subseteq\setexclude{\variables}{\vta[\setId]}$ then $\vtav[\UPindex]\ge0$ so adding more terms only makes it larger.


% \todob{This is an informal justification of the algorithm. It is optimistic, since $\rho_t^a(i)$ is a proper UCB on the lift of arm $a$ in variable $i$. To guarantee that our statistical efficiency scales with $L$ and not $m$, we need to choose up to $L$ variables to act upon in each round. This is done as follows:

% 1) In line 6, we choose variables that are guaranteed to be in $V^a$.

% 2) In line 8, we pad these with the variables with the highest UCBs.

% 3) In line 12, the combination of 1) and 2) yields a proper UCB on the lift of arm $a$.

% Additionally, after arm $a$ is pulled, all estimates $\rho_t^a(i)$ tighten. This is critical to the analysis, because we improve in all variables no matter which variables we acted upon.

% The following structures are used in the proof:

% 1) All decisions are made on uncertain estimates of at most $L$ variables. This is why our statistical efficiency scales with $L$ and not $m$.

% 2) Since the baseline effect is certain, there are no baseline CI widths to hide.}

%In summary, we can now define the uplifting index of arm $\arm$ in round $\run$ as $\vta[\UPindex]=\sum_{\indv\in\vta[\setId]\union\vta[\setLargeUp]}\vtav[\UPindex]$.
%The proposed algorithm, \UpUCBL with known baseline payoffs (\cref{algo:UpUCB-L-BL}),
%follows the general schema of choosing the arm with the largest uplifting index, and enjoys the following regret guarantee

% \begin{restatable}{theorem}{UpUCBLBRegret}
% \label{thm:UpUCB-L-BL-regret}
% Let $\alt{\smallproba}=\smallproba/(2\nArms\nVariables\nRuns)$. If the learner knows  and an upper bound $\nAffected$ on maximum number of variables an action affects and the baseline payoffs, then \UpUCBL, with probability at least $1-\smallproba$, has regret bounded by:
% %
% \begin{gather}
%     \label{eq:UpUCB-L-BL-regret}
%     \vt[\reg][\nRuns] \le
%     \sum_{\arm\in\arms:\va[\gapbandit]>0}
%     \left(\frac{32\nAffected^2\log(2\nArms\nVariables\nRuns/ \smallproba)}{\va[\gapbandit]}+\va[\gapbandit]\right).
%     \raisetag{0.75em}
% \end{gather}
% \end{restatable}

%%%To be added
% \begin{restatable}{theorem}{UpUCBLBRegret}
% \label{thm:UpUCB-L-BL-regret}
% Let $\alt{\smallproba}=\smallproba/(2\nArms\nVariables\nRuns)$. Then the regret of \UpUCBL (\cref{algo:UpUCB-L-BL}), with probability at least $1-\smallproba$, satisfies:
% %
% \begin{gather}
%     \label{eq:UpUCB-L-BL-regret}
%     \vt[\reg][\nRuns] \le
%     \sum_{\arm\in\arms:\va[\gapbandit]>0}
%     \left(\frac{32\nAffected^2\log(2\nArms\nVariables\nRuns/ \smallproba)}{\va[\gapbandit]}+\va[\gapbandit]\right).
%     \raisetag{0.75em}
% \end{gather}
% \end{restatable}

%An important step for proving \cref{thm:UpUCB-L-BL-regret} is to show that $\vta[\UPindexSum]$ does not overestimate the uplift too much.
%This is the case in particular because by construction if $\indv\notin\vta[\setId]$ then $\vav[\meanReward]$ should not differ too much from $\vav[\meanReward][0]$, which guarantees the overestimates contributed by the variables that we add in the padding step is also small.
%In contrast, if we chose the $\nAffected$ variables with the highest $\vtav[\UPindex]$, we could overestimate the uplift significantly when the individual uplift $\vav[\up{\meanReward}]$ is negative for some $\indv$.

%We explained before that $\vta[\UPindexSum]$ in line 9 is a \ac{UCB} of the actual lift. To see why it does not overestimate the lift too much, we observe that by the definition of $\vta[\setId]$, if $\indv\notin\vta[\setId]$ then $\vav[\meanReward]$ should not differ too much from $\vav[\meanReward][0]$, and thus even if the variables chosen in the padding step do not belong to $\va[\variables]$ the overestimate is still small. \todob{Simplify the sentence.} In contrast, if we chose the $\nAffected$ variables with the highest $\vtav[\UPindex]$, we could overestimate the uplift significantly when the uplifting effect $\vav[\up{\meanReward}]$ is negative for some $\indv$.

%The fact that this sum does not overestimate too much the target quantity is ensured by the definition of $\vta[\setId]$, which implies that if $\indv\notin\vta[\setId]$ then $\vav[\meanReward]$ should not differ too much from $\vav[\meanReward][0]$.

% %
% \textcolor{blue}{YG Rewrite: The $\bigoh(\nArms\nAffected^2\log\nRuns/\gapbandit)$ regret in \cref{thm:UpUCB-L-BL-regret} is comparable to \cref{prop:UpUCB-BL-regret} when $\nAffected \approx \va[\nAffected]$ holds for most $\arm\in\arms$. 
% It is also straightforward to adapt \UpUCBL and its analysis to the setting where the learner knows an action-dependent upper bound $\overline{\va[\nAffected]}\ge\va[\nAffected]$. The only change in \eqref{eq:UpUCB-L-BL-regret} is that $\nAffected$ is replaced by $\overline{\va[\nAffected]}$. Thus we recover \eqref{eq:UpUCB-BL-regret} up to a multiplicative constant when $\overline{\va[\nAffected]}=\Theta(\va[\nAffected])$.
% Finally, we would like to highlight that the identification step is important because individual uplift can be negative, in which case choosing the $\nAffected$ variables with the highest $\vtav[\UPindex]$ would overestimate the uplift significantly.}

\subsubsection{Unknown Baseline Payoffs}
Now we focus on the most challenging setting, where also the baseline payoffs are unknown.
%The challenge over \cref{algo:UpUCB-L-BL} is that the baseline effect is unknown, so 
In this case, neither the sets of identified variables nor the uplifting indices of \UpUCBL can be defined.
We also cannot estimate the baseline payoffs using \eqref{eq:mean-estimate-0} since the sets of affected variables are unknown.
%To guarantee that our statistical efficiency scales with $L$ and not $m$, we need to choose up to $O(L)$ variables to act upon in each round.
%\todosk{change the term `baseline action' to something else throughout, to prevent confusion with baseline payoff.}
To overcome these challenges, we note that for any two actions $\arm,\armalt\in\arms$, $\va[\meanReward][\arm]$ and $\va[\meanReward][\armalt]$ only differ on $\va[\variables]\union\va[\variables][\armalt]$, and 
$\card(\va[\variables]\union\va[\variables][\armalt])\le2\nAffected$.
%differ in at most $\va[\nAffected]+\va[\nAffected][\armalt]\le2\nAffected$ variables
Therefore, $\va[\meanReward][\arm]$ and $\va[\meanReward][\armalt]$ differ in at most $2\nAffected$ variables, and we recover a similar problem structure by taking the payoffs of any action as the baseline.

Combining this idea with the elements that we have introduced previously,
%in \UpUCBwb and \UpUCBL, 
we obtain \UpUCBLwb (\cref{algo:UpUCB-L}).
In each round, \UpUCBLwb starts by picking a most frequently taken action $\vt[\mostpullarm]$ (Line 4) whose payoffs are treated as the baseline during this round.
%associated estimates are used to estimate the uplifts of all the actions during this round.
Then, in Line 6, \UpUCBLwb chooses variables that are guaranteed to be either in $\va[\variables]$ or $\va[\variables][\vt[\mostpullarm]]$. 
This generalizes the identification step of \UpUCBL.
%This generalizes line 6 in \cref{algo:UpUCB-L-BL}.
The individual uplifting indices $\vtav[\UPindex]=\vtav[\UCBindex]-\vtav[\UCBindex][\run][\vt[\mostpullarm]]$ are computed in Line 7. The definition as differences of \ac{UCB}s is inspired by similar construction in \UpUCBwb.
%resembles line 5 in \cref{algo:UpUCB}.
Lines 8 and 9 constitute the padding step, during which variables with the highest uplifting indices are selected, and finally in Line 10 we combine the above to get the uplifting index of the action.
%These generalize lines 7 to 9 in \cref{algo:UpUCB-L-BL}.
%
%
% We summarize the important steps below:
% \begin{enumerate}
%     \item In line 4, we fix a baseline action $\vt[\mostpullarm]$ and use it to estimate the uplifting effects of all the actions.
%     \item In line 7, we choose variables that are guaranteed to be either in $\va[\variables]$ or $\va[\variables][\vt[\mostpullarm]]$. This generalizes line 6 in \cref{algo:UpUCB-L-BL}.
%     \item In line 8, we compute the uplifting indices as a difference of \ac{UCB}s
%     \[\vtav[\UPindex]=\vtav[\UCBindex]-\vtav[\UCBindex][\run][\vt[\mostpullarm]].\]
%     This is similar to line 5 in \cref{algo:UpUCB}. \todob{Line 9 is not explained. Without this, the next line does not make sense.}
%     \item In line 10, we pad these with variables with the highest uplifting indices. This generalizes line 8 in \cref{algo:UpUCB-L-BL}.
%     \item In line 11, we combine 2. and 4. to compute the uplifting index.
%     This is a generalization of line 9 in \cref{algo:UpUCB-L-BL}.
% \end{enumerate} \todob{Consolidate in a paragraph, similarly to what I have done before.}
%

The similarity between \UpUCBLwb and \UpUCBL can be shown by supposing that one action has been taken frequently. Then the baseline payoffs are precisely estimated and do not change much between consecutive rounds.
% Therefore, we may use the estimates of any arm as a baseline, as long as these estimates are good enough.
% A natural choice is then to use the arm that has been pulled the most number of times.\footnote{If there are multiple, we just pick one at random.}
% This leads to \cref{algo:UpUCB-L}.
% As in \cref{algo:UpUCB}, the uplifting index is computed as the difference of two \ac{UCB}s (Line 6).
% Moreover, $\vta[\setId]$ is now constructed by looking at the confidence intervals of the arm in question and the arm that serves as the reference at each round.

\subsubsection{Regret Bounds}
Both \UpUCBL and \UpUCBLwb choose $\bigoh(\nAffected)$ variables for estimating the uplift of an action, and the decisions are made based on these estimates.
Therefore, the statistical efficiencies of these algorithms only scale with $\nAffected$ and not $\nVariables$.
This in turn translates into an improvement of the regret, as demonstrated by the theorem below.

% Provided \UpUCBL chooses up to $\nAffected$ variables for estimating the uplifts of the actions, we can again show that the statistical efficiency only scales with $\nAffected$ and the regret is in $\bigoh(\nArms\nAffected^2\log\nRuns/\gapbandit)$.
% While we defer the formal statement and its proof to \cref{apx:upper-bound-unknown-affected}, we would like to highlight this result would not be possible without the identification step.
% In fact, choosing directly the $\nAffected$ variables with the highest $\vtav[\UPindex]$ would overestimate the uplift too much in the presence of negative individual uplift.
% Moreover, it is also straight forward to adapt our algorithm and analysis to the case where instead of $\nAffected$ we indeed have an action-dependent upper bound $\overline{\va[\nAffected]}\ge\va[\nAffected]$.

% Since all decisions are made on uncertain estimates of at most $2\nAffected$ variables, we again expect the regret of the algorithm to scale with $\nAffected$ and not $\nVariables$.
% This is shown in the following theorem.
%In the following theorem, we state a $\bigoh(\nArms\nAffected^2\log\nRuns/\gapbandit)$ regret bound for \UpUCBLwb.
%, which is again in $\bigoh((\nArms\nAffected^2)\log\nRuns/\gapbandit)$.

\input{Algorithms/UpUCB_L_BL}
\input{Algorithms/UpUCB_L_WB}

% \begin{restatable}{theorem}{UpUCBLWBRegret}
% \label{thm:UpUCB-L-regret}
% %maximum number of affected variables
% Let $\alt{\smallproba}=\smallproba/(2\nArms\nVariables\nRuns)$. If the learner knows an upper bound $\nAffected$ on maximum number of variables an action affects, then \UpUCBLwb, with probability at least $1-\smallproba$ has regret bounded by:
% %
% \begin{equation}
%     \label{eq:UpUCB-L-regret}
%     \vt[\reg][\nRuns] \le
%     \sum_{\arm\in\arms:\va[\gapbandit]>0}
%     \left(\frac{512\nAffected^2\log(2\nArms\nVariables\nRuns/\smallproba)}{\va[\gapbandit]}+\va[\gapbandit]\right).
% \end{equation}
% \end{restatable}

\vspace{0.4em}
\begin{restatable}{theorem}{UpUCBLWBRegret}
\label{thm:UpUCB-L-regret}
%maximum number of affected variables
Let $\alt{\smallproba}=\smallproba/(2\nArms\nVariables\nRuns)$. Then the regret of \UpUCBL (\cref{algo:UpUCB-L-BL}) (resp.\ \UpUCBLwb, \cref{algo:UpUCB-L}), with probability at least $1-\smallproba$, satisfies:
%(\cref{algo:UpUCB-L-BL}, \cref{apx:missing})
% (resp.\ , \cref{algo:UpUCB-L}), 
%
\begin{equation}
    \label{eq:UpUCB-L-regret-main}
    \vt[\reg][\nRuns] \le
    \sum_{\arm\in\arms:\va[\gapbandit]>0}
    \left(\frac{\alpha\nAffected^2\log(2\nArms\nVariables\nRuns/\smallproba)}{\va[\gapbandit]}+\va[\gapbandit]\right),
\end{equation}
%
where $\alpha=32$ (resp.\ $512$) in the above inequality.
%for \UpUCBL and $\alpha=512$ for \UpUCBLwb.
\end{restatable}
\vspace{-0.3em}

The proof of \cref{thm:UpUCB-L-regret} (\cref{apx:upper-bound-unknown-affected}) is notable for two reasons.
First, tracking of the identified variables guarantees that the uplifting index $\vta[\UPindexSum]$ does not overestimate the uplift $\va[\uplift]$ much.
Take \UpUCBL as an example.
An alternative to constructing a \ac{UCB} on $\va[\uplift]$ is to choose the $\nAffected$ variables with the highest individual uplifting indices $\vtav[\UPindex]$.
However, this would result in a severe overestimate when a negative individual uplift is present.
Second, to prove \eqref{eq:UpUCB-L-regret-main} for \UpUCBLwb, we use that the widths of confidence intervals of the chosen $\vt[\mostpullarm]$ are always smaller than those of the taken action. This is ensured by taking $\vt[\mostpullarm]$ as the most frequent action (Line 4 in \cref{algo:UpUCB-L}). 
%In fact, the same idea could be applied in \UpUCBwb. This however yields worse performance because the estimates of the baseline payoffs worsen. We confirm this in experiments, which show a larger discrepancy between \UpUCBL and \UpUCBLwb, though both have $\bigoh(\nArms\nAffected^2\log\nRuns/\gapbandit)$ regret bounds. 

%The $\bigoh(\nArms\nAffected^2\log\nRuns/\gapbandit)$ regret in \cref{thm:UpUCB-L-regret} is comparable to \cref{prop:UpUCB-BL-regret} when $\nAffected \approx \va[\nAffected]$ holds for most $\arm\in\arms$. 
% It is also straightforward to adapt \UpUCBL and its analysis to the setting where the learner knows an action-dependent upper bound $\overline{\va[\nAffected]}\ge\va[\nAffected]$. The only change in \eqref{eq:UpUCB-L-BL-regret} is that $\nAffected$ is replaced by $\overline{\va[\nAffected]}$. Thus we recover \eqref{eq:UpUCB-BL-regret} up to a multiplicative constant when $\overline{\va[\nAffected]}=\Theta(\va[\nAffected])$.
% Finally, we would like to highlight that the identification step is important because individual uplift can be negative, in which case choosing the $\nAffected$ variables with the highest $\vtav[\UPindex]$ would overestimate the uplift significantly.}

%
% In addition to reusing ideas from \cref{thm:UpUCB-regret,thm:UpUCB-L-BL-regret}, an important new trick is that the widths of the confidence intervals of the chosen $\vt[\mostpullarm]$ are always smaller than those of the taken action. This is ensured because $\vt[\mostpullarm]$ is the most frequently taken action (Line 4). In fact, the same idea could be applied in \UpUCBwb. However, this yields worse performance because the baseline payoffs estimate worsen. We confirm this in experiments, which show a larger discrepancy between \UpUCBL and \UpUCBLwb, though both have $\bigoh(\nArms\nAffected^2\log\nRuns/\gapbandit)$ regret bounds.
%In terms of regret bound, the upper bound $\nAffected$ would appear in every single term of the summation in \eqref{eq:UpUCB-regret}.

% \todob{This is an informal justification of the algorithm. The challenge over Algorithm 2 is that the baseline effect is unknown. To guarantee that our statistical efficiency scales with $L$ and not $m$, we need to choose up to $O(L)$ variables to act upon in each round. This is done as follows:

% 1) The baseline is fixed within the round. Its choice does not matter as long as it is the same for all arms and affects at most $L$ variables. Let this baseline be $b$.

% 2) In line 7, we choose variables that are guaranteed to be either in $V^a$ or $V^b$. This is a generalization of line 6 in Algorithm 2.

% 2) In line 9, we pad these with variables with the highest UCBs. This is a generalization of line 8 in Algorithm 2.

% 3) In line 13, we combine 1) and 2). This is a generalization of line 12 in Algorithm 2.

% To see that Algorithm 3 is similar to Algorithm 2, think of one arm being pulled very often. Then the baseline is good and does not change much between consecutive rounds.

% The following structures are used in the proof:

% 1) All decisions are made on uncertain estimates of at most $2 L$ variables. This is why our statistical efficiency scales with $L$ and not $m$.

% 2) For any arm $a$, the CI widths of baseline estimates are lower than those of $a$. This is why the baseline is the most pulled arm and we can hide its CI widths in those of $a$. Would the same trick work in Algorithm 1? This would unify the presentation of Algorithms 1 and 3.}

%The regret in \cref{thm:UpUCB-L-regret} is only larger than \cref{thm:UpUCB-L-BL-regret} by a multiplicative constant. Therefore, when only a uniform bound on the number of affected variables is known



%\subsection{Known Lower Bound on Individual Uplifting Effect} \label{sec:part2}

% \input{Algorithms/UpUCB_GapUp_BL}

% \subsection{Known Lower Bound on Individual Uplift}
% \label{sec:part2}
% Another type of knowledge that can help the learner exploit the structure is a lower bound on individual uplift.
% This is defined as $\gapUplift>0$ such that for all $\arm\in\arms$ and $\indv\in\va[\variables]$, $\abs{\vav[\meanReward]-\vav[\meanReward][0]}\ge\gapUplift$.
% Similar assumption were made by \citet{LMT21} to identify which node in the causal graph affects the reward variable.
% Indeed, this gives us an indicator on how many times we need to take each action in order to identify all its affected variables.

% Again in this scenario, we derive regret bounds for both when the baseline payoffs are known or not to the learner. 
% Our algorithms combine UCB, successive elimination \citep{even2006action}, and the idea that the affected variables can be identified after an action is taken sufficiently many times.
% Our regret bounds feature the ratio $\va[\gapbandit]/\gapUplift$, suggesting that this knowledge is helpful when $\gapUplift$ is relatively large. 
% We defer details to~\cref{apx:unknown-affected-2}.
%\todosk{Yu-Guan to add a line about regret bounds here.}

% Hereinafter, for any $x,\alpha,\beta\in\R$ with $\alpha\le\beta$, we use $\clip(x,\alpha,\beta)$ to denote the clipping function that restricts $x$ to the interval $[\alpha,\beta]$, \ie $\clip(x,\alpha,\beta)=\max(\alpha,\min(\beta,x))$.

% \textbf{Known Baseline Payoffs\afterhead}
% Similar to before, if the baseline payoffs $\va[\meanReward][0]=\vav[\meanReward][0]_{\allvariables}$ are known, we can directly check whether $\vav[\meanReward][0]$ is in the confidence interval.
% Moreover, with the knowledge $\abs{\vav[\meanReward]-\vav[\meanReward][0]}\ge\gapUplift$ for all $\indv\in\va[\variables]$, we deduce that $\va[\variables]$ can be identified correctly with probability $1-2\nVariables\alt{\smallproba}$ after $\pullcount_0=\ceil{(8/\gapUplift^2)\log(1/\alt{\smallproba})}$ pulls of arm $\arm$.
% In fact, let $\vta[\valuev][1],\ldots,\vta[\valuev][\pullcount_0]$ be $\pullcount_0$ i.i.d. realizations of $\va[\valuev]\sim\va[\distribution]$ and $\vtav[\tilde{\meanReward}][\pullcount_0]=(\sum_{\run=1}^{\pullcount_0}\vtav[\valuev])/\pullcount_0$ be the empirical mean of variable $\indv$.
% %Choosing $\varepsilon\in(0,\gapUplift)$ such that $\pullcount_0=(8/(\gapUplift-\varepsilon)^2)\log(1/\alt{\smallproba})$.\footnote{Such $\varepsilon$ exists (and of course, is unique) because $\pullcount_0>(8/\gapUplift^2)\log(2\nVariables/\alt{\smallproba})$.}
% Applying the sub-Gaussian concentration inequality \eqref{eq:sub-Gaussian-concentration} gives
% %
% \begin{equation}
%     \prob\left(\abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward]}\ge\frac{\gapUplift}{2}\right)
%     \le2
%     \exp\left(-\frac{\pullcount_0\gapUplift^2}{8}\right)=2\alt{\smallproba}.
%     %\frac{\alt{\smallproba}}{\nVariables}.
% \end{equation}
% %
% With a union bound we conclude that with probability at least $1-2\nVariables\alt{\smallproba}$ it holds for all $\indv$ that $\abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward]}<\gapUplift/2$.
% We distinguish between the following two situations
% %
% \begin{enumerate}
%     \item $\indv\in\va[\variables]$, then $\displaystyle \abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward][0]}\ge\abs{\vav[\meanReward]-\vav[\meanReward][0]}-\abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward]}>\gapUplift-\frac{\gapUplift}{2}=\frac{\gapUplift}{2}$.
%     \item $\indv\notin\va[\variables]$, then $\displaystyle \abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward][0]}=\abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward]}<\frac{\gapUplift}{2}$.
% \end{enumerate}
% %
% This implies that with the choice
% $\va[\setId] = \setdef{\indv\in\variables}{\abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward][0]}>\gapUplift/2}$, we have effectively $\prob(\va[\setId]=\va[\variables])\ge1-2\nVariables\alt{\smallproba}$.
% One natural algorithm is to thus first pull each arm $\pullcount_0$ times and run \UpUCB (from~\cref{subsec:UpUCB-BL}) in the remaining rounds by regarding $\va[\setId]$ as the variables that action $\arm$ affects.
% The regret of this algorithm is in
% $\bigoh(\sum_{\arm\in\arms,\va[\gapbandit]>0}(\va[\gapbandit]/\va[\gapUplift]+\va[\nAffected])^2\log\nRuns/\va[\gapbandit])$.
% %$\bigoh(\pullcount_0\sum_{\arm\in\arms}\va[\gapbandit]+(\nArms\nAffected^2)\log\nRuns/\gapbandit)$.

% However, $\pullcount_0$ can be arbitrarily large when $\gapUplift$ is closer to $0$, and playing an arm much fewer times is probably sufficient to deduce that arm is not optimal (with high probability).
% We thus propose to implement the above idea in a more flexible manner:
% We run \UpUCB with the uplifting indices $\vta[\UPindex]=\sum_{\indv\in\vta[\setId]}(\vtav[\UCBindex]-\vav[\meanReward][0])$, where
% %
% \begin{equation}
%     \notag
%     \vta[\setId] =
%     \begin{cases}
%     \variables & \text{if} ~ \vta[\pullcount]<\pullcount_0,\\
%     \setdef{\indv\in\variables}{\abs{\vtav[\est{\meanReward}][\run][\vt[\arm]]-\vav[\meanReward][0]}>\gapUplift/2} & \text{otherwise}.
%     \end{cases}
% \end{equation}
% %
% %known baseline payoffs by assuming that all the actions affect all the variables.
% %Then, for each arm $\arm$, as long as its pull count exceeds $\pullcount_0$, we switch the index by considering $\va[\setId]$ as the affected set.
% This algorithm is summarized in \cref{algo:UpUCB-GapUp-BL} and has the following regret guarantee.


% \begin{theorem}
% \label{thm:UpUCB-GapUp-BL-regret}
% Let $\alt{\smallproba}=\smallproba/(2\nArms\nVariables\nRuns)$. If the learner, knows a lower bound $\gapUplift$ on uplifting effect and the baseline distribution, then \UpUCBDelta, 
% with probability at least $1-\smallproba$, has regret bounded by:
% %
% \begin{equation}
%     \label{eq:UpUCB-GapUp-BL-regret}
%     \vt[\reg][\nRuns] \le
%     \sum_{\arm\in\arms,\va[\gapbandit]>0}
%     \left(\frac{8\thinspace\clip(\va[\gapbandit]/\gapUplift,\va[\nAffected],\nVariables)^2\log(2\nArms\nVariables\nRuns/\smallproba)}{\va[\gapbandit]}+\va[\gapbandit]\right).
% \end{equation}
% \end{theorem}

% \cref{thm:UpUCB-GapUp-BL-regret} shows that \cref{algo:UpUCB-GapUp-BL} provides a smooth transition between vanilla UCB and the strategy that identifies the affected variables of all the arms.
% When $\va[\gapbandit]/\gapUplift\ge\nVariables$, the loss of pulling arm $\arm$ is so large that UCB prevents it from being pulled being pulled further even if $\vta[\pullcount]\le\pullcount_0$.
% Otherwise, the affected variables get identified after sufficient pulls of an arm and the algorithm benefits from this knowledge to improve the estimate of the uplifting effect.
% It is also quite straightforward to combine \cref{algo:UpUCB-L-BL} with \cref{algo:UpUCB-GapUp-BL} when both $\nAffected$ and $\gapUplift$ are known; this results in a regret bound that replaces $\clip(\va[\gapbandit]/\gapUplift,\va[\nAffected],\nVariables)$ by $\clip(\va[\gapbandit]/\gapUplift,\va[\nAffected],\nAffected)$ in \eqref{eq:UpUCB-GapUp-BL-regret}.

\subsection{Known Lower Bound on Individual Uplift}
\label{sec:part2}
In this second part of this section, we assume a lower bound on individual uplift is known.
This means the learner has access to $\gapUplift>0$ satisfying that for all $\arm\in\arms$ and $\indv\in\va[\variables]$, $\abs{\vav[\meanReward]-\vav[\meanReward][0]}\ge\gapUplift$.
This gives us an indicator on how many times we need to take each action in order to identify all the affected variables. Similar assumption was made by \citet{LMT21} to identify which node in the causal graph affects the reward variable.

Again in this scenario, we derive regret bounds for both when the baseline payoffs are known or not to the learner. 
Our algorithms combine UCB, successive elimination \citep{even2006action}, and the idea that the affected variables can be identified after an action is taken sufficiently many times.
Our regret bounds feature the ratio $\va[\gapbandit]/\gapUplift$, suggesting that this knowledge is helpful when $\gapUplift$ is relatively large. 

%Our regret bound will feature the ratio $\va[\gapbandit]/\gapUplift$, suggesting that this information is helpful when $\gapUplift$ is relatively large.
Hereinafter, for any $x,\alpha,\beta\in\R$ with $\alpha\le\beta$, we use $\clip(x,\alpha,\beta)$ to denote the clipping function that restricts $x$ to the interval $[\alpha,\beta]$, \ie $\clip(x,\alpha,\beta)=\max(\alpha,\min(\beta,x))$. Missing proofs are collected in~\cref{apx:lower-bound-unknown-affected}.
%Again, we consider the cases of whether the baseline payoffs are known or not.

\subsubsection{Known Baseline Payoffs}

As we have seen in \cref{subsubsec:UpUCB-L-BL},
if the baseline payoffs $\va[\meanReward][0]$ are known, we can directly check whether $\vav[\meanReward][0]$ is in the confidence interval.
Moreover, with the knowledge $\abs{\vav[\meanReward]-\vav[\meanReward][0]}\ge\gapUplift$ for all $\indv\in\va[\variables]$, we deduce that $\va[\variables]$ can be identified correctly with probability $1-2\nVariables\alt{\smallproba}$ after action $\arm$ is taken $\pullcount_0=\ceil{(8/\gapUplift^2)\log(1/\alt{\smallproba})}$ times.
In fact, let $\vta[\valuev][1],\ldots,\vta[\valuev][\pullcount_0]$ be $\pullcount_0$ i.i.d. realizations of $\va[\valuev]\sim\va[\distribution]$ and $\vtav[\tilde{\meanReward}][\pullcount_0]=(\sum_{\run=1}^{\pullcount_0}\vtav[\valuev])/\pullcount_0$ be the empirical mean of variable $\indv$.
%Choosing $\varepsilon\in(0,\gapUplift)$ such that $\pullcount_0=(8/(\gapUplift-\varepsilon)^2)\log(1/\alt{\smallproba})$.\footnote{Such $\varepsilon$ exists (and of course, is unique) because $\pullcount_0>(8/\gapUplift^2)\log(2\nVariables/\alt{\smallproba})$.}
Applying the sub-Gaussian concentration inequality (\ref{eq:sub-Gaussian-concentration}, \cref{apx:concentration}) gives
%
\begin{equation}
    \prob\left(\abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward]}\ge\frac{\gapUplift}{2}\right)
    \le2
    \exp\left(-\frac{\pullcount_0\gapUplift^2}{8}\right)
    \le 2\alt{\smallproba}.
    %\frac{\alt{\smallproba}}{\nVariables}.
\end{equation}
%
With a union bound we conclude that with probability at least $1-2\nVariables\alt{\smallproba}$ it holds for all $\indv$ that $\abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward]}<\gapUplift/2$.
We distinguish between the following two situations
%
\begin{enumerate}
    \item $\indv\in\va[\variables]$, then $\displaystyle \abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward][0]}\ge\abs{\vav[\meanReward]-\vav[\meanReward][0]}-\abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward]}>\gapUplift-\frac{\gapUplift}{2}=\frac{\gapUplift}{2}$.
    \item $\indv\notin\va[\variables]$, then $\displaystyle \abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward][0]}=\abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward]}<\frac{\gapUplift}{2}$.
\end{enumerate}
%
This implies that with the choice
$\va[\setId] = \setdef{\indv\in\variables}{\abs{\vtav[\tilde{\meanReward}][\pullcount_0]-\vav[\meanReward][0]}>\gapUplift/2}$, we have effectively $\prob(\va[\setId]=\va[\variables])\ge1-2\nVariables\alt{\smallproba}$.
One natural algorithm is to thus first pull each arm $\pullcount_0$ times and run \UpUCB (\cref{algo:UpUCB-BL}) %(from~\cref{subsec:UpUCB-BL})
in the remaining rounds by regarding $\va[\setId]$ as the variables that action $\arm$ affects.
A direct computation shows that the regret of this algorithm is in
$\bigoh(\sum_{\arm\in\arms:\va[\gapbandit]>0}(\va[\gapbandit]/\gapUplift+\va[\nAffected])^2\log\nRuns/\va[\gapbandit])$ with high probability.
%$\bigoh(\pullcount_0\sum_{\arm\in\arms}\va[\gapbandit]+(\nArms\nAffected^2)\log\nRuns/\gapbandit)$.

However, $\pullcount_0$ can be arbitrarily large when $\gapUplift$ gets closer to $0$, and taking an action much fewer times is probably sufficient to deduce that action is not optimal (with high probability).
We thus propose to implement the above idea in a more flexible manner:
We run \UpUCB with the uplifting indices $\vta[\UPindexSum]=\sum_{\indv\in\vta[\setId]}(\vtav[\UCBindex]-\vav[\meanReward][0])$, where
%
\begin{equation}
    \notag
    \vta[\setId] =
    \begin{cases}
    \variables & \text{if} ~ \vta[\pullcount]<\pullcount_0,\\
    \setdef{\indv\in\variables}{\abs{\vtav[\est{\meanReward}][\run][\vt[\arm]]-\vav[\meanReward][0]}>\gapUplift/2} & \text{otherwise}.
    \end{cases}
\end{equation}
%
%known baseline payoffs by assuming that all the actions affect all the variables.
%Then, for each arm $\arm$, as long as its pull count exceeds $\pullcount_0$, we switch the index by considering $\va[\setId]$ as the affected set.
We refer to this algorithm as \UpUCBDelta, with iLift standing for individual uplift, and summarize it in \cref{algo:UpUCB-GapUp-BL}. \UpUCBDelta has the following regret guarantee.

\input{Algorithms/UpUCB_GapUp_BL}

\begin{restatable}{theorem}{UpUCBGapUpBL}
\label{thm:UpUCB-GapUp-BL-regret}
Let $\alt{\smallproba}=\smallproba/(2\nArms\nVariables\nRuns)$. Then the regret of \UpUCBDelta (\cref{algo:UpUCB-GapUp-BL}), 
with probability at least $1-\smallproba$, satisfies:
%
\begin{equation}
    \label{eq:UpUCB-GapUp-BL-regret}
    \vt[\reg][\nRuns] \le
    \sum_{\arm\in\arms:\va[\gapbandit]>0}
    \left(\frac{8\thinspace\clip(\va[\gapbandit]/\gapUplift,\va[\nAffected],\nVariables)^2\log(2\nArms\nVariables\nRuns/\smallproba)}{\va[\gapbandit]}+\va[\gapbandit]\right).
\end{equation}
\end{restatable}

\cref{thm:UpUCB-GapUp-BL-regret} shows that \cref{algo:UpUCB-GapUp-BL} provides a smooth transition between standard UCB and the naive strategy that tries to identify the affected variables of all the actions.
When $\va[\gapbandit]/\gapUplift\ge\nVariables$, the loss of taking action $\arm$ is so large that UCB prevents it from being taken further even if $\vta[\pullcount]\le\pullcount_0$.
Otherwise, the affected variables get identified after an action is taken sufficient number of times and the algorithm benefits from this knowledge to improve the estimate of the uplift.
It is also quite straightforward to combine \cref{algo:UpUCB-L-BL} with \cref{algo:UpUCB-GapUp-BL} when both $\nAffected$ and $\gapUplift$ are known; this results in a regret bound that replaces $\clip(\va[\gapbandit]/\gapUplift,\va[\nAffected],\nVariables)$ by $\clip(\va[\gapbandit]/\gapUplift,\va[\nAffected],\nAffected)$ in \eqref{eq:UpUCB-GapUp-BL-regret}.

\subsubsection{Unknown Baseline Payoffs}
Several additional challenges emerge when we want to adapt the aforementioned strategies to the case where the baseline payoffs are unknown.
First, without additional assumption, it is impossible to tell whether two arbitrarily close estimates indicate the same effect of two actions on a variable.
Then, without a proper baseline to compare with, we can never exclude the possibility that all the variables are affected by all the actions.
To circumvent this issue, we make the following more stringent assumption.

\begin{assumption}
\label{asm:gapUplift-ubl}
The effect of any two actions on a variable differ by at least $\gapUplift$ as long as one of them affects this variable, \ie for all $\arm\in\arms$, $\indv\in\va[\variables]$, and $\alt{\arm}\in\setexclude{\arms}{\{\arm\}}$, it holds $\abs{\vav[\meanReward]-\vav[\meanReward][\alt{\arm}]}\ge\gapUplift$.
\end{assumption}

\input{Algorithms/UpUCB_GapUp}

In other words, $\gapUplift$ is not only a lower bound on individual uplift, but also a lower bound on (individual) effect gap.
Second, with a UCB-style algorithm, the optimal actions may not be taken sufficiently many times, in which case we can only conservatively assume that they affect all the variables.
This would incur additional regret in the analysis when $\va[\meanReward][0]$ is unknown. 
%While this does not pose a problem when $\va[\meanReward][0]$ is known, it can cause extra regret when we apply the \ac{DiffUCB} principle.
Therefore, we would like to ensure that all the (potentially optimal) actions are taken the same number of times at the point that the affected variables get identified.
This leads to a two-stage method as described in \cref{algo:UpUCB-GapUp}.

In the first stage, we perform successive elimination until the uneliminated actions are taken sufficiently many times.
Here $\vta[\estalt{\reward}][\round]$ is the empirical estimate of the reward associated to action $\arm$ and $\vt[\radiusConf][\round]=\nVariables\sqrt{2\log(1/\alt{\smallproba})/\round}$ is the associated radius of confidence interval.
%After that, we aggregate variables with close estimates.
Subsequently, for each variable $\indv\in\variables$ we construct the set
%
\begin{equation}
    \label{eq:setBaseEst}
    \vv[\setBaseEst]
    = \setdef{\arm\in\arms}{\exists\thinspace \armalt\in\setexclude{\arms}{\{\arm\}}, \vtav[\intConf][\run_0+1]\intersect\vtav[\intConf][\run_0+1][\armalt]\neq\varnothing},
\end{equation}
%
where $\run_0$ is the number of iterations in the elimination phase and the confidence intervals are defined as in \eqref{eq:UCBs-arm}.
If \cref{asm:gapUplift-ubl} is verified, then with high probability $\arm\in\vv[\setBaseEst]$ only if $\indv\notin\va[\variables]$.
Therefore, the observed results from these arms can be used to estimate the baseline payoff of $\indv$.
On the other hand, the identified affected variables for action $\arm\in\arms$ are then $\va[\setId]=\setdef{\indv\in\variables}{\arm\notin\vv[\setBaseEst]}$.

The second stage of the algorithm reuses the idea from \UpUCBwb.
We define the UCB indices following \eqref{eq:UCBs-arm} for $\arm\in\arms$ and for the baseline estimate we choose among $\vv[\setBaseEst]$ the action that is taken the most frequently whenever this set is non-empty. Otherwise we arbitrarily set it to $0$. That is,
%
\begin{equation}
    \label{eq:UCBs-0-UpUCB-GapUp}
    \vtav[\UCBindex][\run][0] = \begin{cases}
    0
    & \text{if} ~ \vv[\setBaseEst]=\varnothing,
    \\
    \vtav[\UCBindex][\run][\vtav[\arm][\run][0]] \text{ where $\vtav[\arm][\run][0]=\argmax_{\arm\in\vv[\setBaseEst]}\vta[\pullcount][\run-1]$} & \text {otherwise}.
    \end{cases}
\end{equation}
%
The uplifting indices that guide the decision of the algorithm are defined by $\vta[\UPindexSum]=\sum_{\indv\in\vta[\setId]}(\vtav[\UCBindex]-\vtav[\UCBindex][\run][0])$.

As shown below, the regret of \cref{algo:UpUCB-GapUp} takes roughly the same form as the one in \cref{thm:UpUCB-GapUp-BL-regret}, but as in \cref{thm:UpUCB-regret}, the number of variables that an optimal action affects also plays a crucial role in the regret bound.


% we form a partition of the remaining arms such that if two arms $\arm, \armalt$ belong to different cells of the partition then the confidence intervals $\vta[\intConf]$ and $\vta[\intConf][\run][\armalt]$ do not overlap.
% Let us denote by $\vav[\arms]$ the cell that arm $\arm$ belongs to. The aggregated empirical means, pull counts, and UCB indices are defined as:
% %
% \begin{equation}
%     \label{eq:UCBs-gapUplift}
%     \vtav[\pullcount] = \sum_{\runalt=1}^{\run}\one\{\vt[\arm]\in\vav[\arms]\},
%     ~~
%     \vtav[\est{\meanReward}] =
%     \frac{\sum_{\runalt=1}^{\run}\vtv[\valuev]\one\{\vt[\arm]\in\vav[\arms]\}}{\max(1, \vtav[\pullcount])},
%     ~~
%     \vtav[\UCBindex]
%     = \vtav[\est{\meanReward}]
%     + \sqrt{\frac{2\log(1/\alt{\smallproba})}{\vtav[\pullcount]}}.
% \end{equation}
% %
% The learner then plays the action with the largest UCB index $\vta[\UCBindex]=\sum_{\indv\in\variables}\vtav[\UCBindex]$.
% %The whole procedure is described in
% Notice that if \cref{asm:gapUplift-ubl} is violated, the aggregation of the estimates may incur an additional regret in $\Theta(\nAffected\nRuns\gapUplift)$. 

% \begin{remark}
% We do not insist on the use of uplifting index here.
% Otherwise, another alternative is to compare with some most pulled armed as in \cref{algo:UpUCB-L}.
% However, we believe aggregating estimates that are close to each other is the most natural thing to do under the assumption that two actions cannot have arbitrarily similar effect on a variable unless they affect the variable in the same way.
% \end{remark}

\begin{restatable}{theorem}{UpUCBGapUpregret}
\label{thm:UpUCB-GapUp-regret}
Let \cref{asm:gapUplift-ubl} hold and $\alt{\smallproba}=\smallproba/(2\nArms\nVariables\nRuns)$.  Then the regret of \UpUCBDeltawb (\cref{algo:UpUCB-GapUp}), with probability at least $1-\smallproba$, satisfies:
%
\begin{equation}
    \label{eq:UpUCB-GapUp-regret}
    \vt[\reg][\nRuns] \le
    \sum_{\arm\in\arms:\va[\gapbandit]>0}
    \left(\frac{8\thinspace\clip(2\va[\gapbandit]/\gapUplift,\va[\nAffected]+\va[\nAffected][\sol[\arm]],2\nVariables)^2\log(2\nArms\nVariables\nRuns/\smallproba)}{\va[\gapbandit]}+\va[\gapbandit]\right).
\end{equation}
\end{restatable}

\vspace{0.4em}
\begin{remark}
A natural candidate for $\vtav[\UCBindex][\run][0]$ is the one that uses aggregated information as in \eqref{eq:mean-estimate-0}.
The problem of this choice is that how we aggregate the observations collected in the first phase are only determined at the end of the the phase, while this choice itself depends on these observations.
Mathematically, this prevents us from defining a suitable martingale difference sequence for which we establish concentration bound.
An easy fix is to only aggregate observations from the second phase, while the use of the observations from the first phase should be limited to those coming from just one arm.
%in $\vv[\setBaseEst]$.
\end{remark}


==> Uplifting bandits - arxiv/Sections/UpBandit.tex <==
We start by formally introducing our uplifting bandit model. We illustrate it in~\cref{fig:model} and summarize our notations in~\cref{tab:notation}. Contextual extensions of this model are discussed in \cref{sec:context}.

%We consider 
A $(\nArms,\nVariables)$-uplifting bandit is
a stochastic bandit with $\nArms$ actions and $\nVariables$ underlying variables.
%, and the reward defined as the sum of these variables.
Each action $\arm\in\arms\defeq\intinterval{1}{\nArms}$ is associated with a distribution $\va[\distribution]$ on $\R^{\nVariables}$. 
%The bandit setup is characterized by a sequence of interactions between the learner and the environment:
At each round $\run$, the learner chooses an action $\vt[\arm]\in\arms$
%as a realization of the random variable $\va[\valuev][\vt[\arm]]\sim\va[\distribution][\vt[\arm]]$
%drawn from $\va[\distribution]$
and receives reward $\vt[\reward]=\sum_{\indv\in\variables}\vtv$ where
$\variables\defeq\intinterval{1}{\nVariables}$ the set of all variables
and $\vt[\valuev]=(\vtv[\valuev])_{\indv\in\variables}\sim\va[\distribution][\vt[\arm]]$ %\footnote{That is, the conditional distribution of the underlying variables given $\vt[\arm][1], \vt[\valuev][1], \ldots, \vt[\arm][\run]$ is $\va[\distribution][\vt[\arm]]$.}
is the payoff vector.\footnote{The terms \emph{reward} and \emph{payoff} distinguish $\vt[\reward]$ and $(\vtv[\valuev])_{\allvariables}$.}
%The goal of the learner is to maximize the cumulative reward up to a time horizon $\nRuns$.
Our model is distinguished by the two assumptions that we describe below. 
%\todobmargin{We may want to have clear terminology that distinguishes individual rewards / lifts from their sums.}
%
\begin{enumerate}[label=\textbf{(\Roman*)}, wide=0pt]
%\begin{list}{{\bf (\alph{enumi})}}{\usecounter{enumi}
%\setlength{\leftmargin}{1ex}
%\setlength{\listparindent}{1ex}
%\setlength{\parsep}{0pt}}
\item \textbf{Limited Number of Affected Variables.}
\label{asm:limited}
%As we discussed in Section~\ref{sec:intro}, in many relevant applications, each action only affects a limited number of variables. 
Let $\va[\variables]\subseteq\variables$ be the subset of variables affected by action $\arm$ and $\va[\distribution][0]$ be the baseline distribution that the variables' payoffs follow when no action is taken.
%We also assume the existence of a baseline distribution $\va[\distribution][0]$ that the variables follow when no arm is pulled.
%We assume that each arm only affects a subset of variables.
%Let $\variables\defeq\intinterval{1}{\nVariables}$ denote the set of variables and $\va[\variables]$ represent the subset of variables that arm $\arm$ affects.
%Then, for each $\arm\in\arms$ there is $\va[\variables]\subseteq\variables$ such that
By definition $\va[\distribution]$ and $\va[\distribution][0]$ have the same marginal distribution on $\setcomplement{\va[\variables]}\defeq\setexclude{\variables}{\va[\variables]}$, the variables unaffected by action $\arm$.\footnote{%
If the actions in fact have small impact on the variables in $\setcomplement{\va[\variables]}$,
%(\eg in example \ref{ex:movie}, the probability that a movie gets watched may slightly decrease if it is not recommended), 
our model is misspecified and incurs additional linear regret whose size is proportional to the impact of the actions on $\setcomplement{\va[\variables]}$.
An interesting question is how we can design algorithms that self-adapt to the degree of misspecification.\label{footnote:small-impact}}
%that still benefits from the structure when the misspecification is small.
%} 
%( $\va[\distribution_{\setcomplement{\va[\variables]}}]=\va[\distribution_{\setcomplement{\va[\variables]}}][0]$).
While the above condition is always satisfied with  $\va[\variables]=\variables$, we are interested in the case of $\va[\nAffected]\defeq\card(\va[\variables])\ll\nVariables$, meaning only a few variables are affected by $\arm$.
%each arm only affects a small number of intermediate variables, so that we can find $\va[\variables]$ with $\va[\nAffected]\defeq\card(\va[\variables])\ll\nVariables$.
We define $\nAffected$ as a uniform bound on $\va[\nAffected]$, so that $\max_{\arm\in\arms}\va[\nAffected]\le\nAffected$.
For convenience of notation, we write $\arms_0=\arms\union\{0\}$ and $\oneto{\nRuns}:=\intinterval{1}{\nRuns}$.
%\todosk{We need to add a footnote to say something about the case, where each action has large impact on small set of variables and non-zero impact on others.}
% \todobmargin{Comment on the role of $A_0$. It does not seem that action $0$ can be taken. So is this just for notation convenience?}
% \todoygmargin{I think it is clear enough, and we will emphasize again action $0$ cannot be taken alter.}

\item\textbf{Observability of Individual Payoff.} 
\label{asm:observability}
In addition to the reward $\vt[\reward]$, we assume that the learner observes all the payoffs $(\vtv[\valuev])_{\indv\in\variables}$ after an action is taken in round $\run$.

%_{\va[\valuev]\sim\va[\distribution]}

%
% For technical reasons, we will also sometimes require the following Bernstein condition to be satisfied for $\noisedev=1$:
% %
% \begin{equation}
%     \label{eq:Bernstein}
%     \ex[\abs{\rv}^{\probmoment}] \le \frac{\probmoment!}{2}\noisedev^{\probmoment-2}\ex[\rv^2]
%     \text{ for all } \probmoment\ge2.
% \end{equation}
% %
% Notice that a sub-Gaussian random variable necessarily satisfy the Bernstein condition but the associated parameter may depend on the variance of the random variable, which is in general unknown to the learner.
% That is why we will force $\noisedev=1$ when we require \eqref{eq:Bernstein}.
%\end{list}
\end{enumerate}
%
%Both these assumptions play an important role in our analysis, as shown by our lower bounds in \cref{sec:lower}. 
%\todob{The next paragraph comes completely out of blue. We need to say that "uplift modeling" is our tool for leveraging sparse feedback.}

\paragraph{Uplift and Noise\afterhead}
Let $\va[\valuev]=(\vav[\valuev])_{\allvariables}$ be a random variable with distribution $\va[\distribution]$. 
%We assume that when the action $\arm$ is taken we observe all of $(\vav[\valuev])_{\allvariables}$.
We define $\vav[\meanReward]=\ex[\vav[\valuev]]$ and $\vav[\snoise]=\vav[\valuev]-\vav[\meanReward]$ respectively as the expected value of and the noise in $\vav[\valuev]$.
%and the noise in this variable.
We use $\va[\meanReward]$ (resp.\ $\vav[\meanReward][0]$) to denote the vector of $(\vav[\meanReward])_{\allvariables}$ (resp.\ $(\vav[\meanReward][0])_{\allvariables}$), and refer to $\va[\meanReward][0]$ as the baseline payoffs.
%The uplift of an action on variable $\allvariables$ 
The \emph{individual} uplift associated to a pair $(\arm,\indv)\in\arms\times\variables$
is defined as $\vav[\meanUplift] =\vav[\meanReward] - \vav[\meanReward][0]$. An individual uplift can be \emph{positive} or \emph{negative}.
We obtain the (total) uplift of an action by summing its individual uplifts over all the variables affected by that action
%
\begin{equation}
\label{eq:total-uplift}
\va[\uplift]
%=\sum_{\indv\in\variables}\vav[\meanUplift]
=\sum_{\indv\in\va[\variables]}\vav[\meanUplift]
=\sum_{\indv\in\va[\variables]}(\vav[\meanReward]-\vav[\meanReward][0]).
\end{equation}
%\vspace{-0.4em}
%
Let $\va[\reward]=\sum_{\indv\in\variables}\vav[\meanReward]$ be the expected reward of an action or of pure observation. We also have $\va[\uplift]=\va[\reward]-\va[\reward][0]$
since $\vav[\meanReward]=\vav[\meanReward][0]$ as long as $\indv\notin\va[\variables]$.

%$\indv$ when arm $\arm$ is pulled (when $\arm\in\arms$) or when the variables follow the baseline distribution (when $\arm=0$).
%The noise in variable $\vav[\valuev]$ is then written as 
A real-value random variable $\rv$ is said to be $\noisedev$-sub-Gaussian 
% \todob{$\sigma^2$-sub-Gaussian is the right capitalization and writing this.} 
if for all $\scalar\in\R$, it holds $\ex[\exp(\scalar\rv)]\le\exp(\noisevar\scalar^2/2)$.
%\footnote{For example, a random variable whose absolute value is almost surely bounded by $\noisedev$ is $\noisedev$-sub-Gaussian.}
Throughout the paper, we assume that $\vav[\snoise]$ is $1$-sub-Gaussian for all $\arm\in\arms_0$ and $\indv\in\variables$.
% The following concentration inequality for $\noisedev$-sub-Gaussian random variables~\citep{vershynin2018high} is crucial to our analysis
% %
% \begin{equation}
%     \label{eq:sub-Gaussian-concentration}
%     \prob(\abs{\rv}\ge\scalar)\le2\exp(-\scalar^2/(2\noisevar)) \text{ for all } \scalar>0.
% \end{equation}
Note that we do not assume that $(\vav[\valuev])_{\indv\in\variables}$ are independent, i.e., the elements in the noise vector $(\vav[\snoise])_{\allvariables}$ may be correlated,
for the following two reasons: 
%\todob{This needs to be discussed in detail. It is nice that our algorithms work in this difficult setting. However, it is also true that one cannot do better than having separate confidence intervals per variable and adding them up. The resulting additive structure is used heavily in our algorithm design.}
\begin{itemize}[leftmargin=*]
    \item The independence assumption is not always realistic.
    In our first example, it excludes any potential correlation between two customers' purchases.
    %the possibility that a customer's decision of purchase get influenced by that of others.
    \item While a learner can exploit their knowledge on the noise covariance matrix to reduce the regret, as for example shown in \citep{DP16}, incorporating such knowledge complicates the algorithm design and the accompanying analysis.
    We however believe this is an interesting future direction to pursue.
    %and is likely to dilute the focus of our paper.
    % \todoyg{This second part is a bit delicate, because we should avoid giving a negative impression.
    % You may be able to do a better job here.}
    % \todosk{I do not like the second part much, especially the bit ``likely to dilute the focus of our paper''.}
    % \todoyg{changed}
\end{itemize}

\input{Figures/Illustration}
% Similarly, we define the vector $\va[\snoise]$.

\paragraph{Regret.}
%In the following, we will write $\vav[\meanReward]=\ex_{\va[\valuev]\sim\va[\distribution]}[\vav[\valuev]]$ for the expected value of variable $\indv$ when arm $\arm$ is pulled (when $\arm\in\arms$) or when the variables follow the baseline distribution (when $\arm=0$).
%By definition, for any $\arm\in\arms$, we have $\vav[\meanReward]=\vav[\meanReward][0]$ when $\indv\notin\va[\variables]$.
The learner's performance is characterized by their regret.
To define it, we denote by $\sol[\arm]\smallin\argmax_{\arm\in\arms}\va[\reward]$ an action with the largest expected reward and
$\sol[\reward]=\va[\reward][\sol[\arm]]=\max_{\arm\in\arms}\va[\reward]$
the largest expected reward.
The regret of the learner after $\nRuns$ rounds is then given by
%
\begin{equation}
    \label{eq:regret-decomp}
    \begin{aligned}[b]
    \reg_{\nRuns} &= \sol[\reward]\nRuns - \sum_{\run=1}^{\nRuns}\va[\reward][\vt[\arm]]
    %= \sol[\uplift]\nRuns - \sum_{\run=1}^{\nRuns}\va[\uplift][\vt[\arm]] 
    %\\
    = \sum_{\arm\in\arms}\sum_{\run=1}^{\nRuns}\one\{\vt[\arm]=\arm\}\va[\gapbandit],
    \end{aligned}
\end{equation}
%
where $\va[\gapbandit]=\sol[\reward]-\va[\reward]$ is the suboptimality gap of action $\arm$.
In words, we compare the learner's cumulative (expected) reward against the best we can achieved by taking  an optimal action at each round.
%that of the optimal policy which consists in taking an optimal action.
For posterity, we write $\gapbandit=\min_{\arm\in\arms,\va[\gapbandit]>0}\va[\gapbandit]$ for the minimum non-zero suboptimality gap and refer to it as the suboptimality gap of the problem.


\paragraph{UCB for Uplifting Bandits.}
%
The \ac{UCB} algorithm~\citep{auer2002using}, at each round, constructs an \acdef{UCB} on the expected reward 
%upper confidence bound (also refer to as UCB index) on the expected reward 
%\todob{This is where a clear distinction between individual rewards and their sum would help.}
of each action and chooses the action with the highest \ac{UCB}.
When applied to our model,
we get a regret of $\bigoh(\nArms\nVariables^2\log\nRuns/\gapbandit)$,
%we get an upper confidence bound of the form $\vta[\UCBindex]=\vta[\est{\reward}]+\vta[\radiusConf]$, where $\vta[\UCBindex]$ is the empirical estimate of $\va[\reward]$ and $\vta[\radiusConf]$ is a confidence interval.
as the noise in the reward is $\nVariables$-sub-Gaussian (recall that we do not assume independence of the payoffs).
%\footnote{Since $(\vav[\valuev])_{\indv\in\variables}$ could be dependent, their sum is not $\sqrt{\nVariables}$-sub-Gaussian, and in general can be bounded only using a $\nVariables$-sub-Gaussian random variable. The covariance of the noises has of course an important impact on the regret, see \eg \citep{DP16}, but providing algorithms that can effectively exploit this knowledge is beyond the scope of this work.} 
However, this approach completely ignores the structure of our problem.
As we show in \cref{sec:UpUCB-BL}, we can achieve much smaller regret by focusing on the uplifts.
%, since it can be estimated with better statistical efficiency.  
%The goal of our work is thus to improve this dependence on $\nVariables$ by taking into account these ingredients, and this is essentially achieved by estimating the expected uplift instead of the expected reward.

%In essence, this is achieved by estimating the expected total uplifting effect $\va[\uplift]$ defined in \eqref{eq:total-uplift}.
%
% \begin{equation}
% \notag
% \va[\uplift]=\va[\reward]-\va[\reward][0]=\sum_{\indv\in\va[\variables]}\vav[\meanUplift]=\sum_{\indv\in\va[\variables]}(\vav[\meanReward]-\vav[\meanReward][0]).
% \end{equation}
%
%This only requires the learner to focus on the affected variables so that the scale of noise becomes potentially much smaller.

\paragraph{Problem Variations.} In the following sections, we study several variants of the above basic problem that differ in the prior knowledge about $(\va[\distribution])_{\arm\in\arms_0}$ that the learner possesses.
\begin{enumerate}[label=\textbf{(\alph*)}, wide=0pt]
% \begin{list}{{\bf (\roman{enumi})}}{\usecounter{enumi}
% \setlength{\leftmargin}{1ex}
% \setlength{\listparindent}{0ex}
% \setlength{\parsep}{0pt}}
% \vspace*{-2ex}
\item\textbf{Knowledge of Baseline Payoffs.} We consider two scenarios based on whether the learner knows the baseline payoffs $\va[\meanReward][0] \coloneqq (\vav[\meanReward][0])_{\allvariables}$ or not.
\item\textbf{Knowledge of Affected Variables.} We again consider two  scenarios based on whether the learner knows the affected variables associated with each action $(\va[\variables])_{\arm\in\arms}$ or not. % has no knowledge of the structure.
%\end{list}
\end{enumerate}
% In the following sections, we provide regret bounds under each combination of these scenarios. \todob{Consolidate the above into a single paragraph.}
% Our results show that while we can completely eliminate the assumption on the learner knowing the baseline, some prior knowledge on how the variables are affected is necessary.

\vspace*{-1ex}
\section{Case of Known Baseline and Known Affected Variables}

%Payoffs and Affected Variables}
\label{sec:UpUCB-BL}
We start with the simplest setting where both the affected variables and the baseline payoffs are known.
To address this problem, we make the crucial observation that
for any two actions, the difference in their rewards equals to that of their uplifts.
As an important consequence, uplift maximization has the same optimal action as total reward maximization, and we can replace rewards by uplifts in the definition of the regret \eqref{eq:regret-decomp}.
Formally, we write $\sol[\uplift]=\va[\uplift][\sol[\arm]]=\max_{\arm\in\arms}\va[\uplift]$ for the largest uplift; then 
\[\reg_{\nRuns} = \sol[\uplift]\nRuns - \sum_{\run=1}^{\nRuns}\va[\uplift][\vt[\arm]].\]
By making this transformation, we gain in statistical efficiency because
$\va[\uplift]=\ex[\sum_{\indv\in\va[\variables]}(\vav[\valuev]-\vav[\meanReward][0])]$ can now be estimated much more efficiently under our notion of sparsity.
Since both $\va[\meanReward][0]$ and $(\va[\variables])_{\arm\in\arms}$ are known, we can directly construct a \ac{UCB} on $\va[\uplift]$. For this, we define
for all rounds $\run\in\oneto{\nRuns}$, actions $\arm\in\arms$, and variables $\indv\in\variables$ the following quantities.
%
\begin{equation}
    \label{eq:mean-estimate-a}
    \begin{aligned}[b]
    \vta[\pullcount] = \sum_{\runalt=1}^{\run}\one\{\vt[\arm][\runalt]=\arm\},
    ~~~
    \vta[\radiusConf] = \sqrt{
    \frac{2\log(1/\alt{\smallproba})}{\vta[\pullcount]}},
    ~~~
    \vtav[\est{\meanReward}] =
    \sum_{\runalt=1}^{\run}
    \frac{\vtv[\valuev][\runalt]\one\{\vt[\arm][\runalt]=\arm\}}{\max(1, \vta[\pullcount])},
    \end{aligned}
\end{equation}
%
where $\alt{\smallproba}>0$ is a tunable parameter.
In words, $\vta[\pullcount]$, $\vtav[\est{\meanReward}]$, and $\vta[\radiusConf]$ represent respectively the number of times that action $\arm$ is taken, the empirical estimate of $\vav[\meanReward]$, and the associated radius of \acl{CI} calculated at the end of round $\run$.
The UCB for action $\arm\in\arms$ and variable $\indv\in\va[\variables]$ at round $\run$ is $\vtav[\UCBindex]=\vtav[\est{\meanReward}][\run-1]+\vta[\radiusConf][\run-1]$.
We further define $\vta[\UPindexSum]=\sum_{\indv\in\va[\variables]}(\vtav[\UCBindex]-\vav[\meanReward][0])$ as the \emph{uplifting index},
and refer to \UpUCB as the algorithm that takes an action with the largest uplifting index $\vta[\UPindexSum]$ at each round $\run$ (\cref{algo:UpUCB-BL}).
Here, the suffix (bl) indicates that the method operates with the knowledge of the baseline payoffs.
%\todob{This naming is confusing. When I see "(b)", I think of something like Figure 1(b), meaning something second after "(a)". However, this is the first algorithm. At the minimum, we should explain what "(b)" stands for.}

\input{Algorithms/UpUCB_BL}

Since \UpUCB is nothing but a standard UCB with transformed rewards $\vt[\alt{\reward}]=\sum_{\indv\in\vt[\variables][\vt[\arm]]}(\vtv[\valuev]-\vav[\meanReward][0])$, and 
$\ex[\vt[\alt{\reward}]]=\va[\uplift][\vt[\arm]]$ defines exactly the same regret as the original reward, a standard analysis for \ac{UCB} yields the following result.
%(recall that $\va[\nAffected]=\card(\va[\variables])\le\nAffected$), which indicates that the new UCB algorithm enjoys a regret in $\bigoh((\nAffected^2\nArms)\log\nRuns/\gapbandit)$.

% \begin{proposition}
% \label{prop:UpUCB-BL-regret}
% Let $\alt{\smallproba}=\smallproba/(2\nArms\nRuns)$. If the learner knows the variables affected by each action and the baseline payoffs, then \UpUCB defined above, with probability at least $1-\smallproba$, has regret bounded by:
% \begin{equation}
%     \label{eq:UpUCB-BL-regret}
%     \vt[\reg][\nRuns] \le
%     \sum_{\arm\in\arms:\va[\gapbandit]>0}
%     \left(\frac{8(\va[\nAffected])^2\log(2\nArms\nRuns/\smallproba)}{\va[\gapbandit]}
%     +\va[\gapbandit]\right).
% \end{equation}
% \end{proposition} 
\begin{proposition}
\label{prop:UpUCB-BL-regret}
Let $\alt{\smallproba}=\smallproba/(2\nArms\nRuns)$. Then the regret of \UpUCB (\cref{algo:UpUCB-BL}), with probability at least $1-\smallproba$, satisfies:
\begin{equation}
     \label{eq:UpUCB-BL-regret}
    \vt[\reg][\nRuns] \le
    \sum_{\arm\in\arms:\va[\gapbandit]>0}
    \left(\frac{8(\va[\nAffected])^2\log(2\nArms\nRuns/\smallproba)}{\va[\gapbandit]}
    +\va[\gapbandit]\right).
\end{equation}
\end{proposition} 

% \todob{A correct way of writing the above is $a \in A: \Delta^a > 0$.}
%
As expected, the regret bound does not depend on $\nVariables$ and scales with $\nAffected^2$.
This is because the transformed reward of action $\arm$ is only $\va[\nAffected]$-sub-Gaussian.
The improvement is significant when $\nAffected\ll\nVariables$. 
%, and the minimax optimality of \eqref{eq:UpUCB-BL-regret}
However, this also comes at a price, as both the baseline payoffs and affected variables need to be known.
We address these shortcomings in \cref{sec:known-affected,sec:unknown-affected}.
%in the rest of the paper.
%Also note that observing the aggregated payoff $\sum_{\indv\in\va[\variables][\vt[\arm]]}\vtv[\valuev]$ is sufficient for this algorithm. 
% \todob{The last sentence does not add anything.}

\paragraph{Estimating Baseline Payoffs from Observational Data.}
In practice, the baseline payoffs $\va[\meanReward][0]$ can be estimated from observational data, which gives confidence intervals where $\vav[\meanReward][0]$ lie with high probability.
The uplifting indices can then be constructed by subtracting the lower confidence bounds of $\vav[\meanReward][0]$ from $\vtav[\UCBindex]$.
If the number of samples is $\nSamples$, the widths of the confidence intervals are in $\bigoh(1/\sqrt{\nSamples})$.
Identification of $a^*$ is possible only when the sum of these widths over $\nAffected$ variables is at most $\gapbandit$, which requires $\nSamples=\Omega(\nAffected^2/\gapbandit^2)$.
Otherwise, these errors persist at each iteration and $\nSamples$ must be in the order of $\nRuns$ to ensure $\bigoh(\sqrt{\nRuns})$ regret.
%Alternatively, we can estimate $\vav[\meanReward][0]$ as well during the interaction phase, and this will be the subject of next section.
%Generally speaking, the problem of warm-starting bandits with side data is also of substantial interest, see \eg \citep{SBSS20,ZAD+19}.

%\vspace{0.4em}
\paragraph{About Expected and Gap-Free Bounds.}
In \cref{prop:UpUCB-BL-regret}, we state a high-probability instance-dependent regret bound, and we will continue to do so for all the regret upper bounds that we present for the non-contextual variants.
This type of result can be directly transformed to bound on $\ex[\vt[\reg][\nRuns]]$ by taking $\smallproba=1/\nRuns$.
%Let us take this opportunity to comment on the form of the regret bounds that are presented in the paper.
Following the routine of separating $\va[\gapbandit]$ into two groups depending on their scale, most of our proofs can also be easily modified to obtain a gap-free regret bound, which is typically in the order of $\bigoh(\nAffected\sqrt{\nArms\nRuns\log(\nRuns)})$.
We will not state these results to avoid unnecessary repetitions.



% \begin{remark}
% For a rigorous analysis, we then also need to take into account the estimation error that rises from this estimate.
% Since our goal here (and in the corresponding parts of \cref{sec:unknown-affected}) is just to illustrate the main idea of the algorithm before tackling the more challenging unknown-baseline scenario, we do not provide such analyses, but these extensions should be straightforward.
% Generally speaking, the problem of warm-starting bandits with side data is also of substantial interest, see \eg \citep{SBSS20,ZAD+19}.
% \end{remark}

%We can then focus on estimating $\va[\meanUplift]$, which is now the mean of a $2\va[\nAffected]$-sub-Gaussian random variable, and if $\va[\nAffected]$ is uniformly bounded by $\nAffected$, \ie $\max_{\arm\in\arms}\va[\nAffected]\le\nAffected$, this should replace $\nVariables$ by $\nAffected$ in the above regret bounds.

\section{Lower Bounds}
\label{sec:lower}

In this section, we discuss the necessity of our modeling assumptions for obtaining the improved regret bounds of \cref{prop:UpUCB-BL-regret}.
%We introduce a general information-theoretic lower bounds for bandit problems with similar design in \cref{apx:lower-bound-information}, based on which we prove
We prove these results in  \cref{apx:lower-bound}, where we also introduce a general information-theoretic lower bounds for bandit problems with similar design.
%The lower bounds presented in this section are proved in \cref{apx:proof-lower-bound}. These proofs are based on a general information-theoretic lower bounds for bandit problems with similar design that we introduce in \cref{apx:lower-bound-information}.
% The complete discussion appears in \cref{apx:lower-bound}.
%Before moving on, we shortly discuss the necessity of the assumptions in \cref{prop:UpUCB-BL-regret}.
%and the optimality of \cref{prop:UpUCB-BL-regret}.
%Formal statement that justify the discussion can be found in \cref{apx:lower-bound}.

Intuitively, the regret can be improved both because the noise in the effect of an action is small, and because the observation of this effect does not heavily deteriorate with noise.
These two points correspond respectively to assumptions \ref{asm:limited} and \ref{asm:observability}.
%If any of these two points are violated, the improvement would be impossible.
Moreover, the knowledge on $(\va[\variables])_{\arm\in\arms}$ allows the learner to distinguish between problems with different structures.
Without such distinction, 
%the learner has no chance to exploit the underlying structure.
there is no chance that the learner can leverage the underlying structure.
%cannot be made by the learner, the structure cannot be exploited and the improvement would again be impossible.
Therefore, the aforementioned three points are crucial for obtaining \eqref{eq:UpUCB-BL-regret}.
%
Below, we establish this formally for algorithms that are {\em consistent} \citep{LR85} over the class of $1$-sub-Gaussian uplifting bandits,
%(\ie the uplifting bandits with $1$-sub-Gaussian noises)
which means the induced regret of the algorithm on any uplifting bandit with $1$-sub-Gaussian noise satisfies $\vt[\reg]=\smalloh(\run^p)$ for all $p>0$.

For conciseness, in the following we say that an uplifting bandit has parameters $(\nArms,\nVariables,(\va[\gapbandit],\va[\nAffected])_{\arm\in\arms})$ if the number of actions, the number of variables, the suboptimality gaps, and the number of affected variables of this instance are respectively $\nArms$, $\nVariables$, $(\va[\gapbandit])_{\arm\in\arms}$, and $(\va[\nAffected])_{\arm\in\arms}$.
%refer to any instance of the uplifting bandit problem as described in \cref{sec:model} with $\nArms$ arms, $\nVariables$ variables, suboptimality gaps $(\va[\gapbandit])_{\arm\in\arms}$, and numbers of affected variables $(\va[\nAffected])_{\arm\in\arms}$ noise as a $1$-sub-Gaussian $(\nArms,\nVariables,(\va[\gapbandit],\va[\nAffected])_{\arm\in\arms})$ uplifting bandit instance.
We focus on instance-dependent lower-bounds and assume that the learner has full knowledge of the baseline distribution. (Of course, the problem only becomes more challenging if the learner does not know the baseline distribution.)
%\footnote{%
%Of course, the problem only becomes more challenging if the learner actually does not know the baseline distribution.}


\begin{proposition}
\label{prop:lower-bound}
Let $\policy$ be a consistent algorithm over the class of $1$-sub-Gaussian uplifting bandits that at most uses knowledge of $\va[\distribution][0]$, $(\va[\variables])_{\arm\in\arms}$, and the fact that the noise is $1$-sub-Gaussian.
Let $\nArms,\nVariables>0$ and sequence $(\va[\nAffected],\va[\gapbandit])_{1\le\arm\le\nArms}\in(\oneto{\nVariables}\times\R_+)^{\nArms}$ satisfy $\va[\gapbandit][1]=0$.
%that at most uses knowledge of $\va[\distribution][0]$, $(\va[\variables])_{\arm\in\arms}$, and the fact that the noise is $1$-sub-Gaussian.
Assume either of the following holds.
\begin{enumerate}[(a)]
    \item 
    \label{low-cond:affected}
    $\va[\nAffected]=\nVariables$ for all $\arm\in\arms$, so that in the bandits considered below all actions affect all variables.
    \item
    \label{low-cond:observed}
    Only the reward is observed.
    %\item The prior knowledge of $\policy$ does not enable it to distinguish between any two bandits with the same baseline and noise distributions.
    \item
    \label{low-cond:knowledge}
    The algorithm $\policy$ does not make use of any prior knowledge about the arms' expected payoffs $(\va[\meanReward])_{\arm\in\arms}$ (in particular, the knowledge of $(\va[\variables])_{\allvariables}$ is not used by $\policy$).
\end{enumerate}
% Then, for any $\nArms,\nVariables>0$ and sequence $(\va[\nAffected],\va[\gapbandit])_{1\le\arm\le\nArms}\in(\oneto{\nVariables}\times\R_+)^{\nArms}$
% %with $\va[\nAffected]\in\oneto{\nVariables}, \va[\nAffected][1]>\va[\gapbandit]\ge\max(0,\va[\nAffected][1]-\va[\nAffected])$ for all $\arm$ 
% with $\va[\gapbandit][1]=0$,\footnote{Necessarily $\va[\nAffected]\equiv\nVariables$ under condition \ref{low-cond:affected}.}
Then, there exists a $1$-sub-Gaussian uplifting bandit 
with parameters $(\nArms,\nVariables,(\va[\gapbandit],\va[\nAffected])_{\arm\in\arms})$
such that the regret induced by $\policy$ on it satisfies: 
\[
\liminf_{\toinf[\nRuns]} \frac{\ex[\vt[\reg][\nRuns]]}{\log\nRuns} \ge \sum_{\arm\in\arms:\va[\gapbandit]>0}\frac{2\nVariables^2}{\va[\gapbandit]}.
\]
\end{proposition}

As discussed above, \cref{prop:lower-bound} shows that there would be a higher regret in absence of any of the following: \begin{enumerate*}[\textup(a\textup)]
\item Limited number of affected variables,
\item Side information about variables beyond reward, and
\item Some prior knowledge on how the variables are affected.
\end{enumerate*}
We discuss below these three points in detail.
%
\begin{enumerate}[(a), wide, topsep=4pt]
    \item This point justifies the necessity of assumption \ref{asm:limited}.
    It can be further refined to account for non-uniform numbers of affected variables.
%
\vspace*{-3pt}
\begin{proposition}
\label{prop:lower-bound-L}
Let $\policy$ be a consistent algorithm over the class of $1$-sub-Gaussian uplifting bandits that at most uses knowledge of $\va[\distribution][0]$, $(\va[\variables])_{\arm\in\arms}$, and the fact that the noise is $1$-sub-Gaussian.
Then, for any $\nArms,\nVariables>0$ and sequence $(\va[\nAffected],\va[\gapbandit])_{1\le\arm\le\nArms}\in(\oneto{\nVariables}\times\R_+)^{\nArms}$
%with $\va[\nAffected]\in\oneto{\nVariables}, \va[\nAffected][1]>\va[\gapbandit]\ge\max(0,\va[\nAffected][1]-\va[\nAffected])$ for all $\arm$ 
with $\va[\gapbandit][1]=0$, there exists a $1$-sub-Gaussian uplifting bandit $(\nArms,\nVariables,(\va[\gapbandit],\va[\nAffected])_{\arm\in\arms})$
%a $1$-sub-Gaussian uplifting bandit instance with $\nArms$ arms, $\nVariables$ variables, suboptimality gaps $(\va[\gapbandit])_{\arm\in\arms}$, and numbers of affected variables $(\va[\nAffected])_{\arm\in\arms}$ 
such that the regret induced by $\policy$ on it satisfies
%
\begin{equation}
    \label{eq:lower-bound-L-1}
    \liminf_{\toinf[\nRuns]} \frac{\ex[\vt[\reg][\nRuns]]}{\log\nRuns} \ge \sum_{\arm\in\arms:\va[\gapbandit]>0}\frac{2(\va[\nAffected])^2}{\va[\gapbandit]}.
\end{equation} 
\end{proposition}
%
%Clearly, \cref{prop:lower-bound} under condition \ref{low-cond:affected} is just a corollary of \cref{prop:lower-bound-L}, and 
\cref{prop:lower-bound-L} essentially posits that the regret must scale with the magnitudes of the noises.
The stated lower bound \eqref{eq:lower-bound-L-1} matches an expected version of \eqref{eq:UpUCB-BL-regret} up to a constant factor,
suggesting the minimax optimatlity of \cref{prop:UpUCB-L-BL-regret}.
One way to argue this lower bound holds is by reducing a carefully designed uplifting bandits with parameters $(\nArms,\nVariables,(\va[\gapbandit],\va[\nAffected])_{\arm\in\arms})$ to a $\nArms$-arm bandit with the corresponding noise scales.
We will take a different approach in \cref{apx:lower-bound} that allows us prove all the lower bounds following the same schema.

\item This point partially justifies assumption \ref{asm:observability}.
Note that it is however not always necessary to observe all the payoffs. For example, observing the aggregated payoff $\sum_{\indv\in\va[\variables][\vt[\arm]]}\vtv[\valuev]$ is sufficient for computing the uplifting indices of \UpUCB.
Having observation of the entire payoff vector $(\vtv[\valuev])_{\indv\in\variables}$ is particularly relevant for the case of unknown affected variables since it helps identify the affected variables relatively easily, as we will see in \cref{sec:unknown-affected}.

\item
This point justifies the learner using knowledge about the affected variables.
To get some more intuition on the meaning of this condition, let us consider two bandits with exactly the same baseline and noise distributions and very close expected payoffs of the arms.
Then, with finite observations, they provide very similar feedback which prevents the learner from distinguishing between the two problems.
However, the two bandits may have completely different structures, and in particular, one of them may have all variables affected by all actions since slight perturbation to the baseline would mean that a variable is affected.
Therefore, the lower bound from \ref{low-cond:affected} applies to this instance.
Now, provided that the learner is doomed to treat the two instances equally, the lower bound applies to the other instance as well.
Of course, one can argue that it is unnatural that the regrets of two similar problems differ significantly even when the learner is provided some prior knowledge.
We believe this is the drawback of the asymptotic analysis that we look at here, since these differences may indeed be small within a reasonable number of runs. This is exactly related to the problem of misspecified model that we mentioned in \cref{footnote:small-impact}.
\end{enumerate}

With \cref{prop:lower-bound}, what remains unclear at this point is whether similar improvement of the regret is still possible when the baseline is unknown or when the learner only has access to more restricted knowledge than $(\va[\variables])_{\arm\in\arms}$.
We give affirmative answers to these two questions in the next two sections.

\vspace{0.4em}
\begin{remark}
Our lower bounds are derived with respect to the worst correlation structure of the noise. It is also possible to obtain lower bounds that depend on the covariance of the noise. % using \cref{lem:lower-bound-instance-dependent}.
For example, if the variables $(\vav[\valuev])_{\allvariables}$ are independent, the lower bound in \eqref{eq:lower-bound-L-1} only scales linearly with $\va[\nAffected]$.
\end{remark}

%two problem instances with different structures (\eg different $(\va[\variables])_{\arm\in\arms}$) can provide arbitrary close information to the learner, and thus the learner is doomed to treat them equally if they are not equipped with any prior knowledge that enables them to distinguish between the two problems.
%Accordingly, the learner is not able to take advantage of the underlying structure, and no improvement of the performance can be achieved.

% 
% Its proof is presented in \cref{apx:lower-bound}, where we also provide another lower bound that justifies the optimality of \cref{prop:UpUCB-BL-regret}.
% A stronger and formal version of \cref{prop:lower-bound}, which also justifies the optimality of \cref{prop:UpUCB-BL-regret}, is stated and proved in \cref{apx:lower-bound}. 
%A general information-theoretic lower bound for bandit problems with similar design based on which \cref{prop:lower-bound} is established is as well provided in \cref{apx:lower-bound}.
%\cref{sec:known-affected,sec:unknown-affected}.

==> Uplifting bandits - arxiv/Sections/UpUCB.tex <==

In this section, we consider the situation where the sets of affected variables $(\va[\variables])_{\arm\in\arms}$ are known by the learner, but not the baseline payoffs. Missing proofs are in~\cref{apx:upper-bound}.

%The hope is that by incorporating these ingredients, we can develop algorithms with much smaller regret bound.
%In fact, since every arm $\arm$ only affects $\va[\nAffected]\ll\nVariables$ variables, it is natural to argue that we only need to look at these variables to estimate the effect of this arm.
%Formally, this leads to the definition of the expected uplifting effect $\va[\meanUplift]=\va[\meanReward]-\va[\meanReward][0]=\sum_{\indv\in\va[\variables]}(\vav[\meanReward]-\vav[\meanReward][0])$.

% \subsection{UpUCB with Known Baseline Payoffs}
% \label{subsec:UpUCB-BL}
% To begin, we assume that the baseline payoffs $\va[\meanReward][0]=(\vav[\meanReward][0])_{\allvariables}$ are also known.
% In this case, we can directly construct an \ac{UCB} on $\va[\uplift]=\ex[\sum_{\indv\in\va[\variables]}(\vav[\valuev]-\vav[\meanReward][0])]$ and proceed as in usual UCB-type methods.
% To state the algorithm, for all time steps $\run\in\oneto{\nRuns}$, arms $\arm\in\arms$, and variables $\indv\in\va[\variables]$, we define
% %
% \begin{equation}
%     \label{eq:mean-estimate-a}
%     \begin{aligned}[b]
%     &\vta[\pullcount] = \sum_{\runalt=1}^{\run}\one\{\vt[\arm][\runalt]=\arm\},
%     ~~~
%     \vta[\radiusConf] = \sqrt{\frac{2\log(1/\alt{\smallproba})}{\vta[\pullcount]}},\\
%     &\vtav[\est{\meanReward}] =
%     \frac{\sum_{\runalt=1}^{\run}\vtv[\valuev][\runalt]\one\{\vt[\arm][\runalt]=\arm\}}{\max(1, \vta[\pullcount])},
%     \end{aligned}
% \end{equation}
% %\todob{$a_t$ and $v_t$ should be $a_s$ and $v_s$, respectively.}
% \todob{$v$ is a non-standard notation for payoffs. Why not $r$ or $y$? Also, do we want to capitalize the random variables?}
% %
% where $\alt{\smallproba}>0$ is a parameter to be specified.
% In words, $\vta[\pullcount]$, $\vtav[\est{\meanReward}]$, and $\vta[\radiusConf]$ represent respectively the number of pulls of $\arm$, the empirical estimate of $\vav[\meanReward]$, and the associated radius of confidence interval that can be calculated at the end of round $\run$.
% The UCB index for arm $\arm\in\arms$ and variable $\indv\in\va[\variables]$ at time $\run$ is then $\vtav[\UCBindex]=\vtav[\est{\meanReward}][\run-1]+\vta[\radiusConf][\run-1]$.
% We further define $\vta[\UPindex]=\sum_{\indv\in\va[\variables]}(\vtav[\UCBindex]-\vav[\meanReward][0])$ as the uplifting index, and refer to UpUCB with known baseline as the algorithm that pulls the arm with the largest uplifting index at each round.
% \todob{This description is clear. To make it crystal clear, point to Algorithm 1 and say we only need to replace the UCB of arm $0$ with the actual mean.}
% \todoyg{Otherwise we can also change the pseudo-code to account for the two cases.}

% In other words, this algorithm applies UCB to the model with transformed rewards $\vt[\alt{\reward}]=\sum_{\indv\in\va[\variables][\vt[\arm]]}(\vav[\valuev][\vt[\arm]]-\vav[\meanReward][0])=\vt[\reward]-\sum_{\indv\in\variables}\vav[\meanReward][0]$.
% This transformation does not modify the cumulative regret of the learner, but the transformed reward of arm $\arm$ is $\va[\nAffected]$-sub-Gaussian. Applying standard regret bound for UCB thus gives the following result.
% %(recall that $\va[\nAffected]=\card(\va[\variables])\le\nAffected$), which indicates that the new UCB algorithm enjoys a regret in $\bigoh((\nAffected^2\nArms)\log\nRuns/\gapbandit)$.

% \begin{proposition}
% \label{prop:UpUCB-BL-regret}
% Let $\alt{\smallproba}=\smallproba/(2\nArms\nRuns)$. With probability at least $1-\smallproba$, the regret of UpUCB with known baseline satisfies:
% %
% \begin{equation}
%     \label{eq:UpUCB-BL-regret}
%     \vt[\reg][\nRuns] \le
%     \sum_{\arm\in\arms,\va[\gapbandit]>0}
%     \left(\frac{8(\va[\nAffected])^2\log(2\nArms\nRuns/\smallproba)}{\va[\gapbandit]}
%     +\va[\gapbandit]\right).
% \end{equation}
% \end{proposition}
% %
% As one may expect, the regret bound does not depend on $\nVariables$ anymore and only scales with $\nAffected^2$. This is an enormous improvement when $\nAffected\ll\nVariables$.
% Moreover, it is also worth noticing that for this specific algorithm, observing the aggregated payoff $\sum_{\indv\in\va[\variables][\vt[\arm]]}\vtv[\valuev]$ is sufficient. As will be demonstrated through our lower bounds, this is generally not the case (i.e., there will be a penalty for regret if we do not observe the individual variables).

% In practice, the baseline payoffs $\va[\meanReward][0]$ can be estimated from observational data, and this gives confidence intervals that $\vav[\meanReward][0]$ lie in with high probability.
% The uplifting index is then constructed by subtracting the lower confidence bound of $\vav[\meanReward][0]$ from $\vtav[\UCBindex]$.
% If the number of samples is $\nSamples$, the width of the confidence intervals of $\vav[\meanReward][0]$'s are in the order of $1/\sqrt{\nSamples}$ and this error persists at each iteration.
% Therefore, to ensure $\bigoh(\sqrt{\nRuns})$ regret, $\nSamples$ must be in the order of $\nRuns$.
% Alternatively, we can try to estimate $\vav[\meanReward][0]$ as well during the interaction phase, which will be the subject of next paragraph.
% Generally speaking, the problem of warm-starting bandits with side data is also of substantial interest, see \eg \cite{SBSS20,ZAD+19}.

% \vspace{0.4em}
% \begin{remark}
% In \cref{prop:UpUCB-BL-regret}, we state a high-probability instance-dependent regret bound, and we will continue to do so for all the regret upper bounds that we present for the non-contextual variants.
% This type of result can be directly transformed to bound on $\ex[\vt[\reg][\nRuns]]$ by taking $\smallproba=1/\nRuns$.
% %Let us take this opportunity to comment on the form of the regret bounds that are presented in the paper.
% Following the routine of separating $\va[\gapbandit]$ into two groups depending on their scale, most of our proofs can also be easily modified to obtain a gap-free regret bound, which is typically in the order of $\bigoh(\nAffected\sqrt{\nArms\nRuns\log(\nRuns)})$.
% We will not state these results to avoid unnecessary repetitions.
% \end{remark}


% \begin{remark}
% For a rigorous analysis, we then also need to take into account the estimation error that rises from this estimate.
% Since our goal here (and in the corresponding parts of \cref{sec:unknown-affected}) is just to illustrate the main idea of the algorithm before tackling the more challenging unknown-baseline scenario, we do not provide such analyses, but these extensions should be straightforward.
% Generally speaking, the problem of warm-starting bandits with side data is also of substantial interest, see \eg \cite{SBSS20,ZAD+19}.
% \end{remark}

%We can then focus on estimating $\va[\meanUplift]$, which is now the mean of a $2\va[\nAffected]$-sub-Gaussian random variable, and if $\va[\nAffected]$ is uniformly bounded by $\nAffected$, \ie $\max_{\arm\in\arms}\va[\nAffected]\le\nAffected$, this should replace $\nVariables$ by $\nAffected$ in the above regret bounds.

% \subsection{UpUCB with Unknown Baseline Payoffs}

%The case of unknown baseline payoffs appears much more challenging, as the uplifting effect in a round is never directly observed. 
%In spite of this, we will show that a simple \ac{DiffUCB} principle can solve the problem and recover optimal regrets in this type of problems.

%In this work, we promote the \ac{DiffUCB} principle for balancing the exploration-exploitation trade-off in uplifting bandits:

%\begin{center}
    %\textit{The difference of two UCBs automatically trades off exploration against exploitation at each variable.} 
    %consists in an optimistic estimate of the uplifting effect.}
%\end{center}

Since the actual uplift at each round is never observed, the uplifts of the actions can hardly be estimated directly without knowing the baseline payoffs.
Instead, we follow a two-model approach.
Leveraging the fact that $\va[\distribution]$ and $\va[\distribution][0]$ have the same marginal distribution on $\setcomplement{\va[\variables]}$, we can estimate the baseline payoffs by aggregating information from the feedback of different actions. This leads to
%
\begin{equation}
    \label{eq:mean-estimate-0}
    \vtav[\pullcount][\run][0] =
    \sum_{\runalt=1}^{\run}\one\{\indv\notin\va[\variables][\vt[\arm][\runalt]]\},
    ~~~
    \vtav[\radiusConf][\run][0] = 
    \sqrt{\frac{2\log(1/\alt{\smallproba})} {\vtav[\pullcount][\run][0]}},
    ~~~
    \vtav[\est{\meanReward}][\run][0] =
    \frac{\sum_{\runalt=1}^{\run}\vtv[\valuev][\runalt]\one\{\indv\notin\va[\variables][\vt[\arm][\runalt]]\}}
    {\max(1, \vtav[\pullcount][\run][0])}.
\end{equation} 
Compared to \eqref{eq:mean-estimate-a}, we notice that both $\vta[\pullcount][\run][0]$ and $\vta[\radiusConf][\run][0]$ are functions of $\indv$.
This is because for each taken action $\arm$, we only increase the counters $\vtav[\pullcount][\run][0]$ for those $\indv\notin\va[\variables]$, which causes a non-uniform increase of $(\vtav[\pullcount][\run][0])_{\allvariables}$.
Then, by looking at all the rounds that variable $\indv$ is not influenced by the chosen action, we manage to compute $\vtav[\est{\meanReward}][\run][0]$, an estimate of $\vav[\meanReward][0]$.
%\todob{The rest of the paragraph has many unnecessary details. We obviously propose a more efficient strategy than trivially taking action $0$. Say it and move on.}
An alternative here is to consider a specific `action $0$' and estimate the baseline payoffs only using feedback from this action.
However, this necessarily requires action $0$ to be taken sufficiently often and would thus result in a very high regret.
As we will see, our algorithm does not make use of this specific action and achieves regret comparable to the one presented in \cref{prop:UpUCB-BL-regret}.
%\todob{Consider dropping the red text. It breaks the flow and it is unclear if this would be sound, because we have not established yet that any action as a baseline would work. That happens only in the last algorithm.}
To proceed, we define the following UCB indices for all the pairs $(\arm,\indv)\in\arms_0\times\variables$
%
\begin{gather}
    \label{eq:UCBs}
    \vtav[\UCBindex] = \begin{cases}
    0
    & \text{if} ~ \arm=0 ~\text{and}~ \indv\in\bigcap_{\arm\in\arms}\va[\variables],
    \\
    \vtav[\est{\meanReward}][\run-1] + \vta[\radiusConf][\run-1] & \text{if} ~ \arm\in\arms ~\text{and}~ \indv\in\va[\variables], \\
    \vtav[\est{\meanReward}][\run-1][0] + \vtav[\radiusConf][\run-1][0]
    & \text{otherwise.}
    \end{cases}
    \raisetag{1em}
\end{gather} 
%
%\todob{Comment on why $c_t^a$ does not depend on $i$ while $c_t^0$ does.} \todob{This leaves open the possibility that arm $0$ can pulled. \cref{algo:UpUCB} does not pull arm $0$.}
%
The second and the third lines of \eqref{eq:UCBs} contain the usual definition of UCBs using the empirical estimates and the radii of the confidence intervals defined in \eqref{eq:mean-estimate-a} and \eqref{eq:mean-estimate-0}.
In the special case that a variable is affected by all the actions
(recall that we do not use `action $0$'),
it is impossible to estimate $\vav[\UCBindex][0]$ but it is enough to compare $\vav[\UCBindex]$ directly against $\vav[\UCBindex][\armalt]$ for any two actions $\arm,\armalt\in\arms$, so we just set $\vtav[\UCBindex][\run][0]$ to $0$ in this case.

%The choice of $0$ in the first line of the definition is arbitrary and does not really matter. \todob{This is not a very good description. Instead of describing the design of $U^a_t(i)$, we talk about its single component that does not matter.}
%In fact, if a variable is affected by all the actions (recall that we do not use `action $0$'), it is impossible to estimate $\vav[\UCBindex][0]$ but it is enough to compare $\vav[\UCBindex]$ directly against $\vav[\UCBindex][\armalt]$ for any two actions $\arm,\armalt\in\arms$.
%\todob{This would be possible if arm $0$ could be pulled. Can it be pulled?}

We outline the proposed method, \UpUCBwb, in~\cref{algo:UpUCB}. 
The uplifting indices are given by
%
$\vta[\UPindexSum]=\sum_{\indv\in\va[\variables]}(\vtav[\UCBindex]-\vtav[\UCBindex][\run][0])$.
%
It may be counter-intuitive to compare the differences between two \ac{UCB}s.
Indeed, $\vta[\UPindexSum]$ is no longer an optimistic estimate of the uplifting effect $\va[\uplift]$, but it captures the essential trade-off between learning action $\arm$'s payoffs and learning the baseline $\va[\meanReward][0]$. 
% \todob{The rest of this paragraph is confusing. Delete it and start explaining why $\vta[\UPindexSum]$ is sound.}
% Importantly, it is only by not taking action $\arm$ that we can learn about the baseline distributions of the variables in $\va[\variables]$.
% %an action that we can learn about the baseline distributions of the variables that the action affects.
% %we can only gain information about baseline distributions of variables that an action affects by not taking this action.
% Therefore, if we subtract lower confidence bounds on the baselines from \ac{UCB}s on the actions' rewards, we may end up by sticking to a suboptimal action if the lower confidence bound of its baseline is badly estimated at the beginning.
To provide some intuition, we give an informal justification of \UpUCBwb in \cref{subfig:UpUCBwb}:
%\todob{I looked at the figure and could not understand it. The text below gives much more insight.}
%\todoyg{If the caption gives some insights that's already good. I am not sure how to improve the figure.}
%\UpUCBwb can be informally justified as follows. 
If a suboptimal action $\arm$ is taken in round $\run$, the estimates of all $\vtav[\UCBindex]$ move closer to the actual mean from above. As a result, $\vta[\UPindexSum]$ decreases, since all $\vtav[\UCBindex]$ for $\indv\in\va[\variables]$ do. Thus action $\arm$ is less likely to be taken next. Moreover, $\vta[\UPindexSum][\run][\sol[\arm]]$ increases, since $\vtav[\UCBindex][\run][0]$ decrease for any $\indv$ affected by $\sol[\arm]$ but not $\arm$. Thus $\sol[\arm]$ is more likely to be taken next.
%We illustrate this intuition in \cref{subfig:UpUCBwb}. 
%The following theorem provides a regret bound for \UpUCBwb.
The effectiveness of \UpUCBwb is confirmed by the following theorem.

%Therefore, the resulting uplifting index is a good indicator about
%In \UpUCBwb, all decisions are made on uncertain estimates of at most $\nAffected$ variables.
%Therefore, its statistical efficiency scales with $\nAffected$ and not $\nVariables$.
%the statistical efficiency should scale with $\nAffected$ and not $\nVariables$.
%This in turns translates into a smaller regret, as testified by the following theorem.

% On one hand, if $\arm\in\arms$ has been chosen just a few times, the radius of the confidence interval $\vta[\radiusConf][\run-1]$, and hence $\sum_{\indv\in\va[\variables]}\vtav[\UCBindex]$, is large, which encourages the learner to choose $\arm$. This is exactly as in UCB.
% However, this is counterbalanced by $-\sum_{\indv\in\va[\variables]}\vtav[\UCBindex][\run][0]$, which is large if the variables in $\va[\variables]$ has been affected too frequently, in which case we should avoid choosing $\arm$ in order to improve our estimate of $\vav[\meanReward][0]$ for $\indv\in\va[\variables]$.


% On the contrary, if we subtract a lower confidence bound of the baseline from an \ac{UCB} of the arm's reward, we may end up by pulling a suboptimal arm too many times when this lower confidence bound of the baseline is too pessimistic.
% This is because by pulling the arm we cannot gain information about the baseline distribution of its affected variables, which prevents us from further improving our estimate about the arm's uplifting effect.


%enables us to design much more efficient implementation of such algorithms in special cases, as we will demonstrate in \cref{sec:up-combi}.

\input{Algorithms/UpUCB_WB}

% \paragraph{Regret\afterhead}
%\label{subsec:UpUCB-regret}
% For \UpUCB-B with unknown baseline, we provide the following high-probability regret bound.
%for UpUCB, which formally demonstrates the benefit of our model.

% \begin{restatable}{theorem}{UpUCBRegret}
% \label{thm:UpUCB-regret}
% %Let \cref{asm:noise} hold and 
% Let $\alt{\smallproba}=\smallproba/(4\nArms\nAffected\nRuns)$. If the learner knows the affected variables for each action, then \UpUCBwb, with probability at least $1-\smallproba$, has regret bounded by: \todob{This claim has many unnecessary details. From the definition of the algorithm, it is clear what is known. Thus this claim can be simplified as "Let $\alt{\smallproba}=\smallproba/(4\nArms\nAffected\nRuns)$. Then the regret of \UpUCBwb, with probability at least $1-\smallproba$, satisfies". Do the same for the other theorems. We will get more savings there.}
% %
% \begin{gather}
%     \label{eq:UpUCB-regret}
%     \vt[\reg][\nRuns] \le
%     \sum_{\substack{\arm\in\arms:\va[\gapbandit]>0}}
%     \left(\frac{8(\va[\nAffected]+\va[\nAffected][\sol[\arm]])^2\log(4\nArms\nAffected\nRuns/\smallproba)}{\va[\gapbandit]}
%     %\max\left(
%     %1, \frac{\va[\gapbandit]}{2\sqrt{2}\va[\nAffected]+16\va[\nAffected][\sol[\arm]]}\right)
%     +\va[\gapbandit]\right).
%     \raisetag{0.75em}
% \end{gather}
% \end{restatable}

\vspace{0.2em}
\begin{restatable}{theorem}{UpUCBRegret}
\label{thm:UpUCB-regret}
%Let \cref{asm:noise} hold and 
Let $\alt{\smallproba}=\smallproba/(4\nArms\nAffected\nRuns)$. Then the regret of \UpUCBwb (\cref{algo:UpUCB}) with probability at least $1-\smallproba$, satisfies:
\vspace{-0.6em}
\begin{gather}
    \label{eq:UpUCB-regret}
    \vt[\reg][\nRuns] \le
    \sum_{\substack{\arm\in\arms:\va[\gapbandit]>0}}
    \left(\frac{8(\va[\nAffected]+\va[\nAffected][\sol[\arm]])^2\log(4\nArms\nAffected\nRuns/\smallproba)}{\va[\gapbandit]}
    %\max\left(
    %1, \frac{\va[\gapbandit]}{2\sqrt{2}\va[\nAffected]+16\va[\nAffected][\sol[\arm]]}\right)
    +\va[\gapbandit]\right).
    \raisetag{0.6em}
\end{gather}
\end{restatable}
%\vspace{-0.6em}

%As discussed previously, the regret bound does not at all depend on $\nVariables$. This is a substantial improvement compared to the $\bigoh((\nArms\nVariables^2)\log\nRuns/\gapbandit)$ regret of vanilla UCB.
As in \cref{prop:UpUCB-BL-regret}, the regret is $\bigoh(\nArms\nAffected^2\log\nRuns/\gapbandit)$.
%There is no dependence on $\nVariables$.
In fact, all decisions in \UpUCBwb are made on uncertain estimates of at most $\nAffected$ variables; thus the statistical efficiency scales with $\nAffected$ and not $\nVariables$.
Moreover, for any action $\arm$, the width of the confidence intervals for baseline estimates $\vtav[\radiusConf][\run][0]$
%\acl{CI} widths of baseline estimates 
are lower than those of $\arm$ whenever $\indv\in\setcomplement{\va[\variables]}$. 
%This is why they only cause the 
%This is why we can hide them in those of $\arm$ in the analysis.
The factors $\vtav[\radiusConf][\run][0]$ thus play a secondary role in the analysis of the regret.
A detailed comparison with \cref{prop:UpUCB-BL-regret} reveals that the difference is in 
the order of $\nArms(\va[\nAffected][\sol[\arm]])^2\log\nRuns/\gapbandit$; this is only significant when 
%all
the optimal actions affect many more variables then the suboptimal ones. 
%\todobmargin{This can be explained more easily as an extra multiplicative factor of $2$.}
%\todoygmargin{I mean the difference can be much larger if $\va[\nAffected][\sol[\arm]]\gg\va[\nAffected][\arm]$ for any suboptimal $\arm$.}
%Therefore, 
%in essence,
Hence, the price of not knowing the baseline payoffs is generally quite small.
%On the other hand, if we simply view the problem as a semi-bandit one without taking into the additional structure, we may conclude that the regret is in $\bigoh((\min(\nArms\nAffected,\nVariables)\nArms\nAffected)\log\nRuns/\gapbandit)$.


%However, by further digging into the analysis, we indeed get a regret bound in $\bigoh((\nArms\nAffected^2)\log\nRuns/\gapbandit)$ as shown in \cref{thm:UpUCB-regret}.
%The improvement is in the order of $\nArms$ in the best case.

%As an immediate corollary of the above result, 
%Finally, following the standard derivation, from our proof we easily get an gap-free regret bound in $\bigoh(\nAffected\sqrt{\nArms\nRuns\log\nRuns})$.

% \todob{This is an informal justification of the algorithm. Let suboptimal arm $a$ be pulled in round $t$. Then the estimates of all $U_t^a(i)$ move closer to the actual mean from above. This has two consequences:

% 1) $\rho_t^a$ decreases, since $U_t^a(i)$ for $i \in V^a$ do. So arm $a$ is less likely to be pulled next.

% 2) $\rho_t^{a^*}$ increases, since $U_t^0(i)$ decrease for any $i$ that is affected by $a^*$ but not $a$. So $a^*$ is more likely to be pulled next.

% I find it interesting that we can get away with estimating the baseline without ever pulling arm $0$. This should be stressed.

% The following structures are used in the proof:

% 1) All decisions are made on uncertain estimates of at most $L$ variables. This is why our statistical efficiency scales with $L$ and not $m$.

% 2) For any arm $a$, the CI widths of baseline estimates are lower than those of $a$. This is why we can hide them in those of $a$.

% These structures are used throughout and we should stress it.}

==> Uplifting bandits - arxiv/Tables/Notations.tex <==

\newcommand\Tstrut{\rule{0pt}{2.8ex}}         % = `top' strut
\newcommand\Bstrut{\rule[-1.4ex]{0pt}{0pt}} 
\begin{table}[!h]
    \caption{Main notations used in the paper.}
    \label{tab:notation}
    \renewcommand{\arraystretch}{0.7}
    \label{tab:notation_full}
    \begin{tabularx}{\textwidth}{@{\hspace{1em}}l@{\hspace{1.6em}}l@{\hspace{1.4em}}X@{\hspace{1em}}}
    \toprule
         & Notation & Explanation \\
         \midrule
         \multirow{12}{*}{Bandits} & $\nArms$ & Number of actions\\
         & $\arm$ & An action\\
         & $\sol[\arm]$ & An optimal action, $\sol[\arm]\in\argmax_{\arm\in\arms}\va[\reward]$\\
         & $\arms$ & The set of actions, $\arms=\intinterval{1}{\nArms}$\\
         & $\run$ & Round index \\
         & $\nRuns$ & Number of rounds / Time horizon \\
         & $\oneto{\nRuns}$ & The set of all the rounds, $\oneto{\nRuns}=\intinterval{1}{\nRuns}$\\
         & $\vt[\reward]$ & Reward received at round $\run$\\
         & $\va[\reward]$ & Expected reward of action $\arm$\\
         & $\sol[\reward]$ & Largest expected reward, $\sol[\reward]=\va[\reward][\sol[\arm]]=\max_{\arm\in\arms}\va[\reward]$ \\
         & $\va[\gapbandit]$ & Suboptimality gap of action $\arm$, $\va[\gapbandit]=\sol[\reward]-\va[\reward]$ \\
         & $\gapbandit$ & 
         Minimum non-zero suboptimality gap, \ie $\gapbandit=\min_{\arm\in\arms,\va[\gapbandit]>0}\va[\gapbandit]$ \Bstrut\\
         \hline
         \multirow{19}{*}{
         Uplifting Bandits} & $\nVariables$ & Number of underlying variables \Tstrut\\
         & $\indv$ & A variable \\
         & $\variables$ & The set of variables, $\variables=\intinterval{1}{\nVariables}$\\
         & $\va[\nAffected]$ & Number of variables affected by action $\arm$ \\
         & $\nAffected$ & 
         Upper bound on number of affected variables, \ie $\nAffected\ge\max_{\arm\in\arms}\va[\nAffected]$\\
         & $\va[\variables]$ & The set of variables affected by action $\arm$\\
         & 0 & A convenient notation to represent all quantities related to the baseline \\
         & $\arms_0$ & A notation to include both the actions and the baseline \\
         & $\va[\reward][0]$ & Baseline reward \\
         & $\va[\uplift]$ & Expected uplift of action $\arm$, $\va[\uplift]=\va[\reward]-\va[\reward][0]$ \\
         & $\sol[\uplift]$ & Largest expected uplift, $\sol[\uplift]=\va[\uplift][\sol[\arm]]=\max_{\arm\in\arms}\va[\uplift]$ \\
         & $\vt[\valuev]$ & Payoffs observed at round $\run$,  $\vt[\valuev]=(\vtv[\valuev])_{\allvariables}$ \\
         & $\va[\meanReward]$ & Expected payoffs of action $\arm$, $\va[\meanReward]=(\vav[\meanReward])_{\allvariables}$ \\
         & $\va[\meanReward][0]$ & Baseline payoffs, $\va[\meanReward][0]=(\vav[\meanReward][0])_{\allvariables}$ \\
         & $\va[\meanUplift]$ & Expected individual uplifts of action $\arm$, $\va[\meanUplift]=(\vav[\meanUplift])_{\allvariables}$\\
         & $\va[\distribution]$ & The distribution of the payoffs associated to action $\arm$ \\
         & $\va[\distribution][0]$ & Baseline distribution of the payoffs \\
         & $\gapUplift$ & 
         \makecell[l]{Lower bound on individual uplift,\\ \ie $\forall\arm\in\arms,~\indv\in\va[\variables]$, $\abs{\vav[\meanReward]-\vav[\meanReward][0]}\ge\gapUplift$}
         \Bstrut\\[8pt]
         \hline
         \multirow{8}{*}{UCB} & $\vta[\pullcount]$ & Number of times action $\arm$ is taken in the first $\run$ rounds \Tstrut\\
         & $\vta[\est{\meanReward}]$ & Empirical estimates of expected payoffs \\
         & $\vta[\radiusConf]$ & Widths of confidence intervals \\
         & $\vta[\intConf]$ & Confidence intervals \\
         & $\vta[\UCBindex]$ & Upper confidence bounds \\
         & $\vta[\UPindexSum]$ & Uplifting index of action $\arm$ \\
         & $\vta[\UPindex]$ & Individual uplifting indices \\
         & $\alt{\smallproba}$ & Error probability provided as input for \ac{UCB}-type algorithms\\
    \bottomrule
    \end{tabularx}
\end{table}  


==> Uplifting bandits - arxiv/Tables/Parameters.tex <==
%----------------------------------------------------------------------
%%% OVERVIEW
%----------------------------------------------------------------------
% !TEX root = ../Main.tex

\begin{table}[t]
\setlength{\tabcolsep}{1pt}
\centering
\caption{Parameter values used for the reported experimental results. TS stands for Thompson sampling. Please refer to the text for a explanation on what is the parameter that we tune for each of the algorithms.}
\label{tab:params}
\vskip 0.4em
\begin{tabularx}{\textwidth}{lcccccc}
    \toprule
    Non-contextual & UCB & \UpUCB & \UpUCBwb & \UpUCBL & \UpUCBLwb & TS \\
    \cmidrule{2-7}
    Gaussian 
    & $2$ & $5$ & $3$ & $5$ & $3$ & $8\cdot 10^{-2}$ \\
    Bernoulli &
    $7 \cdot 10^{-7}$ & $8 \cdot 10^{-5}$ & $8 \cdot 10^{-5}$ &  $5 \cdot 10^{-7}$ & $2 \cdot 10^{-6}$  & $2 \cdot 10^{-7}$
    \\
    \midrule
    Contextual && C2UCB & \CUpUCB(b) & \CUpUCB & $\varepsilon$-greedy\,(b) & $\varepsilon$-greedy \\
    \cmidrule{3-7}
    \multicolumn{2}{l}{Logistic for counterfactual} & 2 & 2 & 2 & 0.2  & 0.1\\
    \multicolumn{2}{l}{Logistic for all} & 2 & 2 & 2 & 0.2  & 0.2\\
    %& & $1/\sqrt{\run}$ &  & &  \\
    \bottomrule
\end{tabularx}
%\vskip -0.1in
\end{table}


==> Uplifting bandits - arxiv/Tables/Regrets.tex <==
\begin{table*}[!t]
\renewcommand{\arraystretch}{1.3}
\setlength\tabcolsep{6pt}
%\hspace*{-.2in}
\begin{center}
\begin{tabularx}{\textwidth}{c|a|cc|c|c}
\toprule
%\multirow{2}{*}{Algorithm} & Standard & \UpU & \UpU &  \UpU & \UpU & \UpU & \UpU \\  
% & UCB & \textup{(b)} & & -\textup{nAff\,(b)} & -\textup{nAff} & -iLift\,\textup{(b)} & -iLift \\ \midrule%\hline
Algorithm & UCB & \UpUCB & \UpUCBwb & \UpUCBLwb &  \UpUCBDeltawb     \\ \hline \hline
Affected variables known & No & Yes & Yes & No & No \\ %\hline
Baseline payoffs known & No & Yes & No &  No &  No \\[2pt] %\hline
\hline
\rule{0ex}{4ex}
Regret Bound
& $\displaystyle \frac{\nArms\nVariables^2}{\gapbandit}$ 
&
\multicolumn{2}{c|}{ $\displaystyle \frac{\nArms\nAffected^2}{\gapbandit}$} & 
\multicolumn{1}{c|}{ $\displaystyle \frac{\nArms\nAffected^2}{\gapbandit}$} & 
\multicolumn{1}{c}{$\displaystyle \frac{\nArms\clip(\gapbandit/\gapUplift,\nAffected,\nVariables)^2}{\gapbandit}$} 
\\[0.4em] \bottomrule
\end{tabularx}
%\vspace{-0.1em}
\caption{Summary of our regret bounds for uplifting bandits. Constant and logarithmic factors are ignored throughout.
%$\nArms$ and $\nVariables$ are respectively the number of arms and the number of variables.
For simplicity, we assume here all actions affect exactly $\nAffected$ of the $\nVariables$ variables and all the suboptimal actions have the same suboptimality gap $\gapbandit$. $K$ and $\gapUplift$ are respectively the number of actions and a lower bound on individual uplift ($\gapUplift$ is formally introduced in \cref{sec:part2}).
The operator $\clip$ restricts the value of its first variable to the range defined by its second and third variable, \ie $\clip(x,\alpha,\beta)=\max(\alpha,\min(\beta,x))$.}
%\todob{It does not seem that we ever refer to this table. We should, since we state it upfront.}}
%\vspace{0.4em}
\vspace{-1.4em}
\label{tab:summary}
\end{center}
\end{table*}



==> Uplifting bandits - arxiv/Tables/RegretsCopy.tex <==
\begin{table*}[!ht]
\renewcommand{\arraystretch}{1.2}
\hspace*{-.2in}
\begin{center}
\begin{small}
\begin{tabularx}{0.97\textwidth}{c|a|cc|cc|cc}
\toprule
%\multirow{2}{*}{Algorithm} & Standard & \UpU & \UpU &  \UpU & \UpU & \UpU & \UpU \\  
% & UCB & \textup{(b)} & & -\textup{nAff\,(b)} & -\textup{nAff} & -iLift\,\textup{(b)} & -iLift \\ \midrule%\hline
Algorithm & UCB & \UpUCB & \UpUCBwb & \UpUCBL & \UpUCBLwb & \UpUCBDelta & \UpUCBDeltawb     \\ \hline \hline
%Affected variables & & & & & & & \\
Affected variables known & No & Yes & Yes & No & No & No & No \\ %\hline
%Baseline payoffs & & & & & & & \\
Baseline payoffs known & No & Yes & No & Yes & No & Yes & No \\[2pt] %\hline
\hline
\rule{0pt}{2.6ex} Regret Bound & $\nArms\nVariables^2/\gapbandit$ & 
\multicolumn{2}{c|}{ $\nArms\nAffected^2/\gapbandit$} & 
\multicolumn{2}{c|}{ $\nArms\nAffected^2/\gapbandit$} & 
\multicolumn{2}{c}{$\nArms\min(\max(\gapbandit/\gapUplift,\nAffected),\nVariables)^2/\gapbandit$}  \\ \bottomrule
\end{tabularx}
\caption{Summary of our regret bounds for uplifting bandits. Constant and logarithmic factors are ignored throughout.
%$\nArms$ and $\nVariables$ are respectively the number of arms and the number of variables.
For simplicity, we assume here all the actions affect exactly $\nAffected$ of the $\nVariables$ variables and all the suboptimal actions have the same suboptimality gap $\gapbandit$.
\todosk{define $K$,$L$,$M$}}
%$\clip$ denotes the clipping function that restricts the value of its first variable to the range defined by its second and third variable, \ie $\clip(x,\alpha,\beta)=\max(\alpha,\min(\beta,x))$.
%\todob{It does not seem that we ever refer to this table. We should, since we state it upfront.}}
%\vspace{0.4em}
\label{tab:summary}
\end{small}
\end{center}
\vspace{-1em}
\end{table*}

==> Uplifting bandits - arxiv/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
